MATEX: A Distributed Framework for Transient Simulation of Power Distribution Networks

We proposed MATEX, a distributed framework for transient simulation of power distribution networks (PDNs). MATEX utilizes matrix exponential kernel with Krylov subspace approximations to solve differential equations of linear circuit. First, the whole simulation task is divided into subtasks based on decompositions of current sources, in order to reduce the computational overheads. Then these subtasks are distributed to different computing nodes and processed in parallel. Within each node, after the matrix factorization at the beginning of simulation, the adaptive time stepping solver is performed without extra matrix re-factorizations. MATEX overcomes the stiff-ness hinder of previous matrix exponential-based circuit simulator by rational Krylov subspace method, which leads to larger step sizes with smaller dimensions of Krylov subspace bases and highly accelerates the whole computation. MATEX outperforms both traditional fixed and adaptive time stepping methods, e.g., achieving around 13X over the trapezoidal framework with fixed time step for the IBM power grid benchmarks.

==> abst.tex <==

We proposed \emph{MATEX}, a distributed framework for
SPICE-level transient simulation of large scale
linear circuits.
MATEX inherits the \underline{MAT}rix \underline{EX}ponentials and Krylov subspace methods to 
solve circuit's differential equations.
First, by decomposing input transitions, the whole simulation task is distributed to 
many computing nodes and 
parallelized.
%parallely processed. 
Within each node, the adaptive time stepping is performed individually without re-factorizing matrices. 
Second, by \emph{rational}  Krylov subspace methods, 
MATEX overcomes the stiffness hinder of previous 
matrix exponential-based circuit simulators, 
leading to larger step size with  
smaller dimensions of Krylov subspace basis. 
%This greatly reduces both memory and computational complexities.
%Since the integration kernel an inherently high polynomial approximation, 
%MATEX can utilize larger time steps to do time marching than
%circuit simulation algorithms using traditional integration kernels, 
%e.g. trapezoidal, backward Euler.
%During the simulation, MATEX has the capability of deploying adaptive time stepping 
%and still reusing factorized matrices at the very beginning, 
% even with different time step sizes,
MATEX outperforms both traditional fixed and adaptive time stepping methods,
%Besides, by utilizing superpositions and
%distributed parallel processing, 
%the scalablity of MATEX reduces runtimes furthermore, 
e.g., achieving around 13X over trapezoidal method with fixed time step in transient computing on IBM power grid benchmarks.



==> abst_v1.tex <==
%Theoritical sound and robust
%algorithm for linear circuit transient simulation is crucial to VLSI design.
%It provides the fundation of fast general-purpose circuit analysis, 
%and computationally demanding power grid analysis. 
%In this paper, 
%For efficient transient simulation of linear circuit simulation, 

We proposed a distributed framework for transient simulation of large scale
linear circuits, \emph{MATEX}.
%is a highly efficient and distributed transient simulation framework of linear circuit. %simulation. 
It uses \underline{MAT}rix \underline{EX}ponentials and Krylov subspace methods to 
solve differential equations of the linear system.
By \emph{rational} and \emph{inverted} Krylov subspace methods, 
MATEX overcomes the stiffness hinder of previous 
matrix exponential-based circuit simulators, 
leading to larger step size with  
smaller dimensions of Krylov subspace basis. 
This greatly reduces both memory and computational complexities.
Since the integration kernel an inherently high polynomial approximation, 
MATEX can utilize larger time steps to do time marching than
circuit simulation algorithms using traditional integration kernels, 
e.g. trapezoidal, backward Euler.
During the simulation, MATEX has the capability of deploying adaptive time stepping 
and still reusing factorized matrices at the very beginning, 
% even with different time step sizes,
outperforming both traditional fixed and adaptive time stepping. 
Besides, by utilizing superpositions and
distributed parallel processing, 
the scalablity of MATEX reduces runtimes furthermore, 
e.g. IBM power grid benchmark, 
archiving around 12X 
over fixed time step.
%without losing any accuracy. 
%But due to the stiff system in circuit
%we devise highly efficient ways of handling the matrix exponential approximation
%and 
%overcome previous stiff system problem brought by the ill-conditioned
%capacitance and inductance matrix. 
% formed by modified nodal analysis.

% when dealing such stiff circuit simulation.
%In this paper, we incooperate into MATEX with these
%three approaches and investigate the pros and cons, respectively.
%In pratical, the rational Krylov subspace is high efficient.
%by Krylov subspace for circuit simulation.
%Besides, the scaling invariant property of Krylov subspace enables
%more efficient time stepping than previous matrix exponential based
%circuit simulation. %~\cite{Weng12_TCAD}.
\begin{comment}

This brings huge boosted performance.

Another major contribution of this work
is that MATEX is, inherently, a scalable framework.
We can divide the whole simulation into sub-tasks in terms of 
the groups of independent input sources, 
and map them to processes seperately.
Based on the superposition property,
by summation of the responses from sub-tasks, it reduces
to the final result of time domain simulation without sacrificing
any accuracy.
\end{comment}
%Then map the 
%computational 
%sub-tasks
%to different processes, so that it achieve huge speedups.
%we propose a parallel framework for linear circuits by utilizing adaptive time stepping. 
%Therefore, the whole task can be divided into sub-tasks, and achieve great speedups because 
%the communication only resides at the begin and end of the simulation. 
%The communications are avoided made during the online simulation via precomputed time anchors. 
%In experiment, 
%We also apply this method for power grid simulation.  
%By using rational and inverted Krylov subspace algorithms, 
%our method relax the stiffness constraints of circuit systems,
%and also avoid regularization for singular $\mbf C$ cases of previous works  
%~\cite{Weng12_TCAD}\cite{Weng12_ICCAD} 
%Both highly accelerate MATEX by xX. 
%%It also can handle exsitence of singular matrix $\mbf C$ in the ordinary
%%differential equation (ODE) system without regularization. 
%Furthemore, our MATEX method enjoys more scalability and time-stepping 
%adaptivity than Back Euler (BE) and Trapezoidal (TRAP) methods.  
%Since the required simulation time is usually long for the power grid design, 
%fixed time step size
%from Trapezoidal and Back Euler method 
%cannot exploit large step size corresponding the 
%low frequency response in the power grid for 
%speedup the overall simulation, 
%which is often the cases from industrial power networks (PDNs) design.
%Therefore, our method's adaptivity 
%% by a simple grouping strategy and supperposition porperty of 
%% linear circuit,
%further speedups the simulation by xX.


\begin{comment}
One well-adopted power grid simulation methodology is to factorize matrix once and perform 
only backward/forward substitution with a deliberately chosen step size along the simulation. 
Since the required simulation time is usually long for the power grid design, the costly 
factorization is amortized. However, such fixed step size cannot exploit larger step size for 
the low frequency response in the power grid to speedup the simulation.  In this work, we utilize 
the matrix exponential method with the rational Krylov subspace approximation to enable adaptive 
step size in the power grid simulation. The kernel operation in our method only demands one factorization 
and backward/forward substitutions. Moreover, the rational Krylov subspace approximation can relax the 
stiffness constraint and avoid regularization process of the previous works~\cite{Weng12_TCAD}\cite{Weng12_ICCAD}. 
The cheap computation of adaptivity in our method could exploit the long low-frequency response in a 
power grid and significantly accelerate the simulation. The experimental results show that our method 
achieves up to 18X speedup over the trapezoidal method with fixed step size. Our method also demonstrates 
a promising parallelism. 


Traditional power grid simulation relies on the backward Euler or the trapezoidal
methods with a fixed step size. It requires only one LU decomposition and following 
backward/forward substitutions. However, such fixed step size cannot utilize larger step 
size for the low frequency behavior in the power grid to further speedup the simulation.  
In this work, we propose the matrix exponential method with the rational Krylov subspace 
approximation to enable adaptive step size in the power grid simulation. The rational 
Krylov subspace approximation can relax the stiffness constraint and avoid regularization 
process of the previous works~\cite{Weng12_TCAD}\cite{Weng12_ICCAD}. Moreover, 
adjusting step size in the matrix exponential method costs negligible computational 
overhead, and thus, the adaptive step size could accelerate the simulation process 
significantly. Our experimental results show that the proposed method can achieve up to 
18X speedup over the trapezoidal method with fixed step size, and also demonstrate a 
promising parallelism. 
\end{comment}



==> adaptive_step_control.tex <==

The new proposed MEXP for the power grid simulation can significantly benefit from the adaptive step size control because 
the rational Krylov subspace still preserves the capability of adaptivity, which has been demonstrated the effectiveness 
in linear circuits~\cite{Weng12_TCAD}. And, with the relaxation of the stiffness constraint, MEXP can now utilize even larger 
step size, e.g., 1\emph{ns}, to perform transient analysis. Such large step size is particularly useful for the power grid 
simulation where the voltage noise usually includes the low frequency behavior of both package and board levels. 

The idea of our adaptive step scheme is to step forward as much as possible so that MEXP can finish the simulation 
quickly. With the insight from Eqn. (\ref{eq:scale}), MEXP is able to adjust $\alpha$ to calculate result of arbitrary 
step size with only performing one Arnoldi process. However, because MEXP has to guarantee slopes of input sources must 
be constant within the step size, the maximum allowed step size is limited. Therefore, MEXP will first compute the rational 
Krylov subspace using $\mbf{x}(t)$, and then results within the maximum allowed step size, which is determined by input 
sources, can be calculated through the step size scaling. 

Algorithm~\ref{algo:adaptive_step} shows MEXP with adaptive step control scheme. In order to comply with the required 
accuracy during the simulation, the allowed error $err_k$ at certain time instant $t_k$ is defined as 
\begin{eqnarray}
    err_k \le \frac{E_{Tol}}{T}\times h_k, \nonumber
\end{eqnarray}
where $E_{Tol}$ is the error tolerance in the whole simulation process, $T$ is the simulation time span, $h_k$ is the 
step size at time $t_k$, and $err_k$ is the posterior error of MEXP from Eqn. (\ref{eq:post_err_est}). Hence, when 
we construct the rational Krylov subspace at the current time, we will increase $m$ until the $err_k$ satisfies the 
error tolerance. 

\begin{algorithm} 
    \label{algo:adaptive_step}
    \caption{MEXP with Adaptive Step Control}
    \KwIn{$\mbf{C}$, $\mbf{G}$, $\mbf{B}$, $\mbf{u}(t)$, $\tau$, error tolerance $E_{Tol}$ and simulation time $T$}
    \KwOut{$\mbf{x}(t)$}
    {
        $t = 0$; 
	$\mbf{x}(0)$ = DC\_analysis\;
        %Choose $\tau$ for rational Krylov subspace method\;
        $[\mbf{L}_{sub},\mbf{U}_{sub}] = $LU($\mbf{C} +\gamma \mbf{G}$)\;
        \While{$t \leq T$}
        {	
	    %Update $v_{k+1}$ with $\mbf{L}, \mbf{U}, \mbf{W}$ by (\ref{eq:blu_f})\;
	    %and update $\mathbf{L},\mathbf{U}$ by (\ref{eq:blu})\;
	    Compute maximum allowed step size $h$ from $\mbf{u}(t)$\;
	    Construct $\mbf{H_m}$, $\mbf{V_m}$ by Arnoldi process until $err_k \le \frac{E_{Tol}}{T}h$\;

	    $\alpha = \frac{h}{\gamma}$ \;
	    Compute $\mbf{x}(t+h)$ by (\ref{eq:scale})\;

	    $t = t+h$; 
	}
    }
\end{algorithm}
The complexity of MEXP with adaptive step size is mainly determined by the total number of required backward/forward
substitutions during the simulation process. This is because the dimension of $\mbf{H_m}$ is small, e.g., around 
$5 \sim 20$, and the computation overhead of the step size scaling is negligible. The number of total substitution 
operations is 
\begin{eqnarray}
    \sum_{i=0}^N m_{i}, \nonumber
\end{eqnarray}
where $N$ is total time steps, and $m_i$ is required dimension of rational Krylov subspace of each time step. Compared to 
the trapezoidal method where the number of substitution operations depends on the fixed step size, MEXP could use less 
substitution operations as long as the maximum allowed step size is much larger than the fixed step size. Our experiments 
in the following section demonstrates it is usually the case for the power grid simulation.


==> append.tex <==
\subsection{Future work}
Wavepipe

\subsection{S-Domain}


Using S-Domain analysis~\cite{Cheng00}, 

\begin{eqnarray}
    \label{eqn:s-ode}
    s\mbf{C}{\mbf{x}}(s) - \mbf C \mbf x(0)
    = - \mbf{G}\mbf{x}(s) + \mbf{B}\mbf{u}(s),
\end{eqnarray}

where, with initial solution 
$\mbf{x}(0)$ from the DC analysis via direct 
or iterative approaches\cite{Davis06}\cite{Saad03}, 

\begin{eqnarray}
    s \mbf{C}{\mbf{x}}(s) -  \mbf C \mbf x(0)
    = - \mbf G\mbf{x}(s) + \mbf{B}\mbf{u}(s),
\end{eqnarray}

\begin{eqnarray}
  (s\mbf C + \mbf G ){\mbf{x}}(s) 
    =   \mbf C \mbf x(0) +  \mbf{B}\mbf{u}(s),
\end{eqnarray}

when the matrix pencil $ (s\mbf C + \mbf G ) $ is regular.

\begin{eqnarray}
  {\mbf{x}}(s) 
    = (s\mbf C + \mbf G )^{-1}  \mbf C \mbf x(0) 
    +  (s\mbf C + \mbf G )^{-1} \mbf{B}\mbf{u}(s),
\end{eqnarray}

For time domain, in MEXP\cite{Weng12_TCAD}\cite{Weng12_ICCAD} it 
uses the analytical solution of ODEs, following as 

\begin{eqnarray}
  {\mbf{x}}(s) 
    = (  s\mbf I + \mbf C^{-1} \mbf G )^{-1} 
        \mbf x(0) 
    +  (  s\mbf I + \mbf C^{-1} \mbf G )^{-1}  
      \mbf C^{-1} \mbf{B}\mbf{u}(s),
\end{eqnarray}



\begin{eqnarray}
    \mbf x(t+h) & = &
\mbf I \mbf x(t) + h \mbf A \mbf x(t)
    + h^2 \mbf A^2 \frac{\mbf x(t)}{2} + \cdots + h^k \mbf A^k \frac{\mbf  x(t)}{k!} 
    \\ \nonumber
    & &+ \mbf I \int_0^{h} \mbf b(t+\tau) d\tau +   \mbf A \int_0^{h} (h-\tau) \mbf b(t+\tau) d\tau
    \\ \nonumber
    & &+ \frac{\mbf A^2\int_0^h (h-\tau)^2\mbf b(t+\tau) d\tau}{2}
    + 
    \cdots +  
    \frac{\mbf A^k \int_0^{h} (h-\tau)^k \mbf b(t+\tau) d\tau}{k!}
%    \\ \nonumber
%    & = & 
%    \mbf I (\mbf x(t) + \int_0^{h} \mbf b(t+\tau) d\tau) +
%\mbf A (h\mbf x(t) + \int_0^{h} (h- \tau) \mbf b(t+\tau) d\tau)
% \\ \nonumber
%   & &	+ \mbf A^2 \frac{(h^2\mbf x(t) +\int_0^h (h-\tau)^2   \mbf b(t+\tau) d\tau)}{2} + 
%   \cdots +  \mbf A^k \frac{(h^k\mbf x(t) + \int_0^{h} (h-\tau)^k \mbf b(t+\tau) d\tau)}{k!}
\end{eqnarray}



In Laplacian Transporamtion~\cite{Cheng00},
\begin{eqnarray}
\mbf X(s) & =&  (s \mbf C + \mbf G)^{-1} \mbf C \mbf x_0 + 
                (s \mbf C + \mbf G)^{-1} \mbf B \mbf u(s) 
	         \\ \nonumber
& = & (\mbf G+ s_0 \mbf C + (s-s_0) \mbf C)^{-1} \mbf C \mbf x_0 
	\\ \nonumber
 & &     + (\mbf G+ s_0 \mbf C + (s-s_0) \mbf C)^{-1} \mbf B \mbf u(s) 
	\\ \nonumber
& =&  (\mbf I + (s-s_0) (\mbf G+s_0\mbf C)^{-1} \mbf C)^{-1}
   (\mbf G+s_0\mbf C)^{-1}  \mbf C \mbf x_0
	\\ \nonumber
 & &   +
  (\mbf I + (s-s_0) (\mbf G+s_0\mbf C)^{-1} \mbf C )^{-1} 
  (\mbf G+s_0\mbf C)^{-1} 
  \mbf B \mbf u(s)
  \\ \nonumber
& =&  (\mbf I + (s-s_0) (\mbf G+s_0\mbf C)^{-1} \mbf C)^{-1}
   (\mbf G+s_0\mbf C)^{-1}  \mbf C \mbf x_0
	\\ \nonumber
 & &   +
  (\mbf I + (s-s_0) (\mbf G+s_0\mbf C)^{-1} \mbf C )^{-1} 
  (\mbf G+s_0\mbf C)^{-1} \mbf C \mbf C^{-1} \mbf B \mbf u(s)
	\\ \nonumber
& = &
  (\mbf s I + ((\mbf G+s_0\mbf C)^{-1} \mbf C)^{-1} -s_0 \mbf I )^{-1} \mbf x_0
	\\ \nonumber
 & &   +
  (\mbf s I + ((\mbf G+s_0\mbf C)^{-1} \mbf C)^{-1} -s_0 \mbf I )^{-1}  \mbf C^{-1} \mbf B \mbf u(s)
\end{eqnarray}

\begin{eqnarray}
\mbf X(s) = p(\mbf A) \mbf A \mbf x(0) + p(\mbf A) \mbf A \mbf C^{-1} \mbf G
\mbf B \mbf u(s)
=
\mbf X(s) = q(\mbf A) \mbf x(0) + q(\mbf A)  \mbf C^{-1} \mbf G
\mbf B \mbf u(s)
\end{eqnarray}

where $q(\mbf A) = p(\mbf A)\mbf A$, 
inverse Laplacian Transformation pop out the exponential function.

By interpreting the method as above, the classical MOR can be treated in 
time domain.
Only different is our method use Krylov subsapce to approximate
the exponential operator, however, the MOR use block Krylov subspace
to the stamping matrix directly. It is noted that the Krylov subspace for 
approximation of exponential method can be views as more accurate model order
reduction.

MEXP is precious solution for DAE system, it takes states of very time steps, 
for the Krylov subspace. 

It is supposed to take less $m$, because we evaluate $exp$
operator, and its denominator is factorial is way faster than
order series. 
So the computation will be compensated. 

It is noted in rational Krylov subspace, the $s_0$ is corresponding to $\gamma$. Because in frequency domain, the method SPRIM take expansion points near the observation frequency.
and it is easy to see the $s_0 = \frac{1}{\gamma}$.




\begin{eqnarray}
  {\mbf{x}}(s) 
 &  = & (s\mbf G^{-1} \mbf C + \mbf I )^{-1} \mbf G^{-1} \mbf C \mbf x(0) 
    +  (s\mbf G^{-1} \mbf C + \mbf I )^{-1} \mbf G^{-1} \mbf{B}\mbf{u}(s)
	\\ \nonumber
 &  =& (s\mbf G^{-1} \mbf C + \mbf I )^{-1} \mbf G^{-1} \mbf C \mbf x(0) 
    +  (s\mbf G^{-1} \mbf C + \mbf I )^{-1} \mbf G^{-1} \mbf C \mbf C^{-1}  \mbf{B}\mbf{u}(s)
	\\ \nonumber
 &  =& (s \mbf I + (\mbf G^{-1} \mbf C)^{-1} )^{-1}  \mbf x(0) 
    +  (s \mbf I + (\mbf G^{-1} \mbf C)^{-1} )^{-1}  \mbf C^{-1}  \mbf{B}\mbf{u}(s)
\end{eqnarray}

\begin{eqnarray} 
\mbf x(t+h) = e^{- ( \mbf G ^{-1} \mbf C)^{-1} h } \mbf x(t)
   + \int_t^{t+h} e^{-( ( \mbf G^{-1} \mbf C)^{-1} ) (h-\tau)  } \mbf C^{-1} \mbf B 
   \mbf u(t+\tau) dt
\end{eqnarray} 


\begin{eqnarray}
\mbf x(s) % & =& 
%(s \mbf C + \mbf G)^{-1} \mbf C \mbf x_0 + 
%                (s \mbf C + \mbf G)^{-1} \mbf B \mbf u(s) 
%	         \\ \nonumber
& = & (\mbf G+ s_0 \mbf C + (s-s_0) \mbf C)^{-1} \mbf C \mbf x_0 
	\\ \nonumber
 & &     + (\mbf G+ s_0 \mbf C + (s-s_0) \mbf C)^{-1} \mbf B \mbf u(s) 
	\\ \nonumber
& =&  (\mbf I + (s-s_0) (\mbf G+s_0\mbf C)^{-1} \mbf C)^{-1}
   (\mbf G+s_0\mbf C)^{-1}  \mbf C \mbf x_0
	\\ \nonumber
 & &   +
  (\mbf I + (s-s_0) (\mbf G+s_0\mbf C)^{-1} \mbf C )^{-1} 
  (\mbf G+s_0\mbf C)^{-1} 
  \mbf B \mbf u(s)
  \\ \nonumber
& =&  (\mbf I + (s-s_0) (\mbf G+s_0\mbf C)^{-1} \mbf C)^{-1}
   (\mbf G+s_0\mbf C)^{-1}  \mbf C \mbf x_0
	\\ \nonumber
 & &   +
  (\mbf I + (s-s_0) (\mbf G+s_0\mbf C)^{-1} \mbf C )^{-1} 
  (\mbf G+s_0\mbf C)^{-1} \mbf C \mbf C^{-1} \mbf B \mbf u(s)
\\ \nonumber
& = &
  (s \mbf  I + ((\mbf G+s_0\mbf C)^{-1} \mbf C)^{-1} -s_0 \mbf I )^{-1} \mbf x_0
	\\ \nonumber
 & &   +
  (s \mbf  I + ((\mbf G+s_0\mbf C)^{-1} \mbf C)^{-1} -s_0 \mbf I )^{-1}  \mbf C^{-1} \mbf B \mbf u(s)
\end{eqnarray}

\begin{eqnarray} 
 \mbf  x(t+h) & = & e^{-( ( (\mbf G + s_0 \mbf C)^{-1} \mbf C)^{-1} -s_0 \mbf I)h } \mbf x(t)
 \\ \nonumber
  & & + \int_t^{t+h} e^{-( ( (\mbf G + s_0 \mbf C)^{-1} 
    \mbf C)^{-1} -s_0 \mbf I) (h-\tau)  } \mbf C^{-1} \mbf B 
   \mbf u(t+ \tau) dt
\end{eqnarray} 


==> intro/intro_2.tex <==

Circuit Simulation is an important and heavily used 
process during the cycle of integrated circuit designs.
The increasing integration between functional modules
and interconnects parasitic effects of modern VLSI design
aggravats such simulation tasks,
rendering the transient simulation of the full-system inefficient. % jobs. 
Therefore, accurate yet fast circuit simulation methods have always
been desired in the integrated circuits (IC) industry.
Theoritical sound and scalable algorithm for linear circuit transient simulation 
is the building block of circuit simulators.
It provides the fundation for fast general-purpose circuit analysis, 
as well as computationally demanding power grid analysis, and \emph{etc}. 
Nowadays, the emerging multi-core, many-core platforms bring
powerful computing resources and opportunities
for parallel and distributed computing in EDA and IC industry.
However, building a scalable transient analysis tools is still a chanllenge.
Previous works 
%\cite{Ye08}, \cite{Dong08}, \cite{Dong09}, \cite{Peng09},\cite{Li11}, \cite{Weng12_ICCAD}, \cite{Weng12_TCAD}
\cite{Dong08, Dong09, Li11, Peng09, Weng12_ICCAD, Weng12_TCAD, Ye08}
have been made in order to improve circuit simulation by novel algorithmics or parallel processing.

Time domain simulation involves solving differential algebra equations (DAEs),
which are derived normally from modified nodal analysis (MNA) \cite{Ho75}.
They describes the transient behavior of circuit and can be solved numerically
in explict, e.g., forward Euler (FE), or implicit ways, e.g, backward Euler (BE), Trapezoid (TR).
Due to the stiffness of the equation systems, which results from
a wide range of time constants of a circuit,
the explicit methods require using small time step sizes 
to ensure the stablity of this numerical integration methods.
The implicit methods can conquer this problem and popularly used by conventional SPICE-like
simulators.
Nonetherless, these implicit methods have to solve a linear system during each time step.

Linear systems resulting from this circuit simulation at each time step is sparse and ofter
ill-conditioned. 
Therefore, the industry often favors direct sparse matrix solvers \cite{Davis06}
%are industry standard approach
for solving these linear systems, because of their reliability and pratical usages.
However, this kind of methods has scalability problem,
the time and memory complexity is $O(n^{1.5})$,
where $n$ is the number of non-zero elements in the matrix of circuit simulation.
Although iterative solver can ease the scalability problem, solving an ill-conditioned matrix
is still a chanllenge. 
%In addition, for smaller problems direct methods are usually faster.  
Additionally, in transient simulations linear circuit, e.g., power grid analysis, 
the direct methods are heavily used and shows their efficiency
%\cite{Yu12}, \cite{Xiong12}, \cite{Yang12}, \cite{Zhao02}.
\cite{Xiong12, Yang12, Yu12, Zhao02}.
It is because that, only one factorization (LU or Cholesky factorization)
is required at the begining of simulation. 
During transient calculation, 
only backward
and forward substitutions are performed by reusing the factorization matrices. 



Beyond the traditional explict and implcit methods, a new class of methods called exponential
time differencing (ETD) has been embraced by Weng \emph{et al.} \cite{Weng11_ASICON, Weng12_TCAD} and 
applied to time domain circuit simulations,
%with matrix exponential computation by Krylov subspace approximation, 
which is called as MEXP.
Based on the piecewise linear (PWL) assumptions of input sourses and nonlinear device models, 
these works solve the DAEs analytically and removes the local truncation error (LTE) of
polynomial expansion approximation. 
% in majority of numerical methods. 
The major computation of MEXP resides in calculating the matrix exponential. 
MEXP utilizes standard Krylov subspace method based on \cite{Moler03} to approximate matrix exponentials.  
Nevertheless, there are still three major limitations for MEXP 
in linear circuit transient simulation as follows.
\begin{itemize}
\item[(1)] 
Stiff circuits require the MEXP to use small step sizes to
reduce approximation error of standard Krylov subspace method, degrading the performance.
%(2)
\item[(2)]
Larger Krylov subspace bases are required by stiff circuits, posing a memory bottleneck
and computational burden in each time step.
\item[(3)]
Time steps are enforced to stay the regions without breaking PWL assumption. It becomes
a trouble when there are many independent input sources with transitions at different
time spots, which is often the case in large-scale VLSI transient simulation. 
\end{itemize}
%which
%we summarize in Sec. \cite{sec:rational_krylov}.
%Recently, Zhuang, \emph{et al.} \cite{Zhuang13_ASICON} deployed
%\emph{rational} Krylov subspace method in stiff power grids to
%overcome limitation (1) and (2). 


\emph{Our Contributions}. In this paper, we aim to 
efficent transient simulations of linear circuit. 
We devise a scalable algorithmic framework, called as MATEX, 
of which time integration is still solved by matrix exponentials and Krylov subspace. 
%to achieve large speedups over previous MEXP. 
%To accelerate matrix exponential computation in stiff circuit simulation,  
%We generalize  \cite{Zhuang13_ASICON}
%with rational Krylov subspace 
%\cite{Zhuang13_ASICON}
\begin{itemize}
\item 
To overcome the stiffness problem of MEXP, 
we incorporate inverted and rational Krylov subspace bases into MATEX respectively. 
Both reduce the dimension of basis for matrix exponential computations, 
remarkably ease the memory demands
and boost computational performance. 
When dealing with singular capacitance/inductance matrix, 
these two methods does not need the regularization process \cite{Chen12_TCAD, Weng12_TCAD}, 
which is required in MEXP\cite{Weng12_TCAD}.  
%, which achieve hundreds speedups over MEXP. 
\item 
After freeing from the constraint of stiffness, MATEX takes advantage of the ETD's property 
(analytically solving the differential equations without LTE) to use very large time size, without losing
accuracy, expediting the whole time domain simulation. 
\item
MATEX is a highly scalable transient simulation by decomposition of the input sources 
and superposition property of linear system, described as follows:
\begin{itemize}
\item[(1)] 
For each input transition within each cluster, it only needs one Krylov subpace calculation. 
%Approximately, the times of Krylov subpsace cacluations is $n/m$, 
%where $n$ and $m$ are the total number of time points and computing clusters, respectively. 
\item[(2)] 
All the following time points (before the next input transtion) can be derived from (1) by scaling Krylov subspace for adaptive time stepping. 
%fully enjoys the resulting more "spacious" regions to do time marching, 
%without recomputing the inverted/rational Krylov subspace basis.
%The required computing time spots (for supperpositions of entire systems) in such region 
%only need to scale the exsiting matrix to obtain the exact solutions.
%This process is scalable and no communication-overhead after precomputing the time anchors 
%according to the set of input sources. 
%can be finished in parallel. 
\item[(3)] 
Other tradtional methods (FE, BE, TR, and \emph{etc}): 
for each cluster, we still need to derive step by step along 
all time points with integration calculations (e.g. LU, Cholesky). 
%the calculation times are still $n$.
Therefore, to them, there is no benefit from such input sources decomposition and linear system's superposition. 
%which expedites MATEX.
%Other traditional methods cannot benefit from this seperations and parallism, 
%due to the smaller time step size by LTE and requirement of matrix refactorization 
%when the change of time step size.  
\end{itemize}
%under the PWL  
\end{itemize}

\begin{comment}
and its adaptive time controlling into MATEX. 
During the transient simulation, 
the input changes cause the updates of matrices. 
However, the updated region resides within only columns of the matrix.
By precomputing block LU calculation beforehand and 
updating that region step by step, MATEX does not require LU factorizations on-the-fly, 
which is very different from that of TR-like methods.
%{\color{red} Only by updating small part of matrices,
%due to the input change,
%MATEX's adaptive time stepping does not require 
%LU factorization on-the-fly.}

We also combine MATEX %together 
with \emph{inverted Krylov subspace} as an alternative technique,
which only requires decomposing the conductance matrix. 
Therefore,
it is advantageous the avoidance of inverting the 
matrix of capacitance and inductance, which may 
include many parasitic energy elements 
with large magnitude variations
after circuit extraction.
%{\color{red}{The connections of these two methods are inspired by the works 
%from model order reduction community, \emph{i.e.,}
%PRIMA \cite{PRIMA98} and SPRIM \cite{SPRIM04}.}}

%These solve the limitations (1) and (2);
Additionally, the parallelism of MATEX
is based on the superposition property of linear circuit.
Within our theoritically sound skeleton,
we split the input sources, use all of divided subset of input sources 
to stimuli the system, seperately, %and efficiently adaptive time stepping,
making the whole simulation task divided
into serveral sub-tasks. 
% and solved seperately 
These sub-tasks can be solved parallel, without sacrificing any accuracy. 
This circumvents the limitation (3).
Besides, the traditional methods (FE, BE, and TR) cannot benefit from this
splitting, due to their limitations not from the side of input sources
but from LTE and stability.
With the advent of inexpensive computer clusters, and multi/many-core technology,
this distributable algorithmic framework is a nice one for future implementations.
\end{comment}

\emph{Paper Organization}.
%The rest of paper is organized as follows.
Section II introduces the background of
linear circuit simulation and matrix exponential formualtions.
Section III presents the different bases of Krylov subspace methods for MATEX.  
Section IV presents the adaptive time controling of MATEX. 
Section V presents the scalable framework.
Section VI shows numerical results and Section VII concludes this paper
and propose some possible future directions.

\begin{comment}


The major reason is that mainstream circuit simulators inherit implicit numerical
integration, e.g. backward Euler, Trapezoidal methods, 
for the sake of stability, where the explicit methods suffer. 
However, implict methods trouble the perspective of scalability
due to the requirement 
of solving large linear systems of differential equations.
On the contrary, the explict methods are more scalable and parallelizable 
for current multi-core and manycore architecture.
The merit of explict methods resides in simple time propogation scheme via 
matrix-vector multiplication who costs relative lower
computation and memory complexity about $O(n)$.
Even though the existence of stability issue, 
explicit methods still become a revived research 
area and verifies their parallelism and scalability 
within modern parallel computer architecture
~\cite{Dong08}\cite{Dong09}\cite{Weng12_ICCAD} during these years. 

One of promising and distinct method for circuit simulation
is matrix exponetial method (MATEX) proposed in 
\cite{Weng12_TCAD}. Apart from the above numerical methods, 
the DAE/ODE system (in one discritized region of certain time step) can  
be solved in analytical way via matrix expoential operator $e^{\mbf A}, 
\mbf A \in \mbf R_{n \times n}$. 
By the analytical property, this distinct class 
of numerical approach removes the local truncation  
and it is A-\emph{stable} for passive circuits. 
Therefore, it is not constraint by the stablity problem. 
{\color{red}{This property matters!}}
%(When $h >  0, h \to \infty$, the $x(h) \to 0$). Very unlike forward
%Euler method that require small time step to let fast damp compoent
%die down first, bring too much time steps. But M
However, the kernel computation of MATEX lies in computing matrix expoential is very high,  
e.g., direct computation consumes around $O(n^3)$ complexity. 
Weng \emph{et al.} \cite{Weng12_TCAD}\cite{Weng12_ICCAD} introduced a \emph{standard Krylov subspace}
method-based MATEX for circuit simulation to solve this problem. 
In addition, unlike the implicit methods (Trapezoidal and Back Euler) 
they both require fixed step size so that they reduce the LU online for linear circuit
transient simulation,
this MATEX can utlize the scaling invariant property of Krylov subspace to do the adaptive time-steping 
without compromising any accuracy.
(1) MATEX can jump further than BE and Trap, because the exponenital 
denomator in the exponential approximation, it is much better
than the Taylor expansion.
(2) Under the (PWL) assumptions, MATEX can also carry 
the input information during the stepping.  
(3) With the help of Krylov subspace scaling invariant, it can re-evaluate
the inter time point without rebuilding Krylov subspace.

%By this strategy, it helps to capture the low frequency response from circuit system and further speedups the whole simulation without fixed step size limitation.
% In recent years, the Krylov subspace method has
Nonetheless, the step size is actually limitted by the stiffness of matrix when utilizing standard Krylov subspace.
It is because the large spectrum of $\mbf A$ and the Arnoldi process focus on capturing %the extreme magnitude
% and
well-distributed eigenvalues, so it ofter misses the dominant factors for the circuit system/for
matrix epxonential operator, which are the ones with smallest magnitudes.
Therefore, the Arnoldi process requires large number of order to preserve the 
accurate of matrix exponential calculation. 
Also, the standard Krylov-Based MATEX requires the process of regularization \cite{Chen12_TCAD} 
to deal with singular matrix $\mbf C$, i.e., nodes without grounded capacitance or 
inductance/voltage branches. Both drag the overall performance of MATEX for circuit simulation.  
% former MATEX~\cite{Weng12_TCAD} requires regularization. 
% In addition, when the matrix $\mbf C$ is stiff, it requires smaller 
%time steps or even larger Krylov subspace 
% order $m$, which degrades the method. 


In this paper, we integrated our previous works on MATEX for linear circuits 
using \emph{rational Krylov subspace}~\cite{Zhuang13_ASICON} and \emph{inverted Krylov subspace}.
%The rational Krylov subpsace uses 
They use 
$(\mbf I-\gamma \mbf A)^{-1}$ and $\mbf A^{-1}$, respectively, 
as the basis instead of $\mbf A$ (\emph{standard Krylov subspace}) in \cite{Weng12_TCAD}. 
The rational basis limits the spectrum of a circuit matrix into a unit circle,
and the inverted operation puts the important eigenvalues with smallest magnitudes from former spectrum
into a large magnitude ones. By using Arnoldi algorithm, the Hessenberg matrix can resemble the former matrix
$\mbf A$ projected onto the new invariant subspace better and contain the more accurate important eigenvalues
for matrix exponential operator.
This method provides a good convergent rate in Arnoldi process within MATEX framework.
The inverted Krylov subspace's convergent rate in Arnoldi process may not be as good as rational basis. However,
it only requires the LU factorization of conductance matrix $\mbf G$. It provides
a strategy dealing with $\mbf C$ is very complicated from post-layout extraction, but
$\mbf G$ is much more simple then. Similarly as rational basis, by the invertion $\mbf A$, the small magnitude eigenvalues 
become the large ones in the transformed spectrum, so that the exponential of a matrix can be accurately approximated.
A very typical and important application for circuit simulation is power grid analysis, which plays an 
important role in IC deisgn methodology. Given current stimulus and power grid structure, designers should verify
and pedict the worst-case voltage noise through the simulation before signing off their design. 
The model order reduction provides good way to reduce matrix of circuit system, e.g. 
PRIMA \cite{PRIMA98} and SPRIM \cite{SPRIM04}. However, with the large number of 
input sources, this kind of strategy cannot benefit from 
the reduction models any more. 
The majority works still use Trapezoidal method with fixed step size
for the power grid simulation.
Till now, accourding to Tau power grid simulation contest 2012 \cite{Li12_Tau}\cite{Yu12}, 
the trapezoidal method with fixed step size using one LU and 
many backward/forward substitutions lead to the best performance. 
The small and fixed time steps bring benefits for the transient power grid analysis 
when dealing the voltage variation 
with high frequency, i.e. the input is changing rapidly or constantly. 

However,
when package has an important impact on accurarte 
on-die power grid analysis~\cite{Pant06}\cite{Pant07}, 
and middle and low frequency phenomena is of interests to the designers, 
trapezoidal method with fixed time step becomes very inefficient. 
It is 
because such mehtod takes long time to represent the steady state of power grid system.
In the architecture analysis, power distribution networks (PDN) 
involves with pakcage and board 
level simulations \cite{PengLi12_ICCAD}\cite{Pant06}\cite{Pant07},
which requires longer timespan of simulation,
e.g. up to few $\mu s$, the simulation process are 
often time-consuming with the limitation of fixed step size to avoid online LU.
Our method can exploit large time step, ``steady region'' of waveform
during the simulation, meanwhile, it only requires one LU factoraization
as trapezoidal method, with backward/froward substitutions.
With equivalent error buget, the krylov subspace MATEX can jump larger time step/fewer 
number of time steps
than trapezoidal
method. Therefore, even though such fully implicit scheme can be used here,
when a sparse LU factorization is affordable,
the simulation burden is higher than our Krylov subspaces MATEX because of 
more time steps need.

The aim of this paper is to present and organize the Krylov subspace based 
MATEX solver in transient simulation of linear circuit.
We list our main contributions of this paper are as follows.
\begin{itemize}
%\item A breakthrough of the circuit simulation matrix exponential.
\item Accelerate MATEX via rational and inverted Krylov 
subspace.
\item Using adaptive time 
stepping strategy for circuit simulation and overcome the 
problem to achieve low-frequency pheonomena of circuit system.
\item Eliminating the regularization process 
for singular matrix $\mbf C$ for explicit method 
of circuit simulation.
\item By input grouping and superposition property of linear circuit 
to further accelerate circuit simulation.
\item Establish the relation of MATEX with previous works on Model Order Reduction. 
\end{itemize}

By such contributions, we are able to achieve hihgly efficient trasient 
simulation. Compared to the works~\cite{Weng12_TCAD}.
It is very nice property from linear system, which they can be 
superposition. 
By this idea, the same system with the parts of inputs send to different
machines, cores, or threads and add together without communication 
during the process, only require on precomputed time stamp/anchors.
It is a nice parallelism framework, we provide such for the further 
extension.
It is noted that Trapezodal cannot achieve this benefit, because
it is not analytical solution, and the inputs are not the 
hurdles during their simulation but the stability and local trancation
error are.

The paper is organized as follows. Section II is the fundemantals 
of circuit simulation and matrix exponential inteperation.
Section III describes the Krylov methods for fast matrix exponential evaluations. 
They are three algorithms for such computation, Standard Krylov subspace, inverted 
Krylov subspace, Rational krylov subspace.
Section IV presents the computational results of simple linear circuit cases, also contains industrial power grid designs and the famous IBM benchmark suite.

\begin{comment}

\begin{itemize}
\item Accelerate MATEX via rational and inverted Krylov subspace and its coresponding adaptive time stepping strategy for circuit simulation.
%    \item And, summarize three Krylov strategies for MATEX, the standard/inverted/rational Krylov subspace.
%  \item Use inverted Krylov subspace, enable the krylov subspace based MATEX without regularization~\cite{Chen12_TCAD}.
\item Eliminating the regularization process for singular matrix $\mbf C$ for explicit method of circuit simulation.
\item Speedups linear circuit simulation, by adaptive time stepping.%  partitioning input sources, and using superposition,
    % \item Using block matrix for Krylov subspace generation.
    % \item Establish the relation of MATEX with previous works on Model Order Reduction. 
    % As a explicit circuit solver, which is also enjoy the model order reduction framework.
    %    \item Generalize the explict method for future parallelism circuit simulation (Stablity).
\end{itemize}
For solving ordinary differential equations $x'=Ax+f(t)$,
it has an anlytical solution $x(t+h)=e^{Ah}x(t)+ \int_{0}^{h}e^{A(h-\tau)}f(t+\tau)d\tau$. 
When $A$ is large, it is very expensive to cacluate the exponential operator directly.  
The explict and implict methods are strategies to approximate the operation of $e^{Ah}$.  
Explicit methods required matrix-by-vector multiplications, however, implicit methods need to solve 
a whole linear system.  
It is known that explicit methods are constraint on the size of the time steps required to make sure stability. 
Compared to explicit methods, Implicit methods have more difficulties on utilizing current 
parallel and distributed machines.  
Recent development of Krylov subspace accelerates the exponential operations.  
The  
\begin{itemize}
\item without regularization, 
    \item Accelerate and enpower MATEX framework via rational Krylov subspace algorithm.
    \item Enabling adaptive time stepping for circuit simulation.
    \item Establish the relation of MATEX with previous works on Model Order Reduction. As a explicit circuit solver, which is also enjoy the model order reduction framework.
    \item ?? Generalize the explict method for future parallelism circuit simulation (Stablity).
\end{itemize}
The MATEX has a good characteristic that the exponential operator bares the propagation in the perspective of
time derivitate,
which the method at Forward Euler (FE), Backward Euler (BE) and Trapezoidal (TRAP) method use time step $h$ to discretize the
dynamical system with respect to time. 
They lead to explicit and implicit methods,
which bring the stability and limitted time step due to the system, e.g. 
stiff systems.
Explicit methods are relatively cheap computation; Implicit methods are usually time consuming because they require
to solve the large linear systems. For this regard, in power grid simulation, it precomputes the matrix 
($\mbf C/h+ \mbf G$) in BE, or ($\mbf C/h + \mbf G/2$) in TRAP. This involes the time step $h$. 

Also, in linear circuit, the the mexponential operator is a explicit method, of which the matrix-vector multiplication
take the major part of computation.



Power grid simulation plays an important role in IC design methodology. Given current stimulus and the power grid structure, 
designers could verify and predict the worst-case voltage noise through the simulation before signing off their design.  
However, with the huge size of modern design, power grid simulation is a time-consuming process. Moreover, manifesting effects 
from the package and the board would require longer simulation time, e.g., up to few $\mu s$, which worsens the performance 
of the power grid simulation. Therefore, an efficient power grid simulation is always a demand from industry. 

Conventionally, the power grid simulation is based on the trapezoidal method where the major computation is to solve a linear 
system by either iterative approaches\cite{Saad03} or direct methods\cite{Davis06}. Many previous 
works~\cite{Chen01_Efficient}\cite{Feng08}\cite{Kozhaya02}\cite{Nassif00_Fast}\cite{Su03} utilize iterative approaches to tackle 
the scalability issue and enable adaptive stepping in the power grid simulation. However, the iterative methods usually suffer
from the convergence problem because of the ill-conditioned matrix from the power grid design. On the other hand, the direct 
methods, i.e., Cholesky or LU factorizations, are more general for solving a linear system. Despite the huge memory 
demanding and computational effort, with a carefully chosen step size, the power grid simulation could perform only one 
factorization at the beginning while the rest of operations are just backward/forward substitutions. Since a power grid design 
usually includes board and package models, a long simulation time is required to manifest the low-frequency response. Hence, 
the cost of expensive factorization can be amortized by many faster backward/forward substitutions. Such general factorization 
and fixed step size strategy~\cite{Xiong12}\cite{Yang12}\cite{Yu12}\cite{Zhao02} is widely adopted in industry.  

Beyond the traditional trapezoidal method, Weng \emph{et al.}~\cite{Weng11_ASICON}\cite{Weng12_TCAD}\cite{Weng12_ICCAD} introduced 
the matrix exponential method (MATEX) for the circuit simulation recently. MEXP has better accuracy and adaptivity because of the 
analytical formulation and the scaling invariant Krylov subspace approximation. Unlike the fixed step size strategy, MATEX could 
dynamically adjust the step size to exploit the low-frequency response of the power grid without expensive computation. However, 
the step size in MATEX is limited by the stiffness of circuit. Furthermore, MEXP has to regularize~\cite{Chen12_TCAD} the 
singularity in power grid, i.e., nodes without grounded capacitance or inductance/voltage branches. Both constraints would drag 
the overall performance of MATEX for the power grid simulation. 

In this work, we tailor MATEX using \emph{rational Krylov subspace} for the power grid simulation with adaptive time stepping. 
The rational Krylov subspace uses $(\mbf{I}-\gamma \mbf{A})^{-1}$ as the basis instead of $\mbf{A}$ used in the conventional Krylov 
subspace. The rational basis limits the spectrum of a circuit so that the exponential of a matrix can be accurately approximated 
even under a large step size. Moreover, the rational avoids $\mbf{C}^{-1}$ and thus eliminates the regularization process. 
As a result, MATEX with rational Krylov subspace is free from the stiffness constraint and the regularization process. The 
simulation can purely enjoy benefits of the adaptivity and the accuracy of MATEX. Even though the rational Krylov subspace still needs 
to solve a linear system as the trapezoidal method does, MATEX can factorize the matrix only once and then constructs the rest of 
rational Krylov subspaces by backward/forward substitutions. Therefore, MATEX can utilize its capability of adaptivity to accelerate 
the simulation with the same kernel operations as the fixed step size strategy. Overall, our MATEX has the following advantages: 
\begin{itemize}
    \item enabling adaptive time stepping for the power grid simulation with only one lu factorization.
    \item eliminating the regularization process for the singular power grid design.  
    \item allowing scaling large step size without compromising the accuracy. 
\end{itemize}
The experimental results demonstrate the effectiveness of MATEX with adaptive step size. The power grid simulation for IBM benchmark 
suite~\cite{Nassif08_Power} and industrial power grid designs can be accelerated 6X and 15X on average compared to the trapezoidal method. 

The rest of paper is organized as follows. Section~\ref{sec:preliminary} presents the background of the power grid simulation and MATEX. 
Sections~\ref{sec:rational_krylov} and~\ref{sec:adaptive_step_control} show the theoretical foundation of the rational Krylov subspace 
and our adaptive step scheme for the power grid simulation, respectively.  Section~\ref{sec:exp_results} presents experimental results 
of the IBM benchmark suite~\cite{Nassif08_Power} and several industrial power grid designs. Finally, Section~\ref{sec:conclusion} concludes 
this paper. 
%Specifically, the contributions of this work are:
%\begin{itemize} 
%    \item Enabling adaptive stepping in the power grid simulation with the computational cost of only one matrix factorization 
%	  and backward/forward substitutions. 
%    \item Using rational Krylov subspace method to ease the stiffness constraint~\cite{Weng12_TCAD}\cite{Weng12_ICCAD}, 
%	  meanwhile, endowing MATEX with the capability of dealing with singular $\mbf C$ without time-consuming 
%	  regularization process.
%\end{itemize}
%
\end{comment}



==> intro/intro_v1.tex <==

\IEEEPARstart{C}{ircuit} simulation (e.g. time domain SPICE-like)
is an important and time-consuming 
process during the cycle of integrated circuit designs.
With the increasing integration density of modern design,
billions variables are formed by modified nodal analysis in circuit simulators. 
This aggravates simulation process and costs days/weeks to finish this task.% jobs. 
The major reason is that mainstream circuit simulators inherit implicit numerical
integration, e.g. backward Euler, Trapezoidal methods, 
for the sake of stability, where the explicit methods suffer. 
However, implict methods trouble the perspective of scalability
due to the requirement 
of solving large linear systems of differential equations.
On the contrary, the explict methods are more scalable and parallelizable 
for current multi-core and manycore architecture.
The merit of explict methods resides in simple time propogation scheme via 
matrix-vector multiplication who costs relative lower
computation and memory complexity about $O(n)$.
Even though the existence of stability issue, 
explicit methods still become a revived research 
area and verifies their parallelism and scalability 
within modern parallel computer architecture
~\cite{Dong08}\cite{Dong09}\cite{Weng12_ICCAD} during these years. 

One of promising and distinct method for circuit simulation
is matrix exponetial method (MEXP) proposed in 
\cite{Weng12_TCAD}. Apart from the above numerical methods, 
the DAE/ODE system (in one discritized region of certain time step) can  
be solved in analytical way via matrix expoential operator $e^{\mbf A}, 
\mbf A \in \mbf R_{n \times n}$. 
By the analytical property, this distinct class 
of numerical approach removes the local truncation  
and it is A-\emph{stable} for passive circuits. 
Therefore, it is not constraint by the stablity problem. 
{\color{red}{This property matters!}}
%(When $h >  0, h \to \infty$, the $x(h) \to 0$). Very unlike forward
%Euler method that require small time step to let fast damp compoent
%die down first, bring too much time steps. But M
However, the kernel computation of MEXP lies in computing matrix expoential is very high,  
e.g., direct computation consumes around $O(n^3)$ complexity. 
Weng \emph{et al.} \cite{Weng12_TCAD}\cite{Weng12_ICCAD} introduced a \emph{standard Krylov subspace}
method-based MEXP for circuit simulation to solve this problem. 
In addition, unlike the implicit methods (Trapezoidal and Back Euler) 
they both require fixed step size so that they reduce the LU online for linear circuit
transient simulation,
this MEXP can utlize the scaling invariant property of Krylov subspace to do the adaptive time-steping 
without compromising any accuracy.
(1) MEXP can jump further than BE and Trap, because the exponenital 
denomator in the exponential approximation, it is much better
than the Taylor expansion.
(2) Under the (PWL) assumptions, MEXP can also carry 
the input information during the stepping.  
(3) With the help of Krylov subspace scaling invariant, it can re-evaluate
the inter time point without rebuilding Krylov subspace.

%By this strategy, it helps to capture the low frequency response from circuit system and further speedups the whole simulation without fixed step size limitation.
% In recent years, the Krylov subspace method has
Nonetheless, the step size is actually limitted by the stiffness of matrix when utilizing standard Krylov subspace.
It is because the large spectrum of $\mbf A$ and the Arnoldi process focus on capturing %the extreme magnitude
% and
well-distributed eigenvalues, so it ofter misses the dominant factors for the circuit system/for
matrix epxonential operator, which are the ones with smallest magnitudes.
Therefore, the Arnoldi process requires large number of order to preserve the 
accurate of matrix exponential calculation. 
Also, the standard Krylov-Based MEXP requires the process of regularization \cite{Chen12_TCAD} 
to deal with singular matrix $\mbf C$, i.e., nodes without grounded capacitance or 
inductance/voltage branches. Both drag the overall performance of MEXP for circuit simulation.  
% former MEXP~\cite{Weng12_TCAD} requires regularization. 
% In addition, when the matrix $\mbf C$ is stiff, it requires smaller 
%time steps or even larger Krylov subspace 
% order $m$, which degrades the method. 

In this paper, we integrated our previous works on MEXP for linear circuits 
using \emph{rational Krylov subspace}~\cite{Zhuang13_ASICON} and \emph{inverted Krylov subspace}.
%The rational Krylov subpsace uses 
They use 
$(\mbf I-\gamma \mbf A)^{-1}$ and $\mbf A^{-1}$, respectively, 
as the basis instead of $\mbf A$ (\emph{standard Krylov subspace}) in \cite{Weng12_TCAD}. 
The rational basis limits the spectrum of a circuit matrix into a unit circle,
and the inverted operation puts the important eigenvalues with smallest magnitudes from former spectrum
into a large magnitude ones. By using Arnoldi algorithm, the Hessenberg matrix can resemble the former matrix
$\mbf A$ projected onto the new invariant subspace better and contain the more accurate important eigenvalues
for matrix exponential operator.
This method provides a good convergent rate in Arnoldi process within MEXP framework.
The inverted Krylov subspace's convergent rate in Arnoldi process may not be as good as rational basis. However,
it only requires the LU factorization of conductance matrix $\mbf G$. It provides
a strategy dealing with $\mbf C$ is very complicated from post-layout extraction, but
$\mbf G$ is much more simple then. Similarly as rational basis, by the invertion $\mbf A$, the small magnitude eigenvalues 
become the large ones in the transformed spectrum, so that the exponential of a matrix can be accurately approximated.
A very typical and important application for circuit simulation is power grid analysis, which plays an 
important role in IC deisgn methodology. Given current stimulus and power grid structure, designers should verify
and pedict the worst-case voltage noise through the simulation before signing off their design. 
The model order reduction provides good way to reduce matrix of circuit system, e.g. 
PRIMA \cite{PRIMA98} and SPRIM \cite{SPRIM04}. However, with the large number of 
input sources, this kind of strategy cannot benefit from 
the reduction models any more. 
The majority works still use Trapezoidal method with fixed step size
for the power grid simulation.
Till now, accourding to Tau power grid simulation contest 2012 \cite{Li12_Tau}\cite{Yu12}, 
the trapezoidal method with fixed step size using one LU and 
many backward/forward substitutions lead to the best performance. 
The small and fixed time steps bring benefits for the transient power grid analysis 
when dealing the voltage variation 
with high frequency, i.e. the input is changing rapidly or constantly. 

However,
when package has an important impact on accurarte 
on-die power grid analysis~\cite{Pant06}\cite{Pant07}, 
and middle and low frequency phenomena is of interests to the designers, 
trapezoidal method with fixed time step becomes very inefficient. 
It is 
because such mehtod takes long time to represent the steady state of power grid system.
In the architecture analysis, power distribution networks (PDN) 
involves with pakcage and board 
level simulations \cite{PengLi12_ICCAD}\cite{Pant06}\cite{Pant07},
which requires longer timespan of simulation,
e.g. up to few $\mu s$, the simulation process are 
often time-consuming with the limitation of fixed step size to avoid online LU.
Our method can exploit large time step, ``steady region'' of waveform
during the simulation, meanwhile, it only requires one LU factoraization
as trapezoidal method, with backward/froward substitutions.
With equivalent error buget, the krylov subspace MEXP can jump larger time step/fewer 
number of time steps
than trapezoidal
method. Therefore, even though such fully implicit scheme can be used here,
when a sparse LU factorization is affordable,
the simulation burden is higher than our Krylov subspaces MEXP because of 
more time steps need.

The aim of this paper is to present and organize the Krylov subspace based 
MEXP solver in transient simulation of linear circuit.
We list our main contributions of this paper are as follows.
\begin{itemize}
\item A breakthrough of the circuit simulation matrix exponential.
\item Accelerate MEXP via rational and inverted Krylov 
subspace.
\item Using adaptive time 
stepping strategy for circuit simulation and overcome the 
problem to achieve low-frequency pheonomena of circuit system.
\item Eliminating the regularization process 
for singular matrix $\mbf C$ for explicit method 
of circuit simulation.
\item By input grouping and superposition property of linear circuit 
to further accelerate circuit simulation.
\item Establish the relation of MEXP with previous works on Model Order Reduction. 
\end{itemize}

By such contributions, we are able to achieve hihgly efficient trasient 
simulation. Compared to the works~\cite{Weng12_TCAD}.
It is very nice property from linear system, which they can be 
superposition. 
By this idea, the same system with the parts of inputs send to different
machines, cores, or threads and add together without communication 
during the process, only require on precomputed time stamp/anchors.
It is a nice parallelism framework, we provide such for the further 
extension.
It is noted that Trapezodal cannot achieve this benefit, because
it is not analytical solution, and the inputs are not the 
hurdles during their simulation but the stability and local trancation
error are.

The paper is organized as follows. Section II is the fundemantals 
of circuit simulation and matrix exponential inteperation.
Section III describes the Krylov methods for fast matrix exponential evaluations. 
They are three algorithms for such computation, Standard Krylov subspace, inverted 
Krylov subspace, Rational krylov subspace.
Section IV presents the computational results of simple linear circuit cases, also contains industrial power grid designs and the famous IBM benchmark suite.

\begin{comment}

\begin{itemize}
\item Accelerate MEXP via rational and inverted Krylov subspace and its coresponding adaptive time stepping strategy for circuit simulation.
%    \item And, summarize three Krylov strategies for MEXP, the standard/inverted/rational Krylov subspace.
%  \item Use inverted Krylov subspace, enable the krylov subspace based MEXP without regularization~\cite{Chen12_TCAD}.
\item Eliminating the regularization process for singular matrix $\mbf C$ for explicit method of circuit simulation.
\item Speedups linear circuit simulation, by adaptive time stepping.%  partitioning input sources, and using superposition,
    % \item Using block matrix for Krylov subspace generation.
    % \item Establish the relation of MEXP with previous works on Model Order Reduction. 
    % As a explicit circuit solver, which is also enjoy the model order reduction framework.
    %    \item Generalize the explict method for future parallelism circuit simulation (Stablity).
\end{itemize}
For solving ordinary differential equations $x'=Ax+f(t)$,
it has an anlytical solution $x(t+h)=e^{Ah}x(t)+ \int_{0}^{h}e^{A(h-\tau)}f(t+\tau)d\tau$. 
When $A$ is large, it is very expensive to cacluate the exponential operator directly.  
The explict and implict methods are strategies to approximate the operation of $e^{Ah}$.  
Explicit methods required matrix-by-vector multiplications, however, implicit methods need to solve 
a whole linear system.  
It is known that explicit methods are constraint on the size of the time steps required to make sure stability. 
Compared to explicit methods, Implicit methods have more difficulties on utilizing current 
parallel and distributed machines.  
Recent development of Krylov subspace accelerates the exponential operations.  
The  
\begin{itemize}
\item without regularization, 
    \item Accelerate and enpower MEXP framework via rational Krylov subspace algorithm.
    \item Enabling adaptive time stepping for circuit simulation.
    \item Establish the relation of MEXP with previous works on Model Order Reduction. As a explicit circuit solver, which is also enjoy the model order reduction framework.
    \item ?? Generalize the explict method for future parallelism circuit simulation (Stablity).
\end{itemize}
The MEXP has a good characteristic that the exponential operator bares the propagation in the perspective of
time derivitate,
which the method at Forward Euler (FE), Backward Euler (BE) and Trapezoidal (TRAP) method use time step $h$ to discretize the
dynamical system with respect to time. 
They lead to explicit and implicit methods,
which bring the stability and limitted time step due to the system, e.g. 
stiff systems.
Explicit methods are relatively cheap computation; Implicit methods are usually time consuming because they require
to solve the large linear systems. For this regard, in power grid simulation, it precomputes the matrix 
($\mbf C/h+ \mbf G$) in BE, or ($\mbf C/h + \mbf G/2$) in TRAP. This involes the time step $h$. 

Also, in linear circuit, the the mexponential operator is a explicit method, of which the matrix-vector multiplication
take the major part of computation.



Power grid simulation plays an important role in IC design methodology. Given current stimulus and the power grid structure, 
designers could verify and predict the worst-case voltage noise through the simulation before signing off their design.  
However, with the huge size of modern design, power grid simulation is a time-consuming process. Moreover, manifesting effects 
from the package and the board would require longer simulation time, e.g., up to few $\mu s$, which worsens the performance 
of the power grid simulation. Therefore, an efficient power grid simulation is always a demand from industry. 

Conventionally, the power grid simulation is based on the trapezoidal method where the major computation is to solve a linear 
system by either iterative approaches\cite{Saad03} or direct methods\cite{Davis06}. Many previous 
works~\cite{Chen01_Efficient}\cite{Feng08}\cite{Kozhaya02}\cite{Nassif00_Fast}\cite{Su03} utilize iterative approaches to tackle 
the scalability issue and enable adaptive stepping in the power grid simulation. However, the iterative methods usually suffer
from the convergence problem because of the ill-conditioned matrix from the power grid design. On the other hand, the direct 
methods, i.e., Cholesky or LU factorizations, are more general for solving a linear system. Despite the huge memory 
demanding and computational effort, with a carefully chosen step size, the power grid simulation could perform only one 
factorization at the beginning while the rest of operations are just backward/forward substitutions. Since a power grid design 
usually includes board and package models, a long simulation time is required to manifest the low-frequency response. Hence, 
the cost of expensive factorization can be amortized by many faster backward/forward substitutions. Such general factorization 
and fixed step size strategy~\cite{Xiong12}\cite{Yang12}\cite{Yu12}\cite{Zhao02} is widely adopted in industry.  

Beyond the traditional trapezoidal method, Weng \emph{et al.}~\cite{Weng11_ASICON}\cite{Weng12_TCAD}\cite{Weng12_ICCAD} introduced 
the matrix exponential method (MEXP) for the circuit simulation recently. MEXP has better accuracy and adaptivity because of the 
analytical formulation and the scaling invariant Krylov subspace approximation. Unlike the fixed step size strategy, MEXP could 
dynamically adjust the step size to exploit the low-frequency response of the power grid without expensive computation. However, 
the step size in MEXP is limited by the stiffness of circuit. Furthermore, MEXP has to regularize~\cite{Chen12_TCAD} the 
singularity in power grid, i.e., nodes without grounded capacitance or inductance/voltage branches. Both constraints would drag 
the overall performance of MEXP for the power grid simulation. 

In this work, we tailor MEXP using \emph{rational Krylov subspace} for the power grid simulation with adaptive time stepping. 
The rational Krylov subspace uses $(\mbf{I}-\gamma \mbf{A})^{-1}$ as the basis instead of $\mbf{A}$ used in the conventional Krylov 
subspace. The rational basis limits the spectrum of a circuit so that the exponential of a matrix can be accurately approximated 
even under a large step size. Moreover, the rational avoids $\mbf{C}^{-1}$ and thus eliminates the regularization process. 
As a result, MEXP with rational Krylov subspace is free from the stiffness constraint and the regularization process. The 
simulation can purely enjoy benefits of the adaptivity and the accuracy of MEXP. Even though the rational Krylov subspace still needs 
to solve a linear system as the trapezoidal method does, MEXP can factorize the matrix only once and then constructs the rest of 
rational Krylov subspaces by backward/forward substitutions. Therefore, MEXP can utilize its capability of adaptivity to accelerate 
the simulation with the same kernel operations as the fixed step size strategy. Overall, our MEXP has the following advantages: 
\begin{itemize}
    \item enabling adaptive time stepping for the power grid simulation with only one lu factorization.
    \item eliminating the regularization process for the singular power grid design.  
    \item allowing scaling large step size without compromising the accuracy. 
\end{itemize}
The experimental results demonstrate the effectiveness of MEXP with adaptive step size. The power grid simulation for IBM benchmark 
suite~\cite{Nassif08_Power} and industrial power grid designs can be accelerated 6X and 15X on average compared to the trapezoidal method. 

The rest of paper is organized as follows. Section~\ref{sec:preliminary} presents the background of the power grid simulation and MEXP. 
Sections~\ref{sec:rational_krylov} and~\ref{sec:adaptive_step_control} show the theoretical foundation of the rational Krylov subspace 
and our adaptive step scheme for the power grid simulation, respectively.  Section~\ref{sec:exp_results} presents experimental results 
of the IBM benchmark suite~\cite{Nassif08_Power} and several industrial power grid designs. Finally, Section~\ref{sec:conclusion} concludes 
this paper. 
%Specifically, the contributions of this work are:
%\begin{itemize} 
%    \item Enabling adaptive stepping in the power grid simulation with the computational cost of only one matrix factorization 
%	  and backward/forward substitutions. 
%    \item Using rational Krylov subspace method to ease the stiffness constraint~\cite{Weng12_TCAD}\cite{Weng12_ICCAD}, 
%	  meanwhile, endowing MEXP with the capability of dealing with singular $\mbf C$ without time-consuming 
%	  regularization process.
%\end{itemize}
%
\end{comment}



==> intro/intro_v3.tex <==


Circuit simulation is an important and 
{\color{red} heavily used process}
during the cycle of integrated circuit (IC) designs.
The increasing integration between functional modules and interconnects
parasitic effects of modern VLSI design aggravates such simulation tasks,
rendering the transient simulation of the full system very inefficient.
Therefore, accurate yet fast circuit simulation methods have always been 
desired in the IC industry. Theoretical sound and scalable algorithm
for linear circuit transient simulation is the building block of circuit simulators.
It provides the foundation for fast general-purpose circuit anaylsis as well as
computationally demanding power grid anaysis, and etc.
Nowadays, the emerging multi-core, many-core platforms bring powerful 
computing resource and opportunities for parallel computing. 
Even more, modern big data challenges drive cloud computing techniques \cite{cloud}, 
making distributed systems scaling to tens of thousands computing nodes
\cite{mesos, mapreduce, spark10, dryad}.
Such distributed systems are also promising computing resources in EDA and IC industry.
However, building scalable or efficient distributed transient analysis simulation framework
is still a challenge.
Previous works 
%\cite{Ye08}, \cite{Dong08}, \cite{Dong09}, \cite{Peng09},\cite{Li11}, \cite{Weng12_ICCAD}, \cite{Weng12_TCAD}
\cite{Dong08, Dong09, Li11, Peng09, Weng12_ICCAD, Weng12_TCAD, Ye08, Wang13}
have been made in order to improve circuit simulation by novel algorithmics, 
parallel processing and distributed computing.

Traditional time domain simulation solves differential algebra equations (DAEs) 
numerically in explicit ways, e.g., forward Euler (FE), or implicit ways, 
e.g., backward Euler (BE), Trapezoidal (TR).
Due to the stiffness of the euqation systems, which results from a wide range of time constants of a circuit,
the explicit methods requrie small time step sizes to ensure the stability.
However, implicit methods can conquer this problem by their larger stability
region. These implicit lmethods have to solve a linear system during each time step.
Linear systems resulted from circuit simulation is sparse and often ill conditioned.
Therefore, direct sparse matrix solver\cite{Davis06} are favored by 
linear circuit transient simulators and used as a state of art in 
current TAU power grid contest\cite{Xiong12, Yu12, Li12_Tau}. 
Only one factorization (LU or Cholesky factorization) is required
at the beginning of simulation.  
By resuing the factorization matrices, the transient computation performs only backward and forward substitions.


Beyond the traditional explict and implcit methods, 
a new class of methods called exponential
time differencing (ETD) has been embraced by 
Weng \emph{et al.} \cite{Weng11_ASICON, Weng12_TCAD} and 
applied to time domain circuit simulations,
%with matrix exponential computation by Krylov subspace approximation, 
which is called as MEXP.
The major computation of MEXP resides in calculating the matrix exponential. 
MEXP utilizes standard Krylov subspace method based on \cite{Moler03} to approximate matrix exponentials.  
These works solve the DAEs with higher 
polynomial expansion approximations \cite{Saad92} than traditional circuit simulators.
% in majority of numerical methods. 
Nevertheless, there are still constraints for above methods. 
\begin{itemize}
\item
The solutions (state of system) at input transitions are required to capture the 
system behaviour. These positions force the adaptive stepping method stop
and solve the linear systems or regenerate Krylov subspace for MEXP.
\item
The small resolution of transition distance constrains the step size of fixed time step method, 
while adaptive stepping brings matrix re-factotrization overhead.
\item
Large dimension of Krylov subspace basis or small time step is required when simulating stiff circuits, 
posing a memory bottleneck and computational burden for MEXP.
\end{itemize}
%which
%we summarize in Sec. \cite{sec:rational_krylov}.
%Recently, Zhuang, \emph{et al.} \cite{Zhuang13_ASICON} deployed
%\emph{rational} Krylov subspace method in stiff power grids to
%overcome limitation (1) and (2). 

\emph{Our Contributions}. 
%In this paper, we aim to efficent transient simulations of linear circuit. 
We devise a distributed algorithmic framework, called as \emph{MATEX}, 
of which the integral is still solved by matrix exponentials 
with variant Krylov subspace-based methods. 
%to achieve large speedups over previous MEXP. 
%To accelerate matrix exponential computation in stiff circuit simulation,  
%We generalize  \cite{Zhuang13_ASICON}
%with rational Krylov subspace 
%\cite{Zhuang13_ASICON}
\begin{itemize}
\item 
MATEX is a distributed framework by leveraging the superposition property of linear system.
By decomposing the input transition points, MATEX puts subsets of 
input transition points to different computing nodes and  process parallelly.
\begin{itemize}
\item
It reduces the chance of Krylov subspace basis generations. Besides, 
it provides more spacious time regions (before the next transtion point) 
so that matrix exponential can enjoy large adaptive time stepping only by scaling latest Krylov subspace basis.
\item
Meanwhile, traditional methods have no benefit from this decomposition, since they still need to derive
solution step by step, either do backward foward substitutions 
or adaptive stepping with solving the linear system using direct or iterative methods.
\end{itemize}
\item 
Overcome the stiffness impediment of MEXP then form an efficient circuit solver within MATEX.
\begin{itemize}
\item 
We  incorporate inverted and rational Krylov subspace bases into MATEX. 
Both reduce the dimension of basis for matrix exponential computations, 
remarkably ease the memory demands
and boost computational performance. 
\item 
After unleashing from the constraint of stiffness, MATEX uses larger time size, expediting the whole time domain simulation.
When dealing with singular capacitance/inductance matrix, 
\item
When dealing with singular capacitance/inductance matrix in DAE, these two methods 
need the regularization process \cite{Chen12_TCAD, Weng12_TCAD}, which is required 
in MEXP\cite{Weng12_TCAD} and bring computational overhead.
\end{itemize}
%, which achieve hundreds speedups over MEXP. 
\end{itemize}
\emph{Paper Organization}.
%The rest of paper is organized as follows.
Section \ref{sec:method} introduces the background of
linear circuit simulation and matrix exponential formualtions.
Section \ref{sec:matex} presents overall framework of MATEX.  
Section \ref{sec:advanced} illustrates how to accelerate MATEX's circuit solver by
utilizing inverted and rational Krylov subspace methods. 
Section \ref{sec:complexity} presents complexity analysis.
Section \ref{sec:exp_results} shows numerical results 
and Section \ref{sec:conclusion} concludes this paper.


\begin{comment}
and its adaptive time controlling into MATEX. 
During the transient simulation, 
the input changes cause the updates of matrices. 
However, the updated region resides within only columns of the matrix.
By precomputing block LU calculation beforehand and 
updating that region step by step, MATEX does not require LU factorizations on-the-fly, 
which is very different from that of TR-like methods.
%{\color{red} Only by updating small part of matrices,
%due to the input change,
%MATEX's adaptive time stepping does not require 
%LU factorization on-the-fly.}

We also combine MATEX %together 
with \emph{inverted Krylov subspace} as an alternative technique,
which only requires decomposing the conductance matrix. 
Therefore,
it is advantageous the avoidance of inverting the 
matrix of capacitance and inductance, which may 
include many parasitic energy elements 
with large magnitude variations
after circuit extraction.
%{\color{red}{The connections of these two methods are inspired by the works 
%from model order reduction community, \emph{i.e.,}
%PRIMA \cite{PRIMA98} and SPRIM \cite{SPRIM04}.}}

%These solve the limitations (1) and (2);
Additionally, the parallelism of MATEX
is based on the superposition property of linear circuit.
Within our theoritically sound skeleton,
we split the input sources, use all of divided subset of input sources 
to stimuli the system, seperately, %and efficiently adaptive time stepping,
making the whole simulation task divided
into serveral sub-tasks. 
% and solved seperately 
These sub-tasks can be solved parallel, without sacrificing any accuracy. 
This circumvents the limitation (3).
Besides, the traditional methods (FE, BE, and TR) cannot benefit from this
splitting, due to their limitations not from the side of input sources
but from LTE and stability.
With the advent of inexpensive computer clusters, and multi/many-core technology,
this distributable algorithmic framework is a nice one for future implementations.


\begin{comment}


The major reason is that mainstream circuit simulators inherit implicit numerical
integration, e.g. backward Euler, Trapezoidal methods, 
for the sake of stability, where the explicit methods suffer. 
However, implict methods trouble the perspective of scalability
due to the requirement 
of solving large linear systems of differential equations.
On the contrary, the explict methods are more scalable and parallelizable 
for current multi-core and manycore architecture.
The merit of explict methods resides in simple time propogation scheme via 
matrix-vector multiplication who costs relative lower
computation and memory complexity about $O(n)$.
Even though the existence of stability issue, 
explicit methods still become a revived research 
area and verifies their parallelism and scalability 
within modern parallel computer architecture
~\cite{Dong08}\cite{Dong09}\cite{Weng12_ICCAD} during these years. 

One of promising and distinct method for circuit simulation
is matrix exponetial method (MATEX) proposed in 
\cite{Weng12_TCAD}. Apart from the above numerical methods, 
the DAE/ODE system (in one discritized region of certain time step) can  
be solved in analytical way via matrix expoential operator $e^{\mbf A}, 
\mbf A \in \mbf R_{n \times n}$. 
By the analytical property, this distinct class 
of numerical approach removes the local truncation  
and it is A-\emph{stable} for passive circuits. 
Therefore, it is not constraint by the stablity problem. 
{\color{red}{This property matters!}}
%(When $h >  0, h \to \infty$, the $x(h) \to 0$). Very unlike forward
%Euler method that require small time step to let fast damp compoent
%die down first, bring too much time steps. But M
However, the kernel computation of MATEX lies in computing matrix expoential is very high,  
e.g., direct computation consumes around $O(n^3)$ complexity. 
Weng \emph{et al.} \cite{Weng12_TCAD}\cite{Weng12_ICCAD} introduced a \emph{standard Krylov subspace}
method-based MATEX for circuit simulation to solve this problem. 
In addition, unlike the implicit methods (Trapezoidal and Back Euler) 
they both require fixed step size so that they reduce the LU online for linear circuit
transient simulation,
this MATEX can utlize the scaling invariant property of Krylov subspace to do the adaptive time-steping 
without compromising any accuracy.
(1) MATEX can jump further than BE and Trap, because the exponenital 
denomator in the exponential approximation, it is much better
than the Taylor expansion.
(2) Under the (PWL) assumptions, MATEX can also carry 
the input information during the stepping.  
(3) With the help of Krylov subspace scaling invariant, it can re-evaluate
the inter time point without rebuilding Krylov subspace.

%By this strategy, it helps to capture the low frequency response from circuit system and further speedups the whole simulation without fixed step size limitation.
% In recent years, the Krylov subspace method has
Nonetheless, the step size is actually limitted by the stiffness of matrix when utilizing standard Krylov subspace.
It is because the large spectrum of $\mbf A$ and the Arnoldi process focus on capturing %the extreme magnitude
% and
well-distributed eigenvalues, so it ofter misses the dominant factors for the circuit system/for
matrix epxonential operator, which are the ones with smallest magnitudes.
Therefore, the Arnoldi process requires large number of order to preserve the 
accurate of matrix exponential calculation. 
Also, the standard Krylov-Based MATEX requires the process of regularization \cite{Chen12_TCAD} 
to deal with singular matrix $\mbf C$, i.e., nodes without grounded capacitance or 
inductance/voltage branches. Both drag the overall performance of MATEX for circuit simulation.  
% former MATEX~\cite{Weng12_TCAD} requires regularization. 
% In addition, when the matrix $\mbf C$ is stiff, it requires smaller 
%time steps or even larger Krylov subspace 
% order $m$, which degrades the method. 


In this paper, we integrated our previous works on MATEX for linear circuits 
using \emph{rational Krylov subspace}~\cite{Zhuang13_ASICON} and \emph{inverted Krylov subspace}.
%The rational Krylov subpsace uses 
They use 
$(\mbf I-\gamma \mbf A)^{-1}$ and $\mbf A^{-1}$, respectively, 
as the basis instead of $\mbf A$ (\emph{standard Krylov subspace}) in \cite{Weng12_TCAD}. 
The rational basis limits the spectrum of a circuit matrix into a unit circle,
and the inverted operation puts the important eigenvalues with smallest magnitudes from former spectrum
into a large magnitude ones. By using Arnoldi algorithm, the Hessenberg matrix can resemble the former matrix
$\mbf A$ projected onto the new invariant subspace better and contain the more accurate important eigenvalues
for matrix exponential operator.
This method provides a good convergent rate in Arnoldi process within MATEX framework.
The inverted Krylov subspace's convergent rate in Arnoldi process may not be as good as rational basis. However,
it only requires the LU factorization of conductance matrix $\mbf G$. It provides
a strategy dealing with $\mbf C$ is very complicated from post-layout extraction, but
$\mbf G$ is much more simple then. Similarly as rational basis, by the invertion $\mbf A$, the small magnitude eigenvalues 
become the large ones in the transformed spectrum, so that the exponential of a matrix can be accurately approximated.
A very typical and important application for circuit simulation is power grid analysis, which plays an 
important role in IC deisgn methodology. Given current stimulus and power grid structure, designers should verify
and pedict the worst-case voltage noise through the simulation before signing off their design. 
The model order reduction provides good way to reduce matrix of circuit system, e.g. 
PRIMA \cite{PRIMA98} and SPRIM \cite{SPRIM04}. However, with the large number of 
input sources, this kind of strategy cannot benefit from 
the reduction models any more. 
The majority works still use Trapezoidal method with fixed step size
for the power grid simulation.
Till now, accourding to Tau power grid simulation contest 2012 \cite{Li12_Tau}\cite{Yu12}, 
the trapezoidal method with fixed step size using one LU and 
many backward/forward substitutions lead to the best performance. 
The small and fixed time steps bring benefits for the transient power grid analysis 
when dealing the voltage variation 
with high frequency, i.e. the input is changing rapidly or constantly. 

However,
when package has an important impact on accurarte 
on-die power grid analysis~\cite{Pant06}\cite{Pant07}, 
and middle and low frequency phenomena is of interests to the designers, 
trapezoidal method with fixed time step becomes very inefficient. 
It is 
because such mehtod takes long time to represent the steady state of power grid system.
In the architecture analysis, power distribution networks (PDN) 
involves with pakcage and board 
level simulations \cite{PengLi12_ICCAD}\cite{Pant06}\cite{Pant07},
which requires longer timespan of simulation,
e.g. up to few $\mu s$, the simulation process are 
often time-consuming with the limitation of fixed step size to avoid online LU.
Our method can exploit large time step, ``steady region'' of waveform
during the simulation, meanwhile, it only requires one LU factoraization
as trapezoidal method, with backward/froward substitutions.
With equivalent error buget, the krylov subspace MATEX can jump larger time step/fewer 
number of time steps
than trapezoidal
method. Therefore, even though such fully implicit scheme can be used here,
when a sparse LU factorization is affordable,
the simulation burden is higher than our Krylov subspaces MATEX because of 
more time steps need.

The aim of this paper is to present and organize the Krylov subspace based 
MATEX solver in transient simulation of linear circuit.
We list our main contributions of this paper are as follows.
\begin{itemize}
%\item A breakthrough of the circuit simulation matrix exponential.
\item Accelerate MATEX via rational and inverted Krylov 
subspace.
\item Using adaptive time 
stepping strategy for circuit simulation and overcome the 
problem to achieve low-frequency pheonomena of circuit system.
\item Eliminating the regularization process 
for singular matrix $\mbf C$ for explicit method 
of circuit simulation.
\item By input grouping and superposition property of linear circuit 
to further accelerate circuit simulation.
\item Establish the relation of MATEX with previous works on Model Order Reduction. 
\end{itemize}

By such contributions, we are able to achieve hihgly efficient trasient 
simulation. Compared to the works~\cite{Weng12_TCAD}.
It is very nice property from linear system, which they can be 
superposition. 
By this idea, the same system with the parts of inputs send to different
machines, cores, or threads and add together without communication 
during the process, only require on precomputed time stamp/anchors.
It is a nice parallelism framework, we provide such for the further 
extension.
It is noted that Trapezodal cannot achieve this benefit, because
it is not analytical solution, and the inputs are not the 
hurdles during their simulation but the stability and local trancation
error are.

The paper is organized as follows. Section II is the fundemantals 
of circuit simulation and matrix exponential inteperation.
Section III describes the Krylov methods for fast matrix exponential evaluations. 
They are three algorithms for such computation, Standard Krylov subspace, inverted 
Krylov subspace, Rational krylov subspace.
Section IV presents the computational results of simple linear circuit cases, also contains industrial power grid designs and the famous IBM benchmark suite.

\begin{comment}

\begin{itemize}
\item Accelerate MATEX via rational and inverted Krylov subspace and its coresponding adaptive time stepping strategy for circuit simulation.
%    \item And, summarize three Krylov strategies for MATEX, the standard/inverted/rational Krylov subspace.
%  \item Use inverted Krylov subspace, enable the krylov subspace based MATEX without regularization~\cite{Chen12_TCAD}.
\item Eliminating the regularization process for singular matrix $\mbf C$ for explicit method of circuit simulation.
\item Speedups linear circuit simulation, by adaptive time stepping.%  partitioning input sources, and using superposition,
    % \item Using block matrix for Krylov subspace generation.
    % \item Establish the relation of MATEX with previous works on Model Order Reduction. 
    % As a explicit circuit solver, which is also enjoy the model order reduction framework.
    %    \item Generalize the explict method for future parallelism circuit simulation (Stablity).
\end{itemize}
For solving ordinary differential equations $x'=Ax+f(t)$,
it has an anlytical solution $x(t+h)=e^{Ah}x(t)+ \int_{0}^{h}e^{A(h-\tau)}f(t+\tau)d\tau$. 
When $A$ is large, it is very expensive to cacluate the exponential operator directly.  
The explict and implict methods are strategies to approximate the operation of $e^{Ah}$.  
Explicit methods required matrix-by-vector multiplications, however, implicit methods need to solve 
a whole linear system.  
It is known that explicit methods are constraint on the size of the time steps required to make sure stability. 
Compared to explicit methods, Implicit methods have more difficulties on utilizing current 
parallel and distributed machines.  
Recent development of Krylov subspace accelerates the exponential operations.  
The  
\begin{itemize}
\item without regularization, 
    \item Accelerate and enpower MATEX framework via rational Krylov subspace algorithm.
    \item Enabling adaptive time stepping for circuit simulation.
    \item Establish the relation of MATEX with previous works on Model Order Reduction. As a explicit circuit solver, which is also enjoy the model order reduction framework.
    \item ?? Generalize the explict method for future parallelism circuit simulation (Stablity).
\end{itemize}
The MATEX has a good characteristic that the exponential operator bares the propagation in the perspective of
time derivitate,
which the method at Forward Euler (FE), Backward Euler (BE) and Trapezoidal (TRAP) method use time step $h$ to discretize the
dynamical system with respect to time. 
They lead to explicit and implicit methods,
which bring the stability and limitted time step due to the system, e.g. 
stiff systems.
Explicit methods are relatively cheap computation; Implicit methods are usually time consuming because they require
to solve the large linear systems. For this regard, in power grid simulation, it precomputes the matrix 
($\mbf C/h+ \mbf G$) in BE, or ($\mbf C/h + \mbf G/2$) in TRAP. This involes the time step $h$. 

Also, in linear circuit, the the mexponential operator is a explicit method, of which the matrix-vector multiplication
take the major part of computation.



Power grid simulation plays an important role in IC design methodology. Given current stimulus and the power grid structure, 
designers could verify and predict the worst-case voltage noise through the simulation before signing off their design.  
However, with the huge size of modern design, power grid simulation is a time-consuming process. Moreover, manifesting effects 
from the package and the board would require longer simulation time, e.g., up to few $\mu s$, which worsens the performance 
of the power grid simulation. Therefore, an efficient power grid simulation is always a demand from industry. 

Conventionally, the power grid simulation is based on the trapezoidal method where the major computation is to solve a linear 
system by either iterative approaches\cite{Saad03} or direct methods\cite{Davis06}. Many previous 
works~\cite{Chen01_Efficient}\cite{Feng08}\cite{Kozhaya02}\cite{Nassif00_Fast}\cite{Su03} utilize iterative approaches to tackle 
the scalability issue and enable adaptive stepping in the power grid simulation. However, the iterative methods usually suffer
from the convergence problem because of the ill-conditioned matrix from the power grid design. On the other hand, the direct 
methods, i.e., Cholesky or LU factorizations, are more general for solving a linear system. Despite the huge memory 
demanding and computational effort, with a carefully chosen step size, the power grid simulation could perform only one 
factorization at the beginning while the rest of operations are just backward/forward substitutions. Since a power grid design 
usually includes board and package models, a long simulation time is required to manifest the low-frequency response. Hence, 
the cost of expensive factorization can be amortized by many faster backward/forward substitutions. Such general factorization 
and fixed step size strategy~\cite{Xiong12}\cite{Yang12}\cite{Yu12}\cite{Zhao02} is widely adopted in industry.  

Beyond the traditional trapezoidal method, Weng \emph{et al.}~\cite{Weng11_ASICON}\cite{Weng12_TCAD}\cite{Weng12_ICCAD} introduced 
the matrix exponential method (MATEX) for the circuit simulation recently. MEXP has better accuracy and adaptivity because of the 
analytical formulation and the scaling invariant Krylov subspace approximation. Unlike the fixed step size strategy, MATEX could 
dynamically adjust the step size to exploit the low-frequency response of the power grid without expensive computation. However, 
the step size in MATEX is limited by the stiffness of circuit. Furthermore, MEXP has to regularize~\cite{Chen12_TCAD} the 
singularity in power grid, i.e., nodes without grounded capacitance or inductance/voltage branches. Both constraints would drag 
the overall performance of MATEX for the power grid simulation. 

In this work, we tailor MATEX using \emph{rational Krylov subspace} for the power grid simulation with adaptive time stepping. 
The rational Krylov subspace uses $(\mbf{I}-\gamma \mbf{A})^{-1}$ as the basis instead of $\mbf{A}$ used in the conventional Krylov 
subspace. The rational basis limits the spectrum of a circuit so that the exponential of a matrix can be accurately approximated 
even under a large step size. Moreover, the rational avoids $\mbf{C}^{-1}$ and thus eliminates the regularization process. 
As a result, MATEX with rational Krylov subspace is free from the stiffness constraint and the regularization process. The 
simulation can purely enjoy benefits of the adaptivity and the accuracy of MATEX. Even though the rational Krylov subspace still needs 
to solve a linear system as the trapezoidal method does, MATEX can factorize the matrix only once and then constructs the rest of 
rational Krylov subspaces by backward/forward substitutions. Therefore, MATEX can utilize its capability of adaptivity to accelerate 
the simulation with the same kernel operations as the fixed step size strategy. Overall, our MATEX has the following advantages: 
\begin{itemize}
    \item enabling adaptive time stepping for the power grid simulation with only one lu factorization.
    \item eliminating the regularization process for the singular power grid design.  
    \item allowing scaling large step size without compromising the accuracy. 
\end{itemize}
The experimental results demonstrate the effectiveness of MATEX with adaptive step size. The power grid simulation for IBM benchmark 
suite~\cite{Nassif08_Power} and industrial power grid designs can be accelerated 6X and 15X on average compared to the trapezoidal method. 

The rest of paper is organized as follows. Section~\ref{sec:preliminary} presents the background of the power grid simulation and MATEX. 
Sections~\ref{sec:rational_krylov} and~\ref{sec:adaptive_step_control} show the theoretical foundation of the rational Krylov subspace 
and our adaptive step scheme for the power grid simulation, respectively.  Section~\ref{sec:exp_results} presents experimental results 
of the IBM benchmark suite~\cite{Nassif08_Power} and several industrial power grid designs. Finally, Section~\ref{sec:conclusion} concludes 
this paper. 
%Specifically, the contributions of this work are:
%\begin{itemize} 
%    \item Enabling adaptive stepping in the power grid simulation with the computational cost of only one matrix factorization 
%	  and backward/forward substitutions. 
%    \item Using rational Krylov subspace method to ease the stiffness constraint~\cite{Weng12_TCAD}\cite{Weng12_ICCAD}, 
%	  meanwhile, endowing MATEX with the capability of dealing with singular $\mbf C$ without time-consuming 
%	  regularization process.
%\end{itemize}
%
\end{comment}



==> intro/intro_v4.tex <==


\begin{comment}
Circuit simulation is an important and 
{\color{red} heavily used process}
during the cycle of integrated circuit (IC) designs.
The increasing integration between functional modules and interconnects
parasitic effects of modern VLSI design aggravates such simulation tasks,
rendering the transient simulation of the full system very inefficient.
Therefore, accurate yet fast circuit simulation methods have always been 
desired in the IC industry. 
\end{comment}
Theoretical sound and scalable algorithms
for linear circuit transient simulation have been always favored in the IC industry. 
It is the building block of all circuit simulators, 
which not only provides the foundation for fast general-purpose circuit anaylsis 
but also shapen the edge dealing with modern computationally demanding power grid anaysis.
Nowadays, the emerging multi-core, many-core platforms bring powerful 
computing resource and opportunities for parallel computing. 
Even more, modern big data challenges drive cloud computing techniques \cite{cloud}, 
making distributed systems scaling to tens of thousands computing nodes
\cite{mesos, mapreduce, spark10, dryad}.
Such distributed systems will be also promising computing resources in EDA and IC industry.
However, building scalable and efficient distributed algorithmic framework for 
transient linear circuit simulation framework is still a challenge to leverage these powerful computing tools.
Previous works 
%\cite{Ye08}, \cite{Dong08}, \cite{Dong09}, \cite{Peng09},\cite{Li11}, \cite{Weng12_ICCAD}, \cite{Weng12_TCAD}
\cite{Dong08, Dong09, Li11, Weng12_ICCAD, Weng12_TCAD, Ye08, Wang13}
have been made in order to improve circuit simulation by novel algorithmics, 
parallel processing and distributed computing.

Traditional method solves differential algebra equations (DAEs) 
numerically in explicit ways, e.g., forward Euler (FE), or implicit ways, 
e.g., backward Euler (BE), Trapezoidal (TR), which are based on low order polynomial approximations for DAE.
Due to the stiffness of systems, which results from a wide range of time constants of a circuit,
the explicit methods requrie small time step sizes to ensure the stability.
However, implicit methods can conquer this problem by their larger stability
region. These implicit lmethods have to solve a linear system during each time step.
Linear systems resulted from circuit simulation is sparse and often ill conditioned.
Therefore, direct sparse matrix solver\cite{Davis06} are favored by 
linear circuit transient simulators and used as a state of art in 
current TAU power grid contest. 
There, only one factorization (LU or Cholesky factorization) is required
at the beginning of simulation.  
By resuing the factorization matrices, 
the transient computation performs only backward and forward substitions 
and achieves better efficiency over adaptive stepping methods \cite{Xiong12, Yu12, Li12_Tau}.

Beyond the traditional ones, 
a new class of methods called exponential
time differencing (ETD) has been embraced by 
Weng \emph{et al.} \cite{Weng12_TCAD} 
%and 
%applied to time domain circuit simulations,
%with matrix exponential computation by Krylov subspace approximation, 
which is called as MEXP.
The major computation of MEXP resides in calculating the matrix exponential. 
MEXP utilizes standard Krylov subspace method based on \cite{Moler03} to approximate matrix exponentials.  
These works solve the DAEs with higher 
polynomial expansion approximations \cite{Saad92} than traditional ones.
Another merit of using MEXP-like SPICE simulation for linear circuit is 
the adaptive time stepping can be proceeded without
refactorizing the matrix on-the-fly, while the traditional counterparts cannot avoid such time counsuming process.
% in majority of numerical methods. 
Nevertheless, there are still constraints for above methods. 

-- The solutions (state of system) at input transitions are required to solved and capture the 
system behaviour, which force the adaptive stepping method to stop
and solve the linear systems or MEXP to regenerate Krylov subspace basis.

-- The small resolution of transition distance constrains the step size of fixed time step method, 
while resorting to adaptive stepping alternatively brings matrix re-factotrization overhead.

-- Large dimension of Krylov subspace basis or small time step is needed to preserve the accuracy of
matrix exponential approximation when simulating stiff circuits, 
posing a memory bottleneck and computational burden for MEXP.

\emph{Our Contributions}. 
%In this paper, we aim to efficent transient simulations of linear circuit. 
We devise a distributed algorithmic framework, called as \emph{MATEX}, 
of which the circuit solver is still based on matrix exponentials. 
%with variant Krylov subspace-based methods. 
%to achieve large speedups over previous MEXP. 
%To accelerate matrix exponential computation in stiff circuit simulation,  
%We generalize  \cite{Zhuang13_ASICON}
%with rational Krylov subspace 
%\cite{Zhuang13_ASICON}

-- MATEX is a distributed framework by leveraging the superposition property of linear system.
Through decomposing the input transition points, MATEX puts subsets of 
input transition points to different computing nodes and  process parallelly.
(1) In each computing node, it locally reduces the chance of Krylov subspace basis generations,
and provides more spacious time regions (before the next transtion point) 
so that its circuit solver can enjoy large adaptive time stepping only by scaling latest Krylov subspace basis.
(2) Meanwhile, traditional methods cannot benefit from this decomposition, since they still need to derive
solution step by step, either performing backward foward substitutions 
or adaptive stepping with solving the linear system using direct or iterative methods.

-- Overcome the stiffness impediment of MEXP then form an efficient circuit solver within MATEX.
(1) We  incorporate inverted and rational Krylov subspace bases into MATEX. 
Both reduce the dimension of basis for matrix exponential computations, 
remarkably ease the memory cousumptions 
and boost computational performance. 
(2) After unleashing from the constraint of stiffness, MATEX uses larger time size, expediting the whole time domain simulation.
%When dealing with singular capacitance/inductance matrix, 
(3) When dealing with singular capacitance/inductance matrix in DAE, these methods removes 
regularization process \cite{Chen12_TCAD, Weng12_TCAD}, which is required 
in MEXP\cite{Weng12_TCAD} and bring extra computational overhead.
\emph{Paper Organization}.
%The rest of paper is organized as follows.
Section \ref{sec:method} introduces the background of
linear circuit simulation and matrix exponential formualtions.
Section \ref{sec:matex} presents overall framework of MATEX.  
Section \ref{sec:advanced} illustrates the techniques to accelerate MATEX's circuit solver by
utilizing inverted and rational Krylov subspace methods. 
Section \ref{sec:complexity} presents complexity analysis.
Section \ref{sec:exp_results} shows numerical results 
and Section \ref{sec:conclusion} concludes this paper.


\begin{comment}
and its adaptive time controlling into MATEX. 
During the transient simulation, 
the input changes cause the updates of matrices. 
However, the updated region resides within only columns of the matrix.
By precomputing block LU calculation beforehand and 
updating that region step by step, MATEX does not require LU factorizations on-the-fly, 
which is very different from that of TR-like methods.
%{\color{red} Only by updating small part of matrices,
%due to the input change,
%MATEX's adaptive time stepping does not require 
%LU factorization on-the-fly.}

We also combine MATEX %together 
with \emph{inverted Krylov subspace} as an alternative technique,
which only requires decomposing the conductance matrix. 
Therefore,
it is advantageous the avoidance of inverting the 
matrix of capacitance and inductance, which may 
include many parasitic energy elements 
with large magnitude variations
after circuit extraction.
%{\color{red}{The connections of these two methods are inspired by the works 
%from model order reduction community, \emph{i.e.,}
%PRIMA \cite{PRIMA98} and SPRIM \cite{SPRIM04}.}}

%These solve the limitations (1) and (2);
Additionally, the parallelism of MATEX
is based on the superposition property of linear circuit.
Within our theoritically sound skeleton,
we split the input sources, use all of divided subset of input sources 
to stimuli the system, seperately, %and efficiently adaptive time stepping,
making the whole simulation task divided
into serveral sub-tasks. 
% and solved seperately 
These sub-tasks can be solved parallel, without sacrificing any accuracy. 
This circumvents the limitation (3).
Besides, the traditional methods (FE, BE, and TR) cannot benefit from this
splitting, due to their limitations not from the side of input sources
but from LTE and stability.
With the advent of inexpensive computer clusters, and multi/many-core technology,
this distributable algorithmic framework is a nice one for future implementations.


\begin{comment}


The major reason is that mainstream circuit simulators inherit implicit numerical
integration, e.g. backward Euler, Trapezoidal methods, 
for the sake of stability, where the explicit methods suffer. 
However, implict methods trouble the perspective of scalability
due to the requirement 
of solving large linear systems of differential equations.
On the contrary, the explict methods are more scalable and parallelizable 
for current multi-core and manycore architecture.
The merit of explict methods resides in simple time propogation scheme via 
matrix-vector multiplication who costs relative lower
computation and memory complexity about $O(n)$.
Even though the existence of stability issue, 
explicit methods still become a revived research 
area and verifies their parallelism and scalability 
within modern parallel computer architecture
~\cite{Dong08}\cite{Dong09}\cite{Weng12_ICCAD} during these years. 

One of promising and distinct method for circuit simulation
is matrix exponetial method (MATEX) proposed in 
\cite{Weng12_TCAD}. Apart from the above numerical methods, 
the DAE/ODE system (in one discritized region of certain time step) can  
be solved in analytical way via matrix expoential operator $e^{\mbf A}, 
\mbf A \in \mbf R_{n \times n}$. 
By the analytical property, this distinct class 
of numerical approach removes the local truncation  
and it is A-\emph{stable} for passive circuits. 
Therefore, it is not constraint by the stablity problem. 
{\color{red}{This property matters!}}
%(When $h >  0, h \to \infty$, the $x(h) \to 0$). Very unlike forward
%Euler method that require small time step to let fast damp compoent
%die down first, bring too much time steps. But M
However, the kernel computation of MATEX lies in computing matrix expoential is very high,  
e.g., direct computation consumes around $O(n^3)$ complexity. 
Weng \emph{et al.} \cite{Weng12_TCAD}\cite{Weng12_ICCAD} introduced a \emph{standard Krylov subspace}
method-based MATEX for circuit simulation to solve this problem. 
In addition, unlike the implicit methods (Trapezoidal and Back Euler) 
they both require fixed step size so that they reduce the LU online for linear circuit
transient simulation,
this MATEX can utlize the scaling invariant property of Krylov subspace to do the adaptive time-steping 
without compromising any accuracy.
(1) MATEX can jump further than BE and Trap, because the exponenital 
denomator in the exponential approximation, it is much better
than the Taylor expansion.
(2) Under the (PWL) assumptions, MATEX can also carry 
the input information during the stepping.  
(3) With the help of Krylov subspace scaling invariant, it can re-evaluate
the inter time point without rebuilding Krylov subspace.

%By this strategy, it helps to capture the low frequency response from circuit system and further speedups the whole simulation without fixed step size limitation.
% In recent years, the Krylov subspace method has
Nonetheless, the step size is actually limitted by the stiffness of matrix when utilizing standard Krylov subspace.
It is because the large spectrum of $\mbf A$ and the Arnoldi process focus on capturing %the extreme magnitude
% and
well-distributed eigenvalues, so it ofter misses the dominant factors for the circuit system/for
matrix epxonential operator, which are the ones with smallest magnitudes.
Therefore, the Arnoldi process requires large number of order to preserve the 
accurate of matrix exponential calculation. 
Also, the standard Krylov-Based MATEX requires the process of regularization \cite{Chen12_TCAD} 
to deal with singular matrix $\mbf C$, i.e., nodes without grounded capacitance or 
inductance/voltage branches. Both drag the overall performance of MATEX for circuit simulation.  
% former MATEX~\cite{Weng12_TCAD} requires regularization. 
% In addition, when the matrix $\mbf C$ is stiff, it requires smaller 
%time steps or even larger Krylov subspace 
% order $m$, which degrades the method. 


In this paper, we integrated our previous works on MATEX for linear circuits 
using \emph{rational Krylov subspace}~\cite{Zhuang13_ASICON} and \emph{inverted Krylov subspace}.
%The rational Krylov subpsace uses 
They use 
$(\mbf I-\gamma \mbf A)^{-1}$ and $\mbf A^{-1}$, respectively, 
as the basis instead of $\mbf A$ (\emph{standard Krylov subspace}) in \cite{Weng12_TCAD}. 
The rational basis limits the spectrum of a circuit matrix into a unit circle,
and the inverted operation puts the important eigenvalues with smallest magnitudes from former spectrum
into a large magnitude ones. By using Arnoldi algorithm, the Hessenberg matrix can resemble the former matrix
$\mbf A$ projected onto the new invariant subspace better and contain the more accurate important eigenvalues
for matrix exponential operator.
This method provides a good convergent rate in Arnoldi process within MATEX framework.
The inverted Krylov subspace's convergent rate in Arnoldi process may not be as good as rational basis. However,
it only requires the LU factorization of conductance matrix $\mbf G$. It provides
a strategy dealing with $\mbf C$ is very complicated from post-layout extraction, but
$\mbf G$ is much more simple then. Similarly as rational basis, by the invertion $\mbf A$, the small magnitude eigenvalues 
become the large ones in the transformed spectrum, so that the exponential of a matrix can be accurately approximated.
A very typical and important application for circuit simulation is power grid analysis, which plays an 
important role in IC deisgn methodology. Given current stimulus and power grid structure, designers should verify
and pedict the worst-case voltage noise through the simulation before signing off their design. 
The model order reduction provides good way to reduce matrix of circuit system, e.g. 
PRIMA \cite{PRIMA98} and SPRIM \cite{SPRIM04}. However, with the large number of 
input sources, this kind of strategy cannot benefit from 
the reduction models any more. 
The majority works still use Trapezoidal method with fixed step size
for the power grid simulation.
Till now, accourding to Tau power grid simulation contest 2012 \cite{Li12_Tau}\cite{Yu12}, 
the trapezoidal method with fixed step size using one LU and 
many backward/forward substitutions lead to the best performance. 
The small and fixed time steps bring benefits for the transient power grid analysis 
when dealing the voltage variation 
with high frequency, i.e. the input is changing rapidly or constantly. 

However,
when package has an important impact on accurarte 
on-die power grid analysis~\cite{Pant06}\cite{Pant07}, 
and middle and low frequency phenomena is of interests to the designers, 
trapezoidal method with fixed time step becomes very inefficient. 
It is 
because such mehtod takes long time to represent the steady state of power grid system.
In the architecture analysis, power distribution networks (PDN) 
involves with pakcage and board 
level simulations \cite{PengLi12_ICCAD}\cite{Pant06}\cite{Pant07},
which requires longer timespan of simulation,
e.g. up to few $\mu s$, the simulation process are 
often time-consuming with the limitation of fixed step size to avoid online LU.
Our method can exploit large time step, ``steady region'' of waveform
during the simulation, meanwhile, it only requires one LU factoraization
as trapezoidal method, with backward/froward substitutions.
With equivalent error buget, the krylov subspace MATEX can jump larger time step/fewer 
number of time steps
than trapezoidal
method. Therefore, even though such fully implicit scheme can be used here,
when a sparse LU factorization is affordable,
the simulation burden is higher than our Krylov subspaces MATEX because of 
more time steps need.

The aim of this paper is to present and organize the Krylov subspace based 
MATEX solver in transient simulation of linear circuit.
We list our main contributions of this paper are as follows.
\begin{itemize}
%\item A breakthrough of the circuit simulation matrix exponential.
\item Accelerate MATEX via rational and inverted Krylov 
subspace.
\item Using adaptive time 
stepping strategy for circuit simulation and overcome the 
problem to achieve low-frequency pheonomena of circuit system.
\item Eliminating the regularization process 
for singular matrix $\mbf C$ for explicit method 
of circuit simulation.
\item By input grouping and superposition property of linear circuit 
to further accelerate circuit simulation.
\item Establish the relation of MATEX with previous works on Model Order Reduction. 
\end{itemize}

By such contributions, we are able to achieve hihgly efficient trasient 
simulation. Compared to the works~\cite{Weng12_TCAD}.
It is very nice property from linear system, which they can be 
superposition. 
By this idea, the same system with the parts of inputs send to different
machines, cores, or threads and add together without communication 
during the process, only require on precomputed time stamp/anchors.
It is a nice parallelism framework, we provide such for the further 
extension.
It is noted that Trapezodal cannot achieve this benefit, because
it is not analytical solution, and the inputs are not the 
hurdles during their simulation but the stability and local trancation
error are.

The paper is organized as follows. Section II is the fundemantals 
of circuit simulation and matrix exponential inteperation.
Section III describes the Krylov methods for fast matrix exponential evaluations. 
They are three algorithms for such computation, Standard Krylov subspace, inverted 
Krylov subspace, Rational krylov subspace.
Section IV presents the computational results of simple linear circuit cases, also contains industrial power grid designs and the famous IBM benchmark suite.

\begin{comment}

\begin{itemize}
\item Accelerate MATEX via rational and inverted Krylov subspace and its coresponding adaptive time stepping strategy for circuit simulation.
%    \item And, summarize three Krylov strategies for MATEX, the standard/inverted/rational Krylov subspace.
%  \item Use inverted Krylov subspace, enable the krylov subspace based MATEX without regularization~\cite{Chen12_TCAD}.
\item Eliminating the regularization process for singular matrix $\mbf C$ for explicit method of circuit simulation.
\item Speedups linear circuit simulation, by adaptive time stepping.%  partitioning input sources, and using superposition,
    % \item Using block matrix for Krylov subspace generation.
    % \item Establish the relation of MATEX with previous works on Model Order Reduction. 
    % As a explicit circuit solver, which is also enjoy the model order reduction framework.
    %    \item Generalize the explict method for future parallelism circuit simulation (Stablity).
\end{itemize}
For solving ordinary differential equations $x'=Ax+f(t)$,
it has an anlytical solution $x(t+h)=e^{Ah}x(t)+ \int_{0}^{h}e^{A(h-\tau)}f(t+\tau)d\tau$. 
When $A$ is large, it is very expensive to cacluate the exponential operator directly.  
The explict and implict methods are strategies to approximate the operation of $e^{Ah}$.  
Explicit methods required matrix-by-vector multiplications, however, implicit methods need to solve 
a whole linear system.  
It is known that explicit methods are constraint on the size of the time steps required to make sure stability. 
Compared to explicit methods, Implicit methods have more difficulties on utilizing current 
parallel and distributed machines.  
Recent development of Krylov subspace accelerates the exponential operations.  
The  
\begin{itemize}
\item without regularization, 
    \item Accelerate and enpower MATEX framework via rational Krylov subspace algorithm.
    \item Enabling adaptive time stepping for circuit simulation.
    \item Establish the relation of MATEX with previous works on Model Order Reduction. As a explicit circuit solver, which is also enjoy the model order reduction framework.
    \item ?? Generalize the explict method for future parallelism circuit simulation (Stablity).
\end{itemize}
The MATEX has a good characteristic that the exponential operator bares the propagation in the perspective of
time derivitate,
which the method at Forward Euler (FE), Backward Euler (BE) and Trapezoidal (TRAP) method use time step $h$ to discretize the
dynamical system with respect to time. 
They lead to explicit and implicit methods,
which bring the stability and limitted time step due to the system, e.g. 
stiff systems.
Explicit methods are relatively cheap computation; Implicit methods are usually time consuming because they require
to solve the large linear systems. For this regard, in power grid simulation, it precomputes the matrix 
($\mbf C/h+ \mbf G$) in BE, or ($\mbf C/h + \mbf G/2$) in TRAP. This involes the time step $h$. 

Also, in linear circuit, the the mexponential operator is a explicit method, of which the matrix-vector multiplication
take the major part of computation.



Power grid simulation plays an important role in IC design methodology. Given current stimulus and the power grid structure, 
designers could verify and predict the worst-case voltage noise through the simulation before signing off their design.  
However, with the huge size of modern design, power grid simulation is a time-consuming process. Moreover, manifesting effects 
from the package and the board would require longer simulation time, e.g., up to few $\mu s$, which worsens the performance 
of the power grid simulation. Therefore, an efficient power grid simulation is always a demand from industry. 

Conventionally, the power grid simulation is based on the trapezoidal method where the major computation is to solve a linear 
system by either iterative approaches\cite{Saad03} or direct methods\cite{Davis06}. Many previous 
works~\cite{Chen01_Efficient}\cite{Feng08}\cite{Kozhaya02}\cite{Nassif00_Fast}\cite{Su03} utilize iterative approaches to tackle 
the scalability issue and enable adaptive stepping in the power grid simulation. However, the iterative methods usually suffer
from the convergence problem because of the ill-conditioned matrix from the power grid design. On the other hand, the direct 
methods, i.e., Cholesky or LU factorizations, are more general for solving a linear system. Despite the huge memory 
demanding and computational effort, with a carefully chosen step size, the power grid simulation could perform only one 
factorization at the beginning while the rest of operations are just backward/forward substitutions. Since a power grid design 
usually includes board and package models, a long simulation time is required to manifest the low-frequency response. Hence, 
the cost of expensive factorization can be amortized by many faster backward/forward substitutions. Such general factorization 
and fixed step size strategy~\cite{Xiong12}\cite{Yang12}\cite{Yu12}\cite{Zhao02} is widely adopted in industry.  

Beyond the traditional trapezoidal method, Weng \emph{et al.}~\cite{Weng12_TCAD, Weng12_ICCAD} introduced 
the matrix exponential method (MATEX) for the circuit simulation recently. MEXP has better accuracy and adaptivity because of the 
analytical formulation and the scaling invariant Krylov subspace approximation. Unlike the fixed step size strategy, MATEX could 
dynamically adjust the step size to exploit the low-frequency response of the power grid without expensive computation. However, 
the step size in MATEX is limited by the stiffness of circuit. Furthermore, MEXP has to regularize~\cite{Chen12_TCAD} the 
singularity in power grid, i.e., nodes without grounded capacitance or inductance/voltage branches. Both constraints would drag 
the overall performance of MATEX for the power grid simulation. 

In this work, we tailor MATEX using \emph{rational Krylov subspace} for the power grid simulation with adaptive time stepping. 
The rational Krylov subspace uses $(\mbf{I}-\gamma \mbf{A})^{-1}$ as the basis instead of $\mbf{A}$ used in the conventional Krylov 
subspace. The rational basis limits the spectrum of a circuit so that the exponential of a matrix can be accurately approximated 
even under a large step size. Moreover, the rational avoids $\mbf{C}^{-1}$ and thus eliminates the regularization process. 
As a result, MATEX with rational Krylov subspace is free from the stiffness constraint and the regularization process. The 
simulation can purely enjoy benefits of the adaptivity and the accuracy of MATEX. Even though the rational Krylov subspace still needs 
to solve a linear system as the trapezoidal method does, MATEX can factorize the matrix only once and then constructs the rest of 
rational Krylov subspaces by backward/forward substitutions. Therefore, MATEX can utilize its capability of adaptivity to accelerate 
the simulation with the same kernel operations as the fixed step size strategy. Overall, our MATEX has the following advantages: 
\begin{itemize}
    \item enabling adaptive time stepping for the power grid simulation with only one lu factorization.
    \item eliminating the regularization process for the singular power grid design.  
    \item allowing scaling large step size without compromising the accuracy. 
\end{itemize}
The experimental results demonstrate the effectiveness of MATEX with adaptive step size. The power grid simulation for IBM benchmark 
suite~\cite{Nassif08_Power} and industrial power grid designs can be accelerated 6X and 15X on average compared to the trapezoidal method. 

The rest of paper is organized as follows. Section~\ref{sec:preliminary} presents the background of the power grid simulation and MATEX. 
Sections~\ref{sec:rational_krylov} and~\ref{sec:adaptive_step_control} show the theoretical foundation of the rational Krylov subspace 
and our adaptive step scheme for the power grid simulation, respectively.  Section~\ref{sec:exp_results} presents experimental results 
of the IBM benchmark suite~\cite{Nassif08_Power} and several industrial power grid designs. Finally, Section~\ref{sec:conclusion} concludes 
this paper. 
%Specifically, the contributions of this work are:
%\begin{itemize} 
%    \item Enabling adaptive stepping in the power grid simulation with the computational cost of only one matrix factorization 
%	  and backward/forward substitutions. 
%    \item Using rational Krylov subspace method to ease the stiffness constraint~\cite{Weng12_TCAD}\cite{Weng12_ICCAD}, 
%	  meanwhile, endowing MATEX with the capability of dealing with singular $\mbf C$ without time-consuming 
%	  regularization process.
%\end{itemize}
%
\end{comment}



==> matex/adaptive.tex <==


With the relaxation of the stiffness constraint, 
by \emph{inverted basis} and \emph{rational basis} methods 
MATEX can now utilize larger step size, so it enjoys 
an significantly benefit from adaptive step size control
more than \emph{standard basis} when dealing with stiff linear circuit
simulation.
%for Krylov subspace-based matrix exponential computation
%still preserves 
%the capability of adaptivity, which has already been demonstrated the effectiveness 
%in ~\cite{Weng12_TCAD} \cite{Weng12_ICCAD}. 
%e.g., 1\emph{ns}, 
%to perform transient analysis. 
The idea of our adaptive step scheme is to 
step forward as long as the allowance of PWL. 
%so that MATEX can finish the simulation quickly. 
In the following sub section, we introduce
adaptive and matrix handling for \emph{inverted basis}
and \emph{rational basis} Krylov subsapce-based MATEX, respectively.
%Preceding the adaptive frameworks, we introduce some 
%matrix constructions under the assumptions of PWL.

\subsection{Inverted Basis Krylov Subspace-Based MATEX}
We do not use $\mbf {\wtd G}$ because the sub block matrix $\mbf J$ is singular. 
%The first issue is the \mbf{G}
So I need to start from Eqn. (\ref{eqn:pwl_exact_sol}), it contains three matrix exponentials,
however, we re-arrange it, so that it only requires one Arnoldi process for matrix exponential computation
at each time step.
\begin{eqnarray} 
\label{eqn:pwl_inverted}
     \mbf{x}(t+h) &=& e^{\mbf{A}h} \left ( \mbf{x}(t) 
		    + \mbf{A}^{-1}\mbf{b}(t)
		    + \mbf{A}^{-2}\frac{\mbf{b}(t+h)-\mbf{b}(t)}{h} \right )  
     \nonumber \\ 
		&-& 
		\left (
		%\mbf{A}^{-1}\mbf{b}(t)  
	        %- (\mbf{A}h+\mbf{I})\mbf{A}^{-2}\frac{\mbf{b}(t+h)-\mbf{b}(t)}{h}.
		 \mbf A^{-1}\mbf b(t+h) + \mbf A^{-2} \frac{\mbf b(t+h) - \mbf b(t)}{h}
		 \right )
		 \nonumber
%		 \\
\end{eqnarray}
Then we obtain,
\begin{eqnarray}
     \mbf{x}(t+h) &=& e^{\mbf{A}h} \mbf y_1(t,h) 
	+ \mbf y_2(t,h)
%    + \mbf{G}^{-1}\mbf{b}(t)  
%	        - (\mbf{A}h+\mbf{I})\mbf{A}^{-2}\frac{\mbf{b}(t+h)-\mbf{b}(t)}{h}.
\end{eqnarray}
where
\begin{eqnarray}
\mbf{y}_1(t,h)  =	  \mbf x(t) + 
	\mbf{w}(t) + 
 \frac{\theta (t+h) - \theta(t)}{h}
	%\mbf{A}^{-1}\frac{\mbf{w}(t+h)-\mbf{w}(t)}{h}
	 \nonumber
\end{eqnarray}
\begin{eqnarray}
\mbf{y}_2(t,h)  =	\mbf{w}(t+h) +
\frac{\theta (t+h) - \theta(t)}{h}
%\mbf{A}^{-1}\frac{\mbf{w}(t+h)-\mbf{w}(t)}{h}
	 \nonumber
\end{eqnarray}
and
\begin{eqnarray}
\mbf w(t) = \mbf A^{-1}\mbf b(t) = \mbf{G}^{-1}\mbf{Bu}(t) \\ 
\mbf w(t) = \mbf A^{-1}\mbf b(t) = -\mbf{G}^{-1}\mbf{Bu}(t)  
\end{eqnarray}
\begin{eqnarray}
\theta(t) = \mbf A^{-2} \mbf b(t) =\mbf G^{-1}\mbf{C} \mbf{w}(t) 
%\mbf U_2 = \mbf{G}^{-1}\mbf{C}\mbf U_1
\end{eqnarray}

In the inverted basis, we have LU matrices for $\mbf G$ at the very beginning, 
so only backward/forward substitutions are used here, and $\mbf w(t+h), \theta (t+h)$ of time
step $t$ can be reused as $\mbf w(t), \theta(t)$ for the next time step $t+h$.

\emph{Adaptive Time Stepping}: 
Within the region of PWL assumption from $[t,t+h]$,
the slope is an constant.
\begin{eqnarray}
s = \Delta \theta(t,t+h) =
\frac{\theta (t+h) - \theta(t)}{h}
\end{eqnarray}
Therefore, $\mbf y_1(t)$ does not change in the region. 
If we scale the $h$, 
it bares the same Krylov invariant basis for this region.
%where $\alpha \le 1$.
based on the scaling invariant property of Krylov subspace, 
%$[t,t+h]$.
%as $e^{h\mbf A} \mbf y_1(t,h) $. 
%reduce backward forward substitutions.
%It is a function of $t$, not $h$ any more $\left (\mbf y_1(t) \right)$.
%The $\mbf y_2(t,h)$ is now the function of $t$, $\alpha$, $\mbf y_2(t,\alpha)$.
The kernel equation for time stepping can be simplified as follows,
\begin{eqnarray}
\label{eq:inv_scale}
\mbf x(t+h) = e^{h \mbf A} \mbf y_1 (t) + \mbf y_2 (t,h) 
\end{eqnarray}
where
\begin{eqnarray}
\label{eq:y_1_t}
\mbf{y}_1(t)  =	  \mbf x(t) + 
	\mbf{w}(t) + 
	\mbf s , \ \  
	%\mbf{A}^{-1}\frac{\mbf{w}(t+h)-\mbf{w}(t)}{h}
\mbf{y}_2(t,h )  =   \mbf{w}( t  + h ) + \mbf s 
%\mbf{A}^{-1}\frac{\mbf{w}(t+h)-\mbf{w}(t)}{h}
	 \nonumber
\end{eqnarray}

In order to comply with the required 
accuracy during the simulation, the allowed error $err_k$
at certain time instant $t_k$ is defined as 
\begin{eqnarray}
    err_k \le \frac{E_{Tol}}{T} %\times
    h_k, \nonumber
\end{eqnarray}
where $E_{Tol}$ is the error tolerance in the whole simulation process, $T$ is the simulation time span, $h_k$ is the 
step size at time $t_k$, and $err_k$ is the posterior error of MATEX from 
Eqn. (\ref{eq:err_inverted_krylov}) or (\ref{eq:err_rational_krylov}). Hence, when 
we construct the rational Krylov subspace at the current time, we will increase $m$ until the $err_k$ satisfies the 
error tolerance. 


The Algorithm (\ref{algo:inv_adaptive_step}) sketches the adaptive process,  

\begin{algorithm} 
    \label{algo:inv_adaptive_step}
    \caption{I-MATEX with Adaptive Step Control}
    \KwIn{$\mbf{C}$, $\mbf{G}$, $\mbf{B}$, $\mbf{u}(t)$, 
    %$\tau$, 
    error tolerance $E_{Tol}$ and simulation time $T$}
    \KwOut{$\mbf{x}(t)$}
    {
        $t = 0$\; 
	$\mbf{x}(0)$ = DC\_analysis\;
	Compute $\mbf w(0)=\mbf G^{-1}\mbf B \mbf u(0)$, 
	$\mbf \theta(0)=\mbf G^{-1} \mbf C\mbf w(0)$\;
	Compute maximum allowed step size $h$ from $\mbf{u}(t)$,
	$\mbf w(h)=\mbf G^{-1}\mbf B \mbf u(h)$,
	$\mbf \theta(h)=\mbf G^{-1} \mbf C\mbf w(h)$\;
        %Choose $\tau$ for rational Krylov subspace method\;
        $[\mbf{L},\mbf{U}] = $LU($\mbf{G}$)\;
        \While{$t \leq T$}
        {	
	    %Update $v_{k+1}$ with $\mbf{L}, \mbf{U}, \mbf{W}$ by (\ref{eq:blu_f})\;
	    %and update $\mathbf{L},\mathbf{U}$ by (\ref{eq:blu})\;
	    Compute maximum allowed step size $h$ from $\mbf{u}(t)$,
%	    Compute $\mbf w(t)=\mbf w(t)$, $\mbf \theta(t)=\mbf \theta(t)$\;
 $\mbf w(t+h)=\mbf G^{-1}\mbf B \mbf u(t+h)$, 
		    $\mbf \theta(t+h)=\mbf G^{-1} \mbf C\mbf w(t+h)$
		    and $\mbf y_1(t)$ by Eqn. (\ref{eq:y_1_t})
		    \;
	    Construct $\mbf{H_m}$, $\mbf{V_m}$ by Arnoldi process with inputs 
	    $\mbf X_1 = \mbf G ~(\mbf L, \mbf U \text{~pair} )$,
	    $\mbf X_2 = \mbf C$, $\mbf v = \mbf y_1(t)$, 
	    until $err \le \frac{E_{Tol}}{T}h$ \;
	   % $\alpha = \frac{h}{\gamma}$ \;
	    Compute $\mbf{x}(t+h)$ by Eqn. (\ref{eq:inv_scale})
	    $\mbf x(t+h) = \lVert \mbf y_1(t) \rVert \mbf V_m e^{\alpha h \mbf H_m} 
	    \mbf e_1 (t) + \mbf y_2 (t, h )$ \; 
	    $t = t+h$; 
	}
    }
\end{algorithm}


\subsection{Rational Basis Krylov Subspace-Based  MATEX}
\label{sec:rational_adaptive}
With the insight from Eqn. (\ref{eq:scale}), 
MATEX is able to adjust $\alpha$ to calculate result of arbitrary 
step size with only performing one Arnoldi process. 
However, because MATEX has to guarantee slopes of input sources 
(in linear circuit, it is only about PWL) must 
be constant within the step size, the maximum allowed step size is limited. 
Therefore, MATEX will first compute the rational 
Krylov subspace using $\mbf{x}(t)$, and then results within the maximum 
allowed step size, which is determined by input 
sources, can be calculated through the step size scaling. 
Before introducing the adaptive framework, we point out a 
Block LU factorization to reuse one LU at the very beginning.

\emph{Block LU factorization}:
%reduce backward forward substitutions.
In practical numerical implementation, in order to avoid 
direct inversion of $\mbf C$ to form $\mbf A$ in Eqn. (\ref{eq:rat_kry}),
the Eqn. (\ref{eq:precond2}) 
\begin{equation}
\label{eq:precond2}
    (\mathbf C  + \gamma \mathbf G )^{-1}\mathbf C
\end{equation}
% here if we deal with singular case the (\ref{eq:precond}) will use 
is used.
%$\mbf C$ may has bad condition number when it is stiff, 
% or does not exsist when it is singular. 
% (\ref{eq:rat_kry}).
Correspondingly, we uses the following equations for Eqn. (\ref{eq:one_exp}),
\begin{equation}
\label{eq:precond1}
    (\mathbf {\wtd C}  - \gamma \mathbf {\wtd G} )^{-1}\mathbf {\wtd C}
\end{equation}
% $ The augmented matrix $\mbf A = \mbf {C'}^{-1}G'$, where

\begin{comment}
where
\begin{eqnarray}
\label{eq:cg_prime}
\mbf  {\wtd C} = 
    \left[
	\begin{array}{*{20}{c}} 
	    \mbf C &  0 \\ 
	    0 & \mbf I
	\end{array}
    \right], \; 
\mbf  {\wtd G} =
    \left[
	\begin{array}{*{20}{c}}
	 \mbf {-G}  & \mbf W \\
	  0 &  \mbf J
	\end{array}
    \right]
\end{eqnarray}
\end{comment}
% will be used for  ${\wtd A}$ of~(\ref{eq:one_exp})  

The Arnoldi process based on Eqn.~(\ref{eq:precond1}) actually only requires 
to solve $\mbf v_{k+1}$ with $\mbf v_k$. 
The linear system
is expressed as
\begin{eqnarray}
   (\mbf {\wtd C } -  \gamma \mbf {\wtd G}) \mbf v_{k+1}=\mbf {\wtd C} \mbf v_k,
\end{eqnarray}
where $\mbf v_{k}$ and $\mbf v_{k+1}$ are $k$-th and 
$(k+1)$-th basis in the rational Krylov subspace. 
If $\mbf{W}$ changes with inputs during 
the simulation, the Arnoldi process has to factorize a matrix every time step. 
However, it is obvious that the majority of matrix components 
in Eqn.~(\ref{eq:cg_prime}) stay the same for this linear system. 
To take advantage of this property, a block LU factorization is devised here
to avoid redundant calculation.

The goal is to obtain two matrices: the lower triangular matrix $\mbf L$ and the upper triangular matrix $\mbf U$, such that 
\begin{eqnarray}
    \label{eq:blu}
    \mbf  {\wtd C} - \gamma \mbf {\wtd G} = \mbf L \mbf U.
\end{eqnarray}

At the beginning of simulation, after LU factorization of 
\begin{eqnarray}
\mbf C + \gamma \mbf G=\mbf L_{sub} \mbf U_{sub} 
\end{eqnarray}
we obtains the lower triangular sub-matrix $\mbf L_{sub}$, and upper triangular 
sub-matrix $\mbf U_{sub}$. Then Eqn. (\ref{eq:blu}) only needs updating 
via  
\begin{eqnarray}
\label{eq:blu1}
%A^{i}\mathbf{v}={({C'}^{-1}G)}^{i}\mathbf{v} \\
\mbf L = 
  \left[
    \begin{array}{*{20}{c}} 
       \mbf L_{sub} & 0\\
       0 & \mbf I
    \end{array}
   \right] , \;\;
\mbf U = 
    \left[
    \begin{array}{*{20}{c}} 
	\mbf U_{sub} &\mbf L^{-1}_{sub} \mbf W\\
	 0 & \mbf I_J
    \end{array}
    \right],
\end{eqnarray}
where $\mbf I$ is an identity matrix, 
$\mbf I_J = \mbf {I + \gamma J}$ is an upper triangular matrix. 
The following equations further reduce 
operation $\mbf L_{sub}^{-1}$ and construct vector $\mbf{v}_{k+1}$.
\begin{eqnarray}
    \label{eq:blu_f}
    \mbf L_{sub} \mbf U_{sub} \; \mbf y_1 = 
	    \mbf b_1- \mbf W \; \mbf y_2, \; \; \; \; 
    \mbf y_2 = \mbf I^{-1}_J \mbf b_2,  
\end{eqnarray}
where 
\begin{eqnarray}
\mbf v_{k+1} = [\mbf y_1, \; \mbf y_2]^{T} , \mbf b_1=[\mbf C, \; 0] \mbf v_k, 
\mbf b_2 = [0, \; \mbf I] \mbf v_k. 
\nonumber
\end{eqnarray}
By doing this, it only needs one LU factorization at the beginning 
of simulation, and with 
cheap updates for the $\mbf L$ and $\mbf U$ at each time step during transient simulation. 

\emph{Adaptive Time Stepping}:
Algorithm~\ref{algo:adaptive_step} shows MATEX with adaptive step control scheme. 
\begin{algorithm} 
    \label{algo:adaptive_step}
    \caption{R-MATEX with Adaptive Step Control}
    \KwIn{$\mbf{C}$, $\mbf{G}$, $\mbf{B}$, $\mbf{u}(t)$, 
    %$\tau$,
    error tolerance $E_{Tol}$ and simulation time $T$}
    \KwOut{$\mbf{x}(t)$}
    {
        $t = 0$\; 
	$\mbf{x}(0)$ = DC\_analysis\;
        %Choose $\tau$ for rational Krylov subspace method\;
        $[\mbf{L}_{sub},\mbf{U}_{sub}] = $LU($\mbf{C} +\gamma \mbf{G}$)\;
        \While{$t \leq T$}
        {	
	    Update
	    %$\mbf v_{k+1}$ with
	    %$\mbf{L}, \mbf{U}, \mbf{W}$ by (\ref{eq:blu_f})\;
	    $\mathbf{L},\mathbf{U}$ by 
	    $\mbf{L}_{sub},\mbf{U}_{sub}  $
	    and Eqn. (\ref{eq:blu})\;
	    Compute maximum allowed step size $h$ from $\mbf{u}(t)$\;
	    Construct $\mbf{H_m}$, $\mbf{V_m}$ by Arnoldi process,
	    with input $\mbf X_1 = (\mbf L, \mbf U)$, $\mbf X_2 = \mbf C$
	    and $\mbf v = \mbf x(t)$,
	    until $err \le \frac{E_{Tol}}{T}h$\;
	    $\alpha = \frac{h}{\gamma}$ \;
	    Compute $\mbf{x}(t+h)$ by Eqn. (\ref{eq:scale})\;
	    $t = t+h$; 
	}
    }
\end{algorithm}

\subsection{Summary}
The complexity of MATEX with adaptive step size is mainly determined by the total number of required backward/forward
substitutions during the simulation process. This is because the dimension of $\mbf{H_m}$ is small, e.g., around 
$4 \sim 20$, and the computation overhead of the step size scaling is negligible. The number of total substitution 
operations is 
\begin{eqnarray}
    \sum_{i=0}^N m_{i}, \nonumber
\end{eqnarray}
where $N$ is total time steps, and $m_i$ is required dimension of rational Krylov subspace of each time step. Compared to 
the trapezoidal method where the number of substitution operations depends on the fixed step size, MATEX could use less 
substitution operations as long as the maximum allowed step size is much larger than the fixed step size. Our experiments 
in the following section demonstrates it is usually the case for the power grid simulation.

Such large step size is particularly useful for the power grid 
simulation where the voltage noise usually 
includes the low frequency behavior of both package and board levels. 




==> matex/complexity.tex <==


\vspace{-0.02in}
Suppose on average 
we have 
Krylov subspace basis dimension $m$ at each time step along the time span,
one pair of backward and forward substitutions has time complexity $O(T)$. 
The time complexity of unparallelized parts is $O(T_s)$, e.g., matrix factorizations,
The matrix exponential evaluations using $\mbf H_m$ is $O(m^3)$, plus extra $T_e$ to form $\mbf x$.
$T$, $T_s$ and $T_e$ are positive proportional to the nonzero terms in operated matrices.
Given $K$ points of GTS, without decomposition of input transitions,
the time complexity is $O(KmT + K (m^3+ T_e)  + T_s)$, 
After dividing the input transitions and send to enough computing nodes, 
we have $k$ points of LTS for each node based on feature extraction and grouping 
(e.g. $k=4$ for ``bump'' shape feature).
%suppose we have enough computing nodes to parallel process all input sets, 
The total computation complexity is $O( kmT + K(m^3 + T_e) + T_s)$.
%Since no commnication required between the different processors, the extra complexity form
The speedup of distributed computing over single MATEX, 
\begin{eqnarray}
%\footnotesize 
%\text{Speedup}=\frac{ O(Km^3)+ O(Ktm)+O_{s} }  {O(Km^3)+O(ktm)+O_{s}}
\text{Speedup}=\frac{ KmT + K(m^3+ T_e)+ T_{s} }  { kmT+ K(m^3+T_e)+T_{s}}
\end{eqnarray}
In R-MATEX, we have very small $m$. Besides, $T$ is larger than $m^3+T_e$. 
Therefore, the most dominating part is the $KmT$.
We can always decompose input transitions, and make $k$ very small compared to $K$.
Compared to traditional method TR with fixed step size, it has $N$ steps for the whole simulation.
The complexity is $NT+T_s$. Then the speedup of distributed MATEX over TR with fixed step size is,
\begin{eqnarray}
\label{eqn:tr_spd}
%\text{Speedup}=\frac{ O(Km^3)+ O(Ktm)+O_{s} }  {O(Km^3)+O(ktm)+O_{s}}
\text{Speedup'}=\frac{ NT+ T_{s} }  { kmT+ K(m^3+T_e)+T_{s}}
\end{eqnarray}
Usually, $N$ is much larger $K$ and $km$. 
Uniform step sizes make $N$ increased due to resolution of input transitions, 
to which $K$ is not so sensitive.
As mentioned before, $k$ can be maintained in a small number.
When elongating time span of simulation,
$N$
%\ref{sec:complexity}) 
will raise,
however, $k$ will not change due to its irrelevant to time span 
(may bring more input transition features and increase computing nodes),
and speedups tend to become larger.
Therefore, our MATEX has more robust and promising theoretical speedups.

%The rational basis Subspace for circuit simulation is supposed to converge evne fast, when the 
%order $m$ large than a small number, and the error is reduced quickly and the estimation can be replaced with 
%$\lVert r_m(h) \rVert = 
%\lVert \mbf v \rVert h_{m+1,m} \left| \mbf e^{\mathbf T} e^{h\mbf {\wtd {H}}_m} \mbf e_1 \right |$
%to approximate Eqn. (\ref{eq:err_rational_krylov}).





==> matex/framework.tex <==
\begin{figure}[ht] 
\scriptsize
    \centering
    \includegraphics[width=3.2in ]{./figs/time_spots.eps}
    \caption{
	{
	    \scriptsize
	{Illustration of input transitions. 
	GTS: Global Transistion Spots; LTS: Local Transition Spots;
	Snapshots: the crossing positions by dashlines and LTS \#$k$ without solid points, 
	that is the snapshots for LTS \#$k$. % which is the set of $GTS \setminus LTS$. 
	Pulse input information:
    t\_delay: initial delay time;
    t\_rise: rise time;
    t\_width: width of pulse-wise; 
    t\_fall: fall time;
    t\_period: period.
	}
	}
    }
    \label{fig:input}
\end{figure}
\begin{figure}[ht]
\scriptsize
    \centering
    \includegraphics[ width=1.8in]{./figs/rc_ckt.eps}
    \caption{Linear circuit with inputs from Fig. \ref{fig:input}}
	\label{fig:rc_ckt}
\end{figure}
\begin{figure}[ht]
\scriptsize
    \centering
    \includegraphics[ width=3.2in ]{./figs/ckt_ts_decomp.eps}
    \caption{
	\scriptsize
	{``Bump'' shape transitions decomposition.
	    Here, the matrix exponential-based method can enjoy large adaptive stepping in each LTS 
	    and also reuse the Krylov subspace basis generated at the last solid points.
	    Meanwhile, traditional methods (TR, BE) still need to do
	    time marching limited by GTS, either by pairs of backward and forward
	    substitutions or adaptive stepping, which re-factorizes matrix if direct solver is used.
	}
    }
	\label{fig:ckt_ts_decomp}
\end{figure}

\vspace{-0.03in}
\subsection{Motivation}
\label{sec:frame_motivation}
%from \emph{Transition Spots} vs. \emph{Snapshots} }
Input transition spots (\emph{TS}) are the places that 
linear circuit's transient computing cannot jump over without {\color{red} computing} touching,
``Touching'' 
which means, at one of TS, solving linear system by traditional adaptive time stepping methods;  
performing a pair of backward and forward substitutions by methods with fixed time step; or 
regenerating Krylov subspace basis for matrix exponential computation by MEXP.
The situation becomes complicated when there are many excitations.
For example, there are three input sources shown in Fig. \ref{fig:input} and \ref{fig:rc_ckt}.
First, if the linear circuit only has one input source excitation, 
so that TS appears as the \emph{Local Transition Spots} (LTS).
For MEXP, the solid points are the places require new Krylov subspace basis generations.
However, when circuit are stimulated by these inputs together,
the three LTSs form the \emph{Global Transition Spots} (GTS).
Therefore, the time steps of simulation are narrowed by the GTS, which limit MEXP's time stepping and 
demands more frequent basis generations.

The antidote to this problem relies on the superposition property of linear system.
We can still solve the problem based on LTS. 
Then the final result is obtained 
via the summation of responses from different inputs.
More aggressively, we extract the feature of pulse inputs, which is ``bump'' shape 
used in common input sources. We decompose the set of inputs based on ``bump'' feature and 
group ones with same (t\_delay, t\_rise, t\_fall, t\_width) in a same input set, 
which is shown in Fig. \ref{fig:ckt_ts_decomp}, e.g., \#1.2 and \#3 can be grouped into one input set. 
There are 4 groups in Fig. \ref{fig:ckt_ts_decomp},
Group 1 contains LTS\#1.1, Group 2 contains LTS\#2.1, Group 2 contains LTS \#2.2, 
and Group 4 contains LTS \#1.2 and \#3.
Then we simulate by groups. 
Note when superposing, all the results of GTS should be computed.
Then \emph{snapshot}s
%for GTS other than LTS(${GTS} \setminus {{LTS}}$, dashlines in 
(seen in Fig. \ref{fig:input} and \ref{fig:ckt_ts_decomp}) 
are kept in each node locally as local results too.
%The complexity of keeping snapshot can be done with only scaling $h\mbf H_m$, the
%reusing previous Krylov subspace basis. 
When $m$ is small, it costs a little extra efforts
to obtain these snapshots, because we can reuse previous Krylov subspace basis by scaling $\mbf H_m$.

\vspace{-0.03in}
\subsection{MATEX Framework}
\label{sec:all_frame}
MATEX is shown in Fig. \ref{fig:matex}. After pre-computing the GTS and decomposing
input transitions based on ``bump'' shape (Fig. \ref{fig:ckt_ts_decomp}) and group them into 
LTS $\#1 \sim \#K$ (\emph{Note: there are alternative decomposition strategies, 
we try to keep this part as simple as possible here. The main purpose is to illustrate our framework}).  
MATEX scheduler sends out GTS and LTS to corresponding MATEX slave node.
Then the simulations are parallel processed.
There are no communication among nodes before the ``write back''.
Within each slave node, ``circuit solver''(Alg. \ref{algo:ckt_solver}) 
computes transient response with varied time steps. 
During the process, solutions are obtained without re-factorizing matrix. 
After finishing all simulations from slave nodes, they writes back the results
and informs the MATEX scheduler.
\begin{figure}[h]
\centering
\includegraphics[ width=3.4in ]{./figs/hierachical_ckt_sim.eps}
\caption{The flow of MATEX framework}
\label{fig:matex}
\end{figure}
%\textbf{Why does MATEX can leverage such distributed computing framework, but trditional methods cannot?}

\vspace{-0.03in}
%\subsection{Circuit Solver Algorithm}
\begin{algorithm}
\label{algo:ckt_solver}
%\caption{Arnoldi process in Matrix Exponential-Based Circuit Simulation with Krylov subspace Method}
\caption{MATEX Circuit Solver Algorithm}
%$\rm K_m(\mbf X_1^{-1}\mbf X_2, \mbf v)$} %~\cite{Weng12_TCAD, Weng12_ICCAD}}
\KwIn{ LTS \#$k$, GTS, Circuit }
%\KwOut{ $\mbf V_m, \mbf H_m,  m$ }
\KwOut{Local solution $\mbf x$ along GTS in node $s \in [0,\cdots,S]$}
    {   
%	[$\mbf L, \mbf U$]=LU($\mbf X_1$)\\
%	Normalize the intial vector 
	$t=T_{start}$;
	$s=T_{start}$\;
	$\mbf x(t) = local\_DC\_analysis$; // DC for input at \#$s$\; 
	%$[\mbf L,\mbf U] = \text{LU\_Decompose}( \mbf C+\gamma \mbf G)$\;
	$[\mbf L,\mbf U] = \text{LU\_Decompose}( \mbf X_1)$\;
	\While { $t \leq T_{end}$}
	{
	Compute maximum allowed step size $h$ based on GTS\;
	\If{$t \in $ set of LTS \#$k$}
	{
	// Reach LTS and update $\mbf V_m, \mbf H_m, \mbf v, s$\;
	$[ \mbf x(t+h), \mbf V_m, \mbf H_m,\mbf v 	]
	= \text{~~~~~MATEX\_Arnoldi}(\mbf L,\mbf U,\mbf X_2, h, t, \mbf x(t), \epsilon )$ \;
%	Update $\mbf x(t +h) $ based on Eq. (\ref{eqn:new_exact})\; 
	$a_{lts} = t$; // put an LTS anchor for current $t$\; 
	}
	\Else{
%	    \For  {$s_i \in (t_i + h,t_{i+1}]$}
	    {
	    // Take snapshots by reusing $\mbf V_m , \mbf H_m, \mbf v$ \;
	    $h_{a} = t + h - a_{lts}$\;
	    $\mbf x(t+h) = \lVert \mbf v \rVert \mbf {V_m} e^{h_{a} \mbf H_m} \mbf e_1 - \mbf P_s(t,h)$\;
%	    Update $\mbf x(t +h) $ based on Eq. (\ref{eqn:new_exact})\; 
	%$\lVert r_m(h) \rVert  =  \lVert \mbf v \rVert \left| h_{m+1,m} e_m^T e^{h\mbf H_m} e_1 \right|$
	    }
	}
	$t= t+h$\;
	}
    }
\end{algorithm}



%\subsection{MATEX Framework for Distributed Computing}




==> matex/framework_v1.tex <==
\begin{figure}[ht] 
\scriptsize
    \centering
    \includegraphics[width=3.2in ]{./figs/time_spots.eps}
    \caption{
	{\scriptsize
	{Illustration of input transitions. 
	GTS: Global Transistion Spots; LTS: Local Transition Spots;
	Snapshots: the crossing positions by dashlines and LTS $k$ without solid points, 
	that is the snapshots for LTS \#$k$. % which is the set of $GTS \setminus LTS$. 
	Pulse input information:
    t\_delay: initial delay time;
    t\_rise: rise time;
    t\_delay: width of pulse-wise; 
    t\_fall: fall time;
    t\_period: period.
	}
	}
    }
    \label{fig:input}
\end{figure}
\begin{figure}
\scriptsize
    \centering
    \includegraphics[ width=1.8in]{./figs/rc_ckt.eps}
    \caption{Linear circuit with inputs from Fig. \ref{fig:input}}
	\label{fig:rc_ckt}
\end{figure}
\begin{figure}[h]
\scriptsize
    \centering
    \includegraphics[ width=3.2in ]{./figs/ckt_ts_decomp.eps}
    \caption{``Bump'' shape transitions decomposition}
	\label{fig:ckt_ts_decomp}
\end{figure}

\vspace{-0.03in}
\subsection{Motivation}
%from \emph{Transition Spots} vs. \emph{Snapshots} }
Input transition spots (\emph{TS}) are the places that 
linear circuit's transient computing cannot jump over without touching.
``Touching'' means, at one of TS, solving linear system by traditional adaptive time stepping methods;  
performing a pair of backward and forward substituions by ones with fixed time step; or 
regenerating Krylov subspace basis for matrix exponential computation by MEXP.
The situation becomes complicated when there are many excitations.
For example, there are three input sources shown in Fig. \ref{fig:input} and \ref{fig:rc_ckt}.
First, if the linear circuit only has one input source excitation, 
so that TS are appeared as the \emph{Local Transition Spots} (LTS).
The solid points are the places require new Krylov subspace basis generations.
However, when circuit are stimulated by these inputs together,
the three LTSs form the \emph{Global Transition Spots} (GTS).
Therefore, the time steps of simulation are narrowed by the GTS, which limit MEXP's time stepping and 
demands more frequent basis generations.

The antidote to this problem relies on the superposition property of linear system.
We can still solve the problem based on LTS. 
Then the final result is obtained 
via the summation of responses from different inputs.
More aggressively, we extract the feature of pulse inputs, which is ``bump'' shape 
used in common input sources. We decompose the set of inputs based on ``bump'' feature and 
group ones with same (t\_delay, t\_rise, t\_fall, width) in a same input set, 
which is shown in Fig. \ref{fig:ckt_ts_decomp}, e.g., \#1.2 and \#3 can be grouped into one input set. 
When superposing, all the results of GTS should be computed.
Then \emph{snapshot}s
%for GTS other than LTS(${GTS} \setminus {{LTS}}$, dashlines in 
(seen in Fig. \ref{fig:input}, \ref{fig:ckt_ts_decomp}) 
are kept in each node locally.
%The complexity of keeping snapshot can be done with only scaling $h\mbf H_m$, the
%reusing previous Krylov subspace basis. 
When $m$ is small, it costs a little extra efforts
to obtain these snapshots, because we can reuse previous Krylov subspace basis by scaling $\mbf H_m$.

\vspace{-0.03in}
\subsection{MATEX Framework}
MATEX is shown in Fig. \ref{fig:matex}. After precomputing the GTS and decomposing
input transtions based on ``bump'' shape (Fig. \ref{fig:ckt_ts_decomp}) and group them into 
LTS $\#1 \sim \#K$ (\emph{Note: there are alternative decomposition strategies, 
we try to keep this part as simple as possible here. The main purpose is to illustrate our framework}).  
MATEX scheduler sends out GTS and LTS to corresponding MATEX slave node.
Then the simulations are parallel processed.
There are no communication among nodes before the ``write back''.
Within each slave node, ``circuit solver'' computes transient response with varied time steps. 
During the process, solutions are obtained without refactorizing matrix. 
After finishing all simulations from slave nodes, they writes back the results
and informs the MATEX scheduler.
\begin{figure}[h]
\centering
\includegraphics[ width=3.4in ]{./figs/hierachical_ckt_sim.eps}
\caption{The flow of MATEX framework}
\label{fig:matex}
\end{figure}
%\textbf{Why does MATEX can leverage such distributed computing framework, but trditional methods cannot?}

\vspace{-0.03in}
\subsection{Discussions}
MATEX stems from Krylov subspace based matrix exponential computation.
With accurate exponential calculation, it can reuse Krylov subspace basis to
carry adaptive time stepping along successive time spots (taking \emph{snapshots}) before hitting the next LTS.
The snapshot can be obtained as \emph{by-products} by scaling Hessenberg matrix 
and matrix expoentnial evaluation based on adaptive time stepping
techniques similar in MEXP \cite{Weng12_TCAD, Zhuang13_ASICON}.
In addition, MATEX benefits a lot from reusing factorized matrices, which come from
the very beginning of simulation, to generate
new Krylov subspace basis once reaching LTS.
%The LTS, GTS in the Fig. \ref{fig:input}, can be precomputed based on the provided input sources
%information and avoid communication among different computing nodes, 
There are no communication overhead during the transient computing,
rendering such framework 
be a good candidate computational problems for large scale computing techniques, e.g. 
MapReduce, Hadoop, Mesos, Spark, etc., which now may scale to tens of thousands of nodes, 
to deal with large number of input sets.

Nevertheless, the major hinder of traditional methods are LTE due to the low order polynomial approximation, 
and incapability of reusing factorized matrices once changing $h$ (e.g. $C/h+G/2$ 
in Eqn. \ref{eqn:trap} need to be refactorized for solving the linear system). 
Within each node, we still need to derive the transient solutions 
step by step along all time spots (GTS) with calculations, 
e.g. LU, 
%Cholesky, 
or pairs of backward and forward substitutions. 
Therefore, to them, there is no benefit from such input transisition decompositions.
Model order reduction techniques can be applied here, however, they are not full model simulation
and cannot control the error on-the-fly, which MATEX serves all the purposes. 

%\subsection{MATEX Framework for Distributed Computing}




==> matex/krylov_app.tex <==
%{\color{red}{start from here}}

%In MATEX framework, 
%Matrix exponential method is expensive if 
%direct computing matrix exponential is
%expensive ($\sim O(n^3)$), when $n$ is huge of large scale
%circuit simulation.
%In this section, we use Krylov subspace to 
\subsection{Merge of Matrix Exponentials into One Matrix Exponential}

The analytical solution Eqn. (\ref{eqn:pwl_exact_sol}) has 
three matrix exponential terms, which are generally referred 
as $\varphi$-functions of the zero, first and second order~\cite{Niesen11}. It has been shown in 
Theorem 2.1 of \cite{Almohy11} that 
one can obtain the sum of them in one shot by computing the exponential 
of a slightly larger $(n+p)\times (n+p)$ matrix, where $n$ is the dimension of $\mbf{A}$ and $p$ is the 
order of the $\varphi$-functions ($p = 2$ in (\ref{eqn:pwl_exact_sol})). Thus, (\ref{eqn:pwl_exact_sol}) 
can be rewritten into
\begin{equation}
\label{eq:one_exp}
\mbf{x}(t + h) = \left[ 
			\begin{array}{*{20}{c}}
			    \mbf{I}_n & 0
			\end{array} 
		 \right]
		 e^{\mbf {\widetilde A} h}
		 \left[ 
			\begin{array}{*{20}{c}}
			    \mbf{x}(t)	\\
			    e_2
			\end{array} 
		\right],
\end{equation}
with
\begin{equation}
    \begin{gathered}
	\mbf {\widetilde A} = \left[ 
			 \begin{array}{*{20}{c}}
			    \mbf{A} & \mbf{W} \\
			    \mbf{0} & \mbf{J}
			\end{array} 
		   \right],\;\;\;
	\mbf{W} = \left[ 
			\begin{array}{*{20}{c}}
			    \frac{\mbf{b}\left(t + h \right) - \mbf{b}\left( t \right)}{h} & \mbf{b}\left( t \right)
			\end{array} 
		  \right] \hfill \\
	\mbf{J} = \left[ 
			\begin{array}{*{20}{c}}
			    0 & 1 \\
      			    0 & 0
			\end{array} 
		  \right],\;\;\;\;\;\;\;\;
	e_2 = \left[ 
		    \begin{array}{*{20}{c}}
			0 \\
      			1
		    \end{array} 
	      \right] \hfill \\
    \end{gathered}
\end{equation}
To keep the notations simple, we use 
$\mbf{A}$ and 
$\mbf{v}$ to represent 
$\mbf{A}'$ and 
$[\mbf{x}(t)\;\; e_2]^\mathsf{T}$ in the following sections, respectively. 
%We call this formulation as MATEX, which is the fundamental in this paper.

\subsection{Krylov Subspace Approximation of Fast Matrix Exponential Computation}
The matrix exponential function of $\mbf A$ is defined by   
\begin{eqnarray}
\label{eq:exp_def}
e^{\mbf A} :=  \mbf I + \mbf A + \frac{\mbf A^2}{2!} + ... +\frac{ \mbf A^{k}}{k!}+... 
\end{eqnarray}
The direct computation of matrix exponential $e^{\mbf A}$ has 
very high computational complexity ($\sim O(n^3)$)
and usually leads to a full matrix. 
Actually, MATEX framework requires the matrix-and-vector 
product of $e^{\mbf A} \mbf v$, 
which could be approximated via Krylov subspace 
algorithms~\cite{Weng12_TCAD, Weng12_ICCAD,Hochbruck97, Saad92}. 
Then, we consider using polynomial approximation to $e^{\mbf A} \mbf v$, that is,  
\begin{eqnarray}
\label{eq:poly}
e^{\mbf A} \mbf v \approx p_{m-1}(\mbf A) \mbf v, 
\end{eqnarray}
where $p_{m-1}$ is a polynomial of degree at most $m-1$,
and $\mbf v$ is $n \times 1$ vector. 
The approximation of Eqn. (\ref{eq:poly}) 
%can be utilized 
can utilize the well-known Krylov subspace \cite{Saad92}.
Suppose an orthogonal basis $\{ \mbf v_1, \mbf v_2, \cdots, \mbf v_m \}
\in \mathbb{R}^{n \times m}
$
of the Krylov subspace. 
Straightforwardly, such basis is built as follows,
\begin{eqnarray}
\label{eq:kryspan}
{\rm K_m}\left(\mbf{A}, \mbf{v}\right) := \text{span} \{ { \mbf v, 
\mbf A \mbf v, \mbf A^2 \mbf v, ..., \mbf A^{m-1} \mbf v}\} 
\end{eqnarray}
%\subsection{Standard Krylov Subspace of Matrix Exponential Computation}
%It is built and stored as the columns of a matrix 
It is stored as the columns of a matrix
$\mbf V_m = [ \mbf v_0, \mbf v_1, \cdots, \mbf v_m ]$.
This $\mbf V_m$ is usually computed by Arnoldi decomposition algorithm.
%If we take $\mbf v_1 = \mbf v/ ||\mbf v||$ as the initial vector, and generate 
%the basis $\mbf V_m$ contains $m$ vectors, with the Arnoldi algorithm. 
Throughout the paper, $\lVert \cdot \rVert$ 
represents the Euclidean vector norm
or induced matrix norm, unless noted specifically.

\begin{algorithm}
\label{algo:arnoldi}
\caption{Arnoldi decomposition} %~\cite{Weng12_TCAD, Weng12_ICCAD}}
\KwIn{ $\mbf A, \mbf v,  m $  }
\KwOut{ $\mbf V_m, \mbf H_m$ }
    {   
	%// Normalize the intial vector 
	$\mbf v_1 = \frac{\mbf v} { \lVert\mbf v \rVert}$\\
	\For  {$j=1:m$}
	{
	   % Calculate 
	    $\mbf w =\mbf A \mbf v_{j}  $\\ 
	    \For {$i = 1:j$}
	    {
	%	// Orthogonalization 
		$h_{i,j} = \mbf w^T \mbf v_{i}$\\ 
		$\mbf w = \mbf w - h_{i,j} \mbf v_{i}$\\
	    }
	   % Normalization 
	    $h_{j+1,j} =  \lVert \mbf w \rVert $ \\
	    %\mbf w^T \mbf v_{i}$\;
	    $\mbf v_{j+1} = \frac{\mbf w}{  h_{j+1,j}}$\\
	}
    }
\end{algorithm}

Then, we have the relation, 
\begin{eqnarray}
\label{eq:kryspan}
\mbf A \mbf V_m =  \mbf V_m \mbf H_m + h_{m+1,m} \mbf v_{m+1} \mbf e^T_m . 
\end{eqnarray}
where
$\mbf e_m$ is the $m$-th unit vector with 
dimension $m \times 1$.
\begin{eqnarray}
\mbf{H_m} = \left[ \begin{array}{*{20}{c}}
		h_{1,1} & h_{1,2}  & \cdots & h_{1,m} \\
		0 &  h_{2,2}  & \cdots & h_{2,m} \\
		0 & 0  & \cdots & h_{3,m} \\
		\cdots & \cdots &	\cdots & \cdots \\
		0 & 0 &\cdots  & h_{m,m} \\
		    \end{array}
		\right]
\end{eqnarray}
\begin{comment}
\begin{eqnarray}
\mbf{H_m} = \left[ \begin{array}{*{20}{c}}
		h_{1,1} & h_{1,2} & h_{1,3} & \cdots & h_{1,m} \\
		0 &  h_{2,2} & h_{2,3} & \cdots & h_{2,m} \\
		0 & 0 & h_{3,3} & \cdots & h_{3,m} \\
		\cdots & \cdots &	\cdots & \cdots & \cdots\\
		0 & \cdots &\cdots  & \cdots & h_{m,m} \\
		    \end{array}
		\right]
\end{eqnarray}
\end{comment}
is the upper-Hessenberg matrix that is the projection of the 
linear transormation $\mbf A$ to 
subspace $\rm K_m$. 
Thus, $\mbf V_m \mbf V_m^T$ denotes the projection onto ${\rm K_m}$; 
$\mbf H_m$ is the operator restricted to ${\rm K_m}$, 
\emph{i. e.,} $\mbf  H_m = \mbf V^{T}_m \mbf A \mbf V_m$ \cite{Orec:12}.
From the Algorithm and Eqn. (\ref{eq:kryspan}), the Krylov subspace is successful, 
if the last term of Eqn. (\ref{eq:kryspan}) 
turns out to be small enough, for some sufficient $m$.
This means the Krylov subspace ${\rm K_m}$ is almost identical to an invariant subspace of $\mbf A$
\cite{Botchev12}.
%are zero 
% which formed by 
%$\mbf V_m = [ \mbf v_0, \mbf v_1, \cdots, \mbf v_m ]$.
\begin{comment}
\begin{eqnarray}
\label{eq:exp_def}
e^{\mbf A}\mbf v:=  \mbf {(I + A + \frac{A^2}{2!} + ... +\frac{ A^{n-1}}{k!}+...)v}. 
\end{eqnarray}
%The Krylov subspace spans by the basis of $m$ vector
%Generally, the orthogonal bases of Krylov subspace can be constructed from Arnoldi.% or Lanczos process. 
\end{comment}

%From the orthogonomal vectors in $\mbf V_m$, 
%$\mbf H_m $ is expressed as 
%\begin{eqnarray}
%\mbf  H_m = \mbf V^{T}_m \mbf A \mbf V_m
%\end{eqnarray}
% Therefore, $e^{\mbf{A}}\mbf{v}$ can be projected onto the Krylov 
% subspace ${\rm K_m}\left(\mbf{A}, \mbf{v}\right)$ with dimension of $m$. 
Suppose a sufficient $m$, we have,
\begin{eqnarray}
\mbf A \mbf v &=& 
(\mbf V_m \mbf V_m^T ) \mbf A (\mbf V_m \mbf V_m^T ) \mbf v 
\\ \nonumber
& =& \mbf V_m ( \mbf V_m^T \mbf A  \mbf V_m) \mbf V_m^T \mbf v
= \mbf V_m \mbf H_m \mbf V_m^T \mbf v
\end{eqnarray}
Similarly, for $\forall i < m$, 
$\mbf A^i \mbf v = \mbf V_m \mbf H_m^i \mbf V_m^T \mbf v$. 
By linearity, $p_{m-1}(\mbf A) \mbf v = \mbf V_m p_{m-1}(\mbf H_m) \mbf V_m^T \mbf v$ \cite{Orec:12}.
Therefore, the Formula ~(\ref{eq:exp_def}) is evaluated by 
\begin{eqnarray}
\label{eq:Krylov_exp}
e^{\mbf A} \mbf v  
%& \approx &
% \mbf {V_m} \mbf {V^T_m}  e^{\mbf A} 
% \mbf v
% = 
& = & 
e^{\mbf A} (\lVert \mbf v \rVert \mbf V_m \mbf e_1)
= 
\lVert \mbf v \rVert e^{\mbf A} \mbf V_m \mbf e_1
%= ||\mbf v|| \mbf {V_m} \mbf {V^T_m}  e^{\mbf A} 
% \mbf V_m \mbf e_1
 \\ \nonumber
% \mbf {V_m}  \mbf {V^T_m v}  
%& =& 
& \approx &
\lVert \mbf v \rVert \mbf {V_m} e^{\mbf H_m} \mbf e_1 
\end{eqnarray}
% It is noted that in experiment for circuit simulation, the order $m$ is usually small, the overall computational complexity of exponential operator is greately reduce, so the scalability of MEXP is better than traditional implicit methods. 
%where $\mbf v = ||\mbf v||_2\mbf V_m \mbf e_1$.
%The Krylov subspace is scaling invariant, in our time domain simulation, 
%Based on the notion of residual $\mbf r$ in~\cite{Botchev2013},  %~\cite{Saad92}.
\begin{comment}
\begin{eqnarray}
\label{eq:eas belowsrr_1}
 || \mbf r_m(h) || 
% & \equiv &
 = || \mbf x_m'(h) - \mbf A \mbf x_m(h)||  
  \\ \nonumber
%  & = & -||\mbf v||_2 h_{m+1,m} 
%  \mbf v_{m+1} \mbf e^T_m e^{h\mbf H_{m}} \mbf e_1 .   
%  \\% \nonumber
%  || \mbf r_m(h) ||  & \le & 
 = ||h_{m+1,m} \mbf e^T_m h e^{h\mbf H_{m}} \mbf e_1|| .   
\end{eqnarray}
is a stop criterion for Krylov subspace 
when $\mbf x_m \approx \mbf x = e^{h\mbf A}\mbf v$, the same as the $Er_2$ in
~\cite{Botchev2013}
~\cite{Saad92}.
\end{comment}
% In pratical, the (\ref{eq:err_2}) is used as follows, 
%\begin{comment}
Since the Krylov subspace assoicate with $\mbf A$ and $h\mbf A$ are identical,
this equation
\begin{eqnarray}
e^{h\mbf A}\mbf v = 
\lVert \mbf v \rVert \mbf {V_m} e^{h\mbf H_m} \mbf e_1 
\end{eqnarray}
still holds. When the dimension of $\mbf H_m$ is small, 
computing $e^{\mbf H_m} \mbf v$ is very fast. 
In \cite{Hochbruck97},
it has been proved
that convergence of Krylov subspace for matrix exponential 
$\mbf x=  e^{h\mbf A} \mbf v$ is faster
than that for the iterave soultion of linear systems 
$(\mbf I + h\mbf A)\mbf x = \mbf v$.
%is much lower than direct computing $\mbf e^{\mbf A} \mbf v$. 

During the time domain simulation, the Arnoldi process is applied.
%on the fly of ETD circuit simulation, 
%The works~\cite{Weng12_TCAD, Weng12_ICCAD}
It computes $\mbf A \mbf v $ in the line 3 of Algorithm (\ref{algo:arnoldi}) 
as $ \mbf{\wtd C}^{-1}(\mbf{\wtd G}\mbf{v})$.
where, 
\begin{eqnarray}
\mbf A = \mbf {\wtd C}^{-1} \mbf {\wtd G} 
\end{eqnarray}
and
\begin{eqnarray}
\mbf {\wtd C} =  {\alpha}
	\left [ 
		    \begin{array}{*{20}{c}}
			\frac{1}{\alpha} \mbf C & \mbf 0 \\ 
			\mbf 0 & \mbf I_2
		    \end{array} 
	\right ], \ 
%\\ \nonumber
\mbf {\wtd G} =  \left [ 
		    \begin{array}{*{20}{c}}
			-\mbf G & \mbf {\wtd W} \\ 
			\mbf 0 & \alpha \mbf J
		    \end{array} 
\right ]
\end{eqnarray}
here $\alpha$ is introduced to balance the magnitude in $\mbf {\wtd C}$ and $\mbf {\wtd G}$.
\begin{eqnarray}
\mbf{\wtd W} = \left [ \frac{\mbf B \mbf u(t+h) - \mbf B u(t) }{h} \ \  \mbf B \mbf u(t) \right]
\end{eqnarray}

In linear circuit, the factorization $\mbf {\wtd C}$ 
is done at the beginning of simulation, 
then the construction of the following subspaces is by backward/forward substitutions.
The Algorithm (\ref{algo:arnoldi_std}) illustrates the details.
%Instead of computing time-consuming $\mbf{C}^{-1}$ explicitly. 
In order to discuss more succintly, first, 
we introduce variables 
%$\mbf X_1 = \mbf {\wtd C}$ 
$[\mbf L, \mbf U] = LU(\mbf {\wtd C})$, 
and $\mbf X_2 = \mbf {\wtd G}$.
This is called as 
\emph{standard basis} of Krylov subspace for  matrix exponential approximation, 
and has been used in \cite{Weng11_ASICON}, \cite{Weng12_TCAD}.
Our following modified versions will replace $\mbf X_1$
and $\mbf X_2$ with futher counterparts.
%represent the counterparts correspondingly.
%In Alg. \ref{algo:arnoldi_std},
%$\mbf X_1 = \mbf C$ and  $\mbf X_2 = \mbf G$. 

The $\epsilon$ 
is a threshold value to determine whether the 
accuracy of Krylov subspace approximation
for matrix expoenential is good enough. 
As we know the prior bound of such error prediction may not be sharp
and is costly to evaluate \cite{Weng12_TCAD},
the posteriori error is practically used.
%\epsilon$ 
The residual-based error  
$r_m(h)$ can be calculated 
based on \cite{Weng12_ICCAD}, \cite{Botchev2013},
%which is,
\begin{eqnarray}
\label{eq:err_std_krylov}
\lVert r_m(h) \rVert 
 =  \lVert \mbf v \rVert \left| h_{m+1,m} \mbf v_{m+1} e_m^T e^{h\mbf H_m} e_1 \right|
\end{eqnarray}

\begin{algorithm}
\label{algo:arnoldi_std}
\caption{Arnoldi process in MATEX}
%$\rm K_m(\mbf X_1^{-1}\mbf X_2, \mbf v)$} %~\cite{Weng12_TCAD, Weng12_ICCAD}}
\KwIn{ $\mbf L, \mbf U, \mbf X_2, h ,\mbf x(t),  \epsilon $  }
%\KwOut{ $\mbf V_m, \mbf H_m,  m$ }
\KwOut{ $\mbf x(t+h)$ }
    {   
%	[$\mbf L, \mbf U$]=LU($\mbf X_1$)\\
%	Normalize the intial vector 
	$\mbf v = \mbf x(t), \mbf v_1 = \frac{\mbf v }{\lVert \mbf v \rVert}$\;
	\For  {$j=1:m$}
	{
	   % Calculate 
%	    $   \mbf w =  \mbf X_1^{-1} \mbf X_2 \mbf v_{j} $ by solving
	    $\mbf w = \mbf U^{-1}  (\mbf L^{-1} (\mbf X_2 \mbf v_{j})) $ \;
	    \For {$i = 1:j$}
	    {
	%	Orthogonalization 
		$h_{i,j} = \mbf w^T\mbf v_{j}$\;
		$\mbf w = \mbf w - h_{i,j} \mbf v_{j}$\;
	    }
	    $h_{j+1,j} = \lVert \mbf w \rVert $\;
	    $\mbf v_{j+1} = \frac{\mbf w }{h_{j+1,j}} $\;
	    % \If {$ h_{i+1,j} < \epsilon $}
	    \If {$ || \mbf r_j(h)|| < \epsilon $}
	    {
		$m = j$\;
		break\;
	    }
	}
	$\mbf x(t) = \lVert \mbf v \rVert \mbf {V_m} e^{h \mbf H_m} \mbf e_1 $\;
	%$\lVert r_m(h) \rVert  =  \lVert \mbf v \rVert \left| h_{m+1,m} e_m^T e^{h\mbf H_m} e_1 \right|$
    }
\end{algorithm}


%In addition, when $\mbf{C}$ has fewer non-zeros and better structure 
%than $(\mbf{C}/h+\mbf{G})$ % of implicit methods 
%solving $\mbf{C}$ is much easier.% and it can enjoy both direct and iterative sparse solvers. 




\begin{comment}

\subsection{Adaptivity}



The ease of adaptively adjusting $h$ is a pleasing feature compared.
The invariant of scaling of Krylov subspace


\subsection{Analysis of Error and Complexity}


The error approximation of \emph{standard basis} matrix exponential calculation
depends on norm of $h\mbf A$. 
\end{comment}


\subsection{Limitations of Standard Krylov Subspace for Matrix Exponential for Circuit Simulation}

Matrix exponential method has advantages of accuracy. 
However, based on such standard Krylov subspace approximation,
there are two limitations: 
%especially when dealing 
%with stiff circuit simulation.
\begin{itemize}
\item[(1)] 
If $\mbf C$ is singular, 
it requires regularization process in \cite{Chen12_TCAD} \cite{Weng12_TCAD}. 
When the scale of problem is large, it is timing-consuming.
\item[(2)] 
It comes from the stiffness problem,
the formula (\ref{eq:exp_def}) requires large $m$ for the matrix exponential approximation.
In large scale circuit, the matrix $\mbf C$ often has wide range magnitudes of entries.
%resulting to a classic stiffness problem. 
Intuitively, the small/large magnitude entries 
of $\mbf C$ are inverted to large/small ones of   
$\mbf A$ (or $\mbf C^{-1}\mbf G$).
%, which become large ones there, 
%and vice versa.
%the circuit belongs to a stiff system. 
Therefore, $\mbf A$ features a large spectrum, 
and requires large value of $m$ or small $h$ value
to ensure the convergence of $e^{h\mbf A}$ of formula (\ref{eq:exp_def}) and $p_{m-1}(h\mbf A) $ of (\ref{eq:poly}). 
%in order to provide sufficient resolution of $h\mbf A$.
%to capture
%more important eigenvalues with small mangitudes for the exponetial operator. 
%In Krylov subspace, 
%$\mbf H_{m}$ provides a good estimation for eigenvalues with well-distributed 
%positions in the spectrum of $\mbf A$~\cite{Olsson2006}~\cite{Starke93}.
%However,% It cause the degraded convergence rate of Arnoildi process, which is resulted
% from ill-conditioned $\mbf A$.  
%It costs much more memory consumptions than nonstiff cases.
%Alternatively, 
Larger $m$ costs memory consumptions and takes more operations
during Arnoldi process; 
Smaller $h$ requires more time steps to finish
the whole transient simulation.
\end{itemize}
%tiny time-step $h$ 
%can be used for reducing the norm of $||\mbf A h||$ in the 
%upper bound (Corollary 4.6 of~\cite{Saad92}) and minimize the error. 
%\begin{eqnarray}
%|| e^{h\mbf A}\mbf v - ||\mbf v||_2 \mbf V_{m} e^{h\mbf H_m}\mbf e_1 || 
%\le 2 || \mbf v||_2 \frac{\rho^{m+1}{e^{\rho}}}{(m+1)!} 
%\end{eqnarray}
%where $\rho = ||h\mbf A||_2$. 
% the error term's value.% match the fast damped component. 
%\cite{Hochbruck97} points out the superlinear error decay requires $m$ 
%are to some extent  
%However, the ``tiny'' time steps requires more operations 
%to complete the whole transient simulation.
%Therefore, these factors become the limitations of 
%large stiff circuit using standard Krylov subspace method.
%for explicit method. 
%which is generated by $\mbf A$.
%First, it is singularity problem of matrix $\mbf C$. 
%It requires the solving the linear system of $\mbf C \mbf w = \mbf G\mbf v_i$.
%The $\mbf C $ could not be singular, and it is likely to exsit
%(i.e., nodes without grounded capacitance or 
%inductance/voltage branches).
%Therefore, extra computational effort are
%proposed as \emph{regularization} in \cite{Chen12_TCAD} to treat this scenario.

As following sections, we demonstrate two methods based
on spectral transformation, which highly accelerate the approximation of matrix exponential
and reduce memory usage compared to MEXP in \cite{Weng11_ASICON}, \cite{Weng12_TCAD}.
Besides, regularization can be eliminated due to their 
avoidance of direct inverting singular $\mbf C$.
%convergent rate of Arnoldi process forming Krylov subspace, and corresponding
%MEXP framework.
%Before introducing these two Krylov subspace algorithm, 


% We borrows the notion of ``spread/gap ratio'' here to help us decide the $\gamma$'s range. 
\begin{comment}
\subsection{Compatibility with Singular $\mbf C$ without Regularization}
%Another benign characteristic using Krylov subspace without inverse of $\mbf C$ 
%is handling singular $\mbf C$ without regularization in the rational Krylov subspace and inverted Krylov subspace. 
Even we cannot formulate Eqn. (\ref{eqn:discrete_sol}) explicitly, but the solution can be still represented as the combination of 
eigenvalues and eigenvectors \cite{Wilk:79}.
% Our method can obtain the Krylov subsapce $\mbf V_m$ and $\mbf H_m$ to  
%To illustrate our idea, 
%considering the homogenous version of Eqn. (\ref{eqn:ode}), 
%$\mbf { C} \mbf {\dot{x}} +  \mbf { G} \mbf x = 0$,
%the % general
%solution bares the form 
%$\mbf x(t+h) = \mbf Q e^{\mbf \Lambda h} \mbf Q^{-1} \mbf x(t)$,
%where $\mbf \Lambda$ is a matrix with only the diagonal terms, which are the eigenvalues of
%matrix pencil $(-\mbf G, \mbf C)$.
%\cite{Weng12_ICCAD},
To calculate such eigenvalues, the problem turns into the generalized eigenvalue problem for matrix pencil $(-\mbf G, \mbf C)$.
There are $n$ eigenvalues $\lambda_1, \lambda_2, \cdots, \lambda_n $, whose real parts are negative in passive circuits.
The solution can be expressed as $ \mbf x(t+h) = \mbf Q_n e^{h\Sigma_{n} } \mbf P_n \mbf x(t), $, where 
$\mbf Q_n \mbf P_n = \mbf I$, and $\mbf I$ is an identity $n \times n$ matrix.  The only hindrance is the existence of ``$-\infty$'' 
eigenvalues without regularization~\cite{Chen12_TCAD}. However, we can prove these eigenvalues can be eliminated in the solution, which 
is given in the following lemma.
\begin{lemma}
When all generalized eigenvalues of matrix pencil ($-\mbf G, \mbf C$) are negative, 
there exist $r$ bounded eigenvalues and $\forall i>r, \; \; \lambda_i = -\infty $.
The formula,
\begin{equation*}
\mbf x(t+h) = \mbf Q_n e^{h\Sigma_{n} } \mbf P_n \mbf x(t),
\end{equation*}
can be written as
\begin{equation*}
\mbf x(t+h) = \mbf Q_r e^{h\Sigma_{r} } \mbf P_r \mbf x(t),
\end{equation*}
where 
\begin{equation*}
\mbf \Sigma_{j} = 
 \left[
      \begin{array}{*{20}{c}} 
      \lambda_1 & 0   &\cdots  &0\\
      0 & \lambda_2   &\cdots  &0 \\
      \vdots & \vdots &\ddots &\vdots \\ 
      0 & 0 &\cdots & \lambda_j
      \end{array}
    \right]
\end{equation*}
$\mbf Q_j = [\mbf q_1, \mbf q_2, \cdots , \mbf q_j]$, 
$\mbf P_j = [\mbf p_1; \mbf p_2; \cdots ; \mbf p_j]$, 
and $\mbf q_i$ is $n\times 1$ vector,  $\mbf p_i$ is $1 \times n$ vector. 
\end{lemma}
\begin{IEEEproof}
\begin{equation*}
\mbf x(t+h) = \mbf Q_n e^{h\Sigma_{n} } \mbf P_n \mbf x(t),
\end{equation*}

\begin{eqnarray*}
\mbf x(t+h)& =& [\mbf Q_r \mbf Q_{n-r}] e^{h 
 \left[
      \begin{array}{*{20}{c}} 
      \mbf \Sigma_r & 0 \\
      0 & \mbf \Sigma_{n-r}
      \end{array}
    \right]
}
 \left[
      \begin{array}{*{20}{c}} 
      \mbf P_r  \\ 
      \mbf P_{n-r}
    \end{array}
\right] \mbf x(t) \\ 
& =& (\mbf Q_r e^{h\mbf \Sigma_r }  \mbf P_r + \mbf Q_{n-r} e^{h \mbf \Sigma_{n-r} }  \mbf P_{n-r} ) \mbf x(t) \\
&= & \mbf Q_r e^{h\mbf \Sigma_r }  \mbf P_r \mbf x(t) 
\end{eqnarray*}
where 
\begin{equation*}
e^{h \mbf \Sigma_{n-r}} = 
 \lim_{\forall i>r, \lambda_i \to -\infty} 
 \left[
      \begin{array}{*{20}{c}} 
     e^{\lambda_{r+1}} & 0   &\cdots  &0\\
      0 & e^{  \lambda_{r+2}}   &\cdots  &0 \\
      \vdots & \vdots &\ddots &\vdots \\ 
      0 & 0 &\cdots & e^{\lambda_{n}}
      \end{array}
    \right]
    \to \mbf 0
\end{equation*}
\end{IEEEproof}
%matrix pencil $(-\mbf G, \mbf C)$
%\cite{Hairer96}\cite{Wilk:79}.
%In \cite{Chen12_TCAD}, such singular $\mbf C$ without regularization makes the 
%eigenvalues contains negative infinite (``$-\infty$'') ones.
%If we put such negative infite ``eigenvalues'' there, 
By this lemma, we can take out the ``$-\infty$'' eigenvalues. 

\end{comment}
\begin{comment}
In addition, it is known that eigenvalues of Hessenberg matrix of Arnoldi process are often used as the estimation for the 
original matrix~\cite{Star:93}.  The rational Krylov subspace is also utilized to preserve the bounded eigenvalues of matrix pencil 
and corresponding eigenvectors as long as $m$ is enough\cite{Lee09}.  Therefore, by using Arnoldi process via the rational Krylov 
subspace for ($-\mbf G, \mbf C$) It holds 
\begin{eqnarray}
\mbf x(t+h) &=& \mbf Q e^{h\mbf \Sigma_n} \mbf P \mbf x(t) = \mbf Q_r e^{h\mbf \Sigma_r }  \mbf P_r \mbf x(t) \nonumber \\
	    &\approx& \mbf{V_m}e^{\alpha \mbf{{\wtd H}_m}}\mbf{V_m}^{T}\mbf x(t). \nonumber
\end{eqnarray}
The above equation illustrates that, without modification of our method using the rational Krylov subspace,
our method is compatible with the cases that contain singular $\mbf C$. 
%, where $\mbf H_m = \mbf {\wtd Q} \mbf \Sigma_m \mbf {\wtd P}$. 

Intuitively speaking, ``$-\infty$'' eigenvalues and corresponding eigenvectors do not effect the whole dynamical system via 
time derivatives here due to the exponential operator; it just forms the algebraic relations in the DAEs \cite{Hairer96}.
Previously, MEXP\cite{Weng12_TCAD}\cite{Weng12_ICCAD} cannot handle $\mbf C$ without regularization is only because the 
Arnoldi process requires to inverse $\mbf C$. Our algorithm never uses the inverse of $\mbf C$ directly.

\end{comment}
% it will hamper the efficiency of calculation.
\begin{comment}
the error is in proportion to the norm of matrix $\mbf A$
When the capacitance matrix is singular, 
the works in~\cite{Weng12_TCAD, Weng12_ICCAD} 
require regularization process. 
This process is not so cheap compared to the whole simulation. 

The Krylov subspace method, using matrix $\mbf A$ directly to form the bases, needs a large $m$ 
or a small $h$ to provide sufficient resolution 
to the spectrum of $\mbf{A}h$. 
Besides that, the large storage of $m$ bases for the high stiffness limits the size of circuit. 
We will address the issue in Section~\ref{sec:rational_krylov}. 
 
\end{comment}



%


==> new.tex <==

this 

and

that 



==> new_abst.tex <==

We proposed \emph{MATEX}, a distributed framework for
SPICE-level transient simulation of large scale
linear circuits.
It inherits the \underline{MAT}rix \underline{EX}ponentials and Krylov subspace methods to 
solve circuit's differential equations.
First, by decomposing input transitions, the whole simulation task is distributed to 
many computing nodes and parallely processed. 
Within each node, the adaptive time stepping is performed individually without refactorizing matrices. 
Second, by \emph{rational}  Krylov subspace methods, 
MATEX overcomes the stiffness hinder of previous 
matrix exponential-based circuit simulators, 
leading to larger step size with  
smaller dimensions of Krylov subspace basis. 
%This greatly reduces both memory and computational complexities.
%Since the integration kernel an inherently high polynomial approximation, 
%MATEX can utilize larger time steps to do time marching than
%circuit simulation algorithms using traditional integration kernels, 
%e.g. trapezoidal, backward Euler.
%During the simulation, MATEX has the capability of deploying adaptive time stepping 
%and still reusing factorized matrices at the very beginning, 
% even with different time step sizes,
MATEX outperforms both traditional fixed and adaptive time stepping methods,
%Besides, by utilizing superpositions and
%distributed parallel processing, 
%the scalablity of MATEX reduces runtimes furthermore, 
e.g., achieving around 12X over fixed time step in transient computing on IBM power grid benchmarks.



==> new_advanced_krylov.tex <==


In \cite{Weng12_TCAD, Weng12_ICCAD},
MEXP has shown the great advantages over TR, BE and FE on adaptive step 
controlling and promising parallelism in matrix-and-vector operations dealing with mild stiff circuits. 
MEXP starts from standard Krylov subspace to approximate matrix exponential.
However, the Hessenberg matrix $\mbf H_{m}$ of standard Krylov subspace tends to approximate the large magnitude eigenvalues of $\mbf A$ \cite{Van06}.
Due to the exponential decay of higher order terms in Taylor's expansion, such components are not the crux of circuit system's behavior \cite{Botchev12, Van06, Orec:12}.
%exponential approximation 
Dealing with stiff circuit, therefore, needs to gather more vectors into subspace basis and increase the size of $\mbf H_{m}$
to fetch more informative components, which incur both memory overhead and computational complexity into Krylov subspace generations during time stepping.
Hence direct deploying MEXP into MATEX's \emph{Circuit Solver} is  inefficient to leverage MATEX's benefits.

In the following subsections, we follow \emph{spectral transformation} \cite{Botchev12, Van06, Orec:12}
to effectively capture small magnitude eigenvalues in $\mbf A$, and then contrive a fast yet accurate \emph{Circuit Solver} for MATEX.


\subsection{Matrix Exponential Computation via
Inverted Krylov Subspace Basis (I-MATEX)}

Based on the rationale that standard Krylov subspace method tends to approximate large magnitude eigenvalues of $\mbf A$. 
Then, instead of $\mbf A$, we use $\mbf A^{-1}$ (or say, $\mbf G^{-1} \mbf C$) as our target matrix, 
%then recover it 
\begin{eqnarray}
{\rm K_m}(\mbf A^{-1} , v) := \text{span}
{\{ \mbf v, \mbf A^{-1}\mbf v, \cdots, \mbf A^{-(m-1)} \mbf v}\}
\end{eqnarray}
Intuitively, by inverting $\mbf A$, the small magnitude eigenvalues become the large ones of $\mbf A^{-1}$.
The resulting $\mbf H'_{m}$ is likely to capture these eigenvalues first. 
Based on Arnoldi algorithm, the inverted Krylov subspace has the relation 
%in pratical computation.
\begin{eqnarray}
 \mbf{A}^{-1}\mbf{V_m} =  
     \mbf V_m \mbf H'_m + 
     h'_{m+1,m} \mbf v_{m+1}\mbf e_m^\mathsf{T} 
\end{eqnarray}
The matrix exponential $e^{\mbf A} \mbf v$ is calculated as
%$\left | \beta \right| \mbf V_m \mbf e^{h\mbf H'^{-1}_m}\mbf e_1$.
$ \lVert \mbf v \rVert \mbf V_m e^{h\mbf {H'}^{-1}_m} \mbf e_1 $,

To put this method into Alg. 1, just by modifying the input variables, 
$[\mbf L,\mbf U] =  \text{LU\_Decompose}( \mbf G) $, 
$\mbf X_1 = \mbf C$.  
In the algorithm, $\mbf H_m = \mbf {H'}^{-1}_m$.
The posterior error approximation 
%$\lVert \mbf r_m(h) \rVert $ is  
\begin{eqnarray}
\label{eq:err_inverted_krylov}
  \lVert \mbf r_m(h) \rVert 
  =
  \lVert \mbf v  \rVert
  \left |  \mbf A  h'_{m+1,m} \mbf v_{m+1} 
  \mbf e^T_m {\mbf H'}^{-1}_{m}
  e^{h {\mbf H'}^{-1}_{m}}
  \mbf e_1 \right |
\end{eqnarray}
which is derived from the residual-based error approximation 
\cite{Botchev12},
%When the $\mbf A$ has large condition number and densely distributed spectrum,
When the matrix has a large condition number, the convergence rate 
will be slow in generation of inverted Krylov subspace basis. 
In the next subsection, we solve this problem by confining the specturm of $\mbf A$ with shift-and-invert Krylov subspace \cite{Van06, Moret04}, and extend the the related work in \cite{Zhuang13_ASICON}.

\subsection{Matrix Exponential Computation 
by Rational Basis of Krylov Subspace (R-MATEX)}

The shift-and-invert Krylov subspace basis is defined as 
\begin{eqnarray}
    \label{eq:rat_kry}
    \mbf {K_m}((\mbf I- \gamma \mbf {A} )^{-1}, \mbf v)   =   
	    span\{ \mbf v, (\mbf I- \gamma\mbf { A} )^{-1}\mbf v,
    \cdots,  \nonumber \\
      (  \mbf I -  \gamma \mbf{A})^{-(m-1)} \mbf v \},
\end{eqnarray}
where $\gamma$ is a predefined parameter.
With this shift, all the eigenvalues' magnitudes are larger than one. 
According to \cite{Botchev12} \cite{Van06}, the shift-and-invert basis for matrix exponential time domain simulation
is not very sensitive and the $\gamma$ can be set as $h/10$, where $h$ is the fixed step size or resolution waveform.
This method is also called as rational Krylov subspace method \cite{Zhuang13_ASICON}.
The Arnoldi process constructs $\mbf{V_m}$ and $\mbf{H_m}$, 
and the relationship is given by
\begin{eqnarray}
    \label{eq:rat_kry2}
    (\mbf{I}-  \gamma \mbf {A})^{-1} \mbf{V_m} =
    \mbf{V_m}\mbf{\widetilde{H}_m} + \tilde{h}_{m+1,m} \mbf v_{m+1} \mbf e^T_m, 
\end{eqnarray}
%where $e_m$ is the $m$-th unit vector with dimension $m \times 1$. 
%Matrix $\mbf{H_m}$ is an upper Hessenberg matrix, and 
%$\mbf{V_m}$ consists of $[\mbf v_1, \mbf v_2, \cdots , \mbf v_m]$. 
After re-arranging (\ref{eq:rat_kry2}), we can project
the $e^{\mbf{\wtd{A}}}$ onto the rational Krylov subspace as follows.
\begin{eqnarray}
    \label{eq:scale}
    e^{\mbf{\wtd A}h} \mbf{v}  \approx
    \left\| \mbf v \right\| \mbf{V_m} e^{h\mbf{  H}_m}e_1,
\end{eqnarray}
where 
${ \mbf{H_m}} = \frac{\mbf I - \mbf {\widetilde{H}}_m^{-1}}{\gamma}$. 
Following the same procedure above and in \cite{Botchev12}, 
we can render the  posterior error approximation into
\begin{eqnarray}
\label{eq:err_rational_krylov}
\lVert \mbf r_m(h) \rVert 
=
\lVert \mbf v \rVert
\left |  
\frac{\mbf I - \gamma \mbf A_m}{\gamma} 
\tilde{h}_{m+1,m}
\mbf v_{m+1} 
\mbf e^T_m \mbf{\widetilde {H}}_m^{-1}  
%{ \phi( h\mbf{\wtd H_m})} 
 e^{ h\mbf{ H}_m} 
 \mbf e_1 \right |
\end{eqnarray}
It should be noted that in practice, instead of 
computing $(\mbf I-\gamma \mbf{A})^{-1}$ directly,
%\begin{eqnarray}
$(\mbf C + \gamma \mbf G)^{-1}\mbf C $ is utilized. %\mbf V_m =  \mbf V_m \mbf H_m + h_{m+1,m}
%\mbf v_{m+1} \mbf e^T_m . 
%\end{eqnarray}
The corresponding Arnoldi process shares  
the same skeleton of Alg. \ref{algo:arnoldi} with input matrices 
%The algorithm for rational basis of Krylov subspace in our MATEX is by setting 
$[\mbf L , \mbf U] = \text{LU\_Decompose}( \mbf {C} + \gamma \mbf {G} )$ and $\mbf X = \mbf {C}$.



\subsection{Regularization-Free Krylov Subspace Basis Generation Methods}

When dealing singular $\mbf C$, MEXP needs regularization process
\cite{Chen12_TCAD} to remove the singularity of DAE in Eq.(\ref{eqn:dae}), because MEXP need to factorize $\mbf C$ in Alg. 1. 
This brings extra computational overhead when a singular case is large. 
However, it is not necessary if we can obtain the generalized eigenvalues and corresponding
eigenvectors for matrix pencil $(-\mbf G, \mbf C)$. 
In \cite{Wilk:79}, we derive the following lemma,
\begin{lemma}
Considering a homogeneous system 
%\begin{equation}
$\mbf C \mbf {  \dot{x}} = -\mbf G \mbf x$, 
%\end{equation}
$\mbf u$ and $\lambda$ are the eigenvector and eigenvalue 
of matrix pencil $(-\mbf G, \mbf C)$, then $\mbf x =  e^{t\lambda} \mbf u$ is a solution of this system.
\end{lemma}
An important observation is that we remove the regularization process in MATEX, because we do need $\mbf C^{-1}$ explicitly during Krylov subspace generation.
Instead, we only factorize $\mbf G$ for inverted Krylov subspace basis generation, 
or $(\mbf C+\gamma\mbf G)$ for rational Krylov.
Besides, $\mbf H'_m$ and $\mbf {\wtd H_m}$ are always invertible, 
and contain corresponding important generalized eigenvalues in 
matrix pencil $(-\mbf G, \mbf C)$, and define the behavior of linear dynamic system in Eqn. (\ref{eqn:dae}). 
%Then obtain the solution of the system
%Therefore, when dealing with singular $\mbf C$, these two variant Krylov subspace methods 
%do not require the regularization process \cite{Chen12_TCAD} anymore, whose main purpose is 
%%to eliminate the singularity of $\mbf C$. 

Because the $\mbf C$ is singular, the $\mbf A$ cannot be formed explicitly. 
However, for a certain lower bound of basis number, these two Krylov subspace methods
begin to converge, and 
%order $m$ large than a certain number (\~20), and 
the error of matrix exponential approximation is reduced quickly. 
Empirically, the estimation can be replaced with 
$\lVert r_m(h) \rVert = \lVert \mbf v \rVert h_{m+1,m} \left| 
\mbf e^{\mathbf T} e^{h\mbf{H}_m} \mbf e_1 \right |$
to approximate Eqn. (\ref{eq:err_inverted_krylov}), where
$\mbf H_m = \mbf {H'}^{-1}_m, h_{m+1,m} = h'_{m+1,m}$
for inverted Krylov method;
$\mbf H_m = \frac{\mbf I - \mbf {\wtd H}_m}{\gamma}, h_{m+1,m} = \wtd{ h}_{m+1,m}$
for rational Krylov method.
We set the error budget $E_{budget}$ for the time step $h$ during the $[t_{start},t_{end}]$ time span. 




==> new_complexity.tex <==



For single MATEX, given $K$ GTS requiring generation of Krylov subspace basis. 
Suppose, on average, each of them generates $m$ order basis along the time axis. 
Since one backward/ forward substitution has $O(T)$, the Krylov subspace generations on average are $O(Tm)$ when matrix exponential evaluations based on $m$ are $\mbf V_m$ and $\mbf H_m$. 
The complexity is $O(Km^3)+O(KmT)$. 
%We have $N$ computing nodes, 
After dividing the input transition, on average, we have $k$ LTS for each computing node.
There are $K-k$ snapshots need to be kept, approximately, 
and their computation take $O((K-k)m^3)$.
%for each matrix exponential computation. 
Therefore, the total computation complexity is $O(Km^3)+O(kmT)$
Since no communication required between the different processors, the extra complexity form
the unserializable parts, we denote it as $O_{s}$, which stands for the overheads of both to single and multi-node MATEX.
The speedups from single-node to multi-node
\begin{eqnarray}
%\text{Speedup}=\frac{ O(Km^3)+ O(Ktm)+O_{s} }  {O(Km^3)+O(ktm)+O_{s}}
\text{Speedup}=\frac{ Km^3+ KmT+ T_{s} }  { Km^3+ kmT +T_{s}}
\end{eqnarray}
In R-MATEX, we have very small $m$, so that the most dominating part is the $KmT$.
We can always to decomposition our input transition to make the $k$ relatively small as compared to $K$.





%The rational basis Subspace for circuit simulation is supposed to converge evne fast, when the 
%order $m$ large than a small number, and the error is reduced quickly and the estimation can be replaced with 
%$\lVert r_m(h) \rVert = 
%\lVert \mbf v \rVert h_{m+1,m} \left| \mbf e^{\mathbf T} e^{h\mbf {\wtd {H}}_m} \mbf e_1 \right |$
%to approximate Eqn. (\ref{eq:err_rational_krylov}).





==> new_framework.tex <==

\subsection{Motivation}
%from \emph{Transition Spots} vs. \emph{Snapshots} }
First,
it is necessary to illustrate how transitions of input sources form a bottleneck for MEXP-based circuit simulator.
We call the whole input transitions as \emph{Transition Spots}(TS).
In linear circuit, TS are the moments, when Krylov subspace generations are strictly required.
In another word, no matter how far a temporal marching step can be extended,
TS place a rigorous \emph{stop sign} ahead of it. 
For example, there are three input sources in 
Fig. \ref{fig:input}
Each has its own TS, \emph{Local TS}(LTS). 
When these inputs are applied to the same circuit, the three LTS form a \emph{global TS}(GTS),
which increase the number of \emph{stop signs} along time axes.
Thus, the solving process of GTS stops more frequently than that of individual LTS does.
However, in such linear system, we can resort to obtain the solutions individually by decomposing the input transitions, 
then combine them into one solution with the superposition property of linear system.
When superposing, all GTS should be computed. Therefore, every decomposed transient simulation should calculate the output at GTS besides LTS. 
Then a \emph{snapshot} for these GTS is kept in each computing node.
If $m$ is small, it cost a few extra efforts to obtain these snapshot, because we can scale the time step $h$ and reuse previous Krylov subspaces.

\subsection{Distributed MATEX framework}
It is noted that, by maintaining the snapshots, 
the summation via superposition can be postponed to the end of simulation. 
The simulation job can be decomposed and mapped to different computing nodes (Fig. \ref{fig:matex}). 
The way to decide the strategy of decomposition can be various. 
In this paper, we decompose based on bump shape (Fig. \ref{fig:ckt_ts_decomp}.
During the simulation, there is no communication overhead among different nodes. 
The snapshot requests have been already stored in the local copy of GTS within each computing node.
After slave nodes finish all simulations, they writes back the results and informs the MATEX scheduler.

\emph{Why does MATEX can leverage such distributed computing framework, but traditional methods
cannot?}
MATEX steps from Krylov subspace are derived from matrix exponential computation.
With accurate exponential calculation, the Krylov subspace can be reused to
carry time stepping along successive time spots (GTS) before encountering the next LTS.
In addition, MATEX benefits a lot from reusing factorized matrices, which come from
the very beginning of simulation, to generate a new Krylov subspace basis once reaching LTS.
The snapshot can be obtained as \emph{by-products} by scaling Hessenberg matrix and matrix exponential evaluation based on adaptive time stepping techniques similar in MEXP \cite{Weng12_TCAD}.
The LTS, GTS in the Fig. \ref{fig:input}, can be precomputed based on the provided input sources
information, and communication among different computing nodes can be avoided.
These properties render such framework a well-conditioned computational problems for large scale computing techniques, e.g. 
MapReduce, Hadoop, Mesos, Spark, MPI, etc., which now may scale to tens of thousands of nodes.

Nevertheless, the major hinders of traditional methods are LTE due to the low order polynomial approximation, 
and incapability of reusing factorized matrices once time step changes $C/h+G/2$ in Eqn. \ref{eqn:trap}. 
Within each node, we still need to derive the transient solutions step by step along all time spots (GTS) with calculations, e.g. LU, Cholesky, or backward forward substitutions. 
Therefore, to them, there is no benefit from such input transition decompositions.
The MOR techniques can be applied here; however, there will be no full model simulation and control of
the error on-the-fly, since our MATEX is still full model circuit solver.


\begin{figure}[ht]
    \centering
    \includegraphics[width=3.6in ]{./figs/time_spots.eps}
    \caption{Input}
	\label{fig:input}
\end{figure}

\begin{figure}[h]
    \centering
    \includegraphics[ width=2.5in]{./figs/rc_ckt.eps}
    \caption{Linear circuit with inputs from Fig. \ref{fig:input}}
	\label{fig:rc_ckt}
\end{figure}


\begin{figure}[ht]
    \centering
    \includegraphics[width=3.5in]{./figs/ckt_ts_decomp.eps}
    \caption{``Bump'' Shape Decomposition}
	\label{fig:ckt_ts_decomp}
\end{figure}



%\subsection{MATEX Framework for Distributed Computing}


\begin{figure}[h]
    \centering
    \includegraphics[ width=4.0in ]{./figs/hierachical_ckt_sim.eps}
    \caption{MATEX framework}
	\label{fig:matex}
\end{figure}



==> new_framework_v1.tex <==



\begin{figure}[ht]
    \centering
    \includegraphics[width=3.6in ]{./figs/time_spots.eps}
    \caption{Input}
	\label{fig:input}
\end{figure}

\begin{figure}[h]
    \centering
    \includegraphics[ width=2.5in]{./figs/rc_ckt.eps}
    \caption{Linear circuit with inputs from Fig. \ref{fig:input}}
	\label{fig:rc_ckt}
\end{figure}


\begin{figure}[ht]
    \centering
    \includegraphics[width=3.5in]{./figs/ckt_ts_decomp.eps}
    \caption{``Bump'' Shape Decomposition}
	\label{fig:ckt_ts_decomp}
\end{figure}











































\subsection{Motivation}
%from \emph{Transition Spots} vs. \emph{Snapshots} }
First,
it is necessary to illustrate how transitions of input sources form a bottleneck for MEXP-based circuit simulator.
We call the whole input transitions as \emph{Transition Spots}(TS).
In linear circuit, TS are the moments, when Krylov subspace generations are strictly required.
In another word, no matter how far a temporal marching step can be extended,
TS place a rigorous \emph{stop sign} ahead of it. 
For example, there are three input sources in 
Fig. \ref{fig:input}
Each has its own TS, \emph{Local TS}(LTS). 
When these inputs are applied to the same circuit, the three LTS form a \emph{global TS}(GTS),
which increase the number of \emph{stop signs} along time axes.
Thus, the solving process of GTS stops more frequently than that of individual LTS does.
However, in such linear system, we can resort to obtain the solutions individually by decomposing the input transitions, 
then combine them into one solution with the superposition property of linear system.
When superposing, all GTS should be computed. Therefore, every decomposed transient simulation should calculate the output at GTS besides LTS. 
Then a \emph{snapshot} for these GTS is kept in each computing node.
If $m$ is small, it cost a few extra efforts to obtain these snapshot, because we can scale the time step $h$ and reuse previous Krylov subspaces.

\subsection{Distributed MATEX framework}
It is noted that, by maintaining the snapshots, 
the summation via superposition can be postponed to the end of simulation. 
The simulation job can be decomposed and mapped to different computing nodes (Fig. \ref{fig:matex}). 
The way to decide the strategy of decomposition can be various. 
In this paper, we decompose based on bump shape (Fig. \ref{fig:ckt_ts_decomp}.
During the simulation, there is no communication overhead among different nodes. 
The snapshot requests have been already stored in the local copy of GTS within each computing node.
After slave nodes finish all simulations, they writes back the results and informs the MATEX scheduler.

\emph{Why does MATEX can leverage such distributed computing framework, but traditional methods
cannot?}
MATEX steps from Krylov subspace are derived from matrix exponential computation.
With accurate exponential calculation, the Krylov subspace can be reused to
carry time stepping along successive time spots (GTS) before encountering the next LTS.
In addition, MATEX benefits a lot from reusing factorized matrices, which come from
the very beginning of simulation, to generate a new Krylov subspace basis once reaching LTS.
The snapshot can be obtained as \emph{by-products} by scaling Hessenberg matrix and matrix exponential evaluation based on adaptive time stepping techniques similar in MEXP \cite{Weng12_TCAD}.
The LTS, GTS in the Fig. \ref{fig:input}, can be precomputed based on the provided input sources
information, and communication among different computing nodes can be avoided.
These properties render such framework a well-conditioned computational problems for large scale computing techniques, e.g. 
MapReduce, Hadoop, Mesos, Spark, MPI, etc., which now may scale to tens of thousands of nodes.

Nevertheless, the major hinders of traditional methods are LTE due to the low order polynomial approximation, 
and incapability of reusing factorized matrices once time step changes $C/h+G/2$ in Eqn. \ref{eqn:trap}. 
Within each node, we still need to derive the transient solutions step by step along all time spots (GTS) with calculations, e.g. LU, Cholesky, or backward forward substitutions. 
Therefore, to them, there is no benefit from such input transition decompositions.
The MOR techniques can be applied here; however, there will be no full model simulation and control of
the error on-the-fly, since our MATEX is still full model circuit solver.



==> new_intro.tex <==


\begin{comment}
Circuit simulation is an important and 
{\color{red} heavily used process}
during the cycle of integrated circuit (IC) designs.
The increasing integration between functional modules and interconnects
parasitic effects of modern VLSI design aggravates such simulation tasks,
rendering the transient simulation of the full system very inefficient.
Therefore, accurate yet fast circuit simulation methods have always been 
desired in the IC industry. 
\end{comment}
Theoretically sound and scalable algorithms
for linear circuit transient simulation have been always favored in the IC industry. 
It is the building block of all circuit simulators, 
which not only provides the foundation for fast general-purpose circuit anaylsis 
but also sharpen the edge dealing with modern computationally demanding power grid anaysis.
Nowadays, the emerging multi-core, many-core platforms bring powerful 
computing resource and opportunities for parallel computing. 
Even more, modern big data challenges drive cloud computing techniques \cite{cloud}, 
making distributed systems scaling to tens of thousands computing nodes
\cite{mesos, mapreduce, spark10, dryad}.
Such distributed systems will be also promising computing resources in EDA and IC industry.
However, building scalable and efficient distributed algorithmic framework for 
transient linear circuit simulation framework is still a challenge to leverage these powerful computing tools.
Previous works 
%\cite{Ye08}, \cite{Dong08}, \cite{Dong09}, \cite{Peng09},\cite{Li11}, \cite{Weng12_ICCAD}, \cite{Weng12_TCAD}
\cite{Dong08, Dong09, Li11, Weng12_ICCAD, Weng12_TCAD, Ye08, Wang13}
have been made in order to improve circuit simulation by novel algorithmics, 
parallel processing and distributed computing.

Traditional method solves differential algebra equations (DAEs) 
numerically in explicit ways, e.g., forward Euler (FE), or implicit ways, 
e.g., backward Euler (BE), Trapezoidal (TR), which are based on low order polynomial approximations for DAE.
Due to the stiffness of systems, which results from a wide range of time constants of a circuit,
the explicit methods require small time step sizes to ensure the stability.
However, implicit methods can conquer this problem by their larger stability
region. These implicit methods have to solve a linear system during each time step.
Linear systems resulted from circuit simulation is sparse and often ill conditioned.
Therefore, direct sparse matrix solver\cite{Davis06} are favored by 
linear circuit transient simulators and used as a state of art in 
current TAU power grid contest. 
There, only one factorization (LU or Cholesky factorization) is required
at the beginning of simulation.  
By reusing the factorization matrices, 
the transient computation performs only backward and forward substitutions 
and achieves better efficiency over adaptive stepping methods \cite{Xiong12, Yu12, Li12_Tau}.

Beyond the traditional ones, 
a new class of methods called exponential
time differencing (ETD) has been embraced by 
Weng \emph{et al.} \cite{Weng12_TCAD} 
%and 
%applied to time domain circuit simulations,
%with matrix exponential computation by Krylov subspace approximation, 
which is called as MEXP.
The major computation of MEXP resides in calculating the matrix exponential. 
MEXP utilizes standard Krylov subspace method based on \cite{Moler03} to approximate matrix exponentials.  
These works solve the DAEs with higher 
polynomial expansion approximations \cite{Saad92} than traditional ones.
% in majority of numerical methods. 
Nevertheless, there are still constraints for above methods. 
\begin{itemize}
\item
The solutions (state of system) at input transitions are required to solved and capture the 
system behavior, which force the adaptive stepping method to stop
and solve the linear systems or MEXP to regenerate Krylov subspace basis.
\item
The small resolution of transition distance constrains the step size of fixed time step method, 
while resorting to adaptive stepping alternatively brings matrix re-factorization overhead.
\item
Large dimension of Krylov subspace basis or small time step is needed to preserve the accuracy of
matrix exponential approximation when simulating stiff circuits, 
posing a memory bottleneck and computational burden for MEXP.
\end{itemize}
%which
%we summarize in Sec. \cite{sec:rational_krylov}.
%Recently, Zhuang, \emph{et al.} \cite{Zhuang13_ASICON} deployed
%\emph{rational} Krylov subspace method in stiff power grids to
%overcome limitation (1) and (2). 

\emph{Our Contributions}. 
%In this paper, we aim to efficent transient simulations of linear circuit. 
We devise a distributed algorithmic framework, called as \emph{MATEX}, 
of which the integral is still solved by matrix exponentials 
with variant Krylov subspace-based methods. 
%to achieve large speedups over previous MEXP. 
%To accelerate matrix exponential computation in stiff circuit simulation,  
%We generalize  \cite{Zhuang13_ASICON}
%with rational Krylov subspace 
%\cite{Zhuang13_ASICON}
\begin{itemize}
\item 
MATEX is a distributed framework leveraging the superposition property of linear system.
Through decomposing the input transition points, MATEX puts subsets of 
input transition points to different computing nodes and  process it parallelly.
\begin{itemize}
\item
In each computing node, it locally reduces the chance of Krylov subspace basis generations,
and provides more temporal interval (before the next transition point) 
so that matrix exponential can take advantage of large adaptive time steps only by scaling latest Krylov subspace basis.
\item
Meanwhile, traditional methods cannot benefit from this decomposition, since they still need to derive
solution step by step, either performing backward and forward substitutions 
or adaptive stepping with solving the linear system using direct or iterative methods.
\end{itemize}
\item 
Incorporating inverted and rational Krylov subspace bases into MATEX, we surmount the stiffness of MEXP and then form an efficient circuit solver within MATEX.
\begin{itemize}
\item 
%We  incorporate inverted and rational Krylov subspace bases into MATEX. 
This efficiently reduces the dimension of MEXP basis, 
remarkably decrease the memory consumptions 
and consequently boost computational performance. 
\item 
After unleashing from the constraint of stiffness, MATEX uses larger time size, expediting the whole time domain simulation.
%When dealing with singular capacitance/inductance matrix, 
\item
When dealing with singular capacitance/inductance matrix in DAE, these methods removes 
regularization process \cite{Chen12_TCAD, Weng12_TCAD}, which is required 
in MEXP\cite{Weng12_TCAD} and bring extra computational overhead.
\end{itemize}
%, which achieve hundreds speedups over MEXP. 
\end{itemize}
\emph{Paper Organization}.
%The rest of paper is organized as follows.
Section \ref{sec:method} introduces the background of
linear circuit simulation and matrix exponential formulations.
Section \ref{sec:matex} presents overall framework of MATEX.  
Section \ref{sec:advanced} illustrates the techniques to accelerate MATEX's circuit solver by
utilizing inverted and rational Krylov subspace methods. 
Section \ref{sec:complexity} presents complexity analysis.
Section \ref{sec:exp_results} shows numerical results 
and Section \ref{sec:conclusion} concludes this paper.


\begin{comment}
and its adaptive time controlling into MATEX. 
During the transient simulation, 
the input changes cause the updates of matrices. 
However, the updated region resides within only columns of the matrix.
By precomputing block LU calculation beforehand and 
updating that region step by step, MATEX does not require LU factorizations on-the-fly, 
which is very different from that of TR-like methods.
%{\color{red} Only by updating small part of matrices,
%due to the input change,
%MATEX's adaptive time stepping does not require 
%LU factorization on-the-fly.}

We also combine MATEX %together 
with \emph{inverted Krylov subspace} as an alternative technique,
which only requires decomposing the conductance matrix. 
Therefore,
it is advantageous the avoidance of inverting the 
matrix of capacitance and inductance, which may 
include many parasitic energy elements 
with large magnitude variations
after circuit extraction.
%{\color{red}{The connections of these two methods are inspired by the works 
%from model order reduction community, \emph{i.e.,}
%PRIMA \cite{PRIMA98} and SPRIM \cite{SPRIM04}.}}

%These solve the limitations (1) and (2);
Additionally, the parallelism of MATEX
is based on the superposition property of linear circuit.
Within our theoritically sound skeleton,
we split the input sources, use all of divided subset of input sources 
to stimuli the system, seperately, %and efficiently adaptive time stepping,
making the whole simulation task divided
into serveral sub-tasks. 
% and solved seperately 
These sub-tasks can be solved parallel, without sacrificing any accuracy. 
This circumvents the limitation (3).
Besides, the traditional methods (FE, BE, and TR) cannot benefit from this
splitting, due to their limitations not from the side of input sources
but from LTE and stability.
With the advent of inexpensive computer clusters, and multi/many-core technology,
this distributable algorithmic framework is a nice one for future implementations.


\begin{comment}


The major reason is that mainstream circuit simulators inherit implicit numerical
integration, e.g. backward Euler, Trapezoidal methods, 
for the sake of stability, where the explicit methods suffer. 
However, implict methods trouble the perspective of scalability
due to the requirement 
of solving large linear systems of differential equations.
On the contrary, the explict methods are more scalable and parallelizable 
for current multi-core and manycore architecture.
The merit of explict methods resides in simple time propogation scheme via 
matrix-vector multiplication who costs relative lower
computation and memory complexity about $O(n)$.
Even though the existence of stability issue, 
explicit methods still become a revived research 
area and verifies their parallelism and scalability 
within modern parallel computer architecture
~\cite{Dong08}\cite{Dong09}\cite{Weng12_ICCAD} during these years. 

One of promising and distinct method for circuit simulation
is matrix exponetial method (MATEX) proposed in 
\cite{Weng12_TCAD}. Apart from the above numerical methods, 
the DAE/ODE system (in one discritized region of certain time step) can  
be solved in analytical way via matrix expoential operator $e^{\mbf A}, 
\mbf A \in \mbf R_{n \times n}$. 
By the analytical property, this distinct class 
of numerical approach removes the local truncation  
and it is A-\emph{stable} for passive circuits. 
Therefore, it is not constraint by the stablity problem. 
{\color{red}{This property matters!}}
%(When $h >  0, h \to \infty$, the $x(h) \to 0$). Very unlike forward
%Euler method that require small time step to let fast damp compoent
%die down first, bring too much time steps. But M
However, the kernel computation of MATEX lies in computing matrix expoential is very high,  
e.g., direct computation consumes around $O(n^3)$ complexity. 
Weng \emph{et al.} \cite{Weng12_TCAD}\cite{Weng12_ICCAD} introduced a \emph{standard Krylov subspace}
method-based MATEX for circuit simulation to solve this problem. 
In addition, unlike the implicit methods (Trapezoidal and Back Euler) 
they both require fixed step size so that they reduce the LU online for linear circuit
transient simulation,
this MATEX can utlize the scaling invariant property of Krylov subspace to do the adaptive time-steping 
without compromising any accuracy.
(1) MATEX can jump further than BE and Trap, because the exponenital 
denomator in the exponential approximation, it is much better
than the Taylor expansion.
(2) Under the (PWL) assumptions, MATEX can also carry 
the input information during the stepping.  
(3) With the help of Krylov subspace scaling invariant, it can re-evaluate
the inter time point without rebuilding Krylov subspace.

%By this strategy, it helps to capture the low frequency response from circuit system and further speedups the whole simulation without fixed step size limitation.
% In recent years, the Krylov subspace method has
Nonetheless, the step size is actually limitted by the stiffness of matrix when utilizing standard Krylov subspace.
It is because the large spectrum of $\mbf A$ and the Arnoldi process focus on capturing %the extreme magnitude
% and
well-distributed eigenvalues, so it ofter misses the dominant factors for the circuit system/for
matrix epxonential operator, which are the ones with smallest magnitudes.
Therefore, the Arnoldi process requires large number of order to preserve the 
accurate of matrix exponential calculation. 
Also, the standard Krylov-Based MATEX requires the process of regularization \cite{Chen12_TCAD} 
to deal with singular matrix $\mbf C$, i.e., nodes without grounded capacitance or 
inductance/voltage branches. Both drag the overall performance of MATEX for circuit simulation.  
% former MATEX~\cite{Weng12_TCAD} requires regularization. 
% In addition, when the matrix $\mbf C$ is stiff, it requires smaller 
%time steps or even larger Krylov subspace 
% order $m$, which degrades the method. 


In this paper, we integrated our previous works on MATEX for linear circuits 
using \emph{rational Krylov subspace}~\cite{Zhuang13_ASICON} and \emph{inverted Krylov subspace}.
%The rational Krylov subpsace uses 
They use 
$(\mbf I-\gamma \mbf A)^{-1}$ and $\mbf A^{-1}$, respectively, 
as the basis instead of $\mbf A$ (\emph{standard Krylov subspace}) in \cite{Weng12_TCAD}. 
The rational basis limits the spectrum of a circuit matrix into a unit circle,
and the inverted operation puts the important eigenvalues with smallest magnitudes from former spectrum
into a large magnitude ones. By using Arnoldi algorithm, the Hessenberg matrix can resemble the former matrix
$\mbf A$ projected onto the new invariant subspace better and contain the more accurate important eigenvalues
for matrix exponential operator.
This method provides a good convergent rate in Arnoldi process within MATEX framework.
The inverted Krylov subspace's convergent rate in Arnoldi process may not be as good as rational basis. However,
it only requires the LU factorization of conductance matrix $\mbf G$. It provides
a strategy dealing with $\mbf C$ is very complicated from post-layout extraction, but
$\mbf G$ is much more simple then. Similarly as rational basis, by the invertion $\mbf A$, the small magnitude eigenvalues 
become the large ones in the transformed spectrum, so that the exponential of a matrix can be accurately approximated.
A very typical and important application for circuit simulation is power grid analysis, which plays an 
important role in IC deisgn methodology. Given current stimulus and power grid structure, designers should verify
and pedict the worst-case voltage noise through the simulation before signing off their design. 
The model order reduction provides good way to reduce matrix of circuit system, e.g. 
PRIMA \cite{PRIMA98} and SPRIM \cite{SPRIM04}. However, with the large number of 
input sources, this kind of strategy cannot benefit from 
the reduction models any more. 
The majority works still use Trapezoidal method with fixed step size
for the power grid simulation.
Till now, accourding to Tau power grid simulation contest 2012 \cite{Li12_Tau}\cite{Yu12}, 
the trapezoidal method with fixed step size using one LU and 
many backward/forward substitutions lead to the best performance. 
The small and fixed time steps bring benefits for the transient power grid analysis 
when dealing the voltage variation 
with high frequency, i.e. the input is changing rapidly or constantly. 

However,
when package has an important impact on accurarte 
on-die power grid analysis~\cite{Pant06}\cite{Pant07}, 
and middle and low frequency phenomena is of interests to the designers, 
trapezoidal method with fixed time step becomes very inefficient. 
It is 
because such mehtod takes long time to represent the steady state of power grid system.
In the architecture analysis, power distribution networks (PDN) 
involves with pakcage and board 
level simulations \cite{PengLi12_ICCAD}\cite{Pant06}\cite{Pant07},
which requires longer timespan of simulation,
e.g. up to few $\mu s$, the simulation process are 
often time-consuming with the limitation of fixed step size to avoid online LU.
Our method can exploit large time step, ``steady region'' of waveform
during the simulation, meanwhile, it only requires one LU factoraization
as trapezoidal method, with backward/froward substitutions.
With equivalent error buget, the krylov subspace MATEX can jump larger time step/fewer 
number of time steps
than trapezoidal
method. Therefore, even though such fully implicit scheme can be used here,
when a sparse LU factorization is affordable,
the simulation burden is higher than our Krylov subspaces MATEX because of 
more time steps need.

The aim of this paper is to present and organize the Krylov subspace based 
MATEX solver in transient simulation of linear circuit.
We list our main contributions of this paper are as follows.
\begin{itemize}
%\item A breakthrough of the circuit simulation matrix exponential.
\item Accelerate MATEX via rational and inverted Krylov 
subspace.
\item Using adaptive time 
stepping strategy for circuit simulation and overcome the 
problem to achieve low-frequency pheonomena of circuit system.
\item Eliminating the regularization process 
for singular matrix $\mbf C$ for explicit method 
of circuit simulation.
\item By input grouping and superposition property of linear circuit 
to further accelerate circuit simulation.
\item Establish the relation of MATEX with previous works on Model Order Reduction. 
\end{itemize}

By such contributions, we are able to achieve hihgly efficient trasient 
simulation. Compared to the works~\cite{Weng12_TCAD}.
It is very nice property from linear system, which they can be 
superposition. 
By this idea, the same system with the parts of inputs send to different
machines, cores, or threads and add together without communication 
during the process, only require on precomputed time stamp/anchors.
It is a nice parallelism framework, we provide such for the further 
extension.
It is noted that Trapezodal cannot achieve this benefit, because
it is not analytical solution, and the inputs are not the 
hurdles during their simulation but the stability and local trancation
error are.

The paper is organized as follows. Section II is the fundemantals 
of circuit simulation and matrix exponential inteperation.
Section III describes the Krylov methods for fast matrix exponential evaluations. 
They are three algorithms for such computation, Standard Krylov subspace, inverted 
Krylov subspace, Rational krylov subspace.
Section IV presents the computational results of simple linear circuit cases, also contains industrial power grid designs and the famous IBM benchmark suite.

\begin{comment}

\begin{itemize}
\item Accelerate MATEX via rational and inverted Krylov subspace and its coresponding adaptive time stepping strategy for circuit simulation.
%    \item And, summarize three Krylov strategies for MATEX, the standard/inverted/rational Krylov subspace.
%  \item Use inverted Krylov subspace, enable the krylov subspace based MATEX without regularization~\cite{Chen12_TCAD}.
\item Eliminating the regularization process for singular matrix $\mbf C$ for explicit method of circuit simulation.
\item Speedups linear circuit simulation, by adaptive time stepping.%  partitioning input sources, and using superposition,
    % \item Using block matrix for Krylov subspace generation.
    % \item Establish the relation of MATEX with previous works on Model Order Reduction. 
    % As a explicit circuit solver, which is also enjoy the model order reduction framework.
    %    \item Generalize the explict method for future parallelism circuit simulation (Stablity).
\end{itemize}
For solving ordinary differential equations $x'=Ax+f(t)$,
it has an anlytical solution $x(t+h)=e^{Ah}x(t)+ \int_{0}^{h}e^{A(h-\tau)}f(t+\tau)d\tau$. 
When $A$ is large, it is very expensive to cacluate the exponential operator directly.  
The explict and implict methods are strategies to approximate the operation of $e^{Ah}$.  
Explicit methods required matrix-by-vector multiplications, however, implicit methods need to solve 
a whole linear system.  
It is known that explicit methods are constraint on the size of the time steps required to make sure stability. 
Compared to explicit methods, Implicit methods have more difficulties on utilizing current 
parallel and distributed machines.  
Recent development of Krylov subspace accelerates the exponential operations.  
The  
\begin{itemize}
\item without regularization, 
    \item Accelerate and enpower MATEX framework via rational Krylov subspace algorithm.
    \item Enabling adaptive time stepping for circuit simulation.
    \item Establish the relation of MATEX with previous works on Model Order Reduction. As a explicit circuit solver, which is also enjoy the model order reduction framework.
    \item ?? Generalize the explict method for future parallelism circuit simulation (Stablity).
\end{itemize}
The MATEX has a good characteristic that the exponential operator bares the propagation in the perspective of
time derivitate,
which the method at Forward Euler (FE), Backward Euler (BE) and Trapezoidal (TRAP) method use time step $h$ to discretize the
dynamical system with respect to time. 
They lead to explicit and implicit methods,
which bring the stability and limitted time step due to the system, e.g. 
stiff systems.
Explicit methods are relatively cheap computation; Implicit methods are usually time consuming because they require
to solve the large linear systems. For this regard, in power grid simulation, it precomputes the matrix 
($\mbf C/h+ \mbf G$) in BE, or ($\mbf C/h + \mbf G/2$) in TRAP. This involes the time step $h$. 

Also, in linear circuit, the the mexponential operator is a explicit method, of which the matrix-vector multiplication
take the major part of computation.



Power grid simulation plays an important role in IC design methodology. Given current stimulus and the power grid structure, 
designers could verify and predict the worst-case voltage noise through the simulation before signing off their design.  
However, with the huge size of modern design, power grid simulation is a time-consuming process. Moreover, manifesting effects 
from the package and the board would require longer simulation time, e.g., up to few $\mu s$, which worsens the performance 
of the power grid simulation. Therefore, an efficient power grid simulation is always a demand from industry. 

Conventionally, the power grid simulation is based on the trapezoidal method where the major computation is to solve a linear 
system by either iterative approaches\cite{Saad03} or direct methods\cite{Davis06}. Many previous 
works~\cite{Chen01_Efficient}\cite{Feng08}\cite{Kozhaya02}\cite{Nassif00_Fast}\cite{Su03} utilize iterative approaches to tackle 
the scalability issue and enable adaptive stepping in the power grid simulation. However, the iterative methods usually suffer
from the convergence problem because of the ill-conditioned matrix from the power grid design. On the other hand, the direct 
methods, i.e., Cholesky or LU factorizations, are more general for solving a linear system. Despite the huge memory 
demanding and computational effort, with a carefully chosen step size, the power grid simulation could perform only one 
factorization at the beginning while the rest of operations are just backward/forward substitutions. Since a power grid design 
usually includes board and package models, a long simulation time is required to manifest the low-frequency response. Hence, 
the cost of expensive factorization can be amortized by many faster backward/forward substitutions. Such general factorization 
and fixed step size strategy~\cite{Xiong12}\cite{Yang12}\cite{Yu12}\cite{Zhao02} is widely adopted in industry.  

Beyond the traditional trapezoidal method, Weng \emph{et al.}~\cite{Weng12_TCAD, Weng12_ICCAD} introduced 
the matrix exponential method (MATEX) for the circuit simulation recently. MEXP has better accuracy and adaptivity because of the 
analytical formulation and the scaling invariant Krylov subspace approximation. Unlike the fixed step size strategy, MATEX could 
dynamically adjust the step size to exploit the low-frequency response of the power grid without expensive computation. However, 
the step size in MATEX is limited by the stiffness of circuit. Furthermore, MEXP has to regularize~\cite{Chen12_TCAD} the 
singularity in power grid, i.e., nodes without grounded capacitance or inductance/voltage branches. Both constraints would drag 
the overall performance of MATEX for the power grid simulation. 

In this work, we tailor MATEX using \emph{rational Krylov subspace} for the power grid simulation with adaptive time stepping. 
The rational Krylov subspace uses $(\mbf{I}-\gamma \mbf{A})^{-1}$ as the basis instead of $\mbf{A}$ used in the conventional Krylov 
subspace. The rational basis limits the spectrum of a circuit so that the exponential of a matrix can be accurately approximated 
even under a large step size. Moreover, the rational avoids $\mbf{C}^{-1}$ and thus eliminates the regularization process. 
As a result, MATEX with rational Krylov subspace is free from the stiffness constraint and the regularization process. The 
simulation can purely enjoy benefits of the adaptivity and the accuracy of MATEX. Even though the rational Krylov subspace still needs 
to solve a linear system as the trapezoidal method does, MATEX can factorize the matrix only once and then constructs the rest of 
rational Krylov subspaces by backward/forward substitutions. Therefore, MATEX can utilize its capability of adaptivity to accelerate 
the simulation with the same kernel operations as the fixed step size strategy. Overall, our MATEX has the following advantages: 
\begin{itemize}
    \item enabling adaptive time stepping for the power grid simulation with only one lu factorization.
    \item eliminating the regularization process for the singular power grid design.  
    \item allowing scaling large step size without compromising the accuracy. 
\end{itemize}
The experimental results demonstrate the effectiveness of MATEX with adaptive step size. The power grid simulation for IBM benchmark 
suite~\cite{Nassif08_Power} and industrial power grid designs can be accelerated 6X and 15X on average compared to the trapezoidal method. 

The rest of paper is organized as follows. Section~\ref{sec:preliminary} presents the background of the power grid simulation and MATEX. 
Sections~\ref{sec:rational_krylov} and~\ref{sec:adaptive_step_control} show the theoretical foundation of the rational Krylov subspace 
and our adaptive step scheme for the power grid simulation, respectively.  Section~\ref{sec:exp_results} presents experimental results 
of the IBM benchmark suite~\cite{Nassif08_Power} and several industrial power grid designs. Finally, Section~\ref{sec:conclusion} concludes 
this paper. 
%Specifically, the contributions of this work are:
%\begin{itemize} 
%    \item Enabling adaptive stepping in the power grid simulation with the computational cost of only one matrix factorization 
%	  and backward/forward substitutions. 
%    \item Using rational Krylov subspace method to ease the stiffness constraint~\cite{Weng12_TCAD}\cite{Weng12_ICCAD}, 
%	  meanwhile, endowing MATEX with the capability of dealing with singular $\mbf C$ without time-consuming 
%	  regularization process.
%\end{itemize}
%
\end{comment}



==> new_matex_method.tex <==


\subsection{Time Domain Formulation of Linear Circuits}

Time domain linear circuit simulation is formulated as DAEs
via modified nodal analysis (MNA),
\begin{eqnarray}
    \label{eqn:dae}
    \mbf{C}\dot{\mbf{x}}(t) = - \mbf{G}\mbf{x}(t) + \mbf{B}\mbf{u}(t),
\end{eqnarray}
where matrix $\mbf{C}$ describes the capacitance and inductance, matrix 
$\mbf{G}$ represents the resistance and the conductance between voltages 
and currents, and matrix $\mbf{B}$ indicates locations of the independent 
sources. $\mbf{x}(t)$ is a vector that stands for the nodal 
voltages and branch currents 
at time $t$, and vector $\mbf{u}(t)$ represents 
the 
%corresponding 
voltage 
and current sources.
% associated to different blocks. 
%\subsection{Matrix Exponential Method}
To solve Eqn. (\ref{eqn:dae}) numerically,
it is, commonly, 
discretized with time step $h$ and transformed
to a linear algebraic system. 
%, respectively as follows: %based on different strategies as follows,
Then, given an initial condition $\mbf x(0)$ from DC analysis, 
or previous time step $\mbf x(t)$,
% of circuit and
%$h$ is the size of time step,
$\mbf x(t+h)$ can be obtained by traditional FE, BE, TR methods.
Take TR for example, 
\begin{eqnarray}
    \label{eqn:trap}
    (\frac{\mbf{C}}{h} + 
    \frac{\mbf G}{2}) {\mbf{x}}(t+h) 
    = (\frac{\mbf C}{h}- \frac{\mbf G}{2} )
    \mbf{x}(t) + \mbf{B} \frac{ \left ( \mbf{u}(t) + \mbf{u}(t+h) \right)} {2}
  %  (2{\mbf{C}} + h{\mbf G}) {\mbf{x}}(t+h )  &   = & (2{\mbf C}- h{\mbf G} ) \mbf{x}(t) 
  %  \\ \nonumber
  % &+ & h\mbf{B}(\mbf{u}(t) +\mbf{u}(t+h))
\end{eqnarray}
which is an implicit second-order method, and probably most often used
strategy in circuit simulation for large scale simulation. It is also known that
TR with fixed time step $h$ is the most efficient academic solution for power
grid simulation
\cite{Yu12, Yang12,Xiong12, Li12_Tau}
%, which is very computational demanding.
, which, for VLSI design process, is a typical and very
important application of linear circuit simulation. 
%power grid formulation is the same as Eqn. (\ref{eqn:dae}).
%TR is the integration kernel, often applied to %the important linear circuit transient
%time domain simulation 


\subsection{Exponential Time Differencing Method with Matrix Exponentials}
There are theory \cite{Leon75} obtaining the solution of Eqn. (\ref{eqn:dae}) analytically. 
To simply illustrate the method, we convert Eqn. (\ref{eqn:dae}) into 
an system of ordinary differential equations (ODEs),
\begin{eqnarray}
\label{eqn:ode}
    \dot{\mbf{x}}(t) = \mbf{A}\mbf{x}(t) + \mbf{b}(t),
\end{eqnarray}
when $\mbf{C}$ is not singular, 
$\mbf{A} = - \mbf{C}^{-1}\mbf{G}$ 
and $\mbf{b}(t) = \mbf{C}^{-1}\mbf{B}\mbf{u}(t)$.
%This is the fundamental framework for our work in this paper,
\begin{eqnarray} 
    \label{eqn:discrete_sol}
    \mbf{x}(t+h) = e^{h\mbf{A}}\mbf{x}(t) + 
    \int^{h}_{0}e^{(h-\tau)\mbf{A}}\mbf{b}(t+\tau)d\tau.
\end{eqnarray}
%Eqn. (\ref{eqn:discrete_sol}) is the fundamental integration
%kernel of our framework MATEX.
Assuming that the input $\mbf{u}(t)$ is PWL (piecewise linear), 
we integrate the last term in 
Eqn. (\ref{eqn:discrete_sol}) analytically, 
turning the solution with matrix exponential operator:
\begin{eqnarray} 
\label{eqn:pwl_exact_sol}
    \mbf{x}(t+h)
    &=& 
    e^{h\mbf{A}}(\mbf{x}(t) + \mbf A^{-1}\mbf b(t) + \mbf A^{-2} \frac{\mbf b(t+h)- \mbf b(t)}{h})
  %  e^{h\mbf{A}}\mbf y(t)
    \nonumber \\
    & & 
    -(\mbf A^{-1}\mbf b(t+h) + \mbf A^{-2} \frac{\mbf b(t+h)- \mbf b(t)}{h})
	%	\\
	%	\nonumber
\end{eqnarray}
The bottleneck of the computation is $e^{\mbf A}$, which cost $O(n^3)$,
where $n$ is the number of unknowns.

\subsection{Matrix Exponential Computation by Standard Krylov Subspace Method}

%The complexity of $e^{\mbf A}$ can be reduced
Krylov subspace method can reduce the complexity of $e^{\mbf A}$,
yet still maintain a high order polynomial approximation \cite{Saad92} deployed by MEXP  \cite{Weng12_TCAD}.
%using Krylov subspace method and still maintained  
%with a high order polynomial approximation \cite{Saad92}, 
%which has been deplyed by MEXP \cite{Weng12_TCAD}.
In this paper, we call the Krylov subspace utilized in MEXP as \emph{standard Krylov subpsace}, due to its
straightforward usage of $\mbf A$ when generating basis through 
Arnoldi process in Alg. \ref{algo:arnoldi}. 
First,
we reformulate Eqn. (\ref{eqn:pwl_exact_sol}) into
\begin{eqnarray}
%\label{eqn:pwl_exact_sol}
    \mbf{x}(t+h)
    =
    \mbf{y}(t+h)
    -(\mbf A^{-1}\mbf b(t+h) + \mbf A^{-2} \frac{\mbf b(t+h)- \mbf b(t)}{h})
    %	\\
\end{eqnarray}
%where,
\begin{eqnarray}
%\label{eqn:pwl_exact_sol}
    \mbf{y}(t+h)
    =
    e^{h\mbf{A}}\mbf{y}(t)	%	\\
\end{eqnarray}
where $\mbf y(t) = 
\mbf{x}(t) + \mbf A^{-1}\mbf b(t) + \mbf A^{-2} \frac{\mbf b(t+h)- \mbf b(t)}{h}$.
The standard Krylov subspace 
${\rm K_m}(\mbf A, v) := \text{span}
{\{ \mbf v, \mbf A\mbf v,
\cdots, \mbf A^{m-1} \mbf v}\}$
obtained by Arnoldi process
has the the relation
$\mbf{A}\mbf{V_m} = 
\mbf V_m \mbf H_m
+ h_{m+1,m} 
\mbf v_{m+1}\mbf e_m^\mathsf{T} 
$, where $h_{m+1,m}$ is the $(m+1,m)$ entry of Hessenberg matrix
$\mbf H_m $. 
The matrix exponential $e^{h\mbf A}$ can be approximated by 
\begin{eqnarray}
 e^{h\mbf A} \approx \lVert \mbf v \rVert \mbf V_m e^{h\mbf {H}_m} \mbf e_1 
 \end{eqnarray}
and the posterior error term is 
$\lVert r_m(h) \rVert = \lVert \mbf v \rVert h_{m+1,m} \left| 
\mbf e^{\mathbf T} e^{h\mbf{H}_m} \mbf e_1 \right |$
% the matrix $\mbf C$, 
Then, 
to generate $\mbf y(t+h)$, 
we use $[\mbf L, ~\mbf U] = LU\_Decompose(\mbf C)$,
%which can be  
%reused the factorized matrices $\mbf L ,\mbf U$ .
$\mbf X = \mbf G$ as inputs of 
Alg. \ref{algo:arnoldi}
\begin{algorithm}
\label{algo:arnoldi}
\caption{Arnoldi process in Matrix Exponential-Based Circuit Simulation with Krylov subspace Method}
%$\rm K_m(\mbf X_1^{-1}\mbf X_2, \mbf v)$} %~\cite{Weng12_TCAD, Weng12_ICCAD}}
\KwIn{ $\mbf L, \mbf U, \mbf X, h ,\mbf y(t),  \epsilon $  }
%\KwOut{ $\mbf V_m, \mbf H_m,  m$ }
\KwOut{ $\mbf y(t+h)$ }
    {   
%	[$\mbf L, \mbf U$]=LU($\mbf X_1$)\\
%	Normalize the intial vector 
	$\mbf v = \mbf x(t), \mbf v_1 = \frac{\mbf v }{\lVert \mbf v \rVert}$\;
	\For  {$j=1:m$}
	{
	   % Calculate 
%	    $   \mbf w =  \mbf X_1^{-1} \mbf X_2 \mbf v_{j} $ by solving
	    $\mbf w = \mbf U^{-1}  (\mbf L^{-1} (\mbf X \mbf v_{j})) $ \;
	    \For {$i = 1:j$}
	    {
	%	Orthogonalization 
		$h_{i,j} = \mbf w^T\mbf v_{i}$; $\mbf w = \mbf w - h_{i,j} \mbf v_{i}$\;
	    }
	    $h_{j+1,j} = \lVert \mbf w \rVert $;
	    $\mbf v_{j+1} = \frac{\mbf w }{h_{j+1,j}} $\;
	    % \If {$ h_{i+1,j} < \epsilon $}
	    \If {$ || \mbf r_j(h)|| < \epsilon $}
	    {
		$m = j$; break\;
	    }
	}
	$\mbf y(t+h) = \lVert \mbf v \rVert \mbf {V_m} e^{h \mbf H_m} \mbf e_1 $\;
	%$\lVert r_m(h) \rVert  =  \lVert \mbf v \rVert \left| h_{m+1,m} e_m^T e^{h\mbf H_m} e_1 \right|$
    }
\end{algorithm}

\subsection{Challenges of MEXP}

First, the input term embedded in Eqn. (\ref{eqn:discrete_sol}) serves a double-edged sword in MEXP.
As long as the exponential computation is accurate enough,
we can always jump in any time spot before next input transition,
which make the time stepping very flexible. 
On the other hand, the region before the next transition may be shortened
when there are a lot of independent input sources injected into the linear system. 
This problem is solved in Section \ref{sec:matex}.

The standard Krylov subspace incurs another challenge when a simulated circuit is stiff.
The larger $m$ of Hessenberg matrix, the more memory is needed to store subspace. 
This degrades the computational performance. 
If a smaller $h$ is chosen to lower the storage requirement, 
it results in a much longer computational time to finish the total transient simulation
with such tiny marching time step.
The problem is very similar to explicit method
in transient solvers based on forward Euler, 
but solved in Section \ref{sec:advanced}.






==> new_sub-concl.tex <==


In this paper, we proposed a MATEX framework for distributed computing 
transient simulation of large scale linear circuits.
It leverages the linear system's property by decomposing the task based on input transitions, 
mapping them to run in parallel, 
and then summing up results by the theory of superpositions.
We also address the stiffness problem of matrix exponential based circuit solver
by modifying the basis of Krylov subspace methods and find 
the rational Krylov subspace (R-MATEX) has the best performance.
Combined with adaptive time stepping technique and a few efforts for error control, 
In the IBM power grid benchmark, MATEX on average achieves 12X speedups of transient time stepping over fixed-step trapezoidal method.
The overall average speedup is 7X.


%We think this framework will shed a light to future architecture of circuit simulator. 
%It can also be combined with other transition partiton strategy and domain-decomposition based
%simulation, as well as exploit the locality analysis.











































==> new_sub-exp_results.tex <==

We implement our proposed MATEX in MATLAB and use UMFPACK package for LU factorization. 
The experiment is carried on Linux workstations with 
Intel Core\texttrademark~i7-4770 3.40GHz processor and 32GB memory on each.

\subsection{MATEX's Circuit Solver Performance using Different Krylov Subspace Basis} 
We test the part of circuit solver within MATEX 
using MEXP~\cite{Weng12_TCAD}, as well as our proposed I-MATEX and R-MATEX.
We create RC mesh cases %that contains 2500 nodes
with different stiffness 
by changing the entries of matrix $\mbf C,~ \mbf G$. 
%the stiffness of $-\mbf C^{-1}\mbf G$ is changed. 
The stiffness here is defined as 
$ \frac{Re(\lambda_{min})}{Re(\lambda_{max})}$,
where $\lambda_{min}$ and $\lambda_{max}$ 
are the minimum and maximum eigenvalues of $-\mbf C^{-1} \mbf G$.
Transient results are simulated $[0,0.3ns]$ with a fixed time step, $5ps$.
Table~\ref{tab:rc_cases} shows 
the average Krylov subspace basis dimension $m_{a}$ and the peak dimension $m_{p}$
used to compute matrix exponential during the transient simulations. 
We also compare the runtime speedups (Spdp) over MEXP. %and speedup of RC case.
The Err (\%) is the relative error opposed to 
backward Euler method with tiny fixed step size $0.05ps$.
%However, in this small but stiff cases,
%There are not so much different from I-MATEX and R-MATEX in this case.
%\subsubsection{Eigenvalues distribution}
%In this subsection, it is comparison among different krylov subspace basis, to
%fetch the $\mbf A$'s eigenvanlue.
\begin{table}[hp]
\footnotesize
    \caption{Comparisions among MEXP, I-MATEX and R-MATEX with RC cases}
    \centering
    \begin{tabular}{|c||c|c|c|c|c|c|}
    \hline
	Method  & $m_{a}$ &   $m_{p} $  & Err(\%)    & Spdp 
	& {Stiffness}  \\ 
	\hline
	MEXP	&  211.4   	&   229  	&  0.510   & -- &
	\multirow{3}{*}{$2.1 \times 10^{16}$ } 
	\\
	\cline{1-5}
	I-MATEX	& 5.7 	&14       &  0.004	   & 2616X   &   \\
	\cline{1-5}
	R-MATEX	& 6.9   & 12   &  0.004   &  2735X   & \\ 
	\hline
	\hline
	MEXP	&  154.2   	&   224  	&  0.004 & --  
	& 	    \multirow{3}{*}{$2.1 \times 10^{12}$ } 
	\\
	\cline{1-5}
	I-MATEX	&  5.7 	& 14       &0.004   &  583X  &   \\
	\cline{1-5}
	R-MATEX	& 6.9  & 12   &  0.004 	   &  611X  & \\ 
	\hline
	\hline
	MEXP &  148.6   	&   223  & 0.004  &  -- & 	    \multirow{3}{*}{$2.1 \times 10^{8}$ } 
	\\
	\cline{1-5}
	I-MATEX	& 5.7  	& 14      & 0.004     & 229X  &   \\
	\cline{1-5}
	R-MATEX	& 6.9  & 12   &  0.004  &  252X  & \\ 
	%\cline{1-6}
	\hline
    \end{tabular}
    \label{tab:rc_cases}
\end{table}

\begin{table*}[t]
%\scriptsize
\footnotesize
%\footfontesize
    \centering
    \caption{Performance comparison TR, I-MATEX and R-MATEX.
    Spdp$^1$: Speedup of I-MATEX over TR ($h=10ps$); 
    Spdp$^2$: Speedup of R-MATEX over Adaptive TR .  
    Spdp$^3$: Speedup of R-MATEX over I-MATEX.  
   }
    \begin{threeparttable}[b]
    \begin{tabular}{|c|r|r||r|r|| r| r|  r| }
    \hline
    \multirow{2}{*}{Design} & 
    \multirow{2}{*}{DC(s)} &
    \multicolumn{1}{c||}{Adaptive TR} & 
    \multicolumn{2}{c||}{I-MATEX} & 
    \multicolumn{3}{c|}{R-MATEX } 
    \\ 
    \cline{3-8} 
    &
			     &Total(s) % s I-M 
			     &Total(s) 
			     &SPDP$^1$
			     &Total(s) 
			     &SPDP$^2$
			     &SPDP$^3$
			     \\ \hline  
	ibmpg1t		     & 0.13     
			      & 29.48
			      & 27.23
			     & 1.3X
			     & 4.93	  
			     & 6.0X 
			     & 5.5X
			     \\ \hline 
    	ibmpg2t 	     & 0.80  
			    & 179.74 
			   &  124.44
			   & 1.4X 
			   & 25.90  
			   & 6.9X 
			   & 4.8X
			    \\ \hline 
    	ibmpg3t 	     & 13.83 
			    & 2792.96 
			   & 1246.69  %1988.98
			   & 2.2X
			   & 244.56  
			   & 11.4X
			   & 5.1X
			   \\ \hline
    	ibmpg4t 	    & 16.69
			    & 1773.14 
			    & 484.83 %625.12
			   & 3.7X 
			    & 140.42 %231.06 
			    & 12.6X
			    & 3.5X
			    \\ \hline
    	ibmpg5t 	    & 8.16 
			   & 2359.11
			    & 1821.60 
			    & 1.3X 
			    & 337.74 
			    & 7.0X
			    & 5.4X 
			    \\ \hline 
    	ibmpg6t 	     & 11.17
		    	& 3184.59
			    & 2784.46 %4059.30
			   & 1.1X
			    & 482.42  
			    &   6.6X 
			   &5.8X 
			    \\ 
    \hline
    \end{tabular}
   % \begin{tablenotes}\scriptsize
%	\item [1] Speedup of I-MATEX (mn) over TR ($h=10ps$) 
%	\item [2] Speedup of R-MATEX (mn)over I-MATEX (mn) 
%	\item [3] Speedup of R-MATEX (mn) over TR ($h=10ps$)
%	\item [4] Speedup of R-MATEX (mn) over TR (adpt)      
%	\vspace{-0.5in}
%    \end{tablenotes}
    \end{threeparttable}
    \label{tab:perf_mexp}
\end{table*}
\begin{table*}[tp]
%\scriptsize
\footnotesize
\centering
\caption{Speed-ups of R-MATEX over TR with fixed
time step $h=10ps$; 
Max. and Avg. Err.: compared to all output nodes' solutions provided by IBM Power Grid Benchmarks;
Spdp$^4$:$ {t_{1000}/t_{adpt}}$ speedups of transient stepping on R-MATEX over TR;
Spdp$^5$: $ {t_{t_total}/t_{r_total}}$ total runtime speedups of R-MATEX over TR. 
}
\begin{tabular}{|c||r|r||r|r| r| r|r|r|r|}
\hline
\multirow{2}{*}{Design}&
\multicolumn{2}{c||}{TR}&
\multicolumn{7}{c|}{R-MATEX}
\\
\cline{2-10}
& $t_{1000}(s)$
& $t_{t_total}(s)$
& Group
& $t_{adpt}(s)$ 
& $t_{r_total}(s)$
& Max. Err
& Avg. Err
& Spdp$^4$
& Spdp$^5$
\\
\hline
 ibmpg1t & 5.94   &   6.20  &  {\color{black} 100}  &  0.50  &  0.85  &  1.4E-4 & 2.5E-5 & 11.9X  & 7.3X  
\\
\hline
 ibmpg2t & 26.98  &   28.61  &  100  &  2.02  &  3.72  &  1.9E-4 &  4.3E-5 & 13.4X  & 7.7X  
\\
\hline
 ibmpg3t & 245.92  & 272.47  &  100  &  20.15  &  45.77 &  2.0E-4 &  3.7E-5 & 12.2X  & 6.0X  
\\
\hline
 ibmpg4t & 329.36  & 368.55  &  {\color{black} 25} & 22.35 &  65.66 &  1.1E-4 &  3.9E-5 & 14.7X  & 5.6X  
\\
\hline
 ibmpg5t & 331.67  & 350.33  &  100 & 35.67 & 54.21 &  0.7E-4 &  1.1E-5 &  9.3X  & 6.5X  
\\
\hline
 ibmpg6t & 542.04  & 567.38  &  100 & 47.27 & 74.94 &  1.0E-4 &  3.4E-5 &  11.5X  & 7.6X  
\\
\hline
\end{tabular}
\label{tab:pg_rmatex}
\end{table*}

The huge speedups by I-MATEX and R-MATEX 
are due to large reductions of Krylov subspace basis $m_a$ and $m_p$. 
%and also save the memory conusmptions.
Exactly as what we have known about, MEXP is good at handling mild stiff circuits \cite{Weng12_TCAD}, 
but inefficient on highly stiff circuits. 
Besides, we also observe that even the basis number is large, there is still possibility with relative larger error
compared to I-MATEX and R-MATEX. 
The average dimension $m_a$ of R-MATEX is a little bit higher than I-MATEX. 
However, the dimensions of R-MATEX used along time points spread more evenly than I-MATEX.
In such small dimension Krylov subspace computation, the total simulation runtime tends to be 
dominated by matrix exponential evaluations on the time points with peak basis dimension($m_p$),
which I-MATEX has more than R-MATEX.
These result to a slightly better runtime performance of R-MATEX over I-MATEX.
% bewteen these two methods in these three cases.
%since the $m_a$ and $m_p$ of MEXP are
%extremely large and consume computational resources (time and memomry), which degrades 
%the overall runtime performance.
%I-MATEX and R-MATEX achieve significant speedups over MEXP 
%with lower demands of Krylov subspace basis dimension. 
%Besides, 

In large scale of linear circuit system and pratical VLSI designs, 
the stiffness may be even more extensive and complicated. %than our toy cases here. 
Many of them may also have large singular $\mbf C$ 
and MEXP cannot handle without regularization process.
These make  I-MATEX and R-MATEX good candidates to deal with these scenarios.
%In the following parts, we apply our I-MATEX and R-MATEX to futher cases and make comparisions 
%with other methods.

%but it spread  more stable along the total simulation in R-MATEX and $m_p$ is smaller.


\subsection{Adaptive Time Stepping}

IBM power grid benchmarks~\cite{Nassif08_Power} are used to
investigate the performance of adaptive time stepping TR based on LTE controlling 
\cite{Weng12_TCAD, Najm10_book} as well as the performance of I-MATEX, and R-MATEX. 
Every experiment is carried out on a single computing node.
The speedups of I-MATEX is not as large as R-MATEX because
I-MATEX with a large spectrum of $\mbf A$ generates large Krylov subspace. 
%in these benchmarks.
In \emph{ibmpg4t} case, the I-MATEX achieves its maximum speedups resulted from
relative small number of input transitions, so does R-MATEX.
%the power grid simulation by 

\subsection{Distributed Computing Performance }
Since R-MATEX is the most efficient circuit solver in our MATEX framework, we focus on it in the following experiments with IBM power grid benchmarks. 
These cases have many input transitions (GTS) that limit the step-size of MATEX.
Exploiting distributed computing, we can easily decompose the inputs proposed in Sec. \ref{sec:matex} 
to obtain fewer transitions of LTS for each computing node.
In IBM power grid benchmarks, we can obtain a fairly small number
of the required computing nodes, which is shown as \emph{Group} in Table. \ref{tab:pg_rmatex}).
To compete TR method we adopt a fixed time step $h=10ps$, which requires 1000 pairs of backward and forward substitutions
for the transient computing after factorizing $(C/h+G/2)$.
%For scalable experiment and simulations, we utilize the equivalent idea 
%of MATLABMPI implementations \cite{matlabmpi}. 

Since MATEX has no  communications during the transient simulation among nodes,
for distributed computing, we emulate the multiple-node environment on our workstations, 
and then select the maximum runtime among all the tasks to sum a total runtime up.
%We also record the computing time for the transient part without LU. 
For R-MATEX, we define the $t_{adpt}$ in Table. \ref{tab:pg_rmatex} as the maximum values among these recorded computing runtimes for the transient part without LU.
%MATEX with grouping is parallelizable by simulating each group in 
%multicore or cluster system.  
Our R-MATEX framework achieves on average 12X 
with respect to pure transient computing $t_{1000}/t_{adpt}$
as well as 7X on the total runtime $t_{t_total}/t_{r_total}$.
With the huge reduction of simulation time on this part, the serial LU and DC parts, which play more dominating roles in MATEX,  can be further improved using advance methods.
%~\cite{nicslu},
%which is another important study area.
%There are other way to decompose the input transitions, we use one simple
%strategy based on ``hump'' shapes, and achieve such large speedups.  

%In order to demonstrate the idea, we simply device a naive grouping scheme, which will take identical input sources together as a group. 
\begin{comment}
We assign each group to one computing nodes. 
In the experiment, we notice the message passing between 
our workstations are extreme small.
Time anchors are generated as a wall-lock, 
that visible to each node, so there are not other
communication overhead.
For example, for the message receiving only takes 0.0007 seconds, which is negligible. 
Table~\ref{tab:perf_mexp_group} shows the performance of MATEX with grouping. 
In this table, ``Groups'' is the number of groups for each 
designs, ``Min. Total`` and ``Max. Total'' is the maximum runtime among different nodes, 
%and ``Ideal Spdp'' records the ideal speedup with parallelization. 
Design ibmpg4t has only 5 groups because the alignment is better. 
The performance of MEXP has a significant improvement after grouping. 
The average ideal speedup over TR is 6 times. 
MATEX shows another parallelism in the power grid simulation from the perspective of 
input sources. 
\end{comment}

\begin{comment}
\begin{table*}[ht]
    \centering
    \caption{Performance of R-MATEX w/ Grouping}
    \begin{tabular}{|c||r |r|r|r|r|r|}
    \hline
    \multirow{2}{*}{Design} & \multirow{2}{*}{TR Trans(s)} & \multicolumn{5}{c|} {R-MATEX w/ grouping}		      \\ \cline{3-7} 
			    &			     & Groups	    & Max. Trans (s)	& Min. Trans (s)  &Spdp1  &Spdp2\\ 
    \hline ibmpg1t 	    & 5.94		     & 25	   & 0.84		& 0.48		  & 7.1X  & 12.4X \\
    \hline ibmpg2t 	    & 26.98                   & 25	   & 3.93		& 2.38		  & 6.7X  & 11.3X \\
    \hline ibmpg3t 	    & 245.92                  & 25	   & 38.09     	&21.96		  & 6.5X & 11.2X \\
    \hline ibmpg4t 	    & 329.36                  & 5	   & 33.55		&30.12		  & 9.8X  & 10.9X \\
    \hline ibmpg5t 	    & 331.67                  & 25	   & 58.54 		& 33.59		  & 5.7X & 9.9X \\
    \hline ibmpg6t 	    & 542.04                  & 25	   & 81.40 		&51.68		  & 6.7X & 28.0X \\
    \hline
    \end{tabular}
    \label{tab:perf_mexp_group}
\end{table*}


\subsection{Complexity}

The performance of MATEX and TR are dominated by the number of backward/forward substitutions. This is because the time span 
is relatively long in a power grid, and therefore, the expensive LU fatorization is amortized during the simulation. In MATEX, 
the number of backward/forward substitutions at each time step is actually $m$, which is the number of vectors forming rational 
Krylov subspace. Since $m$ is small, e.g., $5\sim 6$ in IBM benchmark suite, and MATEX uses large step size than TR, MATEX has 
less numbers of substitution operations in general. Table~\ref{tab:subs} presents number of backward/forward substitions for 
each method. ``Sub.'' is the total number of substituion operations along the simulation. MATEX has less operations but close to
TR because the ill alignment of input sources leads to many tiny step sizes whereas MATEX with grouping has much less operations 
due to well aligned inputs. These results also validate Tables~\ref{tab:perf_mexp} and \ref{tab:perf_mexp_group} where MATEX would 
has less speedup due to ill alignment issue, and the grouping scheme could improve the performance. 

\begin{table}[h]
\centering
    \caption{Number of backward/forward substitutions}
    \begin{tabular} {|c|c|c|c|}
    \hline
    \multirow{2}{*}{Design} &TR	 &MATEX		  &MATEX w/ grouping \\ \cline{2-4} 
			    & \# Sub.	 & \# Sub.        &  \# Max Sub.   \\ \hline
    ibmpg1t   		    & 1000	 &  830		  &  120	    \\ \hline 
    ibmpg2t   		    & 1000  	 &  830   	  &  120 	    \\ \hline
    ibmpg3t   		    & 1000  	 &  874   	  &  120 	    \\ \hline 
    ibmpg4t   		    & 1000  	 &  349   	  &  143 	    \\ \hline  
    ibmpg5t   		    & 1000  	 &  982   	  &  139 	    \\ \hline
    ibmpg6t   		    & 1000  	 &  932   	  &  134 	    \\ 
    \hline 
    \end{tabular}
    \label{tab:subs}
\end{table}
\end{comment}

\begin{comment}

\subsection{Scalable IBM Power Grid Suite with Input Grouping}

Following the previous subsection, we not the input is the limitation for 
adaptive steping in our MATEX framework. 
We utlize input grouping~\ref{sec:group}.
Ideal one input sources per group.

\subsubsection{2 groups}

\subsubsection{4 groups}

\subsubsection{8 groups}

\subsubsection{16 groups}

\subsubsection{32 groups}

\subsubsection{64 groups}




Secondly, we consider a single input to run ibmpg1t-ibmpg6t 
to further illustrate our method. We see there are huge speedups than using trapezoidal method.
\end{comment}
%\subsubsection{Full Solver}
%This is the ideal speedups when computing resources are available.

%\subsubsection{Model Order Reduction Preprocessing}
%In this part, we compare the MOR method and put them into trapezoidal method
%and our MATEX framework, in order to compare our method accurate.



\begin{comment}
\begin{table}[h]
    \caption{Comparisions among MEXP, I-MATEX and R-MATEX with RC cases}
    \centering
    \begin{tabular}{|c||c|c|c|c|}
    \hline
	Method  &   $m_{p} $  & Err(\%)
%	&  Time(s)
	& Speedup 
	& Stiffness\\
	%& {$\frac{Re{\lambda_{smallest}(\mbf A)}}{Re({\lambda_{largest}(A)}}$}  \\ 
	\hline
	MEXP	  	&   229  	
	&  0.510
%	&  601.87  
	& -- &
	\multirow{3}{*}{$2.1 \times 10^{16}$ } 
	\\
	\cline{1-4}
	I-MATEX	 	&14       &  0.004
%	& 0.23
	& 2616X   &   \\
	\cline{1-4}
	R-MATEX	   & 12   &  0.004  
%	& 0.22   
	&  2735X   & \\ 
	\hline
	\hline
	MEXP	  	&   224  	&  0.004  
	%&  134.32
	& --  
	& 	    \multirow{3}{*}{$2.1 \times 10^{12}$ } \\
	\cline{1-4}
	I-MATEX		& 14       &0.004   
	%&   0.23
	&  583X  &   \\
	\cline{1-4}
	R-MATEX	&  12   &  0.004  
%	& 0.20 
	&  611X  & \\ 
	\hline
	\hline
	MEXP	   	&   223  & 0.004  
%	& 52.87  
	&  -- & 	    \multirow{3}{*}{$2.1 \times 10^{8}$ } 
	\\
	\cline{1-4}
	I-MATEX  	& 14      & 0.004   
%	&  0.23 
	& 229X  &   \\
	\cline{1-4}
	R-MATEX	  & 12   &  0.004 
%	& 		0.21  
	&  252X  & \\ 
	%\cline{1-6}
	\hline
    \end{tabular}
    \label{tab:rc_cases}
\end{table}
\end{comment}


\begin{comment}
\begin{table*}[htp]
%\scriptsize
    \centering
    \caption{Performance comparison TR, I-MATEX and R-MATEX of single-node computing (sn)/multi-node simulation (mn) versions,
    Spdp$^1$: Speedup of I-MATEX (mn) over TR ($h=10ps$); 
    Spdp$^2$: Speedup of R-MATEX (mn)over I-MATEX (mn); 
    Spdp$^3$: Speedup of R-MATEX (mn) over TR ($h=10ps$);
    Spdp$^4$: Speedup of R-MATEX (mn) over TR (adpt).  
   }
    \begin{threeparttable}[b]
    \begin{tabular}{|c|r|r|r||r||r|r || r| r|| r| r ||  r|r|r|r| }
    \hline
    \multirow{2}{*}{Design} & 
    \multirow{2}{*}{DC(s)} &
    \multicolumn{2}{c||}{TR ($h=10ps$)} & 
    \multicolumn{1}{c||}{TR (adpt)} & 
    \multicolumn{2}{c||}{I-MATEX(sn)} & 
    \multicolumn{2}{c||}{I-MATEX(mn)} & 
    \multicolumn{2}{c||}{R-MATEX(sn) } & 
    \multicolumn{4}{c|}{R-MATEX(mn)} 
    \\ 
    \cline{3-15} 
			     &		&LU(s)	&Total(s)	
			    % &LU(s)	
			     &Total(s) % s I-M 
			     &LU(s)
			     &Total(s) 
			     &Total(s) 
			     &SPDP\footnote{ over TR }% (/TR.)	
			     % m I-M	
			     &LU(s)	&Total(s) % s R-M	
			     %&Spdp2\footnote{ over TR }
			     %	(/TR.)
			     &Total(s) % m R-M 
			     &SPDP\footnote{ over I-MATEX(mn) } %	(/I- (mn))
			     & SPDP\footnote{ over TR }%  (/TR.)   
			     & SPDP\footnote{ over TR (adpt)}%  (/TR.)   
			     \\ \hline  
	ibmpg1t		     & 0.13     
			      &0.13   &  6.20 	
			      & 29.48
			     & 0.12  & 27.23
			    % & 0.12  
			     & 4.68 
			     & 1.3X
			     & 0.13 & 4.93	  
		%	     & 1.3X
			     %& 0.13 
			     & 1.10
			     & 4.5X 
			     & 5.6X
			     & 26.8X
			     \\ \hline 
    	ibmpg2t 	     & 0.80  
			    & 0.83   & 28.61	
			    & 179.74 
			   & 0.76   &  124.44
			  % & 0.76 
			   & 20.19 
			   & 1.4X
			   & 0.85 
			   & 25.90  
		%	   & 1.1X
			   %& 0.85 
			   & 5.56
			    & 3.6X 
			    & 5.1X
			    & 32.3X
			    \\ \hline 
    	ibmpg3t 	     & 13.83   & 12.72  & 272.47
			    & 2792.96 
			   & 12.87 & 1246.69  %1988.98
			  % & 12.58 
			   & 213.33 %280.66 
			   & 1.3X 
			   & 12.73 
			   & 244.56  
			 %  & 1.1X
			  % & 12.81 
			   & 63.78 
			   & 3.3X 
			   & 4.3X 
			   & 43.8X
			   \\ \hline
    	ibmpg4t 	    & 16.69    & 22.50   &	368.55
			    & 1773.14 
			    & 21.09 & 484.83 %625.12
			   % & 20.99 
			    & 148.45 %231.06 
			    & 2.5X
			    & 22.09  & 140.42    
			 %   & 2.6X
			   % & 22.02  
			    & 76.55  
			    & 1.9X  
			    & 4.8X
			    & 23.1X
			    \\ \hline
    	ibmpg5t 	    & 8.16    & 10.50  & 350.33  	
			   & 2359.11
			    & 9.92 & 1821.60 
			   % & 10.03 
			    & 304.72 %413.77
			    & 1.1X
			    & 10.77 &  337.74 
			 %   & 1.0X
			   % & 10.51  
			    &  78.99 
			    &    3.9X 
			    & 4.4X
			    & 29.9X
			    \\ \hline 
    	ibmpg6t 	     & 11.17    &14.17  & 567.38
		    	& 3184.59
			    & 13.19 & 2784.46 %4059.30
			   % & 13.55 
			    & 479.79 %856.09
			   & 1.2X
			    & 14.18 & 482.42  
		%	    & 1.2X
			   % & 14.15 
			    & 108.92 
			   & 4.4X 
			    &   5.2X 
			   & 29.2X 
			    \\ 
    \hline
    \end{tabular}
   % \begin{tablenotes}\scriptsize
%	\item [1] Speedup of I-MATEX (mn) over TR ($h=10ps$) 
%	\item [2] Speedup of R-MATEX (mn)over I-MATEX (mn) 
%	\item [3] Speedup of R-MATEX (mn) over TR ($h=10ps$)
%	\item [4] Speedup of R-MATEX (mn) over TR (adpt)      
%	\vspace{-0.5in}
%    \end{tablenotes}
    \end{threeparttable}
    \label{tab:perf_mexp}
\end{table*}
\end{comment}


%Note that even though previous works\cite{Chen01_Efficient}\cite{Su03} show that using iterative approach in TR 
%could also achieve adaptive step control, long simulation time span in power grid designs make direct 
%method with fixed step size more desirable\cite{Xiong12}\cite{Yang12}\cite{Zhao02}. 
%Our benchmark includes different industrial power distribution networks (PDNs), which contain the model of 
%board and package, and also includes IBM power grid suite~\cite{Nassif08_Power}. 
%The details and simulation results of 
%both industrial designs and IBM power grid suite are presented in the following subsections. 




==> sub-concl_1.tex <==

In this paper, we proposed the MATEX framework for distributed computing 
transient simulation of large scale linear circuits.
We also address the stiffness problem of matrix exponential based circuit solver
by modifying the basis of Krylov subspace methods and find 
the rational Krylov subspace (R-MATEX) has the best perforamnce.

We propose an adaptive time stepping method for large scale power grid simulation based on MATEX. 
This method utilizes rational Krylov subspace approximation, which solves stiffness constraint and 
eliminates the regularization requirement for singular $\mbf{C}$. For the time-consuming impulse 
response simulation for industrial PDN designs, the proposed method has more than 15 times speedup on 
average over the widely-adopted fixed-step trapezoidal method. Also, the proposed method shows a
promising parallelism. The naive grouping scheme could further accelerate the power grid simulation 
about 6X on average for the IBM power grid benchmark.

In addition, the matrix exponential kernel can be a good candidate for future thermal modeling.

And linear system time domain simulation. 



{\color{red}{ reuse factorized matrices to do time stepping, and converge very fast
via matrix exponential operator}}
Note that a similar step-size control have been applied
in commercial SPICE-like simulators, such as HSPICE, to
constrain the LTE of each time step. Yet the adaptivity of
implicit methods and matrix exponential approach is quite
different in the following aspects.
1) When a step size is changed, the linear system in the
implicit methods will also change, such as C/h − G/2
in TRAP. Thus, the implicit methods must solve the
linear system again for every time-step reversal. In
practice, it is often seen that HSPICE takes a long time
to perform one-time stepping because the LTE control
forces the simulator to solve a linear system many times
to find a feasible h. MEXP is free from this overhead
when adjusting time step owing to the scaling invariant
property of Krylov subspace projection.
2) Since in implicit methods there is no easy update of
solution for a different step size, an increase in step size,
if possible, can only happen in the next step. In contrast,
    with simple scaling and reevaluation of a small matrix
    exponential, one can apply the largest permissible step
    size right in the same step.
    3) Varying order of approximation, e.g., automatic switch
    between first, second, and higher order of implicit methods
    is difficult. On the other hand, the matrix exponential
    approach allows a simultaneous adjustment of h and
    m within a wide range to optimize the computational
    efficiency.


In the future, there are many things to imporve.
Matrix decomposition method can be imported here besides the UMPACK package.

In each node computing, like GPU acceleration
the matrix-and-vector mulitpication. More tight bound error estimation. 




==> sub-exp_results_v1.tex <==

In this section, we conduct the experiments to test our methods.
First, we compare standard Krylov-Based MATEX(S-MATEX)~\cite{Weng12_TCAD},
with our inverted Krylov-Based MATEX(I-MATEX) and rational Krylov-Based MEXP (R-MATEX) and show
I-MATEX and R-MATEX are good at dealing with stiff circuit simulations.
Secondly, we compare performance of %the power grid simulation by 
I-MATEX, R-MATEX and the trapezoidal method (TR) for linear circuit simulation,
we also use IBM power grid benchmark~\cite{Nassif08_Power} to validate the efficiency
of our method for power grid application and scalablity.

%MATEX with adaptive step size control follows Algorithm~\ref{algo:adaptive_step}. 
%We set $\gamma$ as $10^{-10}$ .
%(similar as the strategy in \cite{Van06}).
%and restrict the maximum allowed step size within $1ns$ to have enough time instants to plot the figure.
%It is possible to have more fine-grain time instants, e.g., $10ps$, with only negligible cost by adjusting 
%$\alpha$ in Eqn. (\ref{eq:scale}). TR is in fixed step size in order to minimize the cost 
%of LU factorization. Both methods only perform factorization once, and rest of operations is mainly backward/forward 
%substitution. 
We implement both methods in MATLAB and use UMFPACK package for LU factorization. 
For distributed Computing, we utilize the equivalent idea of MATLABMPI \cite{matlabmpi} 
combined with shared files in network file systems.
%Note that even though previous works\cite{Chen01_Efficient}\cite{Su03} show that using iterative approach in TR 
%could also achieve adaptive step control, long simulation time span in power grid designs make direct 
%method with fixed step size more desirable\cite{Xiong12}\cite{Yang12}\cite{Zhao02}. 

%Our benchmark includes different industrial power distribution networks (PDNs), which contain the model of 
%board and package, and also includes IBM power grid suite~\cite{Nassif08_Power}. 
%The details and simulation results of 
%both industrial designs and IBM power grid suite are presented in the following subsections. 

\begin{comment}
\subsection{Comparisions on FE, BE, TR and MATEXs}
\end{comment}

\subsection{Efficiency Comparisions on S-MATEX, I-MATEX and R-MATEX of Different Stiff Systems}

We construct a RC case that contains 2500 nodes. By changing the entries of matrix $\mbf C$, 
the stiffness of $-\mbf C^{-1}\mbf G$ is changed. 
The stiffness is defined as 
$ \frac{Re(\lambda_{min})}{Re(\lambda_{max})}$, where $\lambda_{min}$ and $\lambda_{max}$ are
the minimum and maximum eigenvalues of $\mbf C^{-1} \mbf G$.

\subsubsection{$ \frac{Re(\lambda_{min})}{Re(\lambda_{max})}= 2.12 \times 10^{3}$}
The extreme values of the circuit system are shown in Table.~\ref{tab:extreme_values}
The corresponding maximum eigenvalue of $-\mbf C^{-1}\mbf G$ is $-1.88 \times 10^{9}$
and minimum eigenvalue is $-3.98 \times 10^{17}$. 

\begin{table}[htp]
  \caption{Exteme Values in $\mbf C$ and $\mbf G$}
  \centering
  \begin{tabular}{cccc}%cccc}
%    \multicolumn{2}{c}{$\mbf C$} &\multicolumn{2}{c}{$\mbf G$}\\ % &\multicolumn{2}{c}{M6} &\multicolumn{2}{c}{RDL}\\
    \hline $\mbf C_{min}$ & $\mbf C_{max}$  & $\mbf G_{min}$ & $\mbf G_{max}$ \\ % &pitch &width  &pitch &width \\
    \hline $5.04 \times 10^{-19}$   & $1.00 \times 10^{-15}$  & $1.09 \times 10^{-2}$ &$1.00 \times 10^2$ \\% &30 &4 &400 &30\\
    \hline 
  \end{tabular}
  \label{tab:extreme_values}
\end{table}


The Table.~\ref{tab:rc_cases} shows the average order $m_{avg}$ used in matrix exponential with Krylov subspace 
method, and the peak order $m_{peak}$. We also compare the total simulation time and speedup of RC case.
The experiments are performed 
on a Linux workstation with an Intel i7 2.67GHz processor and 12GB memory. T

\begin{table}[h]
    \caption{Comparision among Different MATEX with RC cases(Fixed $h=1ps$)}
    \centering
    \begin{tabular}{|c||c|c|c|c|c|c|}
    \hline
	Method  & $m_{avg}$ &   $m_{peak}$  & $E_{avg}$  & $E_{max} $ & Time & Spdp  \\ \hline
	S-MATEX	&    	&   	&   &   &  & 	   \\ \hline
	I-MATEX	&  	&       &		&     &   &   \\ \hline
	R-MATEX	&   &    &    & 	   &    & \\ \hline
    \end{tabular}
    \label{tab:rc_cases}
\end{table}



\subsubsection{$ \frac{Re(\lambda_{min})}{Re(\lambda_{max})}= 2.12 \times 10^{8}$}
In this case, the extreme values of the circuit system are shown in Table.~\ref{tab:extreme_values}
The corresponding maximum eigenvalue of $-\mbf C^{-1}\mbf G$ is $-1.88 \times 10^{9}$
and minimum eigenvalue is $-3.98 \times 10^{17}$. 
%The stiffness defined here is 
%$ \frac{Re(\lambda_{min})}{Re(\lambda_{max})}= 2.12 \times 10^{8}$ .
%The reference values $x_{ref}$ are obtained by 
%(1) running trapezoidal method with
%the very small time step $t_{small}$ to 
%$h = \sum_1^{m} t_{small}$;
%(2) the small case, we use analytical solution 
%by MATLAB's expm$(h\mbf A)\mbf v$.
%The relateive errors are caculated by $||x-x_{ref}||/||x_{ref}||$ 
%We shows with 
%We use the linear circuit from Table I~\cite{Weng12_TCAD}(D1-D5). 
% In this section, we construct a case with increasing the ``coupling'' structure of $\mbf C$.
% This means
\begin{comment}
\begin{table}[htp]
  \caption{Exteme Values in $\mbf C$ and $\mbf G$}
  \centering
  \begin{tabular}{cccc}%cccc}
%    \multicolumn{2}{c}{$\mbf C$} &\multicolumn{2}{c}{$\mbf G$}\\ % &\multicolumn{2}{c}{M6} &\multicolumn{2}{c}{RDL}\\
    \hline $\mbf C_{min}$ & $\mbf C_{max}$  & $\mbf G_{min}$ & $\mbf G_{max}$ \\ % &pitch &width  &pitch &width \\
    %\hline $5.04 \times 10^{-19}$   & $1.00 \times 10^{-15}$  & $1.09 \times 10^{-2}$ &$1.00 \times 10^2$ \\% &30 &4 &400 &30\\
    \hline $XX \times 10^{-19}$   & $XX \times 10^{-15}$  & $XX \times 10^{-2}$ &$XX \times 10^2$ \\% &30 &4 &400 &30\\
    \hline 
  \end{tabular}
  \label{tab:extreme_values}
\end{table}
\end{comment}

\begin{table}[htp]
  \caption{Exteme Values in $\mbf C$ and $\mbf G$}
  \centering
  \begin{tabular}{cccc}%cccc}
%    \multicolumn{2}{c}{$\mbf C$} &\multicolumn{2}{c}{$\mbf G$}\\ % &\multicolumn{2}{c}{M6} &\multicolumn{2}{c}{RDL}\\
    \hline $\mbf C_{min}$ & $\mbf C_{max}$  & $\mbf G_{min}$ & $\mbf G_{max}$ \\ % &pitch &width  &pitch &width \\
    \hline $5.04 \times 10^{-19}$   & $1.00 \times 10^{-15}$  & $1.09 \times 10^{-2}$ &$1.00 \times 10^2$ \\% &30 &4 &400 &30\\
    \hline 
  \end{tabular}
  \label{tab:extreme_values}
\end{table}


The Table.~\ref{tab:rc_cases} shows the average order $m_{avg}$ used in matrix exponential with Krylov subspace 
method, and the peak order $m_{peak}$. We also compare the total simulation time and speedup of RC case.
%The experiments are performed 
%on a Linux workstation with an Intel i7 2.67GHz processor and 12GB memory. 

\begin{comment}
\begin{table}[h]
%    \caption{Comparision among Different MATEX with RC cases(Fixed $h=1ps$)}
    \centering
    \begin{tabular}{|c||c|c|c|c|}
    \hline
	Method  & $m_{avg}$	& $m_{peak}$    & Time (s) & Speedup	   \\ \hline
	S-MATEX	& 101		& $250$	    	& 570.1	   & -	   \\ \hline
	I-MATEX	& $1.94$  	& 9		& 3.548    & 161   \\ \hline
	R-MATEX	& $2.24$  	& 7		& 2.397	   & 238   \\ \hline
    \end{tabular}
    \label{tab:rc_cases}
\end{table}
\end{comment}
\begin{table}[h]
    \caption{Comparision among Different MATEX with RC cases(Fixed $h=1ps$)}
    \centering
    \begin{tabular}{|c||c|c|c|c|c|c|}
    \hline
	Method  & $m_{avg}$ &   $m_{peak}$  & $E_{avg}$  & $E_{max} $ & Time & Spdp  \\ \hline
	S-MATEX	&    	&   	&   &   &  & 	   \\ \hline
	I-MATEX	&  	&       &		&     &   &   \\ \hline
	R-MATEX	& 4.26  &  10  &  1.04e-9   & 	   &    & \\ \hline
    \end{tabular}
    \label{tab:rc_cases}
\end{table}

The speedups are significant compared to S-MATEX. 
It is because the large dimension of basis required to form Krylov subsapce 
of matrix exponential approximations in S-MATEX. 
Especially in large scale of linear circuit system, the stiffness are even big
than our toy case here. Therefore, in the following sub-sections, 
we only apply our I-MATEX and R-MATEX to futher cases and make comparisions 
with other methods.
%There are not so much different from I-MATEX and R-MATEX in this case.
%\subsubsection{Eigenvalues distribution}
%In this subsection, it is comparison among different krylov subspace basis, to
%fetch the $\mbf A$'s eigenvanlue.

\begin{comment}
\subsection{Handling Post-Layout-like Matrix $\mbf C$}
In this subsection, we increase the complexity of capactiance matrix $\mbf C$
by incremental adding coupling capacitance 
\cite{Zhuang2012}~\cite{Yu2013}~\cite{Moselhy2010}.  
We know the capacitances in chip have ``geometrically'' longer 
relationship than resistor.
They are formed by the different distances from the 
corresponding master conductor
~\cite{Zhuang2012}~\cite{Yu2013}~\cite{Moselhy2010}. 
On the notion of random walk for capacitance, the coupling capacitance 
propogate in a certain distance, and result different range 
of parameters, which is not good for 
limitation of standard Krylov subspace by stiffness.
When the number of coupling capacitances is large, the nonzero entries weakens the sparsity 
of matrix $\mbf C$.
Inverted Krylov subspace is good for this scenario, 

We constructed dense capacitance matrix, and test the fluctuation of $m$ order.

It is observed that 

So it bares more possibility for coupling issues, and result in
more dense capacitance matrix than conduction matrix. 

In the following part, we shows the inverted version of Krylov subspace can handle
very dense matrix, while trapezoidal, backeuler, MATEX(std) and MATEX(rational) all
failed because out of memory.
\end{comment}

%\subsection{Industrial PDN Designs}
\subsection{Adaptive Time-Steping Examples}

We utilize industrial power distribution network cases, which is often stiff system to show MATEX's adaptivity.
The rationale is that designers rely on the simulation result of impulse response of the 
PDN design in order to characterize the design. 
Many previous works \cite{Du10}\cite{Tian96}\cite{Hu12_TVLSI}
have proposed different PDN analysis based on the impulse 
response. The nature of impulse response of the PDN design, which contains low-, mid- and high-frequency components, 
can significantly enjoy the adaptive step size in MATEXs.  
We would also like to mention that the impulse response 
based analysis is not only for the PDN design, but also for worst-case eye opening analysis in the high speed interconnect
\cite{Analui05}\cite{Shi08}. 

The industrial PDN design are given, including
on-chip power grid, package and board. The power grid consists of four metal 
layers: M1, M3, M6 and RDL. The physical parameters of each metal layer is listed in Table~\ref{tab:spec_metal_layers}. 
The package is modeled as an RL series at each C4 bump, and the board is modeled as a lumped RLC network. The
specification of each PDN design is listed in Table~\ref{tab:spec_pdn_designs} where the size of each design 
ranges from $45.7$K to $7.40$M. 

\begin{table}[htp]
  \caption{Widths and pitches of metal layers in the PDN design($\mu m$).}
  \centering
  \begin{tabular}{cccccccc}
    \multicolumn{2}{c}{M1} &\multicolumn{2}{c}{M3} &\multicolumn{2}{c}{M6} &\multicolumn{2}{c}{RDL}\\
    \hline pitch &width  &pitch &width  &pitch &width  &pitch &width \\
    \hline 2.5   &0.2  &8.5  &0.25  &30 &4 &400 &30\\
    \hline 
  \end{tabular}
  \label{tab:spec_metal_layers}
\end{table}

\begin{table}[htp]
    \caption{Specifications of PDN Designs}
    \centering
    \begin{tabular}{|c||c|c|c|c|r|}
    \hline
	Design  & Area ($mm^2$)	& \# R	    & \# C	& \# L	    & \# Nodes  \\ \hline
	D1	& $0.35^2$	& 23221	    & 15193	& 15193	    & 45.7K	\\ \hline
	D2	& $1.40^2$  	& 348582    & 228952	& 228952    & 688K	\\ \hline
	D3	& $2.80^2$  	& 1468863   & 965540	& 965540    & 2.90M	\\ \hline
	D4	& $5.00^2$  	& 3748974   & 2467400	& 2464819   & 7.40M	\\ 
    \hline
    \end{tabular}
    \label{tab:spec_pdn_designs}
\end{table}

The impulse response can be derived from the simulation result of a step input from $0$V to $1$V with a small transition
time. Hence, we inject a step input to each PDN design and compare the performance of adaptive time-stepping 
MATEX (I-MATEX, S-MATEX) and  TR (fixed time step $h=10ps$) and adaptive time-steping TR. 
The transition time of 
the step input and the simulation time span is $10ps$ and $1\mu s$ 
for observing both high- and low-frequency behavior. 
Table~\ref{tab:results_pdn_cases} shows the simulation runtime of MATEXs and TRs 
%where the fixed step size is set as $10ps$ 
to comply with the transition time. In the table, ``DC'', ``LU'' and ``Time'' indicate the runtime for DC analysis, LU 
factorization and the overall simulation, respectively. DC analysis is also via the LU factorization. We can also adopt 
other techniques \cite{Xiong12}\cite{Yang12}\cite{Yu12} to improve the performance of DC analysis for both methods. 
``Spdp'' shows the speedup of R-MATEX over TR. 
\begin{table*}[htp]
    \centering
    \caption{Simulation runtime of PDN designs}
    \begin{tabular}{|c||r|| r|r|| r|| r| r || r|r|r|}
    \hline
	\multirow{2}{*}{Design} & \multirow{2}{*}{DC(s)} 
	&\multicolumn{2}{c||}{TR ($h=10ps$)} 
	&\multicolumn{1}{c||}{TR (Adaptive)} 
	& \multicolumn{2}{c||}{I-MATEX }  
	& \multicolumn{3}{c|}{S-MATEX ($\gamma=10^{-10}$) }  
	\\ 
	\cline{3-10} 
				 &	  &LU(s)   &Total   
				 &Total	
				 &LU(s)	 &Total		  
				 &LU(s)	 &Total		& Spdp 
				 \\ \hline
        D1			& 0.11	  & 0.12   & 392.46s	
				&           % TR A
				& 0.13    & 29.00s    % I-MATEX 
				& 0.13    & 23.76s	
				&  \\ \hline
        D2 			& 2.72 
				&3.41    & 2.80h	
				&       
				& 3.78   & 1120.07s   
				& 3.98	 & 678.01s
				&  \\ \hline
        D3 			& 17.86   
				&23.22 &  12.59h	
				&      
				&       &
				& 23.80	 & 2450.04	
				&  \\ \hline
        D4 			& 62.11 
				& 76.07  & 37.24h 
				&    
				&       &  
				& 77.96	 & 7362.78s 
				& 	\\ 
    \hline
    \end{tabular}
    \label{tab:results_pdn_cases}
\end{table*}
\begin{comment}
\begin{table}[htp]
    \centering
    \caption{Simulation runtime of PDN designs}
    \begin{tabular}{|c||r|r|r||r|r|r|}
    \hline
	\multirow{2}{*}{Design} & \multirow{2}{*}{DC(s)} &\multicolumn{2}{c||}{TR ($h=10ps$)} & \multicolumn{3}{c|}{MATEX ($\gamma=10^{-10}$) }  \\ 
	\cline{3-7} 
				 &	  &LU(s)   &Total	&LU(s)	 &Total		& Spdp  \\ \hline
        D1			 &0.71	  &0.67	   &44.85m	&0.68	 &2.86m		& 15.73 \\ \hline
        D2 			 &12.21	  &15.60   &15.43h	&15.48	 &54.57m	& 16.96 \\ \hline
        D3 			 &69.59   &91.60   &76.92h	&93.28	 &4.30h		& 17.91 \\ \hline
        D4 			 &218.89  &293.81  &203.64h	&298.83	 &11.26h	& 18.08	\\ 
    \hline
    \end{tabular}
    \label{tab:results_pdn_cases}
\end{table}
\end{comment}

MATEX has significant speedup over TR because MATEX can exploit much large step size to simulate the design whereas TR can 
only step in $10ps$ for whole $1\mu s$ time span. The average speedup is 17X.  Figure~\ref{fig:result_pdn_case1} shows the 
simulation result of design D1 at a node on M1. As we can see, the result by MATEX and TR are very close to the result of 
HSPICE, which is as our reference result here. The errors of MATEX and TR to HSPICE are $7.33\times10^{-4}$ and $7.47\times10^{-4}$.  
This figure also demonstrates that a PDN design has low-, mid- and high-frequncy response so that long simulation time span is necessary. 

\begin{figure}[ht]
    \centering
    \includegraphics[width=3.0in]{./figs/result_pdn_case1.eps}
    \caption{Result of D1}
    \label{fig:result_pdn_case1}
\end{figure}



%\subsection{IBM Power Grid Suite}
\subsection{Scalable MATEX using Input Sources Grouping and Distributed Computing}

We compare MATEX and TR using the IBM power grid suite~\cite{Nassif08_Power}. 
These cases have very large input sources, that limit the step-size of MATEX, however, the circuit
systems are linear.

The simulation time is $10ns$, and TR uses fixed step size in $10ps$. 
Table~\ref{tab:spec_ibmpg} shows the details of each benchmark circuit of which size ranges from $54$K up to $3$M.
The experiment is carried on the workstations, and each node has Intel Core i7-4770 and 32G memory.

\begin{table}[h]
    \centering
    \caption{Specifications of IBM power grid suite}
    \begin{tabular}{|c|r|r|r|r|r|r|r|} 
    \hline
        Design    & \#R     & \#C      & \#L  & \#I    & \#V  & \#Nodes  \\ \hline
	ibmpg1t   & 40801   & 10774    & 277  & 10774  &14308  &54265   \\ \hline
	ibmpg2t   & 245163  & 36838    & 330  & 36838  &330    &164897  \\  \hline
	ibmpg3t   & 1602626 & 201054   & 955  & 201054 &955    &1043444 \\ \hline
	ibmpg4t   & 1826589 & 265944   & 962  & 265944 &962    &1214288 \\ \hline
	ibmpg5t   & 1550048 & 473200   & 277  & 473200 &539087 &2092148 \\ \hline
	ibmpg6t   & 2410486 & 761484   & 381  & 761484 &836249 &3203802 \\ \hline
    \end{tabular}
    \label{tab:spec_ibmpg}
\end{table}

\subsubsection{Single-Node Computing}

\begin{table*}[htp]
%\scriptsize
    \centering
    \caption{Performance comparison TR, single-node(sn)/multi-node(mn) S-MATEX and R-MATEX ($\gamma=10^{-10}$)}
    \begin{tabular}{|c|r|r|r||r|r || r| r|| r| r||  r|r|r| }
    \hline
    \multirow{2}{*}{Design} & 
    \multirow{2}{*}{DC(s)} &
    \multicolumn{2}{c||}{TR ($h=10ps$)} & 
    \multicolumn{2}{c||}{I-MATEX(sn)} & 
    \multicolumn{2}{c||}{I-MATEX(mn)} & 
    \multicolumn{2}{c||}{R-MATEX(sn) } & 
    \multicolumn{3}{c|}{R-MATEX(mn)} 
    \\ 
    \cline{3-13} 
			     &		&LU(s)	&Total(s)	
			     &LU(s)	&Total(s) % s I-M 
			     &LU(s)	&Total(s) % m I-M	
			     &LU(s)	&Total(s) % s R-M	
			     &LU(s)	&Total(s) % m R-M 
			     & Spdp     \\ \hline  
	ibmpg1t		     & 0.13     &0.13   &  6.20 	
			     & 0.12  & 40.16
			     & 0.12  & 6.40
			     & 0.13 & 4.93	  
			     & 0.13 & 1.10
			     &     \\ \hline 
    	ibmpg2t 	     & 0.80  & 0.83   & 28.61	
			   & 0.76   &  177.75
			   & 0.76  & 26.92
			   & 0.85 & 25.90  
			   & 0.85 & 5.56
			    &      \\ \hline 
    	ibmpg3t 	     & 13.83   & 12.72  & 272.47
			   & 12.87 & 1988.98
			   & 12.58 & 280.66 
			   & 12.73 & 244.56  
			   & 12.81 & 63.78 
			   &      \\ \hline
    	ibmpg4t 	    & 16.69    & 22.50   &	368.55
			    & 21.09 & 625.12
			    & 20.99 & 231.06 
			    & 22.09  & 140.42    
			    & 22.02  & 76.55  
			    &      \\ \hline
    	ibmpg5t 	    & 8.16    & 10.50  & 350.33  	
			    & 9.92 & 2590.23
			    & 10.03  & 413.77
			    & 10.77 &  337.74 
			    & 10.51  &  78.99 
			    &    
			    \\ \hline 
    	ibmpg6t 	     & 11.17    &14.17  & 567.38
			    & 13.19 & 4059.30
			    & 13.55 & 856.09
			    & 14.18 & 482.42  
			    & 14.15 & 108.92 
			    &     \\ 
    \hline
    \end{tabular}
    \label{tab:perf_mexp}
\end{table*}

\begin{figure}[ht]
    \centering
    \includegraphics[width=3.0in]{./figs/result_ibmpg6t.eps}
    \caption{Result of ibmpg6t}
    \label{fig:result_ibmpg6t}
\end{figure}


Table~\ref{tab:perf_mexp} presents the performance gains from MATEX compared to TR. 
Single Node MATEX shows a little speedup over TR that is 
not significant as that of the industrial PDN designs. 
The average of the speedup is $1.42$ times. 
The reason behind the little speedup 
in IBM benchmark suite is the fact that hundreds 
of thousands of input sources limits the maximum allowed step size. 
The simulation results 
of ibmpg6t via MATEX and TR are shown 
in Figure~\ref{fig:result_ibmpg6t} where MATEX has many small step sizes 
so that the benefit of large 
step size does not improve the performance drastically. 
As we mentioned in Section~\ref{sec:adaptive_step_control}, 
the maximum allowed 
step size is actually determined by the slope of input sources 
over a time interval. Figure~\ref{fig:align} illustrates the concept 
where $I_1$ and $I_2$ are input sources and ``max. step'' shows the maximum allowed step size 
during the simulation. As we can see, 
ill alignment causes tiny step size because MATEX 
has to guarantee constant slopes within a step size so that Eqn.~(\ref{eqn:pwl_exact_sol}) 
can be held. 
The ibmpg4t has better alignment than the other benchmark circuits, 
and thus, MATEX achieves $2.95$ speedup in ibmpg4t over TR. 

\begin{figure}[ht]
    \centering
    \includegraphics[width=3.5in]{figs/alignment.eps} 
    \caption{Input sources alignment} 
    \label{fig:align}
\end{figure}

\subsubsection{Multi-Node Computing}

Our MATEX is a highly scalable method.
%We can avoid the ill alignment issue by simply grouping ``similiar'' 
%input sources and then simulate them in separately. 
Due to the linearity of the power grid, 
the final result is just the superposition of the simulation result with each group of inputs. 
By doing so, MATEX can simulate in much larger step size in each group, e.g. rising/falling slew 
and pulse width of $I_1$ in Figure~\ref{fig:align}, 
than the step size originally in ill aligned input sources. 
MATEX with grouping is parallelizable by simulating each group in 
multicore or cluster system.  

%In order to demonstrate the idea, we simply device a naive grouping scheme, which will take identical input sources together as a group. 
We assign each group to one computing nodes. 
In the experiment, we notice the message passing between 
our workstations are extreme small.
Time anchors are generated as a wall-lock, that visible to each node, so there are not other
communication overhead.
For example, for the message receiving only takes 0.0007 seconds, which is negligible. 
Table~\ref{tab:perf_mexp_group} shows the performance of MATEX with grouping. 
In this table, ``Groups'' is the number of groups for each 
designs, ``Min. Total`` and ``Max. Total'' is the maximum runtime among different nodes, 
%and ``Ideal Spdp'' records the ideal speedup with parallelization. 
Design ibmpg4t has only 5 groups because the alignment is better. 
The performance of S-MATEX has a significant improvement after grouping. 
The average ideal speedup over TR is 6 times. 
MATEX shows another parallelism in the power grid simulation from the perspective of 
input sources. 


\begin{table}[h]
    \centering
    \caption{Performance of S-MATEX w/ Grouping}
    \begin{tabular}{|c||r |r|r|r|r|}
    \hline
    \multirow{2}{*}{Design} & \multirow{2}{*}{DC(s)} & \multicolumn{4}{c|} {MATEX w/ grouping ($\gamma=10^{-10}$)} \\ \cline{3-6} 
			    &			     & Groups	  &LU(s)  & Max. Total (s)	& Min. Total (s)   \\ 
    \hline ibmpg1t 	    & 0.28		     & 25	  &0.22   & 1.63		& 	    \\
    \hline ibmpg2t 	    & 1.12                   & 25	  &1.32   & 7.93		& 	    \\
    \hline ibmpg3t 	    & 17.72                  & 25	  &18.75  & 86.24		& 	    \\
    \hline ibmpg4t 	    & 22.04                  & 5	  &31.55  & 124.16		& 	    \\
    \hline ibmpg5t 	    & 12.40                  & 25	  &16.35  & 111.97		& 	    \\
    \hline ibmpg6t 	    & 17.66                  & 25	  &29.85  & 166.34		& 	    \\
    \hline
    \end{tabular}
    \label{tab:perf_mexp_group}
\end{table}

\begin{comment}
\subsection{Complexity}

The performance of MATEX and TR are dominated by the number of backward/forward substitutions. This is because the time span 
is relatively long in a power grid, and therefore, the expensive LU fatorization is amortized during the simulation. In MATEX, 
the number of backward/forward substitutions at each time step is actually $m$, which is the number of vectors forming rational 
Krylov subspace. Since $m$ is small, e.g., $5\sim 6$ in IBM benchmark suite, and MATEX uses large step size than TR, MATEX has 
less numbers of substitution operations in general. Table~\ref{tab:subs} presents number of backward/forward substitions for 
each method. ``Sub.'' is the total number of substituion operations along the simulation. MATEX has less operations but close to
TR because the ill alignment of input sources leads to many tiny step sizes whereas MATEX with grouping has much less operations 
due to well aligned inputs. These results also validate Tables~\ref{tab:perf_mexp} and \ref{tab:perf_mexp_group} where MATEX would 
has less speedup due to ill alignment issue, and the grouping scheme could improve the performance. 

\begin{table}[h]
\centering
    \caption{Number of backward/forward substitutions}
    \begin{tabular} {|c|c|c|c|}
    \hline
    \multirow{2}{*}{Design} &TR	 &MATEX		  &MATEX w/ grouping \\ \cline{2-4} 
			    & \# Sub.	 & \# Sub.        &  \# Max Sub.   \\ \hline
    ibmpg1t   		    & 1000	 &  830		  &  120	    \\ \hline 
    ibmpg2t   		    & 1000  	 &  830   	  &  120 	    \\ \hline
    ibmpg3t   		    & 1000  	 &  874   	  &  120 	    \\ \hline 
    ibmpg4t   		    & 1000  	 &  349   	  &  143 	    \\ \hline  
    ibmpg5t   		    & 1000  	 &  982   	  &  139 	    \\ \hline
    ibmpg6t   		    & 1000  	 &  932   	  &  134 	    \\ 
    \hline 
    \end{tabular}
    \label{tab:subs}
\end{table}
\end{comment}

\begin{comment}

\subsection{Scalable IBM Power Grid Suite with Input Grouping}

Following the previous subsection, we not the input is the limitation for 
adaptive steping in our MATEX framework. 
We utlize input grouping~\ref{sec:group}.
Ideal one input sources per group.

\subsubsection{2 groups}

\subsubsection{4 groups}

\subsubsection{8 groups}

\subsubsection{16 groups}

\subsubsection{32 groups}

\subsubsection{64 groups}




Secondly, we consider a single input to run ibmpg1t-ibmpg6t 
to further illustrate our method. We see there are huge speedups than using trapezoidal method.
\end{comment}
%\subsubsection{Full Solver}
%This is the ideal speedups when computing resources are available.

%\subsubsection{Model Order Reduction Preprocessing}
%In this part, we compare the MOR method and put them into trapezoidal method
%and our MATEX framework, in order to compare our method accurate.





==> sub-exp_results_v2.tex <==

In this section, %we conduct the experiments to test our methods.
first, we compare standard Krylov-Based MATEX(S-MATEX)~\cite{Weng12_TCAD}, 
our inverted Krylov-Based MATEX(I-MATEX) and rational Krylov-Based MEXP (R-MATEX) and show
I-MATEX and R-MATEX are good at dealing with pratical circuit simulations, especially with stiff systems.
Secondly, we compare performance of 
%the power grid simulation by 
I-MATEX, R-MATEX and the trapezoidal method (TR) for linear circuit simulation,
we also use power distributions networks (PDNs) 
and IBM power grid benchmark~\cite{Nassif08_Power} 
to validate the efficiency
of our methods for power grid application by taking advantages of 
the property of analytical solutions and its scalablity.
%MATEX with adaptive step size control follows Algorithm~\ref{algo:adaptive_step}. 
%We set $\gamma$ as $10^{-10}$ .
%(similar as the strategy in \cite{Van06}).
%and restrict the maximum allowed step size within $1ns$ to have enough time instants to plot the figure.
%It is possible to have more fine-grain time instants, e.g., $10ps$, with only negligible cost by adjusting 
%$\alpha$ in Eqn. (\ref{eq:scale}). TR is in fixed step size in order to minimize the cost 
%of LU factorization. Both methods only perform factorization once, and rest of operations is mainly backward/forward 
%substitution. 
We implement methods in MATLAB and use UMFPACK package for LU factorization. 
For scalable experiment and simulations, we utilize the equivalent idea 
of MATLABMPI implementations \cite{matlabmpi}.
%combined with shared files and network file systems.
All the experiment is carried on Linux workstations with 
Intel Core\texttrademark~i7-4770 3.40GHz processor and 32GB memory each.
%Note that even though previous works\cite{Chen01_Efficient}\cite{Su03} show that using iterative approach in TR 
%could also achieve adaptive step control, long simulation time span in power grid designs make direct 
%method with fixed step size more desirable\cite{Xiong12}\cite{Yang12}\cite{Zhao02}. 
%Our benchmark includes different industrial power distribution networks (PDNs), which contain the model of 
%board and package, and also includes IBM power grid suite~\cite{Nassif08_Power}. 
%The details and simulation results of 
%both industrial designs and IBM power grid suite are presented in the following subsections. 

\subsection{Efficiency Comparisions on S-MATEX, I-MATEX and R-MATEX of Different Stiff Systems}

In this sub-sections, we show the influence of different stiffness of circuit systems 
to S-/I-/R-/MATEX. 
We construct RC mesh cases that contains 2500 nodes with different stiffness 
by changing the entries of matrix $\mbf C$. 
%the stiffness of $-\mbf C^{-1}\mbf G$ is changed. 
The stiffness is defined as 
$ \frac{Re(\lambda_{min})}{Re(\lambda_{max})}$, where $\lambda_{min}$ and $\lambda_{max}$ are
the minimum and maximum eigenvalues of $-\mbf C^{-1} \mbf G$.
We run the transient simulations $[0,0.3ns]$ with fixed time step $5ps$.
\begin{comment}
\subsubsection{$ \frac{Re(\lambda_{min})}{Re(\lambda_{max})}= 2.12 \times 10^{3}$}
The extreme values of the circuit system are shown in Table.~\ref{tab:extreme_values}
The corresponding maximum eigenvalue of $-\mbf C^{-1}\mbf G$ is $-1.88 \times 10^{9}$
and minimum eigenvalue is $-3.98 \times 10^{17}$. 
\begin{table}[htp]
  \caption{Exteme Values in $\mbf C$ and $\mbf G$}
  \centering
  \begin{tabular}{cccc}%cccc}
%    \multicolumn{2}{c}{$\mbf C$} &\multicolumn{2}{c}{$\mbf G$}\\ % &\multicolumn{2}{c}{M6} &\multicolumn{2}{c}{RDL}\\
    \hline $\mbf C_{min}$ & $\mbf C_{max}$  & $\mbf G_{min}$ & $\mbf G_{max}$ \\ % &pitch &width  &pitch &width \\
    \hline $5.04 \times 10^{-19}$   & $1.00 \times 10^{-15}$  & $1.09 \times 10^{-2}$ &$1.00 \times 10^2$ \\% &30 &4 &400 &30\\
    \hline 
  \end{tabular}
  \label{tab:extreme_values}
\end{table}
\end{comment}
Table~\ref{tab:rc_cases} shows the average dimensions $m_{a}$ 
and the peak dimension $m_{p}$
used in the matrix exponential approximations during the transient simulations 
by different strategies of Krylov subspace basis. 
We also compare the total simulation time and speedups (Spdp) to S-MATEXs. %and speedup of RC case.
The Err (\%) is the relative error opposed to 
backward Euler method with fixed step size $0.05ps$.
\begin{table}[h]
    \caption{Comparisions among S-/I-/R-MATEX with RC cases}
    \centering
    \begin{tabular}{|c||c|c|c|c|c|c|}
    \hline
	Method  & $m_{a}$ &   $m_{p} $  & Err(\%)  &  Time(s)  & Spdp 
	& {Stiffness}  \\ 
	\hline
	S-MATEX	&  211.4   	&   229  	&  0.510  &  601.87  & -- &
	\multirow{3}{*}{$2.1 \times 10^{16}$ } 
	\\
	\cline{1-6}
	I-MATEX	& 5.7 	&14       &  0.004		& 0.23    & 2616X   &   \\
	\cline{1-6}
	R-MATEX	& 6.9   & 12   &  0.004  & 0.22   &  2735X   & \\ 
	\hline
	\hline
	S-MATEX	&  154.2   	&   224  	&  0.004  &      134.32 & --  
	& 	    \multirow{3}{*}{$2.1 \times 10^{12}$ } 
	\\
	\cline{1-6}
	I-MATEX	&  5.7 	& 14       &0.004   &   0.23  &  583X  &   \\
	\cline{1-6}
	R-MATEX	& 6.9  & 12   &  0.004  & 0.20 	   &  611X  & \\ 
	\hline
	\hline
	S-MATEX	&  148.6   	&   223  & 0.004  & 52.87  &  -- & 	    \multirow{3}{*}{$2.1 \times 10^{8}$ } 
	\\
	\cline{1-6}
	I-MATEX	& 5.7  	& 14      & 0.004   &  0.23   & 229X  &   \\
	\cline{1-6}
	R-MATEX	& 6.9  & 12   &  0.004  & 	0.21   &  252X  & \\ 
	%\cline{1-6}
	\hline
    \end{tabular}
    \label{tab:rc_cases}
\end{table}
S-MATEX is good to handle mild stiff circuits \cite{Weng12_TCAD}.
However, these cases show that the S-MATEX are senstive to the stiffness, especially 
it becomes large.
It is not efficient on highly stiff circuits, since the $m_a$ and $m_p$ of S-MATEX are
extremely large and consume computational resources (time and memomry), which degrades 
the overall runtime performance.

%However, in this small but stiff cases,
Meanwhile, I-MATEX and R-MATEX achieve significant speedups over S-MATEX 
by the lower demands of
Krylov subspace basis dimension. 
The average dimension $m_a$ of R-MATEX is higher than I-MATEX, 
but the peak $m_p$ are smaller.
Besides, the dimensions of R-MATEX used in each time step spread more evenly than I-MATEX,
These result to the similar runtime performance bewteen these two methods in these three cases.
% R-MATEX as I-MATEX.
%However, the high stiffness are very common in VLSI designs,

As we known, in large scale of linear circuit system and pratical VLSI designs, 
the stiffness may be even bigger and complicated than our toy cases here.
Compared to S-MATEX,  
proposed I-MATEX and R-MATEX are good candidates to deal with these scenarios.
It is because the smaller dimension of basis required to form Krylov subsapce 
of matrix exponential approximations. 
%in S-MATEX. 
Therefore, in the following sub-sections, 
we only apply our I-MATEX and R-MATEX to futher cases and make comparisions 
with other methods.
%There are not so much different from I-MATEX and R-MATEX in this case.
%\subsubsection{Eigenvalues distribution}
%In this subsection, it is comparison among different krylov subspace basis, to
%fetch the $\mbf A$'s eigenvanlue.

\begin{comment}
\subsection{Handling Post-Layout-like Matrix $\mbf C$}

In this subsection, we increase the complexity of capactiance matrix $\mbf C$
by incremental adding coupling capacitance 
\cite{Zhuang2012}~\cite{Yu2013}~\cite{Moselhy2010}.  
We know the capacitances in chip have ``geometrically'' longer 
relationship than resistor.
They are formed by the different distances from the 
corresponding master conductor
~\cite{Zhuang2012}~\cite{Yu2013}~\cite{Moselhy2010}. 
On the notion of random walk for capacitance, the coupling capacitance 
propogate in a certain distance, and result different range 
of parameters, which is not good for 
limitation of standard Krylov subspace by stiffness.
When the number of coupling capacitances is large, the nonzero entries weakens the sparsity 
of matrix $\mbf C$.
Inverted Krylov subspace is good for this scenario, 

We constructed dense capacitance matrix, and test the fluctuation of $m$ order.

It is observed that 

So it bares more possibility for coupling issues, and result in
more dense capacitance matrix than conduction matrix. 

In the following part, we shows the inverted version of Krylov subspace can handle
very dense matrix, while trapezoidal, backeuler, MATEX(std) and MATEX(rational) all
failed because out of memory.
\end{comment}

%\subsection{Industrial PDN Designs}
\subsection{Adaptive Time-Steping Examples}

We utilize industrial power distribution network cases to show MATEX's adaptivity.
The rationale is that designers rely on the simulation result of impulse response of the 
PDN design in order to characterize the design. 
Many previous works \cite{Du10}\cite{Tian96}\cite{Hu12_TVLSI}
have proposed different PDN analysis based on the impulse 
response. 
The nature of impulse response of the PDN design, 
which contains low-, mid- and high-frequency components, 
can significantly enjoy the adaptive step size in MATEX.  
We would also like to mention that the impulse response 
based analysis is not only for the PDN design, 
but also for worst-case eye opening analysis in the high speed interconnect
\cite{Analui05}\cite{Shi08}. 

The industrial PDN design are given, including
on-chip power grid, package and board. 
The power grid consists of four metal 
layers: M1, M3, M6 and Redistribution Layer (RDL). 
The physical parameters of each metal layer 
is listed in Table~\ref{tab:spec_metal_layers}. 
The package is modeled as an RL series at each C4 bump, 
and the board is modeled as a lumped RLC network. The
specification of each PDN design is listed in Table~\ref{tab:spec_pdn_designs} 
where the size of each design 
ranges from $45.7$K to $7.40$M. 
\begin{table}[htp]
  \caption{Widths and pitches of metal layers in the PDN design($\mu m$).}
  \centering
  \begin{tabular}{cccccccc}
    \multicolumn{2}{c}{M1} &\multicolumn{2}{c}{M3} 
    &\multicolumn{2}{c}{M6} &\multicolumn{2}{c}{RDL}\\
    \hline pitch &width  &pitch &width  &pitch &width  &pitch &width \\
    \hline 2.5   &0.2  &8.5  &0.25  &30 &4 &400 &30\\
    \hline 
  \end{tabular}
  \label{tab:spec_metal_layers}
\end{table}

\begin{table}[htp]
    \caption{Specifications of PDN Designs}
    \centering
    \begin{tabular}{|c||r|r|r|r|r|}
    \hline
	Design  & Area ($mm^2$)	& \# R	    & \# C	& \# L	    & \# Nodes  \\ \hline
	D1	& $0.35^2$	& 23221	    & 15193	& 15193	    & 45.7K	\\ \hline
	D2	& $1.40^2$  	& 348582    & 228952	& 228952    & 688K	\\ \hline
	D3	& $2.80^2$  	& 1468863   & 965540	& 965540    & 2.90M	\\ \hline
	D4	& $5.00^2$  	& 3748974   & 2467400	& 2464819   & 7.40M	\\ 
    \hline
    \end{tabular}
    \label{tab:spec_pdn_designs}
\end{table}
The impulse response can be derived from the simulation result 
of a step input from $0$V to $1$V with a small transition time. 
Hence, we inject a step input to each PDN design and 
compare the performance of adaptive time-stepping 
MATEXs (I-MATEX, S-MATEX), and TR (fixed time step $h=10ps$), adaptive time-steping TR. 
The transition time of 
the step input and the simulation time span is $10ps$ and $1\mu s$ 
for observing both high- and low-frequency behavior. 
For such large size application, in the respective of memory counsumption, 
we limit the Krylov subspace order $m$ within $[6,~30]$. During the simulation. 
We find such region can provide enough accuracy for matrix exponential approximation by I-MATEX and S-MATEX.
Table~\ref{tab:results_pdn_cases} shows the simulation runtime of MATEXs and TRs 
%where the fixed step size is set as $10ps$ 
to comply with the transition time. 
In the table, ``DC'', ``LU'' and ``Total'' 
indicate the runtime for DC analysis, LU 
factorization and the overall simulation, respectively. 
DC analysis is also via the LU factorization. 
For large cases, we can also adopt 
other techniques \cite{Xiong12}\cite{Yang12}\cite{Yu12} 
to improve the performance of DC analysis for both methods. 
``Spdp1'' shows the speedup of R-MATEX over fixed time step TR ($h=10ps$). 
``Spdp2'' shows the speedup of R-MATEX over TR (Adaptive). 
``Spdp3'' shows the speedup of R-MATEX over I-MATEX. 

\begin{table*}[htp]
    \centering
    \caption{Simulation runtime of PDN designs}
    \begin{tabular}{|c||r|| r|r|| r|| r| r || r|r|r| r| r|}
    \hline
	\multirow{2}{*}{Design} & \multirow{2}{*}{DC(s)} 
	&\multicolumn{2}{c||}{TR ($h=10ps$)} 
	&\multicolumn{1}{c||}{TR (Adaptive)} 
	& \multicolumn{2}{c||}{I-MATEX }  
	& \multicolumn{5}{c|}{S-MATEX ($\gamma=10^{-10}$) }  
	\\ 
	\cline{3-12} 
				 &	  &LU(s)   &Total   
				 & \multicolumn{1}{c||}{Total}	
				 &LU(s)	 &Total		  
				 &LU(s)	 &Total		& Spdp1 
				 & Spdp2
				 & Spdp3
				 \\ \hline
        D1			& 0.11	  & 0.12   & 392.46s	
				& 52.44s %44.80s         % TR A
				& 0.13    & 33.67s    % I-MATEX 
				& 0.13    & 23.76s	
				& 16.5X 
				& 2.2X 
				& 1.4X 
				\\ \hline
        D2 			& 2.72 
				& 3.41   & 2.80h	
				& 0.27h        
				& 3.78   & 0.21h   
				& 3.98	 & 0.19h
				& 14.7X
				& 1.4X 
				& 1.1X \\ \hline
        D3 			& 17.86   
				& 23.22 &  12.59h	
				& 1.42h %0.26h        
				& 24.88 & 1.06h   
				& 23.80	 &  0.68h	
				& 18.5X 
				& 2.1X
				& 1.5X 
				\\ \hline
        D4 			& 62.11 
				& 76.07  & 37.24h 
				& 4.27h 
				& 88.82  & 3.26h 
				& 77.96	 & 2.05h 
				& 18.2X
				& 2.1X 
				& 1.5X \\ 
    \hline
    \end{tabular}
    \label{tab:results_pdn_cases}
\end{table*}
\begin{comment}
\begin{table}[htp]
    \centering
    \caption{Simulation runtime of PDN designs}
    \begin{tabular}{|c||r|r|r||r|r|r|}
    \hline
	\multirow{2}{*}{Design} & \multirow{2}{*}{DC(s)} &\multicolumn{2}{c||}{TR ($h=10ps$)} & \multicolumn{3}{c|}{MATEX ($\gamma=10^{-10}$) }  \\ 
	\cline{3-7} 
				 &	  &LU(s)   &Total	&LU(s)	 &Total		& Spdp  \\ \hline
        D1			 &0.71	  &0.67	   &44.85m	&0.68	 &2.86m		& 15.73 \\ \hline
        D2 			 &12.21	  &15.60   &15.43h	&15.48	 &54.57m	& 16.96 \\ \hline
        D3 			 &69.59   &91.60   &76.92h	&93.28	 &4.30h		& 17.91 \\ \hline
        D4 			 &218.89  &293.81  &203.64h	&298.83	 &11.26h	& 18.08	\\ 
    \hline
    \end{tabular}
    \label{tab:results_pdn_cases}
\end{table}
\end{comment}

Overall, R-MATEX has impressive speedup over other methods.
R-MATEX can exploit much large step size to simulate the design whereas fixed step size TR can 
only step in $10ps$ for whole $1\mu s$ time span. The average speedup is 17X.  
Adaptive TR cannot jump too large time steps due to instrinsic LTE problem.
However, MATEX can jump large without losing accuracy, due to its property of solving system analytically.
The error is 
larger than I-MATEX, R-MATEX. Trying to reduce such error, will restrict the step size and slow down the
simulation.
%But in these PDNs simulation, the extemley stiffness even singular, 
%the I-MATEX take large dimensions of Krylov subspace basis, that degrades the overal performance.
%R-MATEX can easily handle this issue because the shift-and-invert making the spectrum of systems still
%reside in a unit circle region.
Figure~\ref{fig:result_pdn_case1} shows the 
I-MATEX can achieve 
simulation result of design D1 at a node on M1. 
%As we can see, the result by MATEX and TR are very close to the result of 
%HSPICE, which is as our reference result here. 
%The differences of R-MATEX and TR to HSPICE are $7.33\times10^{-4}$ and $7.47\times10^{-4}$.  
The large size of TR cannot capture the high-frequency behavior, meanwhile, MATEX can enjoy extremely large time step,
to provide enough resolution of waveform, we require MATEX is $1ns$. It is noted even the step size larger than $1ns$,
MATEX still obtain the solutions in these cases.
%This figure also demonstrates that a PDN design has low-, mid- and high-frequncy response so that long simulation time span is necessary. 

\begin{figure}[ht]
    \centering
    \includegraphics[width=3.0in]{./figs/result_pdn_case1.eps}
    \caption{Result of D1}
    \label{fig:result_pdn_case1}
\end{figure}



%\subsection{IBM Power Grid Suite}
\subsection{Scalable MATEX using Input Sources Grouping and Distributed Computing}

We compare MATEX and TR using the IBM power grid suite~\cite{Nassif08_Power}. 
These cases have very large input sources, that limit the step-size of MATEX, however, the circuit
systems are linear.

The simulation time is $10ns$, and TR uses fixed step size in $10ps$. 
Table~\ref{tab:spec_ibmpg} shows the details of each benchmark circuit of which size ranges from $54$K up to $3$M.
The experiment is carried on the workstations, and each node has Intel Core i7-4770 and 32G memory.

\begin{table}[h]
    \centering
    \caption{Specifications of IBM power grid suite}
    \begin{tabular}{|c|r|r|r|r|r|r|r|} 
    \hline
        Design    & \#R     & \#C      & \#L  & \#I    & \#V  & \#Nodes  \\ \hline
	ibmpg1t   & 40801   & 10774    & 277  & 10774  &14308  &54265   \\ \hline
	ibmpg2t   & 245163  & 36838    & 330  & 36838  &330    &164897  \\  \hline
	ibmpg3t   & 1602626 & 201054   & 955  & 201054 &955    &1043444 \\ \hline
	ibmpg4t   & 1826589 & 265944   & 962  & 265944 &962    &1214288 \\ \hline
	ibmpg5t   & 1550048 & 473200   & 277  & 473200 &539087 &2092148 \\ \hline
	ibmpg6t   & 2410486 & 761484   & 381  & 761484 &836249 &3203802 \\ \hline
    \end{tabular}
    \label{tab:spec_ibmpg}
\end{table}

\subsubsection{Single-Node Computing}

\begin{table*}[htp]
%\scriptsize
    \centering
    \caption{Performance comparison TR, single-node(sn)/multi-node(mn) S-MATEX and R-MATEX ($\gamma=10^{-10}$)}
    \begin{tabular}{|c|r|r|r||r|r || r| r|| r| r||  r|r|r| }
    \hline
    \multirow{2}{*}{Design} & 
    \multirow{2}{*}{DC(s)} &
    \multicolumn{2}{c||}{TR ($h=10ps$)} & 
    \multicolumn{2}{c||}{I-MATEX(sn)} & 
    \multicolumn{2}{c||}{I-MATEX(mn)} & 
    \multicolumn{2}{c||}{R-MATEX(sn) } & 
    \multicolumn{3}{c|}{R-MATEX(mn)} 
    \\ 
    \cline{3-13} 
			     &		&LU(s)	&Total(s)	
			     &LU(s)	&Total(s) % s I-M 
			     &LU(s)	&Total(s) % m I-M	
			     &LU(s)	&Total(s) % s R-M	
			     &LU(s)	&Total(s) % m R-M 
			     & Spdp     \\ \hline  
	ibmpg1t		     & 0.13     &0.13   &  6.20 	
			     & 0.12  & 40.16
			     & 0.12  & 6.40
			     & 0.13 & 4.93	  
			     & 0.13 & 1.10
			     &     \\ \hline 
    	ibmpg2t 	     & 0.80  & 0.83   & 28.61	
			   & 0.76   &  177.75
			   & 0.76  & 26.92
			   & 0.85 & 25.90  
			   & 0.85 & 5.56
			    &      \\ \hline 
    	ibmpg3t 	     & 13.83   & 12.72  & 272.47
			   & 12.87 & 1988.98
			   & 12.58 & 280.66 
			   & 12.73 & 244.56  
			   & 12.81 & 63.78 
			   &      \\ \hline
    	ibmpg4t 	    & 16.69    & 22.50   &	368.55
			    & 21.09 & 625.12
			    & 20.99 & 231.06 
			    & 22.09  & 140.42    
			    & 22.02  & 76.55  
			    &      \\ \hline
    	ibmpg5t 	    & 8.16    & 10.50  & 350.33  	
			    & 9.92 & 2590.23
			    & 10.03  & 413.77
			    & 10.77 &  337.74 
			    & 10.51  &  78.99 
			    &     
			    \\ \hline 
    	ibmpg6t 	     & 11.17    &14.17  & 567.38
			    & 13.19 & 4059.30
			    & 13.55 & 856.09
			    & 14.18 & 482.42  
			    & 14.15 & 108.92 
			    &     \\ 
    \hline
    \end{tabular}
    \label{tab:perf_mexp}
\end{table*}

\begin{figure}[ht]
    \centering
    \includegraphics[width=3.0in]{./figs/result_ibmpg6t.eps}
    \caption{Result of ibmpg6t}
    \label{fig:result_ibmpg6t}
\end{figure}


Table~\ref{tab:perf_mexp} presents the performance gains from MATEX compared to TR. 
Single Node MATEX shows a little speedup over TR that is 
not significant as that of the industrial PDN designs. 
The average of the speedup is $1.42$ times. 
The reason behind the little speedup 
in IBM benchmark suite is the fact that hundreds 
of thousands of input sources limits the maximum allowed step size. 
The simulation results 
of ibmpg6t via MATEX and TR are shown 
in Figure~\ref{fig:result_ibmpg6t} where MATEX has many small step sizes 
so that the benefit of large 
step size does not improve the performance drastically. 
As we mentioned in Section~\ref{sec:adaptive_step_control}, 
the maximum allowed 
step size is actually determined by the slope of input sources 
over a time interval. Figure~\ref{fig:align} illustrates the concept 
where $I_1$ and $I_2$ are input sources and ``max. step'' shows the maximum allowed step size 
during the simulation. As we can see, 
ill alignment causes tiny step size because MATEX 
has to guarantee constant slopes within a step size so that Eqn.~(\ref{eqn:pwl_exact_sol}) 
can be held. 
The ibmpg4t has better alignment than the other benchmark circuits, 
and thus, MATEX achieves $2.95$ speedup in ibmpg4t over TR. 

\begin{figure}[ht]
    \centering
    \includegraphics[width=3.5in]{figs/alignment.eps} 
    \caption{Input sources alignment} 
    \label{fig:align}
\end{figure}

\subsubsection{Multi-Node Computing}

Our MATEX is a highly scalable method.
%We can avoid the ill alignment issue by simply grouping ``similiar'' 
%input sources and then simulate them in separately. 
Due to the linearity of the power grid, 
the final result is just the superposition of the simulation result with each group of inputs. 
By doing so, MATEX can simulate in much larger step size in each group, e.g. rising/falling slew 
and pulse width of $I_1$ in Figure~\ref{fig:align}, 
than the step size originally in ill aligned input sources. 
MATEX with grouping is parallelizable by simulating each group in 
multicore or cluster system.  

%In order to demonstrate the idea, we simply device a naive grouping scheme, which will take identical input sources together as a group. 
We assign each group to one computing nodes. 
In the experiment, we notice the message passing between 
our workstations are extreme small.
Time anchors are generated as a wall-lock, that visible to each node, so there are not other
communication overhead.
For example, for the message receiving only takes 0.0007 seconds, which is negligible. 
Table~\ref{tab:perf_mexp_group} shows the performance of MATEX with grouping. 
In this table, ``Groups'' is the number of groups for each 
designs, ``Min. Total`` and ``Max. Total'' is the maximum runtime among different nodes, 
%and ``Ideal Spdp'' records the ideal speedup with parallelization. 
Design ibmpg4t has only 5 groups because the alignment is better. 
The performance of S-MATEX has a significant improvement after grouping. 
The average ideal speedup over TR is 6 times. 
MATEX shows another parallelism in the power grid simulation from the perspective of 
input sources. 


\begin{table}[h]
    \centering
    \caption{Performance of S-MATEX w/ Grouping}
    \begin{tabular}{|c||r |r|r|r|r|}
    \hline
    \multirow{2}{*}{Design} & \multirow{2}{*}{DC(s)} & \multicolumn{4}{c|} {MATEX w/ grouping ($\gamma=10^{-10}$)} \\ \cline{3-6} 
			    &			     & Groups	  &LU(s)  & Max. Total (s)	& Min. Total (s)   \\ 
    \hline ibmpg1t 	    & 0.28		     & 25	  &0.22   & 1.63		& 	    \\
    \hline ibmpg2t 	    & 1.12                   & 25	  &1.32   & 7.93		& 	    \\
    \hline ibmpg3t 	    & 17.72                  & 25	  &18.75  & 86.24		& 	    \\
    \hline ibmpg4t 	    & 22.04                  & 5	  &31.55  & 124.16		& 	    \\
    \hline ibmpg5t 	    & 12.40                  & 25	  &16.35  & 111.97		& 	    \\
    \hline ibmpg6t 	    & 17.66                  & 25	  &29.85  & 166.34		& 	    \\
    \hline
    \end{tabular}
    \label{tab:perf_mexp_group}
\end{table}

\begin{comment}
\subsection{Complexity}

The performance of MATEX and TR are dominated by the number of backward/forward substitutions. This is because the time span 
is relatively long in a power grid, and therefore, the expensive LU fatorization is amortized during the simulation. In MATEX, 
the number of backward/forward substitutions at each time step is actually $m$, which is the number of vectors forming rational 
Krylov subspace. Since $m$ is small, e.g., $5\sim 6$ in IBM benchmark suite, and MATEX uses large step size than TR, MATEX has 
less numbers of substitution operations in general. Table~\ref{tab:subs} presents number of backward/forward substitions for 
each method. ``Sub.'' is the total number of substituion operations along the simulation. MATEX has less operations but close to
TR because the ill alignment of input sources leads to many tiny step sizes whereas MATEX with grouping has much less operations 
due to well aligned inputs. These results also validate Tables~\ref{tab:perf_mexp} and \ref{tab:perf_mexp_group} where MATEX would 
has less speedup due to ill alignment issue, and the grouping scheme could improve the performance. 

\begin{table}[h]
\centering
    \caption{Number of backward/forward substitutions}
    \begin{tabular} {|c|c|c|c|}
    \hline
    \multirow{2}{*}{Design} &TR	 &MATEX		  &MATEX w/ grouping \\ \cline{2-4} 
			    & \# Sub.	 & \# Sub.        &  \# Max Sub.   \\ \hline
    ibmpg1t   		    & 1000	 &  830		  &  120	    \\ \hline 
    ibmpg2t   		    & 1000  	 &  830   	  &  120 	    \\ \hline
    ibmpg3t   		    & 1000  	 &  874   	  &  120 	    \\ \hline 
    ibmpg4t   		    & 1000  	 &  349   	  &  143 	    \\ \hline  
    ibmpg5t   		    & 1000  	 &  982   	  &  139 	    \\ \hline
    ibmpg6t   		    & 1000  	 &  932   	  &  134 	    \\ 
    \hline 
    \end{tabular}
    \label{tab:subs}
\end{table}
\end{comment}

\begin{comment}

\subsection{Scalable IBM Power Grid Suite with Input Grouping}

Following the previous subsection, we not the input is the limitation for 
adaptive steping in our MATEX framework. 
We utlize input grouping~\ref{sec:group}.
Ideal one input sources per group.

\subsubsection{2 groups}

\subsubsection{4 groups}

\subsubsection{8 groups}

\subsubsection{16 groups}

\subsubsection{32 groups}

\subsubsection{64 groups}




Secondly, we consider a single input to run ibmpg1t-ibmpg6t 
to further illustrate our method. We see there are huge speedups than using trapezoidal method.
\end{comment}
%\subsubsection{Full Solver}
%This is the ideal speedups when computing resources are available.

%\subsubsection{Model Order Reduction Preprocessing}
%In this part, we compare the MOR method and put them into trapezoidal method
%and our MATEX framework, in order to compare our method accurate.





==> sub-exp_results_v3.tex <==

In this section, %we conduct the experiments to test our methods.
first, we compare standard Krylov-Based MATEX(S-MATEX)~\cite{Weng12_TCAD}, 
our inverted Krylov-Based MATEX(I-MATEX) and rational Krylov-Based MEXP (R-MATEX) and show
I-MATEX and R-MATEX are good at dealing with pratical circuit simulations, especially with stiff systems.
Secondly, we compare performance of 
%the power grid simulation by 
I-MATEX, R-MATEX and the trapezoidal method (TR) for linear circuit simulation,
we also use power distributions networks (PDNs) 
and IBM power grid benchmark~\cite{Nassif08_Power} 
to validate the efficiency
of our methods for power grid application by taking advantages of 
the property of analytical solutions and its scalablity.
%MATEX with adaptive step size control follows Algorithm~\ref{algo:adaptive_step}. 
%We set $\gamma$ as $10^{-10}$ .
%(similar as the strategy in \cite{Van06}).
%and restrict the maximum allowed step size within $1ns$ to have enough time instants to plot the figure.
%It is possible to have more fine-grain time instants, e.g., $10ps$, with only negligible cost by adjusting 
%$\alpha$ in Eqn. (\ref{eq:scale}). TR is in fixed step size in order to minimize the cost 
%of LU factorization. Both methods only perform factorization once, and rest of operations is mainly backward/forward 
%substitution. 
We implement methods in MATLAB and use UMFPACK package for LU factorization. 
For scalable experiment and simulations, we utilize the equivalent idea 
of MATLABMPI implementations \cite{matlabmpi}.
%combined with shared files and network file systems.
All the experiment is carried on Linux workstations with 
Intel Core\texttrademark~i7-4770 3.40GHz processor and 32GB memory each.
%Note that even though previous works\cite{Chen01_Efficient}\cite{Su03} show that using iterative approach in TR 
%could also achieve adaptive step control, long simulation time span in power grid designs make direct 
%method with fixed step size more desirable\cite{Xiong12}\cite{Yang12}\cite{Zhao02}. 
%Our benchmark includes different industrial power distribution networks (PDNs), which contain the model of 
%board and package, and also includes IBM power grid suite~\cite{Nassif08_Power}. 
%The details and simulation results of 
%both industrial designs and IBM power grid suite are presented in the following subsections. 

\subsection{Efficiency Comparisions on S-MATEX, I-MATEX and R-MATEX of Different Stiff Systems}

In this sub-sections, we show the influence of different stiffness of circuit systems 
to S-/I-/R-/MATEX. 
We construct RC mesh cases that contains 2500 nodes with different stiffness 
by changing the entries of matrix $\mbf C$. 
%the stiffness of $-\mbf C^{-1}\mbf G$ is changed. 
The stiffness is defined as 
$ \frac{Re(\lambda_{min})}{Re(\lambda_{max})}$, where $\lambda_{min}$ and $\lambda_{max}$ are
the minimum and maximum eigenvalues of $-\mbf C^{-1} \mbf G$.
We run the transient simulations $[0,0.3ns]$ with fixed time step $5ps$.
\begin{comment}
\subsubsection{$ \frac{Re(\lambda_{min})}{Re(\lambda_{max})}= 2.12 \times 10^{3}$}
The extreme values of the circuit system are shown in Table.~\ref{tab:extreme_values}
The corresponding maximum eigenvalue of $-\mbf C^{-1}\mbf G$ is $-1.88 \times 10^{9}$
and minimum eigenvalue is $-3.98 \times 10^{17}$. 
\begin{table}[htp]
  \caption{Exteme Values in $\mbf C$ and $\mbf G$}
  \centering
  \begin{tabular}{cccc}%cccc}
%    \multicolumn{2}{c}{$\mbf C$} &\multicolumn{2}{c}{$\mbf G$}\\ % &\multicolumn{2}{c}{M6} &\multicolumn{2}{c}{RDL}\\
    \hline $\mbf C_{min}$ & $\mbf C_{max}$  & $\mbf G_{min}$ & $\mbf G_{max}$ \\ % &pitch &width  &pitch &width \\
    \hline $5.04 \times 10^{-19}$   & $1.00 \times 10^{-15}$  & $1.09 \times 10^{-2}$ &$1.00 \times 10^2$ \\% &30 &4 &400 &30\\
    \hline 
  \end{tabular}
  \label{tab:extreme_values}
\end{table}
\end{comment}
Table~\ref{tab:rc_cases} shows the average dimensions $m_{a}$ 
and the peak dimension $m_{p}$
used in the matrix exponential approximations during the transient simulations 
by different strategies of Krylov subspace basis. 
We also compare the total simulation time and speedups (Spdp) to S-MATEXs. %and speedup of RC case.
The Err (\%) is the relative error opposed to 
backward Euler method with fixed step size $0.05ps$.
\begin{table}[h]
    \caption{Comparisions among S-/I-/R-MATEX with RC cases}
    \centering
    \begin{tabular}{|c||c|c|c|c|c|c|}
    \hline
	Method  & $m_{a}$ &   $m_{p} $  & Err(\%)  &  Time(s)  & Spdp 
	& {Stiffness}  \\ 
	\hline
	S-MATEX	&  211.4   	&   229  	&  0.510  &  601.87  & -- &
	\multirow{3}{*}{$2.1 \times 10^{16}$ } 
	\\
	\cline{1-6}
	I-MATEX	& 5.7 	&14       &  0.004		& 0.23    & 2616X   &   \\
	\cline{1-6}
	R-MATEX	& 6.9   & 12   &  0.004  & 0.22   &  2735X   & \\ 
	\hline
	\hline
	S-MATEX	&  154.2   	&   224  	&  0.004  &      134.32 & --  
	& 	    \multirow{3}{*}{$2.1 \times 10^{12}$ } 
	\\
	\cline{1-6}
	I-MATEX	&  5.7 	& 14       &0.004   &   0.23  &  583X  &   \\
	\cline{1-6}
	R-MATEX	& 6.9  & 12   &  0.004  & 0.20 	   &  611X  & \\ 
	\hline
	\hline
	S-MATEX	&  148.6   	&   223  & 0.004  & 52.87  &  -- & 	    \multirow{3}{*}{$2.1 \times 10^{8}$ } 
	\\
	\cline{1-6}
	I-MATEX	& 5.7  	& 14      & 0.004   &  0.23   & 229X  &   \\
	\cline{1-6}
	R-MATEX	& 6.9  & 12   &  0.004  & 	0.21   &  252X  & \\ 
	%\cline{1-6}
	\hline
    \end{tabular}
    \label{tab:rc_cases}
\end{table}
S-MATEX is good to handle mild stiff circuits \cite{Weng12_TCAD}.
However, these cases show that the S-MATEX are senstive to the stiffness, especially 
it becomes large.
It is not efficient on highly stiff circuits, since the $m_a$ and $m_p$ of S-MATEX are
extremely large and consume computational resources (time and memomry), which degrades 
the overall runtime performance.

%However, in this small but stiff cases,
Meanwhile, I-MATEX and R-MATEX achieve significant speedups over S-MATEX 
by the lower demands of
Krylov subspace basis dimension. 
The average dimension $m_a$ of R-MATEX is higher than I-MATEX, 
but the peak $m_p$ are smaller.
Besides, the dimensions of R-MATEX used in each time step spread more evenly than I-MATEX,
These result to the similar runtime performance bewteen these two methods in these three cases.
% R-MATEX as I-MATEX.
%However, the high stiffness are very common in VLSI designs,

As we known, in large scale of linear circuit system and pratical VLSI designs, 
the stiffness may be even bigger and complicated than our toy cases here.
Compared to S-MATEX,  
proposed I-MATEX and R-MATEX are good candidates to deal with these scenarios.
It is because the smaller dimension of basis required to form Krylov subsapce 
of matrix exponential approximations. 
%in S-MATEX. 
Therefore, in the following sub-sections, 
we only apply our I-MATEX and R-MATEX to futher cases and make comparisions 
with other methods.
%There are not so much different from I-MATEX and R-MATEX in this case.
%\subsubsection{Eigenvalues distribution}
%In this subsection, it is comparison among different krylov subspace basis, to
%fetch the $\mbf A$'s eigenvanlue.

\begin{comment}
\subsection{Handling Post-Layout-like Matrix $\mbf C$}

In this subsection, we increase the complexity of capactiance matrix $\mbf C$
by incremental adding coupling capacitance 
\cite{Zhuang2012}~\cite{Yu2013}~\cite{Moselhy2010}.  
We know the capacitances in chip have ``geometrically'' longer 
relationship than resistor.
They are formed by the different distances from the 
corresponding master conductor
~\cite{Zhuang2012}~\cite{Yu2013}~\cite{Moselhy2010}. 
On the notion of random walk for capacitance, the coupling capacitance 
propogate in a certain distance, and result different range 
of parameters, which is not good for 
limitation of standard Krylov subspace by stiffness.
When the number of coupling capacitances is large, the nonzero entries weakens the sparsity 
of matrix $\mbf C$.
Inverted Krylov subspace is good for this scenario, 

We constructed dense capacitance matrix, and test the fluctuation of $m$ order.

It is observed that 

So it bares more possibility for coupling issues, and result in
more dense capacitance matrix than conduction matrix. 

In the following part, we shows the inverted version of Krylov subspace can handle
very dense matrix, while trapezoidal, backeuler, MATEX(std) and MATEX(rational) all
failed because out of memory.
\end{comment}

%\subsection{Industrial PDN Designs}
\subsection{Adaptive Time-Steping Examples}

We utilize industrial power distribution network cases to show MATEX's adaptivity.
The rationale is that designers rely on the simulation result of impulse response of the 
PDN design in order to characterize the design. 
Many previous works \cite{Du10}\cite{Tian96}\cite{Hu12_TVLSI}
have proposed different PDN analysis based on the impulse 
response. 
The nature of impulse response of the PDN design, 
which contains low-, mid- and high-frequency components, 
can significantly enjoy the adaptive step size in MATEX.  
We would also like to mention that the impulse response 
based analysis is not only for the PDN design, 
but also for worst-case eye opening analysis in the high speed interconnect
\cite{Analui05}\cite{Shi08}. 

The industrial PDN design are given, including
on-chip power grid, package and board. 
The power grid consists of four metal 
layers: M1, M3, M6 and Redistribution Layer (RDL). 
The physical parameters of each metal layer 
is listed in Table~\ref{tab:spec_metal_layers}. 
The package is modeled as an RL series at each C4 bump, 
and the board is modeled as a lumped RLC network. The
specification of each PDN design is listed in Table~\ref{tab:spec_pdn_designs} 
where the size of each design 
ranges from $45.7$K to $7.40$M. 
\begin{table}[htp]
  \caption{Widths and pitches of metal layers in the PDN design($\mu m$).}
  \centering
  \begin{tabular}{cccccccc}
    \multicolumn{2}{c}{M1} &\multicolumn{2}{c}{M3} 
    &\multicolumn{2}{c}{M6} &\multicolumn{2}{c}{RDL}\\
    \hline pitch &width  &pitch &width  &pitch &width  &pitch &width \\
    \hline 2.5   &0.2  &8.5  &0.25  &30 &4 &400 &30\\
    \hline 
  \end{tabular}
  \label{tab:spec_metal_layers}
\end{table}

\begin{table}[htp]
    \caption{Specifications of PDN Designs}
    \centering
    \begin{tabular}{|c||r|r|r|r|r|}
    \hline
	Design  & Area ($mm^2$)	& \# R	    & \# C	& \# L	    & \# Nodes  \\ \hline
	D1	& $0.35^2$	& 23221	    & 15193	& 15193	    & 45.7K	\\ \hline
	D2	& $1.40^2$  	& 348582    & 228952	& 228952    & 688K	\\ \hline
	D3	& $2.80^2$  	& 1468863   & 965540	& 965540    & 2.90M	\\ \hline
	D4	& $5.00^2$  	& 3748974   & 2467400	& 2464819   & 7.40M	\\ 
    \hline
    \end{tabular}
    \label{tab:spec_pdn_designs}
\end{table}
The impulse response can be derived from the simulation result 
of a step input from $0$V to $1$V with a small transition time. 
Hence, we inject a step input to each PDN design and 
compare the performance of adaptive time-stepping 
MATEXs (I-MATEX, S-MATEX), and TR (fixed time step $h=10ps$), adaptive time-steping TR. 
The transition time of 
the step input and the simulation time span is $10ps$ and $1\mu s$ 
for observing both high- and low-frequency behavior. 
For such large size application, in the respective of memory counsumption, 
we limit the Krylov subspace order $m$ within $[6,~30]$. During the simulation. 
We find such region can provide enough accuracy for matrix exponential approximation by I-MATEX and S-MATEX.
Table~\ref{tab:results_pdn_cases} shows the simulation runtime of MATEXs and TRs 
%where the fixed step size is set as $10ps$ 
to comply with the transition time. 
In the table, ``DC'', ``LU'' and ``Total'' 
indicate the runtime for DC analysis, LU 
factorization and the overall simulation, respectively. 
DC analysis is also via the LU factorization. 
For large cases, we can also adopt 
other techniques \cite{Xiong12}\cite{Yang12}\cite{Yu12} 
to improve the performance of DC analysis for both methods. 
``Spdp1'' shows the speedup of R-MATEX over fixed time step TR ($h=10ps$). 
``Spdp2'' shows the speedup of R-MATEX over TR (Adaptive). 
``Spdp3'' shows the speedup of R-MATEX over I-MATEX. 

\begin{table*}[htp]
    \centering
    \caption{Simulation runtime of PDN designs}
    \begin{tabular}{|c||r|| r|r|| r|| r| r || r|r|r| r| r|}
    \hline
	\multirow{2}{*}{Design} & \multirow{2}{*}{DC(s)} 
	&\multicolumn{2}{c||}{TR ($h=10ps$)} 
	&\multicolumn{1}{c||}{TR (Adaptive)} 
	& \multicolumn{2}{c||}{I-MATEX }  
	& \multicolumn{5}{c|}{S-MATEX ($\gamma=10^{-10}$) }  
	\\ 
	\cline{3-12} 
				 &	  &LU(s)   &Total   
				 & \multicolumn{1}{c||}{Total}	
				 &LU(s)	 &Total		  
				 &LU(s)	 &Total		& Spdp1 
				 & Spdp2
				 & Spdp3
				 \\ \hline
        D1			& 0.11	  & 0.12   & 392.46s	
				& 52.44s %44.80s         % TR A
				& 0.13    & 33.67s    % I-MATEX 
				& 0.13    & 23.76s	
				& 16.5X 
				& 2.2X 
				& 1.4X 
				\\ \hline
        D2 			& 2.72 
				& 3.41   & 2.80h	
				& 0.27h        
				& 3.78   & 0.21h   
				& 3.98	 & 0.19h
				& 14.7X
				& 1.4X 
				& 1.1X \\ \hline
        D3 			& 17.86   
				& 23.22 &  12.59h	
				& 1.42h %0.26h        
				& 24.88 & 1.06h   
				& 23.80	 &  0.68h	
				& 18.5X 
				& 2.1X
				& 1.5X 
				\\ \hline
        D4 			& 62.11 
				& 76.07  & 37.24h 
				& 4.27h 
				& 88.82  & 3.26h 
				& 77.96	 & 2.05h 
				& 18.2X
				& 2.1X 
				& 1.5X \\ 
    \hline
    \end{tabular}
    \label{tab:results_pdn_cases}
\end{table*}
\begin{comment}
\begin{table}[htp]
    \centering
    \caption{Simulation runtime of PDN designs}
    \begin{tabular}{|c||r|r|r||r|r|r|}
    \hline
	\multirow{2}{*}{Design} & \multirow{2}{*}{DC(s)} &\multicolumn{2}{c||}{TR ($h=10ps$)} & \multicolumn{3}{c|}{MATEX ($\gamma=10^{-10}$) }  \\ 
	\cline{3-7} 
				 &	  &LU(s)   &Total	&LU(s)	 &Total		& Spdp  \\ \hline
        D1			 &0.71	  &0.67	   &44.85m	&0.68	 &2.86m		& 15.73 \\ \hline
        D2 			 &12.21	  &15.60   &15.43h	&15.48	 &54.57m	& 16.96 \\ \hline
        D3 			 &69.59   &91.60   &76.92h	&93.28	 &4.30h		& 17.91 \\ \hline
        D4 			 &218.89  &293.81  &203.64h	&298.83	 &11.26h	& 18.08	\\ 
    \hline
    \end{tabular}
    \label{tab:results_pdn_cases}
\end{table}
\end{comment}

Overall, R-MATEX has impressive speedup over other methods.
R-MATEX can exploit much large step size to simulate the design whereas fixed step size TR can 
only step in $10ps$ for whole $1\mu s$ time span. The average speedup is 17X.  
Adaptive TR cannot jump too large time steps due to instrinsic LTE problem.
However, MATEX can jump large without losing accuracy, due to its property of solving system analytically.
The error is 
larger than I-MATEX, R-MATEX. Trying to reduce such error, will restrict the step size and slow down the
simulation.
%But in these PDNs simulation, the extemley stiffness even singular, 
%the I-MATEX take large dimensions of Krylov subspace basis, that degrades the overal performance.
%R-MATEX can easily handle this issue because the shift-and-invert making the spectrum of systems still
%reside in a unit circle region.
Figure~\ref{fig:result_pdn_case1} shows the 
I-MATEX can achieve 
simulation result of design D1 at a node on M1. 
%As we can see, the result by MATEX and TR are very close to the result of 
%HSPICE, which is as our reference result here. 
%The differences of R-MATEX and TR to HSPICE are $7.33\times10^{-4}$ and $7.47\times10^{-4}$.  
The large size of TR cannot capture the high-frequency behavior, meanwhile, MATEX can enjoy extremely large time step,
to provide enough resolution of waveform, we require MATEX is $1ns$. It is noted even the step size larger than $1ns$,
MATEX still obtain the solutions in these cases.
%This figure also demonstrates that a PDN design has low-, mid- and high-frequncy response so that long simulation time span is necessary. 

\begin{figure}[ht]
    \centering
    \includegraphics[width=3.0in]{./figs/result_pdn_case1.eps}
    \caption{Result of D1}
    \label{fig:result_pdn_case1}
\end{figure}



%\subsection{IBM Power Grid Suite}
\subsection{Scalable MATEX using Input Sources Grouping and Distributed Computing}

We compare MATEX and TR using the IBM power grid suite~\cite{Nassif08_Power}. 
These cases have very large input sources, that limit the step-size of MATEX, however, the circuit
systems are linear.

The simulation time is $10ns$, and TR uses fixed step size in $10ps$. 
Table~\ref{tab:spec_ibmpg} shows the details of each benchmark circuit of which size ranges from $54$K up to $3$M.
The experiment is carried on the workstations, and each node has Intel Core i7-4770 and 32G memory.

\begin{table}[h]
    \centering
    \caption{Specifications of IBM power grid suite}
    \begin{tabular}{|c|r|r|r|r|r|r|r|} 
    \hline
        Design    & \#R     & \#C      & \#L  & \#I    & \#V  & \#Nodes  \\ \hline
	ibmpg1t   & 40801   & 10774    & 277  & 10774  &14308  &54265   \\ \hline
	ibmpg2t   & 245163  & 36838    & 330  & 36838  &330    &164897  \\  \hline
	ibmpg3t   & 1602626 & 201054   & 955  & 201054 &955    &1043444 \\ \hline
	ibmpg4t   & 1826589 & 265944   & 962  & 265944 &962    &1214288 \\ \hline
	ibmpg5t   & 1550048 & 473200   & 277  & 473200 &539087 &2092148 \\ \hline
	ibmpg6t   & 2410486 & 761484   & 381  & 761484 &836249 &3203802 \\ \hline
    \end{tabular}
    \label{tab:spec_ibmpg}
\end{table}

\subsubsection{Single-Node Computing}

\begin{table*}[htp]
%\scriptsize
    \centering
    \caption{Performance comparison TR, single-node(sn)/multi-node(mn) S-MATEX and R-MATEX ($\gamma=10^{-10}$)}
    \begin{tabular}{|c|r|r|r||r|r || r| r|| r| r||  r|r|r| }
    \hline
    \multirow{2}{*}{Design} & 
    \multirow{2}{*}{DC(s)} &
    \multicolumn{2}{c||}{TR ($h=10ps$)} & 
    \multicolumn{2}{c||}{I-MATEX(sn)} & 
    \multicolumn{2}{c||}{I-MATEX(mn)} & 
    \multicolumn{2}{c||}{R-MATEX(sn) } & 
    \multicolumn{3}{c|}{R-MATEX(mn)} 
    \\ 
    \cline{3-13} 
			     &		&LU(s)	&Total(s)	
			     &LU(s)	&Total(s) % s I-M 
			     &LU(s)	&Total(s) % m I-M	
			     &LU(s)	&Total(s) % s R-M	
			     &LU(s)	&Total(s) % m R-M 
			     & Spdp1     
			     \\ \hline  
	ibmpg1t		     & 0.13     &0.13   &  6.20 	
			     & 0.12  & 27.23
			     & 0.12  & 4.68 
			     & 0.13 & 4.93	  
			     & 0.13 & 1.10
			     &     \\ \hline 
    	ibmpg2t 	     & 0.80  & 0.83   & 28.61	
			   & 0.76   &  124.44
			   & 0.76  & 20.19 
			   & 0.85 & 25.90  
			   & 0.85 & 5.56
			    &      \\ \hline 
    	ibmpg3t 	     & 13.83   & 12.72  & 272.47
			   & 12.87 & 1246.69  %1988.98
			   & 12.58 & 213.33 %280.66 
			   & 12.73 & 244.56  
			   & 12.81 & 63.78 
			   &      \\ \hline
    	ibmpg4t 	    & 16.69    & 22.50   &	368.55
			    & 21.09 & 484.83 %625.12
			    & 20.99 & 148.45 %231.06 
			    & 22.09  & 140.42    
			    & 22.02  & 76.55  
			    &      \\ \hline
    	ibmpg5t 	    & 8.16    & 10.50  & 350.33  	
			    & 9.92 & 1821.60 
			    & 10.03  & 304.72 %413.77
			    & 10.77 &  337.74 
			    & 10.51  &  78.99 
			    &     
			    \\ \hline 
    	ibmpg6t 	     & 11.17    &14.17  & 567.38
			    & 13.19 & 2784.46 %4059.30
			    & 13.55 & 479.79 ? %856.09
			    & 14.18 & 482.42  
			    & 14.15 & 108.92 
			    &     \\ 
    \hline
    \end{tabular}
    \label{tab:perf_mexp}
\end{table*}

\begin{figure}[ht]
    \centering
    \includegraphics[width=3.0in]{./figs/result_ibmpg6t.eps}
    \caption{Result of ibmpg6t}
    \label{fig:result_ibmpg6t}
\end{figure}


Table~\ref{tab:perf_mexp} presents the performance gains from MATEX compared to TR. 
Single Node MATEX shows a little speedup over TR that is 
not significant as that of the industrial PDN designs. 
The average of the speedup is $1.42$ times. 
The reason behind the little speedup 
in IBM benchmark suite is the fact that hundreds 
of thousands of input sources limits the maximum allowed step size. 
The simulation results 
of ibmpg6t via MATEX and TR are shown 
in Figure~\ref{fig:result_ibmpg6t} where MATEX has many small step sizes 
so that the benefit of large 
step size does not improve the performance drastically. 
As we mentioned in Section~\ref{sec:adaptive_step_control}, 
the maximum allowed 
step size is actually determined by the slope of input sources 
over a time interval. Figure~\ref{fig:align} illustrates the concept 
where $I_1$ and $I_2$ are input sources and ``max. step'' shows the maximum allowed step size 
during the simulation. As we can see, 
ill alignment causes tiny step size because MATEX 
has to guarantee constant slopes within a step size so that Eqn.~(\ref{eqn:pwl_exact_sol}) 
can be held. 
The ibmpg4t has better alignment than the other benchmark circuits, 
and thus, MATEX achieves $2.95$ speedup in ibmpg4t over TR. 

\begin{figure}[ht]
    \centering
    \includegraphics[width=3.5in]{figs/alignment.eps} 
    \caption{Input sources alignment} 
    \label{fig:align}
\end{figure}

\subsubsection{Multi-Node Computing}

Our MATEX is a highly scalable method.
%We can avoid the ill alignment issue by simply grouping ``similiar'' 
%input sources and then simulate them in separately. 
Due to the linearity of the power grid, 
the final result is just the superposition of the simulation result with each group of inputs. 
By doing so, MATEX can simulate in much larger step size in each group, e.g. rising/falling slew 
and pulse width of $I_1$ in Figure~\ref{fig:align}, 
than the step size originally in ill aligned input sources. 
MATEX with grouping is parallelizable by simulating each group in 
multicore or cluster system.  

%In order to demonstrate the idea, we simply device a naive grouping scheme, which will take identical input sources together as a group. 
We assign each group to one computing nodes. 
In the experiment, we notice the message passing between 
our workstations are extreme small.
Time anchors are generated as a wall-lock, that visible to each node, so there are not other
communication overhead.
For example, for the message receiving only takes 0.0007 seconds, which is negligible. 
Table~\ref{tab:perf_mexp_group} shows the performance of MATEX with grouping. 
In this table, ``Groups'' is the number of groups for each 
designs, ``Min. Total`` and ``Max. Total'' is the maximum runtime among different nodes, 
%and ``Ideal Spdp'' records the ideal speedup with parallelization. 
Design ibmpg4t has only 5 groups because the alignment is better. 
The performance of S-MATEX has a significant improvement after grouping. 
The average ideal speedup over TR is 6 times. 
MATEX shows another parallelism in the power grid simulation from the perspective of 
input sources. 


\begin{table*}[ht]
    \centering
    \caption{Performance of R-MATEX w/ Grouping}
    \begin{tabular}{|c||r |r|r|r|r|r|}
    \hline
    \multirow{2}{*}{Design} & \multirow{2}{*}{TR Trans(s)} & \multicolumn{5}{c|} {R-MATEX w/ grouping}		      \\ \cline{3-7} 
			    &			     & Groups	    & Max. Trans (s)	& Min. Trans (s)  &Spdp1  &Spdp2\\ 
    \hline ibmpg1t 	    & 5.94		     & 25	   & 0.84		& 0.48		  & 7.1X  & 12.4X \\
    \hline ibmpg2t 	    & 26.98                   & 25	   & 3.93		& 2.38		  & 6.7X  & 11.3X \\
    \hline ibmpg3t 	    & 245.92                  & 25	   & 38.09     	&21.96		  & 6.5X & 11.2X \\
    \hline ibmpg4t 	    & 329.36                  & 5	   & 33.55		&30.12		  & 9.8X  & 10.9X \\
    \hline ibmpg5t 	    & 331.67                  & 25	   & 58.54 		& 33.59		  & 5.7X & 9.9X \\
    \hline ibmpg6t 	    & 542.04                  & 25	   & 81.40 		&51.68		  & 6.7X & 28.0X \\
    \hline
    \end{tabular}
    \label{tab:perf_mexp_group}
\end{table*}

\begin{comment}
\subsection{Complexity}

The performance of MATEX and TR are dominated by the number of backward/forward substitutions. This is because the time span 
is relatively long in a power grid, and therefore, the expensive LU fatorization is amortized during the simulation. In MATEX, 
the number of backward/forward substitutions at each time step is actually $m$, which is the number of vectors forming rational 
Krylov subspace. Since $m$ is small, e.g., $5\sim 6$ in IBM benchmark suite, and MATEX uses large step size than TR, MATEX has 
less numbers of substitution operations in general. Table~\ref{tab:subs} presents number of backward/forward substitions for 
each method. ``Sub.'' is the total number of substituion operations along the simulation. MATEX has less operations but close to
TR because the ill alignment of input sources leads to many tiny step sizes whereas MATEX with grouping has much less operations 
due to well aligned inputs. These results also validate Tables~\ref{tab:perf_mexp} and \ref{tab:perf_mexp_group} where MATEX would 
has less speedup due to ill alignment issue, and the grouping scheme could improve the performance. 

\begin{table}[h]
\centering
    \caption{Number of backward/forward substitutions}
    \begin{tabular} {|c|c|c|c|}
    \hline
    \multirow{2}{*}{Design} &TR	 &MATEX		  &MATEX w/ grouping \\ \cline{2-4} 
			    & \# Sub.	 & \# Sub.        &  \# Max Sub.   \\ \hline
    ibmpg1t   		    & 1000	 &  830		  &  120	    \\ \hline 
    ibmpg2t   		    & 1000  	 &  830   	  &  120 	    \\ \hline
    ibmpg3t   		    & 1000  	 &  874   	  &  120 	    \\ \hline 
    ibmpg4t   		    & 1000  	 &  349   	  &  143 	    \\ \hline  
    ibmpg5t   		    & 1000  	 &  982   	  &  139 	    \\ \hline
    ibmpg6t   		    & 1000  	 &  932   	  &  134 	    \\ 
    \hline 
    \end{tabular}
    \label{tab:subs}
\end{table}
\end{comment}

\begin{comment}

\subsection{Scalable IBM Power Grid Suite with Input Grouping}

Following the previous subsection, we not the input is the limitation for 
adaptive steping in our MATEX framework. 
We utlize input grouping~\ref{sec:group}.
Ideal one input sources per group.

\subsubsection{2 groups}

\subsubsection{4 groups}

\subsubsection{8 groups}

\subsubsection{16 groups}

\subsubsection{32 groups}

\subsubsection{64 groups}




Secondly, we consider a single input to run ibmpg1t-ibmpg6t 
to further illustrate our method. We see there are huge speedups than using trapezoidal method.
\end{comment}
%\subsubsection{Full Solver}
%This is the ideal speedups when computing resources are available.

%\subsubsection{Model Order Reduction Preprocessing}
%In this part, we compare the MOR method and put them into trapezoidal method
%and our MATEX framework, in order to compare our method accurate.





==> sub-exp_results_v4.tex <==

We implement our MATEX in MATLAB and use UMFPACK package for LU factorization. 
All the experiment is carried on Linux workstations with 
Intel Core\texttrademark~i7-4770 3.40GHz processor and 32GB memory each.

\subsection{MATEX's Circuit Solver Performance using Different Krylov Subspace Basis} 
\begin{table}[hp]
\footnotesize
    \caption{Comparisions among MEXP, I-MATEX and R-MATEX with RC cases}
    \centering
    \begin{tabular}{|c||c|c|c|c|c|c|}
    \hline
	Method  & $m_{a}$ &   $m_{p} $  & Err(\%)    & Spdp 
	& {Stiffness}  \\ 
	\hline
	MEXP	&  211.4   	&   229  	&  0.510   & -- &
	\multirow{3}{*}{$2.1 \times 10^{16}$ } 
	\\
	\cline{1-5}
	I-MATEX	& 5.7 	&14       &  0.004	   & 2616X   &   \\
	\cline{1-5}
	R-MATEX	& 6.9   & 12   &  0.004   &  2735X   & \\ 
	\hline
	\hline
	MEXP	&  154.2   	&   224  	&  0.004 & --  
	& 	    \multirow{3}{*}{$2.1 \times 10^{12}$ } 
	\\
	\cline{1-5}
	I-MATEX	&  5.7 	& 14       &0.004   &  583X  &   \\
	\cline{1-5}
	R-MATEX	& 6.9  & 12   &  0.004 	   &  611X  & \\ 
	\hline
	\hline
	MEXP &  148.6   	&   223  & 0.004  &  -- & 	    \multirow{3}{*}{$2.1 \times 10^{8}$ } 
	\\
	\cline{1-5}
	I-MATEX	& 5.7  	& 14      & 0.004     & 229X  &   \\
	\cline{1-5}
	R-MATEX	& 6.9  & 12   &  0.004  &  252X  & \\ 
	%\cline{1-6}
	\hline
    \end{tabular}
    \label{tab:rc_cases}
\end{table}
We test the part of circuit solver within MATEX 
using MEXP~\cite{Weng12_TCAD}, as well as our proposed I-MATEX and R-MATEX.
We create RC mesh cases %that contains 2500 nodes
with different stiffness 
by changing the entries of matrix $\mbf C,~ \mbf G$. 
%the stiffness of $-\mbf C^{-1}\mbf G$ is changed. 
Here, the stiffness is defined as 
$ \frac{Re(\lambda_{min})}{Re(\lambda_{max})}$,
where $\lambda_{min}$ and $\lambda_{max}$ 
are the minimum and maximum eigenvalues of $-\mbf C^{-1} \mbf G$.
We run the transient simulations $[0,0.3ns]$ with fixed time step $5ps$.
Table~\ref{tab:rc_cases} shows 
the average Krylov subspace basis dimension $m_{a}$ and the peak dimension $m_{p}$
used to compute matrix exponential during the transient simulations. 
We also compare the runtime speedups (Spdp) over MEXP. %and speedup of RC case.
The Err (\%) is the relative error opposed to 
backward Euler method with tiny fixed step size $0.05ps$.
%However, in this small but stiff cases,
%There are not so much different from I-MATEX and R-MATEX in this case.
%\subsubsection{Eigenvalues distribution}
%In this subsection, it is comparison among different krylov subspace basis, to
%fetch the $\mbf A$'s eigenvanlue.
\begin{table*}[t]
%\scriptsize
\footnotesize
%\footfontesize
    \centering
    \caption{Performance comparison TR, I-MATEX and R-MATEX
    Spdp$^1$: Speedup of I-MATEX over TR ($h=10ps$); 
    Spdp$^2$: Speedup of R-MATEX over Adaptive TR .  
    Spdp$^3$: Speedup of R-MATEX over I-MATEX.  
   }
    \begin{threeparttable}[b]
    \begin{tabular}{|c|r|r||r|r|| r| r|  r| }
    \hline
    \multirow{2}{*}{Design} & 
    \multirow{2}{*}{DC(s)} &
    \multicolumn{1}{c||}{Adaptive TR} & 
    \multicolumn{2}{c||}{I-MATEX} & 
    \multicolumn{3}{c|}{R-MATEX } 
    \\ 
    \cline{3-8} 
    &
			     &Total(s) % s I-M 
			     &Total(s) 
			     &SPDP1
			     &Total(s) 
			     &SPDP2
			     &SPDP3
			     \\ \hline  
	ibmpg1t		     & 0.13     
			      & 29.48
			      & 27.23
			     & 1.3X
			     & 4.93	  
			     & 6.0X 
			     & 5.5X
			     \\ \hline 
    	ibmpg2t 	     & 0.80  
			    & 179.74 
			   &  124.44
			   & 1.4X 
			   & 25.90  
			   & 6.9X 
			   & 4.8X
			    \\ \hline 
    	ibmpg3t 	     & 13.83 
			    & 2792.96 
			   & 1246.69  %1988.98
			   & 2.2X
			   & 244.56  
			   & 11.4X
			   & 5.1X
			   \\ \hline
    	ibmpg4t 	    & 16.69
			    & 1773.14 
			    & 484.83 %625.12
			   & 3.7X 
			    & 140.42 %231.06 
			    & 12.6X
			    & 3.5X
			    \\ \hline
    	ibmpg5t 	    & 8.16 
			   & 2359.11
			    & 1821.60 
			    & 1.3X 
			    & 337.74 
			    & 7.0X
			    & 5.4X 
			    \\ \hline 
    	ibmpg6t 	     & 11.17
		    	& 3184.59
			    & 2784.46 %4059.30
			   & 1.1X
			    & 482.42  
			    &   6.6X 
			   &5.8X 
			    \\ 
    \hline
    \end{tabular}
   % \begin{tablenotes}\scriptsize
%	\item [1] Speedup of I-MATEX (mn) over TR ($h=10ps$) 
%	\item [2] Speedup of R-MATEX (mn)over I-MATEX (mn) 
%	\item [3] Speedup of R-MATEX (mn) over TR ($h=10ps$)
%	\item [4] Speedup of R-MATEX (mn) over TR (adpt)      
%	\vspace{-0.5in}
%    \end{tablenotes}
    \end{threeparttable}
    \label{tab:perf_mexp}
\end{table*}
\begin{table*}[tp]
%\scriptsize
\footnotesize
\centering
\caption{Speed-ups of R-MATEX over TR with fixed
time step $h=10ps$; 
Max. and Avg. Err.: compared to all output nodes' solutions provided by IBM Power Grid Benchmarks;
Spdp4:$ {t_{1000}/t_{adpt}}$;
Spdp5: total runtime speedups of R-MATEX over TR 
}
\begin{tabular}{|c||r|r||r|r| r| r|r|r|r|}
\hline
\multirow{2}{*}{Design}&
\multicolumn{2}{c||}{TR}&
\multicolumn{7}{c|}{R-MATEX}
\\
\cline{2-10}
& $t_{1000}(s)$
& $t_{total}(s)$
& Group
& $t_{adpt}(s)$ 
& $t_{total}(s)$
& Max. Err
& Avg. Err
& Spdp4
& Spdp5
\\
\hline
 ibmpg1t & 5.94   &   6.20  &  {\color{red} 100}  &  0.50  &  0.85  &  1.4E-4 & 2.5E-5 & 11.9X  & 7.3X  
\\
\hline
 ibmpg2t & 26.98  &   28.61  &  100  &  2.02  &  3.72  &  1.9E-4 &  4.3E-5 & 13.4X  & 7.7X  
\\
\hline
 ibmpg3t & 245.92  & 272.47  &  100  &  20.15  &  45.77 &  2.0E-4 &  3.7E-5 & 12.2X  & 6.0X  
\\
\hline
 ibmpg4t & 329.36  & 368.55  &  {\color{red}25} & 22.35 &  65.66 &  1.1E-4 &  3.9E-5 & 14.7X  & 5.6X  
\\
\hline
 ibmpg5t & 331.67  & 350.33  &  100 & 35.67 & 54.21 &  0.7E-4 &  1.1E-5 &  9.3X  & 6.5X  
\\
\hline
 ibmpg6t & 542.04  & 567.38  &  100 & 47.27 & 74.94 &  1.0E-4 &  3.4E-5 &  11.5X  & 7.6X  
\\
\hline
\end{tabular}
\label{tab:pg_rmatex}
\end{table*}


The huge speedups by I-MATEX and R-MATEX 
are due to large reductions of Krylov subspace basis $m_a$ and $m_p$. 
%and also save the memory conusmptions.
As we known, MEXP is good at handling mild stiff circuits \cite{Weng12_TCAD}, 
but not efficient on highly stiff circuits. 
Besides,
we also observe even the basis number is large, 
there is still possiblility with relative larger error
compared to I-MATEX and R-MATEX. 
The average dimension $m_a$ of R-MATEX is a little bit higher than I-MATEX. 
However, the dimensions of R-MATEX used along time points spread more evenly than I-MATEX.
In such small dimension Krylov subspace computation, the total simulation runtime tends to be 
influenced by matrix exponential evaluations on the time points with peak basis dimension($m_p$),
which I-MATEX has more than R-MATEX.
These result to a slightly better runtime performance of R-MATEX over I-MATEX.
% bewteen these two methods in these three cases.
%since the $m_a$ and $m_p$ of MEXP are
%extremely large and consume computational resources (time and memomry), which degrades 
%the overall runtime performance.
%I-MATEX and R-MATEX achieve significant speedups over MEXP 
%with lower demands of Krylov subspace basis dimension. 
%Besides, 

As we known, in large scale of linear circuit system and pratical VLSI designs, 
the stiffness may be even bigger and complicated. %than our toy cases here. 
Many of them may also have large singular $\mbf C$ 
and MEXP cannot handle without regularization process.
These make  I-MATEX and R-MATEX are good candidates to deal with these scenarios.
In the following parts, we apply our I-MATEX and R-MATEX to futher cases and make comparisions 
with other methods.

%but it spread  more stable along the total simulation in R-MATEX and $m_p$ is smaller.


\subsection{Adaptive Time Stepping}

IBM power grid benchmarks~\cite{Nassif08_Power} are used here to
investigate the performance of SPICE-like adaptive time stepping TR based on LTE controling 
\cite{Weng12_TCAD, Najm10_book} as well as
our proposed I-MATEX, and R-MATEX. All are running on single computing node.
The speedups of I-MATEX is not as large as R-MATEX due to
the large Krylov subspace dimesnsion in these benchmarks.
In \emph{ibmpg4t} case, the I-MATEX gains its largest speedups, due to
the input sources make transition relative less, and it can enjoy
more adaptive stepping.
The same is to R-MATEX in this case.
%the power grid simulation by 

\subsection{Distributed Computing Performance }
Since R-MATEX is the most efficient circuit solver in our MATEX
framework. We use it on IBM power grid benchmarks. 
These cases have many input transistion that limit the step-size of MATEX.
Combined with distributed computing,
we can easily decompose the inputs based on ``bumps'' 
to minimize LTS for one computing nodes.
In IBM power grid benchmarks, we can obtain reasonable number
of group to on identical ``bumps'' shapes  
(the required computing node number is shown 
in \emph{Group} in Table. \ref{tab:pg_rmatex}).
It is used to compete fixed time step $h=10ps$ TR method,
which requires 1000 time steps 
for the transient simulation.
%For scalable experiment and simulations, we utilize the equivalent idea 
%of MATLABMPI implementations \cite{matlabmpi}. 
Since there is not  communications during the transient simulation among
each node, for distributed computing, we utilize our workstations to 
emulate the multiple-node environment, 
and then select the maximum runtime among all the task as the total runtime.
We also record the computing time for the transient part without LU. 
For R-MATEX
we use the maximum values among this 
to define the $t_{adpt}$ in Table. \ref{tab:pg_rmatex}.
%MATEX with grouping is parallelizable by simulating each group in 
%multicore or cluster system.  

Our R-MATEX framework is able to achieve 12X on average
withe respect to pure transient computing  as
well as 7X on the total wall-clock time.
It is because we extract the 
With the huge reduction of time on part, the serial LU and DC parts
in our MATEX
take larger  portion. 
It can be further improved further using the advance methods~\cite{nicslu},
which is another important study area.
There are other way to decompose the input transitions, we use one simple
strategy based on ``hump'' shapes, and achieve such large speedups.  


%In order to demonstrate the idea, we simply device a naive grouping scheme, which will take identical input sources together as a group. 
\begin{comment}
We assign each group to one computing nodes. 
In the experiment, we notice the message passing between 
our workstations are extreme small.
Time anchors are generated as a wall-lock, 
that visible to each node, so there are not other
communication overhead.
For example, for the message receiving only takes 0.0007 seconds, which is negligible. 
Table~\ref{tab:perf_mexp_group} shows the performance of MATEX with grouping. 
In this table, ``Groups'' is the number of groups for each 
designs, ``Min. Total`` and ``Max. Total'' is the maximum runtime among different nodes, 
%and ``Ideal Spdp'' records the ideal speedup with parallelization. 
Design ibmpg4t has only 5 groups because the alignment is better. 
The performance of MEXP has a significant improvement after grouping. 
The average ideal speedup over TR is 6 times. 
MATEX shows another parallelism in the power grid simulation from the perspective of 
input sources. 
\end{comment}

\begin{comment}
\begin{table*}[ht]
    \centering
    \caption{Performance of R-MATEX w/ Grouping}
    \begin{tabular}{|c||r |r|r|r|r|r|}
    \hline
    \multirow{2}{*}{Design} & \multirow{2}{*}{TR Trans(s)} & \multicolumn{5}{c|} {R-MATEX w/ grouping}		      \\ \cline{3-7} 
			    &			     & Groups	    & Max. Trans (s)	& Min. Trans (s)  &Spdp1  &Spdp2\\ 
    \hline ibmpg1t 	    & 5.94		     & 25	   & 0.84		& 0.48		  & 7.1X  & 12.4X \\
    \hline ibmpg2t 	    & 26.98                   & 25	   & 3.93		& 2.38		  & 6.7X  & 11.3X \\
    \hline ibmpg3t 	    & 245.92                  & 25	   & 38.09     	&21.96		  & 6.5X & 11.2X \\
    \hline ibmpg4t 	    & 329.36                  & 5	   & 33.55		&30.12		  & 9.8X  & 10.9X \\
    \hline ibmpg5t 	    & 331.67                  & 25	   & 58.54 		& 33.59		  & 5.7X & 9.9X \\
    \hline ibmpg6t 	    & 542.04                  & 25	   & 81.40 		&51.68		  & 6.7X & 28.0X \\
    \hline
    \end{tabular}
    \label{tab:perf_mexp_group}
\end{table*}


\subsection{Complexity}

The performance of MATEX and TR are dominated by the number of backward/forward substitutions. This is because the time span 
is relatively long in a power grid, and therefore, the expensive LU fatorization is amortized during the simulation. In MATEX, 
the number of backward/forward substitutions at each time step is actually $m$, which is the number of vectors forming rational 
Krylov subspace. Since $m$ is small, e.g., $5\sim 6$ in IBM benchmark suite, and MATEX uses large step size than TR, MATEX has 
less numbers of substitution operations in general. Table~\ref{tab:subs} presents number of backward/forward substitions for 
each method. ``Sub.'' is the total number of substituion operations along the simulation. MATEX has less operations but close to
TR because the ill alignment of input sources leads to many tiny step sizes whereas MATEX with grouping has much less operations 
due to well aligned inputs. These results also validate Tables~\ref{tab:perf_mexp} and \ref{tab:perf_mexp_group} where MATEX would 
has less speedup due to ill alignment issue, and the grouping scheme could improve the performance. 

\begin{table}[h]
\centering
    \caption{Number of backward/forward substitutions}
    \begin{tabular} {|c|c|c|c|}
    \hline
    \multirow{2}{*}{Design} &TR	 &MATEX		  &MATEX w/ grouping \\ \cline{2-4} 
			    & \# Sub.	 & \# Sub.        &  \# Max Sub.   \\ \hline
    ibmpg1t   		    & 1000	 &  830		  &  120	    \\ \hline 
    ibmpg2t   		    & 1000  	 &  830   	  &  120 	    \\ \hline
    ibmpg3t   		    & 1000  	 &  874   	  &  120 	    \\ \hline 
    ibmpg4t   		    & 1000  	 &  349   	  &  143 	    \\ \hline  
    ibmpg5t   		    & 1000  	 &  982   	  &  139 	    \\ \hline
    ibmpg6t   		    & 1000  	 &  932   	  &  134 	    \\ 
    \hline 
    \end{tabular}
    \label{tab:subs}
\end{table}
\end{comment}

\begin{comment}

\subsection{Scalable IBM Power Grid Suite with Input Grouping}

Following the previous subsection, we not the input is the limitation for 
adaptive steping in our MATEX framework. 
We utlize input grouping~\ref{sec:group}.
Ideal one input sources per group.

\subsubsection{2 groups}

\subsubsection{4 groups}

\subsubsection{8 groups}

\subsubsection{16 groups}

\subsubsection{32 groups}

\subsubsection{64 groups}




Secondly, we consider a single input to run ibmpg1t-ibmpg6t 
to further illustrate our method. We see there are huge speedups than using trapezoidal method.
\end{comment}
%\subsubsection{Full Solver}
%This is the ideal speedups when computing resources are available.

%\subsubsection{Model Order Reduction Preprocessing}
%In this part, we compare the MOR method and put them into trapezoidal method
%and our MATEX framework, in order to compare our method accurate.



\begin{comment}
\begin{table}[h]
    \caption{Comparisions among MEXP, I-MATEX and R-MATEX with RC cases}
    \centering
    \begin{tabular}{|c||c|c|c|c|}
    \hline
	Method  &   $m_{p} $  & Err(\%)
%	&  Time(s)
	& Speedup 
	& Stiffness\\
	%& {$\frac{Re{\lambda_{smallest}(\mbf A)}}{Re({\lambda_{largest}(A)}}$}  \\ 
	\hline
	MEXP	  	&   229  	
	&  0.510
%	&  601.87  
	& -- &
	\multirow{3}{*}{$2.1 \times 10^{16}$ } 
	\\
	\cline{1-4}
	I-MATEX	 	&14       &  0.004
%	& 0.23
	& 2616X   &   \\
	\cline{1-4}
	R-MATEX	   & 12   &  0.004  
%	& 0.22   
	&  2735X   & \\ 
	\hline
	\hline
	MEXP	  	&   224  	&  0.004  
	%&  134.32
	& --  
	& 	    \multirow{3}{*}{$2.1 \times 10^{12}$ } \\
	\cline{1-4}
	I-MATEX		& 14       &0.004   
	%&   0.23
	&  583X  &   \\
	\cline{1-4}
	R-MATEX	&  12   &  0.004  
%	& 0.20 
	&  611X  & \\ 
	\hline
	\hline
	MEXP	   	&   223  & 0.004  
%	& 52.87  
	&  -- & 	    \multirow{3}{*}{$2.1 \times 10^{8}$ } 
	\\
	\cline{1-4}
	I-MATEX  	& 14      & 0.004   
%	&  0.23 
	& 229X  &   \\
	\cline{1-4}
	R-MATEX	  & 12   &  0.004 
%	& 		0.21  
	&  252X  & \\ 
	%\cline{1-6}
	\hline
    \end{tabular}
    \label{tab:rc_cases}
\end{table}
\end{comment}


\begin{comment}
\begin{table*}[htp]
%\scriptsize
    \centering
    \caption{Performance comparison TR, I-MATEX and R-MATEX of single-node computing (sn)/multi-node simulation (mn) versions,
    Spdp$^1$: Speedup of I-MATEX (mn) over TR ($h=10ps$); 
    Spdp$^2$: Speedup of R-MATEX (mn)over I-MATEX (mn); 
    Spdp$^3$: Speedup of R-MATEX (mn) over TR ($h=10ps$);
    Spdp$^4$: Speedup of R-MATEX (mn) over TR (adpt).  
   }
    \begin{threeparttable}[b]
    \begin{tabular}{|c|r|r|r||r||r|r || r| r|| r| r ||  r|r|r|r| }
    \hline
    \multirow{2}{*}{Design} & 
    \multirow{2}{*}{DC(s)} &
    \multicolumn{2}{c||}{TR ($h=10ps$)} & 
    \multicolumn{1}{c||}{TR (adpt)} & 
    \multicolumn{2}{c||}{I-MATEX(sn)} & 
    \multicolumn{2}{c||}{I-MATEX(mn)} & 
    \multicolumn{2}{c||}{R-MATEX(sn) } & 
    \multicolumn{4}{c|}{R-MATEX(mn)} 
    \\ 
    \cline{3-15} 
			     &		&LU(s)	&Total(s)	
			    % &LU(s)	
			     &Total(s) % s I-M 
			     &LU(s)
			     &Total(s) 
			     &Total(s) 
			     &SPDP\footnote{ over TR }% (/TR.)	
			     % m I-M	
			     &LU(s)	&Total(s) % s R-M	
			     %&Spdp2\footnote{ over TR }
			     %	(/TR.)
			     &Total(s) % m R-M 
			     &SPDP\footnote{ over I-MATEX(mn) } %	(/I- (mn))
			     & SPDP\footnote{ over TR }%  (/TR.)   
			     & SPDP\footnote{ over TR (adpt)}%  (/TR.)   
			     \\ \hline  
	ibmpg1t		     & 0.13     
			      &0.13   &  6.20 	
			      & 29.48
			     & 0.12  & 27.23
			    % & 0.12  
			     & 4.68 
			     & 1.3X
			     & 0.13 & 4.93	  
		%	     & 1.3X
			     %& 0.13 
			     & 1.10
			     & 4.5X 
			     & 5.6X
			     & 26.8X
			     \\ \hline 
    	ibmpg2t 	     & 0.80  
			    & 0.83   & 28.61	
			    & 179.74 
			   & 0.76   &  124.44
			  % & 0.76 
			   & 20.19 
			   & 1.4X
			   & 0.85 
			   & 25.90  
		%	   & 1.1X
			   %& 0.85 
			   & 5.56
			    & 3.6X 
			    & 5.1X
			    & 32.3X
			    \\ \hline 
    	ibmpg3t 	     & 13.83   & 12.72  & 272.47
			    & 2792.96 
			   & 12.87 & 1246.69  %1988.98
			  % & 12.58 
			   & 213.33 %280.66 
			   & 1.3X 
			   & 12.73 
			   & 244.56  
			 %  & 1.1X
			  % & 12.81 
			   & 63.78 
			   & 3.3X 
			   & 4.3X 
			   & 43.8X
			   \\ \hline
    	ibmpg4t 	    & 16.69    & 22.50   &	368.55
			    & 1773.14 
			    & 21.09 & 484.83 %625.12
			   % & 20.99 
			    & 148.45 %231.06 
			    & 2.5X
			    & 22.09  & 140.42    
			 %   & 2.6X
			   % & 22.02  
			    & 76.55  
			    & 1.9X  
			    & 4.8X
			    & 23.1X
			    \\ \hline
    	ibmpg5t 	    & 8.16    & 10.50  & 350.33  	
			   & 2359.11
			    & 9.92 & 1821.60 
			   % & 10.03 
			    & 304.72 %413.77
			    & 1.1X
			    & 10.77 &  337.74 
			 %   & 1.0X
			   % & 10.51  
			    &  78.99 
			    &    3.9X 
			    & 4.4X
			    & 29.9X
			    \\ \hline 
    	ibmpg6t 	     & 11.17    &14.17  & 567.38
		    	& 3184.59
			    & 13.19 & 2784.46 %4059.30
			   % & 13.55 
			    & 479.79 %856.09
			   & 1.2X
			    & 14.18 & 482.42  
		%	    & 1.2X
			   % & 14.15 
			    & 108.92 
			   & 4.4X 
			    &   5.2X 
			   & 29.2X 
			    \\ 
    \hline
    \end{tabular}
   % \begin{tablenotes}\scriptsize
%	\item [1] Speedup of I-MATEX (mn) over TR ($h=10ps$) 
%	\item [2] Speedup of R-MATEX (mn)over I-MATEX (mn) 
%	\item [3] Speedup of R-MATEX (mn) over TR ($h=10ps$)
%	\item [4] Speedup of R-MATEX (mn) over TR (adpt)      
%	\vspace{-0.5in}
%    \end{tablenotes}
    \end{threeparttable}
    \label{tab:perf_mexp}
\end{table*}
\end{comment}


%Note that even though previous works\cite{Chen01_Efficient}\cite{Su03} show that using iterative approach in TR 
%could also achieve adaptive step control, long simulation time span in power grid designs make direct 
%method with fixed step size more desirable\cite{Xiong12}\cite{Yang12}\cite{Zhao02}. 
%Our benchmark includes different industrial power distribution networks (PDNs), which contain the model of 
%board and package, and also includes IBM power grid suite~\cite{Nassif08_Power}. 
%The details and simulation results of 
%both industrial designs and IBM power grid suite are presented in the following subsections. 




==> sub-group.tex <==

\subsection{Superposition of Linear Circuit System in MATEX Framework}

In thie linear circuit simulation, the equation, 
\begin{eqnarray} 
    \mbf{x}(t+h) = e^{\mbf{A}h}\mbf{x}(t) + 
    \int^{h}_{0}e^{\mbf{A}(h-\tau)}\mbf{b}(t+\tau)d\tau.
\end{eqnarray}
can be views as the summation of sub-systems,
 
\begin{eqnarray} 
   & \mbf{x}(t+h) &= e^{\mbf{A}h}\mbf{x}(t) + 
    \int^{h}_{0}e^{\mbf{A}(h-\tau)}\sum_i^N \mbf{b_i}(t+\tau)d\tau
    \nonumber
    \\ \nonumber
    &=&  e^{\mbf{A}h}\mbf{x}_1(t) + \int^{h}_{0}e^{\mbf{A}(h-\tau)}\mbf{b_1}(t+\tau)d\tau
    \\ \nonumber
    & &(\text{sub-problem } 1)
    \\ \nonumber
    &+& e^{\mbf{A}h}\mbf{x}_2(t) + \int^{h}_{0}e^{\mbf{A}(h-\tau)}\mbf{b_2}(t+\tau)d\tau
    \\ \nonumber
    & &(\text{sub-problem } 2)
    \\ \nonumber
    &+& \cdots
    \\ \nonumber
    &+& e^{\mbf{A}h}\mbf{x}_N(t) + \int^{h}_{0}e^{\mbf{A}(h-\tau)}\mbf{b_N}(t+\tau)d\tau 
    \\ \nonumber
    & &(\text{sub-problem } N)
\end{eqnarray}
where
 $\mbf x(t) = \sum_i^N \mbf x_i(t)$, $\mbf x_i(t)$ is DC solution for sub problem $i$. 
$\mbf b = \sum_i^N \mbf b_i$, and $N$ is
the number of total inputs, including voltage and current
sources.
The merit of this application of superposition theory within MATEX 
framework is theoritically beautiful for future 
parallel and distributed simulation.

\subsection{Generation of Time Anchors and Grouping of Input Sources}

With the assumption of PWL, the transition of input vectors is another
cause to set the limitation of time step length of MATEX. 
If the input vectors change at different time, it results to small
time step length.
However, with the respect to one input or several inputs with identical
feature, which are with 
similar $t_{delay}$, $t_{rise}$, $t_{flat}$, $t_{fall}$, $t_{period}$), 
the changes 
can behave well.
The communications among precessors are via ``time anchors'', 
which are computed and can be seen as ``globally'' wall clock.

To a specific processor, in term of ``global time anchors'', 
only the ``local time anchors'' limit the step length of time. 
If the number of processors are limited to a number $g$, 
we need to group as identical input as possible 
to avoid the ``local time anchors'' limitation.
The algorithm for such time anchor generation and source grouping is summarized 
in Algorithm~\ref{algo:time_anchor}.
\begin{algorithm} 
    \label{algo:time_anchor}
    \caption{Precomputed Time Anchor and Grouping Input Source}
    \KwIn{Input source $\mbf{b}(=\mbf{Bu})$, with pulse information, 
    including $t_{delay}$, $t_{rise}$, $t_{flat}$, $t_{fall}$, $t_{period}$ }
    \KwOut{$\{t^{anchors}\}$, and $\{\mbf b\}_{i}, i=1,2, \cdots , g $ is the total number of input source grouping}
    {
	//Time Anchors Generation\;
	\For{ $i \in 1,2,..., \beta $}
	{
	    \{$t^{anchors}_{temp}$\} = ComputeTransistionTimePoint($\mbf{u}_i(t)$)\;
	   \{$t^{anchors}$\} = MergeAndSort(\{$t^{anchors}$\},\{$t^{anchors}_{temp}$\})\; 
	   {
	       //Input Grouping\;
	       \If{Grouping is required}
	       {
		   \eIf{ MatchFeature(${\mbf M_{map}}$,~${\mbf b_i}$)== ${\mbf b_j}$ }{
		       $\{\mbf b\}_j$= AddToGroupWith(${\mbf b_i}$); 
		   }
		   {
		       RegisterTheFeatureIntoMap$({\mbf M_{map}}, ~{\mbf b_i}  )$\;
		   }
	       }
	   }
	}
    }
\end{algorithm}
Based on previous modified Krylov subspace method, MATEX can
jump a large time step with the error budget for each time step and the assumption of PWL.
This is called as ``JUMP'' operation (JOpt). 
JOpt may go across several time anchors. 
Then MATEX need to compute those 
inter points of ``time anchors'' by looking the wall clock, from current time point
to the last time point. 
This is called as ``LOOK-BACK'' opearation (LBOpt).
MATEX is based on more analytical solution with 
Krylov scaling invariance with the order $m$ is always small, 
$e^{h\mbf A} \mbf v = \beta \mbf V_m e^{\alpha \mbf H_m}$ can be 
calculate very efficiently for the inner time points. 
On the other hand, the method like FE, BE and TRAP methods cannot have such property.
Firstly, $h$ in these methods fix the time step size, otherwise, it cannot reuse LU matrices or use slow
iterative methods with adaptive controling
(another benefit of Krylov subspace in matrix exponentials has better convergent rate than previous iterative solver~\cite{Hochbruck97}).
Contrary, the $\gamma$ in rational method does not enforce the time step, 
because Krylov subspace is scaling invariant, $h\mbf{\wtd H}$ will help to 
look back during one time step.
Therefore, as long as 
the Krylov basis number $m$ is small, with the scaling invariant
of Krylov subspace method, LBOpt is relatively cheap and also accurate. 
The time points can be pre-computed via the shape from input sourses.
%these ``time anchor'' tell the processors, 
After all, the time cost $T_{total}$ is
\begin{eqnarray}
 T_{total} = T_{map} + T_{slowest\_task} + T_{reduce}
\end{eqnarray}
where $T_{map}$ contains the one LU factorization, and the matrix send to 
different processors; 
the $T_{slowest\_task}$ represents the slowest sub-problems runtime consumptions;
the $T_{reduce}$ contains the time of collect the output
from other processors, and the summation based on the superposition method. 

\subsection{Scalable Framework with Time Anchors}
This whole algorithm is summarized as  
\begin{algorithm} 
    \label{algo:adaptive_step_group}
    \caption{%(Parallel Linear Circuit Simulation)
     S-MATEX with Source Decompositions with Time Anchors}
    \KwIn{$\mbf{C}$, $\mbf{G}$, $\mbf{B}$, $\mbf{u}(t)$, $\tau$, error tolerance $E_{Tol}$ and simulation time $T$}
    \KwOut{$\mbf{x}(t)$}
    {
        $t = 0$, $\mbf{x}(0)$ = DC\_analysis\;
        %Choose $\tau$ for rational Krylov subspace method\;
        %LU($\mbf{C}, \mbf{G}$)\;
        LU($\mbf{C} + \gamma \mbf{G}$)\;
	// Divide task into sub-tasks and \\
	// mapping them to processes\;
	Proc. \#0 sends matrices, input vector, and time anchors ($\mbf{L}_{sub}$ ,$\mbf{U}_{sub}$, 
	$\mbf b_i, \{ t^{anchors}\}$) to Procs. \#1, \#2, $\dots$, \#N\;
	// Computing sub-task at Proc. \#k\;
        \While{$t \leq T$}
        {	
	    %Update $v_{k+1}$ with $\mbf{L}, \mbf{U}, \mbf{W}$ by (\ref{eq:blu_f})\;
	    %and update $\mathbf{L},\mathbf{U}$ by (\ref{eq:blu})\;
	    // JOpt to jump as far as possible \;
	    Compute maximum allowed step size $h$ from $\mbf{u}_k(t)$\;
	    Construct $\mbf{H_m}$, $\mbf{V_m}$ by Arnoldi process until $err_k \le \frac{E_{Tol}}{T}h$\;
	    $\alpha = \frac{h}{\gamma}$ \;
	    Compute $\mbf{x}(t+h)$\; 
	    % by Eqn. (\ref{eq:scale})\;
	    \For{$t_i^{anchors} \in (t,t+h)$}
	    {
		$h_i = t_i^{anchors}-t$\;
		$\alpha_i = \frac{h_i}{\gamma}$\; 
		Compute $\mbf{x}(t+h_i)$ by Eqn. (\ref{eq:scale})\;
	    }
	    $t = t+h$; 
	}
	// Reduce sub-tasks into the whole problems\;
	Proc. \#0 collects $\{x\}_i$ series from Proc. \#i. 
	After receiving all $\{x\}_1$, $\{x\}_2$, $\cdots$, $\{x\}_N$, add up with  
	$\{x\} = \sum_{i=1}^{N}{\{x\}_i} $	
	by time anchors\;
    }
\end{algorithm}


For limited computing resource,
we can avoid the ill alignment issue as much as possible by 
simply grouping ``similiar'' input sources 
and then simulate them in separately. Due to the 
linearity of the power grid, the final result is just 
the superposition of the simulation result with each group of inputs. By doing
so, MATEX can simulate in much larger step size in each group, 
e.g. rising/falling slew and pulse width of $I_1$ in Figure~\ref{fig:align}, 
than the step size originally in ill aligned input sources. 
Moreover, MATEX with grouping is parallelizable by simulating each group in 
multicore or cluster system.  

In order to demonstrate the idea, we simply device a naive grouping scheme, 
which will take identical input sources together as a group. 
Table~\ref{tab:perf_mexp_group} shows the performance of 
MATEX with grouping. In this table, ``Groups'' is the number of groups for each 
designs, ``Max. Total'' is the maximum runtime among the groups, and ``Ideal Spdp'' records the ideal speedup with parallelization. 
Design ibmpg4t has only 4 groups because the alignment is better. The performance of MATEX has a significant improvement after grouping. 
The average ideal speedup over TRAP is 6 times. MATEX shows another parallelism in the power grid simulation from the perspective of 
input sources. 




==> sub-inverted_krylov.tex <==


\begin{eqnarray} 
\label{eqn:pwl2}
    \mbf{x}(t+h)&=& e^{\mbf{-C^{-1}G}h}\mbf{x}(t) \nonumber \\
		&+& (e^{\mbf{-C^{-1}G}h} - \mbf{I})(\mbf{-G}^{-1}\mbf{C})
		\mbf{C^{-1}B}u(t) \nonumber \\
	        &+& (e^{\mbf{-C^{-1}G}h}-(\mbf{-C^{-1}G}h+\mbf{I}))
		(-\mbf{G^{-1}C})(-\mbf{G^{-1}C})\frac{\mbf{C^{-1}B}u(t+h)-
		\mbf{C^{-1}B}(t)}{h}.
\end{eqnarray}

\begin{comment}
\begin{eqnarray} 
\label{eqn:pwl3}
    \mbf{x}(t+h)&=& e^{\mbf{-C^{-1}G}h}\mbf{x}(t) \nonumber \\
		&-& (e^{\mbf{-C^{-1}G}h} - \mbf{I})\mbf{G}^{-1}\mbf{B}u(t)
		\nonumber \\
	        &+& (e^{\mbf{-C^{-1}G}h}+\mbf{C^{-1}G}h-\mbf{I})
		\mbf{G^{-1}C}\mbf{G^{-1}}\frac{\mbf{B}u(t+h)-
		\mbf{B}(t)}{h}.
\end{eqnarray}

\begin{eqnarray} 
\label{eqn:pwl3}
    \mbf{x}(t+h)&=& e^{\mbf{-C^{-1}G}h}
		    (\mbf{x}(t) - \mbf{G}^{-1}\mbf{B}u(t) +
		    \mbf{G^{-1}C}\mbf{G^{-1}}\frac{\mbf{B}u(t+h)-
					\mbf{B}u(t)}{h}
				       ) \nonumber \\
		&+&  \mbf{G}^{-1}\mbf{B}u(t) \nonumber \\
	        &+& (\mbf{C^{-1}G}h+\mbf{I})
		\mbf{G^{-1}C}\mbf{G^{-1}}\frac{\mbf{B}u(t+h)-
		\mbf{B}u(t)}{h}.
\end{eqnarray}
% will be used for  ${\wtd A}$ of~(\ref{eq:one_exp})  
\end{comment}


\begin{eqnarray} 
\label{eqn:pwl5}
    \mbf{x}(t+h)&=& e^{\mbf{-C^{-1}G}h}
		    (\mbf{x}(t) - \mbf{G}^{-1}\mbf{B}u(t) +
		    \mbf{G^{-1}C}\mbf{G^{-1}}\frac{\mbf{B}u(t+h)-
					\mbf{B}u(t)}{h}
				       ) \nonumber \\
	        &-&  \mbf{G^{-1}C}\mbf{G^{-1}}\frac{\mbf{B}u(t+h)-
		\mbf{B}u(t)}{h}
		+
		\mbf{G^{-1}}({\mbf{B}u(t+h)})
\end{eqnarray}

%

\begin{eqnarray} 
\label{eqn:pwl6}
    \mbf{x}(t+h)&=& e^{\mbf{-C^{-1}G}h}
		    (\mbf{x}(t) - \mbf T_t  +
		    \frac{1}{h}
		    \mbf{G^{-1}C} (\mbf T_{t+h} - \mbf T_{t})) \nonumber \\
	        &-&  \frac{1}{h} \mbf{G^{-1}C} (\mbf T_{t+h} - \mbf T_{t})
		+ \mbf T_{t+h}
\end{eqnarray}

where
$\mbf T_t = \mbf{G}^{-1}\mbf{B}\mbf u(t) $,
this reuses the 
$\mbf T_{t+h}$ at last time step. 

So 
during the current solve $\mbf T_{t+h}$ by 
$\mbf G \mbf T_{t+h} = \mbf B \mbf u(t+h)$
once,
and 

$h \mbf G \mbf v = \mbf C(\mbf T_{t+h}-\mbf T_t) $.
$h \mbf L \mbf U \mbf v = \mbf C(\mbf T_{t+h}-\mbf T_t) $.
reused the DC. 

Complexity for this multiplication operations: 

$O((nnz(L)+nnz(U))\times 2+ nnz(B) + nnz(C) ) $

The expm complexity due to the convergence property of $\mbf G^{-1}$
say $m$ is the order of krylov subspace, the complexity is

$O((nnz(L)+nnz(U))*m )$


This method overcome the inhibitive of inverse of $\mbf{C} $.
The convergence for the 





==> sub-mor.tex <==

MEXP and Krylov-Subspace can be consider as a special case of model order
reduction.

There are PRIMA and SPRIM. 

\subsection{PRIMA v.s. I-MEXP}

\subsection{SPRIM v.s. R-MEXP}


\begin{comment}
In the last decades, in order to accelertion of circuit simulation, 
   there are enormous research carried on macromodelling and 
   model order reduction (MOR).

   PRIMA~\cite{PRIMA98}, SPRIM~\cite{SPRIM04}
   are the classic works in this area. 

   It is noted that, the basic matrix from PRIMA~\cite{PRIMA98}, it uses 
   $\mbf A_{p} = -\mbf G^{-1} \mbf C$
   and
   $\mbf R_{p} = \mbf G^{-1} \mbf B$.
   It is quite the same with MEXP's inverted-Krylov subspace in~\ref{ssec:inverted-krylov} 


   Meanwhile the work in SPRIM~\cite{SPRIM04}, 
   the $\mbf A_s = -(\mbf G + s_0 \mbf C)^{-1} \mbf C$
   and
   $\mbf R_s = (\mbf G+s_0 \mbf C)^{-1}\mbf B $.
   It is quite the same with MEXP's rational-Krylov subspace in~\ref{ssec:inverted-krylov} 


   if $p_{m-1}(\mbf A)$ is a polynomials to approximate $e^{\mbf A}v$

   Then Eqn.~\ref{eqn:kernel} can be expressed as

   \begin{eqnarray}
\mbf{x}(t+h) - \mbf{G}^{-1}\mbf{B}\mbf{u}(t+h) 
    - (\mbf{-G}^{-1}\mbf{C}) \mbf{G}^{-1}\mbf{B}\mbf{u}'(t+h)
    %mbf+ (\mbf{-G}^{-1}\mbf{C})^2 \mbf{G}^{-1}\mbf{B}\mbf{u}''(t+h)
%%mbf+ (\mbf{-G}^{-1}\mbf{C})^3 \mbf{G}^{-1}\mbf{B}\mbf{u}^{(3)}(t+h)
    %%mbf+ \dots 
    %dots- \sum_{k=2}^n (\mbf{-G}^{-1}\mbf{C})^k \mbf{G}^{-1}\mbf{B}\mbf{u}^{(k)}(t+h) & 
    %mbf\\ \nonumber
%nonumber     \mbf{x}(t)
%mbf   -  \mbf{G}^{-1}\mbf{B}\mbf{u}(t) 
    %mbf- (\mbf{-G}^{-1}\mbf{C}) \mbf{G}^{-1}\mbf{B}\mbf{u}'(t)
    %%mbf+ (\mbf{-G}^{-1}\mbf{C})^2 \mbf{G}^{-1}\mbf{B}\mbf{u}''(t+h)
    %%mbf\\ \nonumber
%%nonumber+ (\mbf{-G}^{-1}\mbf{C})^3 \mbf{G}^{-1}\mbf{B}\mbf{u}^{(3)}(t+h)
    %%mbf+ \dots 
%dots- \sum_{k=2}^n(\mbf{-G}^{-1}\mbf{C})^k \mbf{G}^{-1}\mbf{B}\mbf{u}^{(k)}(t)
    %mbf\}
    %\end{eqnarray}
    %
    %where $\mbf A$ can be 
    %$-\mbf C^{-1}\mbf G$ when $\mbf C$ is non-singular, or 
    %$-\mbf G^{-1}\mbf C$ when $\mbf G$ is non-singular.
    %
    %In addition $-(\mbf G+ \gamma \mbf C)^{-1} \mbf C$ when $(\mbf G+ \gamma \mbf C)$ is regular.
    %\subsection{Weakness of PRIMA and SPRIM}
    %As we know the Krylov subspace is relate to the $\mbf x(t)$
    %, when this drives the subspace away from the 
    %$span(\mbf A, \mbf A \mbf R, \mbf A^2 \mbf R, \cdots \mbf A^{m-1} \mbf R)$. 
    %The reduced model cannot be used in time domain simulation.
    %Dectect the PRIMA's error and recalculate Krylov
    %
    \end{comment}
    %
    %





==> sub-nume_results.tex <==



==> sub-pwr_grid_formulation.tex <==
%DO WE NEED A POWER GRID FIGURE TO SHOW MORE DETAILS ABOUT THE FORMULATION?

A power grid can be formulated as a system of 
Differential Algebraic Equations (DAEs)
% Ordinary Differential Equations(ODEs) 
via Modified Nodal Analysis (MNA) as below:
\begin{eqnarray}
    \label{eqn:ode}
    \mbf{C}\dot{\mbf{x}}(t) = - \mbf{G}\mbf{x}(t) + \mbf{B}\mbf{u}(t),
\end{eqnarray}
where matrix $\mbf{C}$ describes the capacitance and inductance, matrix 
$\mbf{G}$ represents the resistance and the incidence between voltages 
and currents, and matrix $\mbf{B}$ indicates locations of the independent 
sources. Vector $\mbf{x}(t)$ describes the nodal voltages and branch currents 
at time $t$, and vector $\mbf{u}(t)$ represents the corresponding supply voltage 
and current sources associated to different blocks. 

In order to stimulate the worst-case voltage noise, those current sources, which 
represent the behavior of underlying blocks of a power grid, are often pre-characterized
with pre-designed vectors. Many previous works\cite{Bodapati02}\cite{Du10}\cite{Ferzli10} 
have developed different methodologies to generate worst-case stimulus currents.  
In this work, we assume those input sources are given and in the format of \emph{piece-wise linear}. 


==> sub-rational_krylov.tex <==
% \subsubsection{Rational Krylov Subspace Method }
%\subsection{Krylov Subspace}


In~\cite{Weng12_TCAD}\cite{Weng12_ICCAD}, the Eqn.~(\ref{eq:one_exp})
is calculated via Krylov Subspace algorithm, using Arnoldi method, 
\begin{eqnarray}
\label{eq:kry_A}
  \mbf {K_m}(\mbf{ \widetilde A, v}) = 
     span\{\mbf v, \mbf { \wtd Av}, \cdots, \mbf {\wtd A}^{m-1} \mbf v \}
\end{eqnarray}
where $\mbf v$ is an initial vector.
The Arnoldi method is good at finding approximations
to the eigenvalues which are nicely separated from the other eigenvalues
in the spectrum.
But when dealing with the stiff circuit system, 
$\mbf {\wtd A}$ is a large ill-conditioned matrix. 
Besides, the exponential function $e^{\mbf {\wtd A} h}$ is 
a quickly decaying function when $\mbf {\wtd A} $'s eigenvalues are 
all non-positive, which is the case in 
power grid circuit simulation based on Eqn. (\ref{eqn:ode}).
It is known that $e^{\mbf{\wtd A}h}$ is mostly determined by 
the eigenvalues with smallest real magnitudes and their corresponding 
invariant subspaces. 
In this scenario, due to
the existence of eigenvalues with large magnitude in $\mbf {\wtd A}$, Arnoldi method
with Eqn.~(\ref{eq:kry_A}) cannot find the first couple important 
eigenvalues and invariant spaces
for exponenetial operator quickly. % and requires large $m$ or extremely small $h$, 
In order to preserve the accuracy, the time steps are constrainted, which is discussed in~\cite{Weng12_ICCAD}.
%This kind of system behaviors multiscally in nature and demands computation for 
%very small and large time steps.
This suggests us to make transformation of the specturm in order to 
put more emphasis on those eigenvalues with small magnitudes 
and corresponding invariant subspaces, who are really contributors
to the exponential operator.
For this regard, we make such transformation based on the idea of 
\emph{rational Krylov subspace method}~\cite{Moret04}\cite{Van06}
 to solve this problem.  
%which will be discussed in the following subsections.

\subsection{Fast Rational Krylov Subspace Approximation of Matrix Exponential}

For the purpose of finding the eigenvalues with smallest magnitude first,
we uses a preconditioner $ (\mbf I - \gamma \mbf{\wtd A})^{-1} $,
instead of using $\mbf {\wtd A}$ directly. It is known as rational Krylov subspace~\cite{Moret04}~\cite{Van06}. 
The formula for rational Krylov subspace is 
\begin{eqnarray}
    \label{eq:rat_kry}
    \mbf {K_m}((\mbf I- \gamma \mbf {\wtd A} )^{-1}, \mbf v)   =   
	    span\{ \mbf v, (\mbf I- \gamma\mbf {\wtd A} )^{-1}\mbf v,
    \cdots,  \nonumber \\
      (  \mbf I -  \gamma \mbf{\wtd A})^{-(m-1)} \mbf v \}
\end{eqnarray}
where $\gamma$ is a predifined paramenter which corresponds to time step in our work.
% the eigenvalue context~\cite{Bai87}, 
The Arnoldi method is based on the relation between $\mbf V_m$ and $\mbf H_m$, which is given by
\begin{eqnarray}
    \label{eq:rat_kry2}
    (\mbf I-  \gamma \mbf {\wtd A})^{-1} \mbf V_m =
    \mbf V_m \mbf H_m + \mbf H(m+1,m) \mbf v_{m+1} e^T_m 
\end{eqnarray}
where $e_m$ is the $m$-th unit vector with dimension $m \times 1$. 
%Because of the negligible error term 
%and the orthogonality of columns in $\mbf V_m,\; \mbf H_m$ can be approximately expressed as  
\begin{comment}


%Another merit of rational Krylov subspace method is very
%similar to the QZ decomposition
%method for generalized eigenvalue problem.
\begin{eqnarray}
 \mbf {\wtd } = \mbf Q \mbf \Lambda \mbf Q^{-1} .
\mbf u(t+h) = e^{\mbf \Lambda h} \mbf x(t),
\end{eqnarray}
With the eigenvalue decompostion 
$\mbf x(t+h) = \mbf Q e^{\mbf \Lambda h} \mbf Q^{-1} \mbf x(t)$
\cite{Weng12_ICCAD},
we have 
\begin{eqnarray}
\mbf y(t+h) = e^{\mbf \Lambda h} \mbf y(t),
\end{eqnarray}
where $\mbf y(t) = \mbf  Q^{-1} \mbf x(t+h) $. %= \mbf Q e^{\mbf \Lambda h} \mbf Q^{-1} \mbf x(t)$
$ \mbf {\wtd A} = \mbf Q \mbf \Lambda \mbf Q^{-1} $.


And the work in \cite{Lee09} shows that Hessenberg bares a very 
good approximation property for eigenvalues from the original system,
here is the matrix pencil $(\mbf G, \mbf C)$.
So  $ \mbf {\wtd } = \mbf Q \mbf \Lambda \mbf Q^{-1} $.
is
the solutions
of the homogeneous system 
$\mbf { C} \mbf {\dot{x}} +  \mbf { G} \mbf x = 0$,
~\cite{Wilk:79}\cite{Hairer96}.
The singular $\mbf C$ in our circuit simulation makes the generalized eigenvalues of matrix pencil 
contain ``$-\inf$''.  
This implies that every variable in $\mbf y(t)$ has a relation with its previous stage and change with 
exponential operator with coressponding eigenvalues. 
If $\mbf C$ is singular matrix, the (\ref{eqn:ode}) contains the variables 
only satisfy algebraic equations. 
We have a matrix pencil $(\mbf C, \mbf G)$, it becomes an generalized eigenvalue problem
~\cite{Wilk:79}\cite{Hairer96}.
We can still obtain the bounded eigenvalues~\cite{Wilk:79}\cite{Lee09}. 
Say from $i$ the $y(t)$ has not relation with respect to time. which means  
In \cite{Chen12_TCAD}, such system without regularization contains negative infinite ``eigenvalues".
If we put such negative infite ``eigenvalues'' there, 



\begin{eqnarray}
\label{eq:prekry_3}
   \frac{1}{\gamma}(\mathbf I  - \mathbf H^{-1}_m) =  
 \nonumber \\
  \mathbf V_m^{T}( \mathbf { {\wtd A}}   
  - (\mbf I - \gamma \mbf {\wtd A}) \mbf H(m+1,m) \mbf v_{m+1} \mbf e^T_m  \mbf H^{-1}_m
  )\mathbf V_m . %e^{ \mathbf {C^{-1}G} {\tau}}
\end{eqnarray}
\end{comment}
%If the error term is small, we use 
\begin{eqnarray}
\label{eq:prekry_2}
  \frac{1}{\gamma}(\mathbf I  - \mathbf H^{-1}_m) \approx 
  \mathbf V_m^{T} \mathbf { {\wtd A}}   
  \mathbf V_m . %e^{ \mathbf {C^{-1}G} {\tau}}
\end{eqnarray}

This strategy resembles those works in~\cite{Drus:09_sol}\cite{Moret04}\cite{Van06}. 
%The advantage is applying Arnoldi method on the 
The shift-and-invert matrix $(\mbf I - \gamma \mbf {\wtd A})^{-1}$
emphasizes the eigenvalues   
important to expoential operator, which is contained in the Hessenberg matrix $\mbf H$ after conducting Arnoldi method
based on Eqn.~(\ref{eq:rat_kry}). 
Intuitively, the original eigenvalues with small magnitudes  
in $\mbf  {\wtd A} $ pop out and become larger than the original ones using Eqn. (\ref{eq:kry_A}) 
with large magnitudes, which approach to zero by the ``shift-and-invert''. 
% \subsection{Scaling for Adaptive Step Size Control}
%The following equation is used to calculte system states at different time steps. 
Now given a time step $h$, the matrix exponential $e^{\mbf {\wtd A} h} \mbf v$ can be calculated as   
\begin{eqnarray}
\label{eq:scale}
e^{\mbf {\wtd A}h } \mbf v & \approx & 
			    \mbf V_m \mbf V^T_m e^{\mbf  {\wtd A}h } \mbf v 
		    = \left\|
		       v 
			\right\|_2
			\mbf V_m \mbf V^T_m e^{\mbf  {\wtd A} h} \mbf V_m e_1  \nonumber \\
		  & = &  	\left\|
		       v 
			\right\|_2	\mbf V_m e^{ \alpha  \mbf {\widetilde H}_m }  e_1		
\end{eqnarray}
where $\mbf {\widetilde{H}}_m = \mbf I - \mbf H^{-1}_m $, $\alpha =\frac {h}{\gamma}$ is the tuning parameters for 
control of adaptive time step size in the later Section \ref{sec:adaptive_step_control}.
%When time steps are different from the $\gamma$, we only need to change a scale parameter, because we know the 
%scaling invariant property of the Krylov subspace method avoids the re-calculation of Arnoldi process
%and requires only evaluation of with scaled Hm lpha in (\ref{eq:tgam}) accordingly, without changing $\gamma$ and recalculating 
%in~(\ref{eq:rat_kry}). The following equantions is used,
%\subsection{Posteriori error estimation} 
%\begin{eqnarray}
%\mbf V_m \alpha \mbf H_m \mbf V_h = A h - h{(\mbf I - \gamma A)}^{-1} \beta \mbf v_{m+1} e^{T}_m *\mbf H^{-1}_m; 
%\end{eqnarray}
\begin{comment}
\begin{eqnarray}
\label{eq:prekry_3}
    \alpha \mathbf {\wtd H_M} =  
 \nonumber \\
  \mathbf V_m^{T}( h \mathbf {  {\wtd A}}   
   - h (\mbf I - \gamma \mbf {\wtd A}) \mbf H(m+1,m) \mbf v_{m+1} \mbf e^T_m  \mbf H^{-1}_m
  )\mathbf V_m . %e^{ \mathbf {C^{-1}G} {\tau}}
\end{eqnarray}
\end{comment}

It is neccessary to point out that the error bound for Eqn. (\ref{eq:scale}) does not longer depend on the norm 
$\left\| \mbf {\wtd A}h \right\|$, which is different from the work in~\cite{Weng12_TCAD}\cite{Weng12_ICCAD}. 
It is only the first (smallest magnitude) eigenvalue of $\mbf {\wtd A}$ %\cite{Van06}. 
The lemma is given as follow and the proof is given in \cite{Van06}.
%\newtheorem{lemma}{Lemma}[section]
\begin{lemma}
\label{lem:err}
(Lemma 3.1 in~\cite{Van06}) Let $\mu$ be such that
$ - \mbf {\wtd A} - \mu \mbf I $ is positive semidefinite. Then
\begin{eqnarray}
  \left\| \left\| v \right\|_2 \mbf V_m e^{\alpha \mbf {\wtd H} } e_1 
  - e^{ \alpha\gamma \mbf {\wtd A}} \mbf v \right\|
   \leq 2 e^{-\alpha\gamma\mu} E^{m-1}_{m-1}(\wtd{\gamma} ) 
\end{eqnarray}
   with % $\wtd{\gamma} = \frac{\gamma}{ h(1+\gamma \mu)}$, 
   $ E^{i}_{j}(\wtd{\gamma} ) := \inf_{r \in R^j_i} \sup_{t \le 0}\left | {r(t) - e^{-t}}\right | $,
   $ R^j_i = \{ p(t)(1-\gamma t)^{-i} | p \in \Pi_j \} $, the space $\Pi_{m-1}$ is the space of all
   polynomials of degree $m-1$ ir less.  
%   is defined in \cite{Van06}.
\end{lemma}

What we want to mention is that the $E^{m-1}_{m-1}$ can be approximated as a constant upper bound here. 
And the eigenvalues of $-\mbf  {\wtd A}$ are all larger than a positive $\mu$. 
With increasing $h$ (equivalently $\alpha$) and predefined $\gamma$,
it brings much tigher trend of error bound than smaller $\alpha$.
That explains, in numerical experiment, we observe 
that the large $\alpha$ provides less error under the same order $m$.
 An intuitive explantion is also given by the \cite{Van06}, 
the larger $\alpha$ combined with
exponential operators, the relatively smaller portion of the eigenvalues with smallest magnitude
determine the final vector.
Actually, it is quite a nice feature, espeically 
for power grid simulation, where the voltage noise 
usually contains low frequency behavior from board and package levels. 
Therefore, the users want to see the simulation in a long time span.
Our method can step forward as much as possible to accelerate simulation, 
and also still maintain the high accuracy. The sacrifice resides in the 
small time step when more eigenvalues determine the final vector. So we should 
choose a appropriate parameter $\gamma$ or increase the order $m$ to balance the accuracy and efficiency. Even though the increasing $m$ results more 
backward/forward substitutions, the $m$ is still quite small ($5 \sim 20$) 
in such power grid simulation. Therefore, it does not degrade our method too much.
It illustrates that our method achieves impressive speedups over 
``de facto'' trapezoidal method, 
meanwhile, preserves both low and high frequency characteristic
in the case of industrial power distribution network 
design of Section \ref{sec:exp_results}.A.

The formula of posterior 
error estimation is required for controling adaptive step size.
%In order to preserve well estimation 
%of error trend as well as computation efficiency during 
%online adaptive time stepping,  
We use the formula derived from \cite{Van06},
\begin{eqnarray}
    \label{eq:post_err_est}
    err(m,\alpha) 
    =
    \frac{\left\| v \right\|_2}{\gamma} \mbf {\wtd H}(m+1,m) 
				 \left\| 
				 e^T_m e^ {( \alpha \mbf {  \widetilde{H}}_m)} e_1 
				 \right\|  
				 \left\| (\mbf I - \gamma \mbf {\wtd{A}}) v_{m+1} \right\|
		   % \left\|  \mbf {H^{-1}_m}  \right\|^{2} 
\end{eqnarray}
\begin{comment}
\begin{eqnarray}
    \label{eq:post_err_est}
    err(m,\alpha) 
    =
    \frac{\left\| v \right\|_2}{\alpha} \mbf {\wtd H}(m+1,m) 
				 \left\| 
				 e^T_m e^ {( \alpha \mbf {  \widetilde{H}}_m)} e_1 
				 \right\|  
		   % \left\|  \mbf {H^{-1}_m}  \right\|^{2} 
\end{eqnarray}
\end{comment}
This formula provides a good approximation for 
the error trend with respect to $m$ and $\alpha$ in our numerical experiment.
%it only overestimate too much when $\alpha$ is too small and $m$ is 1  
%where
%$%\begin{eqnarray}
%$   \phi_1(x) = \frac{e^x-1}{x}. $
%$%\end{eqnarray}
% which is very similar to ~\cite{Van06}\cite{Chen12_ICCAD}. 
%It is noted that the error here is no longer limitted by the time step.
%It is influenced directly by input sources, 

\subsection{Block LU factorization}
In pratical numerical implementation, in order to avoid 
direct inversion of $\mbf C$ to form $\mbf A$ in Eqn. (\ref{eq:rat_kry}),
the Eqn. (\ref{eq:precond2}) 
\begin{equation}
\label{eq:precond2}
    (\mathbf C  + \gamma \mathbf G )^{-1}\mathbf C
\end{equation}
% here if we deal with singular case the (\ref{eq:precond}) will use 
is used.
%$\mbf C$ may has bad condition number when it is stiff, 
% or does not exsist when it is singular. 
% (\ref{eq:rat_kry}).
Correspondingly, we uses the following equations for Eqn. (\ref{eq:one_exp}),
\begin{equation}
\label{eq:precond1}
    (\mathbf {\wtd C}  - \gamma \mathbf {\wtd G} )^{-1}\mathbf {\wtd C}
\end{equation}
% $ The augmented matrix $\mbf A = \mbf {C'}^{-1}G'$, where
where
\begin{eqnarray}
\label{eq:cg_prime}
\mbf  {\wtd C} = 
    \left[
	\begin{array}{*{20}{c}} 
	    \mbf C &  0 \\ 
	    0 & \mbf I
	\end{array}
    \right], \; 
\mbf  {\wtd G} =
    \left[
	\begin{array}{*{20}{c}}
	 \mbf {-G}  & \mbf C \mbf W \\
	  0 &  \mbf J
	\end{array}
    \right]
\end{eqnarray}
% will be used for  ${\wtd A}$ of~(\ref{eq:one_exp})  

Applying Arnoldi method based on Eqn.~(\ref{eq:precond1}) contains solving
$\mbf v_{k+1}$ based on $\mbf v_k$, with the linear system
\begin{eqnarray}
   (\mbf {\wtd C } -  \gamma \mbf {\wtd G}) \mbf v_{k+1}=\mbf {\wtd C} \mbf v_k,
\end{eqnarray}
where $\mbf v_{k}$ and $\mbf v_{k+1}$ are
generated basis vectors in $k$ and $k+1$ iterations. 
%, respectively, for Krylov subspace 
This process carries on LU factorizations, if $\mbf W$
in Eqn.~(\ref{eq:cg_prime})
changes with inputs during the simulation. 
However, it is obvious that the majority of matrix components 
in Eqn.~(\ref{eq:cg_prime}) stay the same for this linear system.
To take advantage of this property, a block LU factorization is devised here
to avoid redundant calculation.

The target is to obtain two matrices, 
the lower triangular matrix $\mbf L$, and the 
upper triangular matrix $\mbf U$, where
\begin{eqnarray}
\label{eq:blu}
\mbf  {\wtd C} - \gamma \mbf {\wtd G} = \mbf L \mbf U.
\end{eqnarray}
At the beginning of simulation, after LU factorization of $\mbf C + \gamma \mbf G=\mbf L_{sub} \mbf U_{sub} $
we obtains the lower triangular sub-matrix $\mbf L_{sub}$, and upper triangular 
sub-matrix $\mbf U_{sub}$. Then Eqn. (\ref{eq:blu}) only needs updating 
via  
\begin{eqnarray}
\label{eq:blu1}
%A^{i}\mathbf{v}={({C'}^{-1}G)}^{i}\mathbf{v} \\
\mbf L = 
  \left[
    \begin{array}{*{20}{c}} 
       \mbf L_{sub} & 0\\
       0 & \mbf I
    \end{array}
   \right] , \;\;
\mbf U = 
    \left[
    \begin{array}{*{20}{c}} 
	\mbf U_{sub} &\mbf L^{-1}_{sub} \mbf{C} \mbf W\\
	 0 & \mbf I_J
    \end{array}
    \right],
\end{eqnarray}
where $\mbf I$ is identity matrix, $\mbf I_J = \mbf {I + J}$ is an upper triangular matrix. 
Following equations further reduces the operations for the inversion of $\mbf L_{sub}$ and form the 
vector $\mbf v_k+1$,
\begin{eqnarray}
\label{eq:blu_f}
    \mbf L_{sub} \mbf U_{sub} \; \mbf y_1 = 
	    \mbf b_1- \mbf{C}\mbf W \; \mbf y_2, \; \; \; \; 
    \mbf y_2 = \mbf I^{-1}_J \mbf b_2,  
\end{eqnarray}
where $\mbf v_{k+1} = [\mbf y_1, \; \mbf y_2]^{T} , \mbf b_1=[\mbf C, \; 0] \mbf v_k, 
\mbf b_2 = [0, \; \mbf I] \mbf v_k$. 
By doing this, it only needs one LU factorization at the beginning of simulation, and with 
cheap updates for the $\mbf L$ and $\mbf U$ at each time step during transient simulation. 

% of backward-forward substitutions, which is even smaller than that of the counterparts 
%within the trapozoidal method.
% {\color{red} Emphasize some points here ... }

\subsection{Compatibility with Singular $\mbf C$ without Regularization}
\label{ssec:singC}
Another contribution of our method, it can handle singular $\mbf C$ without regularization. 
Even though, we cannot formula the equation Eqn.(\ref{eqn:discrete_sol}) explicitly, but the solution can be 
still represent as the combination of eigenvalue and eigenvectors.
Our method can obtain the Krylov subsapce $\mbf V_m$ and $\mbf H_m$ to 
To illustrate our idea, 
considering the homogenous version of Eqn. (\ref{eqn:ode}), 
$\mbf { C} \mbf {\dot{x}} +  \mbf { G} \mbf x = 0$,
the % general
solution bares the form 
$\mbf x(t+h) = \mbf Q e^{\mbf \Lambda h} \mbf Q^{-1} \mbf x(t)$,
where $\mbf \Lambda$ is a matrix with only the diagonal terms, which are the eigenvalues of
matrix pencil $(-\mbf G, \mbf C)$.
%\cite{Wilk:79}.
%\cite{Weng12_ICCAD},
If $\mbf C$ is singular, 
we obtain the generalized eigenvalues to matrix pencil $(-\mbf G, \mbf C)$
%matrix pencil $(-\mbf G, \mbf C)$
\cite{Hairer96}\cite{Wilk:79}.
In \cite{Chen12_TCAD}, such singular $\mbf C$ without regularization makes the 
eigenvalues contains negative infinite (``$-\infty$'') ones.
%If we put such negative infite ``eigenvalues'' there, 
However, ``$-\infty$'' eigenvalues and corresponding eigenvectors does 
not effects the whole dynamical system via time derivatives here 
due to the exponential operator ($e^{-\infty} \to 0$).  
Mathematically speaking, it shows that centain part of space does not 
influenced by the dynamical systems via time deriviatives, and
it just forms the algebraic relations in the DAE system \cite{Hairer96}.
Preivously, MEXP\cite{Weng12_TCAD}\cite{Weng12_ICCAD}
cannot handle $\mbf C$ without regularization is only because  
the Arnoldi method requires to inverse $\mbf C$. 
Our algorithm never 
use this inverse $\mbf C$ directly.

!!! State as Theoroem
In other words, the merit of rational Krylov subspace here is to 
extract the subspace and Hessenberg matrix without the influence by 
eigenvalues with the ``$\infty$'' magnitudes and maintain the important
eigenpairs property~\cite{Lee09}.
It is found that matrix $\mbf C$ in the IBM power grid 
suite~\cite{Nassif08_Power}(in Section \ref{sec:exp_results}.B) are all singular ones. 
It validates that our method based on rational Krylov subspace
method addresses the problem without regularization. 

% ----------------------------------------------
% ----------------------------------------------
% End of Section 
% ----------------------------------------------
% ----------------------------------------------
%
%
\begin{comment}
There is not inversion of $\mbf C$ when it is singular. However, it
can still be cast into this MEXP general framework 
without regularization~\cite{Chen12_TCAD}. 
%It is well-known that 
%$\mbf C$ in a general circuit is asymmetric and 
%it could be poorly conditioned and even close to singular, 
%notice that although regularization can
%remove the structural singularity of $\mbf C$, but cannot remove the numerical
%singularity. In this subsection, we discuss the idea how to tackle such 
%problems gracefully. For simplifying the explanation, firstly, consider following homogenous system, 
end{eqnarray}
%The solution is 
%\begin{eqnarray}
%\label{eq:gen2}
%    \mbf x(h) = e^{ - (\mbf C^{-1} \mbf G)h} \mbf  x(0) ,
%\end{eqnarray}
%where $\mbf C$ is a nonsingular matrix.
%Otherwise, if $\mbf C$ is singular matrix, the solutions of (\ref{eq:gen1}) exist,
%The solution can still be written% as exponential operator~\cite{Cox02}.
If $\mbf C + \lambda \mbf G $ is a regular matrix pencil. % , thehas solutions. 
so the problem can be simplified into generalized eigenvalue problem~\cite{Wilk:79}\cite{Hairer96}.
\begin{eqnarray}
\label{eq:gen}
 \mbf { G} \mbf x = -\mbf \lambda \mbf { C} \mbf {{x}} 
\end{eqnarray}
where $\lambda$ and $\mbf u$ are the eigenvalue and eigenvector of Eqn.~(\ref{eq:gen}).
is the solution to
\begin{eqnarray}
\mbf x = e^{{\lambda}h }\mbf u 
\end{eqnarray}
is a solution of Eqn. (\ref{eq:gen1}).
\begin{eqnarray}
\label{eq:gen1}
\mbf { C} \mbf {\dot{x}} +  \mbf { G} \mbf x = 0,
~\cite{Wilk:79}\cite{Hairer96}.
\end{eqnarray}
If we take eigenvalues $\lambda_i$ and their corresponding eigenvectors $\mbf u_i$
% If the eigenvalues are infinite, there will be not corrsponding non-zero eigenvectors belong to 
% null space of (\ref{eq:gen}),
% ,the solution should be the linear combination of $ e^{\lambda_{i}h}\mbf u_i$. 
% bounded eigenvalues and their corrsponding eigenvectors
% \begin{eqnarray}
% $ \mbf x(h) =  [\mbf u_1, \mbf u_2, \cdots, \mbf u_r] e^{\mbf {\Lambda}h } [ c_1, c_2 , \cdots, c_r ]^T$ 
% \end{eqnarray}
\begin{eqnarray}
\mbf \Lambda = 
    \left[
      \begin{array}{*{20}{c}} 
      \lambda_1 & 0   &\cdots    & 0     &0   &\cdots &0\\
      0 & \lambda_2   &\cdots    & 0     &0   &\cdots &0 \\
      \vdots & \vdots &\ddots    & \vdots & \vdots &\ddots &\vdots \\ 
      0 & 0 & \cdots  &\lambda_r & 0      &\cdots & 0    \\
      0 & 0 & \cdots  & 0        & \xi    &\cdots & 0 \\
      \vdots &\vdots  &\ddots    &\vdots & \vdots &\ddots & 0 \\
      0 & 0 &\cdots   & 0     & 0      &\cdots & \xi
      \end{array}
    \right]
\end{eqnarray}
when $r=n$ it returns to the nonsingular case, the $\xi \to \infty $. 
For such generalized eigenvalue problem, rational Krylov subspace/Arnoldi iteration is particular good for 
this computing task~\cite{Lee09}. By this insight, we can use this method for our matrix exponential operator
without necessity of non-exist $\mbf C^{-1}$.
the eigenvalue of matrix pencil $(\mbf C, \mbf G)$ contains infinte ones when $\mbf C$~\cite{Weng12_ICCAD}. Which means 
we can think the power grid with singluar $\mbf C$ is a special case of extreme stiff one. 
\begin{comment}
Starting from the (\ref{eqn:ode}),
standard transformation leads to the \emph{Kroncker canonical form} 
~\cite{Deuf:87}. In our problem, the equation can be written as  
\begin{eqnarray}
\label{eq:singular}
  \left[
    \begin{array}{*{20}{c}} 
	\mathbf I_r &  0 \\
	0 & 0 \\%\mathbf{\Lambda^{(\epsilon)}_{{22}}}\\
    \end{array}
   \right]
\dot{
  \left[
    \begin{array}{*{20}{c}} 
	\mathbf z_1 \\ 
	\mathbf z_2
    \end{array}
\right]
} 
= & - 
  \left[
    \begin{array}{*{20}{c}} 
	\mathbf G_{11} & \mathbf G_{12}\\
	\mathbf G_{21} & \mathbf G_{22}
    \end{array}
\right]
  \left[
    \begin{array}{*{20}{c}} 
	\mathbf z_1\\
	\mathbf z_2
    \end{array}
\right]
 \nonumber \\ 
 &+  \left[
    \begin{array}{*{20}{c}} 
	\mathbf B_1\\
	\mathbf B_2
    \end{array}
\right] {u}(t),
\end{eqnarray}
where, $\mbf I_r$ is $r \times r$ identity matrix
% $\Lambda = [\lambda_1, \lambda_2, \cdots, \lambda_r]$ are the eigenvalues 
and $r$ is the $rank(\mbf C)$, $\mbf z_1, \mbf z_2$ $\mbf x_1, \mbf x_2$, 
$\mbf G_{11},\mbf G_{12}, \mbf G_{21},\mbf G_{22}, \mbf B_1, \mbf B_2  $
are transformed from~(\ref{eqn:ode})
after corresponding standard transformations.  
The approach III in~\cite{Deuf:87} illustrates using 
$\epsilon$-embedding, when $\epsilon \to 0$, still preserve 
the system property, similar techniques are deployed in~\cite{Hairer96}. 
Therefore, \ref{eq:stiff} is uesd to represent $\epsilon$-embedding method. 
\begin{eqnarray}
\label{eq:stiff}
  \left[
    \begin{array}{*{20}{c}} 
	\mathbf{ I_r }& 0 \\
	0 & \mathbf {\epsilon} \mbf I_{n-r}\\
    \end{array}
   \right]
\dot{
  \left[
    \begin{array}{*{20}{c}} 
	\mathbf z_1 \\ 
	\mathbf z_2
    \end{array}
\right]
}
 = & - \left[
    \begin{array}{*{20}{c}} 
	\mathbf G_{11} & \mathbf G_{12}\\
	\mathbf G_{21} & \mathbf G_{22}
    \end{array}
\right]
  \left[
    \begin{array}{*{20}{c}} 
	\mathbf z_1\\
	\mathbf z_2
    \end{array}
\right] \nonumber \\ 
 & +   \left[
    \begin{array}{*{20}{c}} 
	\mathbf B_1\\
	\mathbf B_2
    \end{array}
\right] {u}(t),
\end{eqnarray}
% where, %$\mbf \Lambda_\epsilon = diag[\epsilon, \epsilon, \cdots, \epsilon]_{n-r}$
In our case, the equivalent matrix exponential form is always feasible
and similar 
to~(\ref{eqn:discrete_sol}) in current conext, where
\begin{eqnarray}
\label{eq:eqmexp}
\mbf {\wtd A} = 
-
  \left[
    \begin{array}{*{20}{c}} 
	\mathbf I_r &  0  \\
	0 & \mathbf{\epsilon}^{-1} \mbf I_{n-r} \\
    \end{array}
   \right]
\left[
    \begin{array}{*{20}{c}} 
	\mathbf G_{11} & \mathbf G_{12}\\
	\mathbf G_{21} & \mathbf G_{22}
    \end{array}
\right]
\end{eqnarray}
It is equivalent ODE formulation still maintain associated convergent 
property~\cite{Deuf:87}\cite{Hairer96}.
The inversion of $\mbf {\epsilon} \mbf I_{n-r}$ will not 
cause numerical problems during our simulation. Firstly, we never 
numerically calculate inversion of ill-conditioned 
matrices when following the rational Krylov subspace in this paper.  
In addition, mathematically, it has non-positive eigenvalue and 
the negative infinite magnitudes caused by this inversion will maintain
inherent algbraic equations relations.
Such property is preserved by rational Krylov 
subspace~(\ref{eq:rat_kry}), (\ref{eq:rat_kry2}), (\ref{eq:prekry_2}). Here, 
we focus on the most influential eigenvalues, which are 
not the infinite large magnitude ones in (\ref{eq:kry_A}). So we gracefully, 
avoid the trouble from inversion.
Under this assumption, the singular $\mbf C$ still meet our framework. 
\end{comment}




==> sub-rkwolu.tex <==

Try to avoid the inversion of $\mbf C$


STOC paper 

Despite our block LU has good efficiency to prevent online LU factorization.
But usually the matrix $\mbf L$ and $\mbf U$ contain much more non-zero
fill-ins than $\mbf C $ and $\mbf G$. For example, in our ibmpg1t case, 
when the total nodes (for one matrix) is 54265,
the $\mbf C$ has 19,188 nonzero elements, 
and the $\mbf G$ has 167,975 nonzero elements.
Meanwhile, the $\mbf L$ contains 401,910 nonzero elements,
and the $\mbf L$ contains 515,575 nonzero elements.

A modified CG method will give to fit the framework 
when dealing with general PSD matrxi~\cite{Orec:12}.

When the 

\begin{eqnarray}
\label{eq:cg_p2}
\mbf  {\wtd A} = 
    \left[
	\begin{array}{*{20}{c}} 
	    \mbf C^{-1} G &  \mbf C^{-1}\mbf W  \\ 
	    0 & \mbf I^{-1}\mbf J
	\end{array}
    \right], \; 
    \left[
	\begin{array}{*{20}{c}} 
	    \mbf C^{-1} G &  \mbf C^{-1}\mbf W  \\ 
	    0 & \mbf J
	\end{array}
    \right], \; 
    \\ \nonumber
\mbf  {\wtd C^{-1}} = 
    \left[
	\begin{array}{*{20}{c}} 
	    \mbf C^{-1} &  0 \\ 
	    0 & \mbf J
	\end{array}
    \right], \; 
\mbf  {\wtd G} =
    \left[
	\begin{array}{*{20}{c}}
	 \mbf {-G}  & \mbf W \\
	  0 &  \mbf I
	\end{array}
    \right]
\end{eqnarray}
% will be used for  ${\wtd A}$ of~(\ref{eq:one_exp})  









